Directly comparing GW150914 with numerical solutions of Einstein's equations for binary black hole coalescence

We compare GW150914 directly to simulations of coalescing binary black holes in full general relativity, accounting for all the spin-weighted quadrupolar modes, and separately accounting for all the quadrupolar and octopolar modes. Consistent with the posterior distributions reported in LVC_PE[1] (at 90% confidence), we find the data are compatible with a wide range of nonprecessing and precessing simulations. Followup simulations performed using previously-estimated binary parameters most resemble the data. Comparisons including only the quadrupolar modes constrain the total redshifted mass Mz \in [64 - 82M_\odot], mass ratio q = m2/m1 \in [0.6,1], and effective aligned spin \chi_eff \in [-0.3, 0.2], where \chi_{eff} = (S1/m1 + S2/m2) \cdot\hat{L} /M. Including both quadrupolar and octopolar modes, we find the mass ratio is even more tightly constrained. Simulations with extreme mass ratios and effective spins are highly inconsistent with the data, at any mass. Several nonprecessing and precessing simulations with similar mass ratio and \chi_{eff} are consistent with the data. Though correlated, the components' spins (both in magnitude and directions) are not significantly constrained by the data. For nonprecessing binaries, interpolating between simulations, we reconstruct a posterior distribution consistent with previous results. The final black hole's redshifted mass is consistent with Mf,z between 64.0 - 73.5M_\odot and the final black hole's dimensionless spin parameter is consistent with af = 0.62 - 0.73. As our approach invokes no intermediate approximations to general relativity and can strongly reject binaries whose radiation is inconsistent with the data, our analysis provides a valuable complement to LVC_PE[1].

==> simulation-rankings_100.tex <==
\begin{longtable}{l|l|lrrrrrr|rr}
\caption{\label{tab:SimulationRanks:100}\textbf{Peak Marginalized $\ln L$ II: Probing the final state}: Peak value of the marginalized log likelihood $\ln L_*$ evaluated using a lowerfrequency $f_{low}=100\unit{Hz}$ and all modes with $l \le 2$.  By adopting this cutoff, our comparison probesstrong-field physics during and after merger, notably including the black hole's final mass and spin.  Because of thelow precession rate prior to coalescence, the impact ofprecession should be most accessible during the merger phase (e.g., via the relative amplitudes of quasinormal modesduring ringdown).}\\ \hline\hline $\ln L$ & Key & q & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ &  $\xi$ & $M_z/M_\odot$  \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot
127.08 & \verb|115| & 1.07 & 0.019 & 0.013 & -0.204 & 0.243 & -0.067 & 0.291 & 0.04 & 71.0 \\
127.06 & \verb|hu_a7_th_120_ph_130| & 1.0 & -0.478 & -0.401 & -0.361 & 0.478 & 0.401 & -0.361 & -0.36 & 63.8 \\
127.04 & \verb|a8_th_120_ph_0| & 1.005 & -0.062 & 0.702 & -0.407 &-&-&-& -0.20 & 66.6 \\
127.03 & \verb|130| & 1.38 & 0.164 & 0.037 & -0.014 & 0.293 & 0.060 & 0.343 & 0.14 & 70.3 \\
126.86 & \verb|198| & 1.202 & - & - & - & - & - &-& 0.00 & 69.2 \\
126.8 & \verb|127| & 1.34 & 0.010 & -0.077 & -0.017 & -0.061 & -0.065 & -0.179 & -0.09 & 67.5 \\
126.78 & \verb|q200_a8_a0_th_30_ph_30| & 2 &-&-&-& 0.346 & 0.200 & 0.693 & 0.23 & 66.7 \\
126.78 & \verb|BBH_SKS_d14.3_q1.22_sA_0_0_0.330_sB_0_0_-0.440| & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.02 & 70.0 \\
126.76 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 68.9 \\
126.74 & \verb|119| & 1.12 & -0.012 & 0.068 & 0.260 & 0.078 & -0.003 & 0.006 & 0.14 & 72.2 \\
126.73 & \verb|131| & 1.55 & 0.042 & -0.014 & -0.070 & 0.105 & 0.017 & -0.175 & -0.11 & 65.9 \\
126.72 & \verb|129| & 1.36 & -0.001 & - & 0.088 & 0.193 & -0.289 & -0.075 & 0.02 & 68.7 \\
126.72 & \verb|(0.0,1.1,'M160','D9')| & 1.1 &-&-&-&-&-&-& 0.00 & 68.2 \\
126.69 & \verb|116| & 1.08 & -0.078 & 0.065 & 0.033 & 0.185 & 0.007 & 0.103 & 0.07 & 70.8 \\
126.68 & \verb|(0.0,1.15)| & 1.15 &-&-&-&-&-&-& 0.00 & 69.0 \\
126.67 & \verb|2| & 1.0 &-& - &-&-&-&-& 0.00 & 69.6 \\
126.63 & \verb|(-0.2,1,'M200','D11')| & 1 & - & - & -0.200 & - & - & -0.200 & -0.20 & 67.6 \\
126.63 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 67.7 \\
126.61 & \verb|100| & 1.5 & - & - &-&-& - &-& 0.00 & 67.2 \\
126.57 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 68.7 \\
126.57 & \verb|(0.0,1.0,'M240','D11')| & 1.0 &-&-&-&-&-&-& 0.00 & 69.3 \\
126.55 & \verb|149| & 1.0 &-& - & -0.200 & - &-& -0.200 & -0.20 & 65.2 \\
126.51 & \verb|('Unbalanced',1,0.0,0.2,'M160','D11')| & 1 &-&-&-&-&-& 0.200 & 0.10 & 71.3 \\
126.49 & \verb|(0.0,1.7,'M160','D9')| & 1.7 &-&-&-&-&-&-& 0.00 & 68.5 \\
126.49 & \verb|a8_th_135_ph_150| & 1.005 & -0.259 & -0.498 & -0.590 & - & - &-& -0.30 & 65.1 \\
126.48 & \verb|133| & 1.63 & 0.098 & 0.042 & -0.134 & -0.107 & -0.110 & -0.021 & -0.09 & 66.0 \\
126.47 & \verb|BBH_SKS_d14.3_q1.22_sA_0_0_0_sB_0_0_0| & 1.221 & - &-&-& - & - &-& 0.00 & 67.7 \\
126.47 & \verb|(0.0,1.4,'M160','D9')| & 1.4 &-&-&-&-&-&-& 0.00 & 68.7 \\
126.47 & \verb|4| & 1.0 & - & - & -0.500 & - & - &-& -0.25 & 65.9 \\
126.46 & \verb|150| & 1.0 &-& - & 0.200 & - &-& 0.200 & 0.20 & 72.8 \\
126.45 & \verb|194| & 1.518 &-& - &-& - &-& - & -0.00 & 67.3 \\
126.45 & \verb|('Unbalanced',1,0.0,0.4,'M160','D11')| & 1 &-&-&-&-&-& 0.400 & 0.20 & 72.8 \\
126.44 & \verb|123| & 1.1 & 0.267 & 0.020 & -0.415 & 0.038 & -0.054 & 0.126 & -0.16 & 67.5 \\
126.44 & \verb|125| & 1.27 & 0.012 & 0.045 & -0.058 & 0.389 & 0.241 & 0.070 & -0.00 & 69.9 \\
126.43 & \verb|(0.0,1.45)| & 1.45 &-&-&-&-&-&-& 0.00 & 67.9 \\
126.43 & \verb|137| & 1.76 & -0.248 & -0.319 & -0.034 & -0.071 & 0.151 & -0.190 & -0.09 & 65.7 \\
126.41 & \verb|(0.0,1.5,'M200','D11')| & 1.5 &-&-&-&-&-&-& 0.00 & 67.9 \\
126.41 & \verb|q200_a8_a0_th_135_ph_120| & 2 &-&-&-& -0.283 & 0.490 & -0.566 & -0.19 & 64.4 \\
126.39 & \verb|147| & 1.0 & 0.404 & 0.294 & -0.001 & -0.404 & -0.294 & -0.001 & -0.00 & 69.7 \\
126.38 & \verb|120| & 1.12 & 0.138 & -0.200 & -0.008 & -0.065 & -0.241 & -0.099 & -0.05 & 67.8 \\
126.38 & \verb|124| & 1.26 & 0.250 & -0.058 & 0.071 & 0.075 & -0.095 & 0.286 & 0.17 & 71.4 \\
126.37 & \verb|88| & 1.0 & 0.495 & 0.067 &-&-&-&-& 0.00 & 69.8 \\
126.32 & \verb|173| & 1.5 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.14 & 66.4 \\
126.31 & \verb|121| & 1.12 & -0.061 & -0.109 & 0.356 & -0.323 & -0.127 & -0.297 & 0.05 & 71.9 \\
126.29 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 66.2 \\
126.28 & \verb|a8_th_165_ph_90| & 1.005 & -0.211 &-& -0.786 & - &-& - & -0.39 & 61.7 \\
126.28 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 68.3 \\
126.28 & \verb|a8_q1_KoL_th135_ph_120| & 1.0 & -0.272 & -0.157 & 0.757 & -0.272 & -0.157 & -0.757 & -0.00 & 68.5 \\
126.27 & \verb|122| & 1.17 & -0.019 & 0.061 & -0.477 & 0.041 & 0.050 & -0.364 & -0.42 & 63.2 \\
126.26 & \verb|a8_th_165_ph_0| & 1.005 & -0.009 & 0.195 & -0.790 & - & - & - & -0.40 & 61.9 \\
126.24 & \verb|169| & 2.0 & - & - &-&-&-&-& 0.00 & 64.6 \\
126.23 & \verb|(0.0,1.8,'M160','D9')| & 1.8 &-&-&-&-&-&-& 0.00 & 67.2 \\
126.23 & \verb|82| & 1.501 & 0.496 & 0.053 & - &-&-&-& -0.00 & 68.9 \\
126.23 & \verb|97| & 1.501 & 0.495 & 0.065 & 0.001 &-&-&-& 0.00 & 69.0 \\
126.22 & \verb|hu_a7_th_135_ph_30| & 1.0 & -0.281 & 0.434 & -0.502 & 0.255 & -0.441 & -0.510 & -0.51 & 62.3 \\
126.21 & \verb|146| & 1.97 & -0.156 & -0.102 & -0.037 & -0.098 & 0.027 & -0.357 & -0.14 & 64.2 \\
126.2 & \verb|q150_a8_a0_th_60_ph_120| & 1.492 & - & - &-& -0.595 & -0.380 & 0.405 & 0.16 & 69.7 \\
126.2 & \verb|a8_th_120_ph_90| & 1.005 & -0.706 & -0.033 & -0.403 & - &-& - & -0.20 & 65.9 \\
126.18 & \verb|135| & 1.64 & -0.110 & 0.027 & 0.024 & 0.211 & -0.144 & -0.229 & -0.07 & 67.5 \\
126.18 & \verb|q200_a8_a0_th_90_ph_0| & 2 &-&-&-& 0.800 &-&-& 0.00 & 65.6 \\
126.17 & \verb|a8_th_135_ph_0| & 1.005 & -0.034 & 0.576 & -0.574 &-&-&-& -0.29 & 62.9 \\
126.17 & \verb|163| & 1.0 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.02 & 70.6 \\
126.16 & \verb|141| & 1.84 & -0.182 & 0.052 & 0.086 & -0.093 & 0.124 & 0.040 & 0.07 & 68.7 \\
126.15 & \verb|(0.2,1.25,'M100')| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 74.7 \\
126.14 & \verb|a8_th_135_ph_120| & 1.005 & -0.498 & -0.288 & -0.576 & - & - & - & -0.29 & 64.2 \\
126.14 & \verb|103| & 1.501 & 0.496 & 0.058 &-&-&-&-& 0.00 & 70.7 \\
126.14 & \verb|a8_th_165_ph_150| & 1.005 & -0.105 & -0.182 & -0.786 & - & - & - & -0.39 & 64.1 \\
126.13 & \verb|q200_a8_a0_th_30_ph_60| & 2 &-&-&-& 0.200 & 0.346 & 0.693 & 0.23 & 66.8 \\
126.13 & \verb|132| & 1.63 & -0.005 & -0.114 & -0.007 & 0.041 & -0.087 & 0.310 & 0.11 & 70.5 \\
126.13 & \verb|a8_q1_KoL_th135_ph_150| & 1.0 & -0.157 & -0.272 & 0.757 & -0.157 & -0.272 & -0.757 & -0.00 & 68.3 \\
126.12 & \verb|a8_th_120_ph_60| & 1.005 & -0.643 & 0.299 & -0.399 &-& - & - & -0.20 & 66.9 \\
126.12 & \verb|a8_th_120_ph_30| & 1.005 & -0.408 & 0.580 & -0.399 & - &-& - & -0.20 & 66.9 \\
126.11 & \verb|96| & 1.501 & 0.497 & 0.051 & - &-&-&-& -0.00 & 68.9 \\
126.08 & \verb|q200_a8_a0_th_135_ph_90| & 2 &-&-&-&-& 0.566 & -0.566 & -0.19 & 62.8 \\
126.07 & \verb|a8_q1_up_dn_th_45_ph_30| & 1.0 & -0.337 & 0.463 & 0.585 & 0.290 & -0.502 & -0.579 & 0.00 & 68.2 \\
126.07 & \verb|a8_q1_up_dn_th_45_ph_60| & 1.0 & -0.537 & 0.242 & 0.570 & 0.502 & -0.290 & -0.579 & -0.00 & 67.9 \\
126.07 & \verb|126| & 1.29 & -0.250 & -0.237 & 0.091 & -0.358 & 0.172 & 0.215 & 0.15 & 71.0 \\
126.06 & \verb|a8_th_135_ph_30| & 1.005 & -0.343 & 0.468 & -0.571 & - & - & - & -0.29 & 64.9 \\
126.06 & \verb|q200_a8_a0_th_135_ph_150| & 2 &-&-&-& -0.490 & 0.283 & -0.566 & -0.19 & 62.8 \\
126.06 & \verb|128| & 1.35 & 0.041 & 0.005 & 0.134 & -0.048 & 0.103 & 0.397 & 0.25 & 72.6 \\
126.05 & \verb|a8_th_120_ph_150| & 1.005 & -0.322 & -0.617 & -0.422 & - & - &-& -0.21 & 66.6 \\
126.03 & \verb|29| & 1.5 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.00 & 70.4 \\
126.03 & \verb|a8_th_165_ph_120| & 1.005 & -0.187 & -0.098 & -0.786 & - &-& - & -0.39 & 63.0 \\
126.03 & \verb|(-0.4,1,'M200','D11')| & 1 & - & - & -0.400 & - & - & -0.400 & -0.40 & 64.0 \\
126.02 & \verb|q200_a8_a0_th_90_ph_120| & 2 &-&-&-& -0.400 & 0.693 &-& 0.00 & 65.3 \\
126.01 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 65.8 \\
126.01 & \verb|145| & 1.96 & 0.017 & 0.029 & -0.049 & 0.091 & -0.002 & 0.027 & -0.02 & 65.6 \\
126.01 & \verb|78| & 1.501 & 0.497 & 0.049 & - &-&-&-& -0.00 & 68.8 \\
126.0 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 65.6 \\
126.0 & \verb|a8_q1_KoL_th45_ph_165| & 1.0 & -0.119 & -0.558 & 0.588 & -0.150 & -0.560 & -0.579 & 0.00 & 69.9 \\
125.99 & \verb|a8_th_135_ph_90| & 1.005 & -0.579 & -0.025 & -0.572 & - &-& - & -0.29 & 65.6 \\
125.99 & \verb|148| & 1.0 &-&-& -0.438 & - & - & -0.438 & -0.44 & 61.7 \\
125.99 & \verb|5| & 1.0 &-&-& 0.499 & - & - &-& 0.25 & 74.4 \\
125.98 & \verb|98| & 1.501 & 0.486 & 0.114 & 0.002 &-&-&-& 0.00 & 69.0 \\
125.98 & \verb|134| & 1.63 & -0.230 & 0.184 & -0.012 & -0.001 & 0.032 & 0.176 & 0.06 & 68.8 \\
125.97 & \verb|q200_a8_a0_th_90_ph_90| & 2 &-&-&-&-& 0.800 &-& 0.00 & 64.8 \\
125.97 & \verb|q200_a8_a0_th_135_ph_60| & 2 &-&-&-& 0.283 & 0.490 & -0.566 & -0.19 & 62.8 \\
125.96 & \verb|(0.0,2.05)| & 2.05 &-&-&-&-&-&-& 0.00 & 65.3 \\
125.95 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 70.6 \\
125.95 & \verb|101| & 1.501 &-& - & -0.500 & - & - &-& -0.30 & 61.3 \\
125.94 & \verb|q200_a8_a0_th_135_ph_30| & 2 &-&-&-& 0.490 & 0.283 & -0.566 & -0.19 & 64.5 \\
125.94 & \verb|a8_q1_up_dn_th_45_ph_90| & 1.0 & -0.591 & -0.053 & 0.565 & 0.568 & -0.003 & -0.591 & -0.01 & 68.3 \\
125.92 & \verb|q200_a8_a0_th_60_ph_120| & 2 &-&-&-& -0.346 & 0.600 & 0.400 & 0.13 & 66.6 \\
125.91 & \verb|q200_a8_a0_th_90_ph_60| & 2 &-&-&-& 0.400 & 0.693 &-& 0.00 & 65.3 \\
125.91 & \verb|a8_th_135_ph_60| & 1.005 & -0.520 & 0.265 & -0.568 &-& - &-& -0.28 & 63.1 \\
125.9 & \verb|a8_q1_KoL_th135_ph_90| & 1.0 & -0.331 & -0.026 & 0.749 & -0.314 & -0.007 & -0.757 & -0.00 & 66.4 \\
125.9 & \verb|(0.2,1.0,'M200','D11')| & 1 &-&-& 0.200 &-&-& 0.200 & 0.20 & 73.5 \\
125.9 & \verb|a8_th_120_ph_120| & 1.005 & -0.611 & -0.353 & -0.407 &-&-& - & -0.20 & 65.3 \\
125.89 & \verb|hu_a7_th_120_ph_315| & 1.0 & 0.442 & 0.442 & -0.361 & -0.442 & -0.442 & -0.361 & -0.36 & 63.1 \\
125.89 & \verb|(0.0,2.3499999999999996)| & 2.35 &-&-&-&-&-&-& 0.00 & 63.6 \\
125.88 & \verb|10| & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.26 & 64.5 \\
125.87 & \verb|a8_th_165_ph_60| & 1.005 & -0.182 & 0.105 & -0.786 &-& - &-& -0.39 & 63.3 \\
125.86 & \verb|140| & 1.82 & 0.115 & -0.367 & -0.209 & -0.066 & 0.062 & 0.087 & -0.10 & 66.4 \\
125.85 & \verb|161| & 1.0 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.29 & 67.9 \\
125.85 & \verb|hu_a7_th_120_ph_90| & 1.0 & -0.629 & -0.027 & -0.353 & 0.625 &-& -0.361 & -0.36 & 63.7 \\
125.84 & \verb|q200_a8_a0_th_60_ph_30| & 2 &-&-&-& 0.600 & 0.346 & 0.400 & 0.13 & 65.7 \\
125.83 & \verb|142| & 1.91 & -0.291 & -0.230 & -0.052 & 0.004 & 0.001 & 0.110 & 0.00 & 66.3 \\
125.82 & \verb|(0.0,2.1,'M160','D9')| & 2.1 &-&-&-&-&-&-& 0.00 & 65.8 \\
125.82 & \verb|q200_a8_a0_th_60_ph_150| & 2 &-&-&-& -0.600 & 0.346 & 0.400 & 0.13 & 66.5 \\
125.82 & \verb|(0.0,2.3,'M160','D9')| & 2.3 &-&-&-&-&-&-& 0.00 & 64.6 \\
125.8 & \verb|144| & 1.94 & 0.061 & 0.104 & -0.288 & -0.050 & -0.022 & 0.215 & -0.12 & 63.0 \\
125.78 & \verb|q200_a8_a0_th_90_ph_30| & 2 &-&-&-& 0.693 & 0.400 &-& 0.00 & 65.3 \\
125.77 & \verb|q50_a0_a8_th_90_ph_90| & 2.0 &-& 0.800 &-&-&-&-& 0.00 & 68.3 \\
125.75 & \verb|a8_th_165_ph_30| & 1.005 & -0.103 & 0.188 & -0.785 & - &-& - & -0.39 & 61.7 \\
125.75 & \verb|q200_a8_a0_th_30_ph_120| & 2 &-&-&-& -0.200 & 0.346 & 0.693 & 0.23 & 67.2 \\
125.73 & \verb|138| & 1.7 & -0.044 & 0.425 & 0.042 & -0.012 & -0.008 & -0.111 & -0.01 & 68.4 \\
125.71 & \verb|(0.0,2.4,'M160','D9')| & 2.4 &-&-&-&-&-&-& 0.00 & 64.2 \\
125.71 & \verb|(0.2,1.75,'M100')| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 70.5 \\
125.71 & \verb|hu_a7_th_135_ph_0| & 1.0 & -0.028 & 0.512 & -0.506 &-& -0.510 & -0.510 & -0.51 & 62.0 \\
125.71 & \verb|a8_th_60_ph_150| & 1.005 & -0.353 & -0.612 & 0.408 & - &-& - & 0.20 & 73.1 \\
125.7 & \verb|q200_a8_a0_th_60_ph_60| & 2 &-&-&-& 0.346 & 0.600 & 0.400 & 0.13 & 66.0 \\
125.7 & \verb|a8_th_60_ph_90| & 1.005 & -0.716 & -0.035 & 0.389 & - & - &-& 0.20 & 72.6 \\
125.7 & \verb|q200_a8_a0_th_60_ph_90| & 2 &-&-&-&-& 0.693 & 0.400 & 0.13 & 65.3 \\
125.69 & \verb|q200_a8_a0_th_90_ph_150| & 2 &-&-&-& -0.693 & 0.400 &-& 0.00 & 65.1 \\
125.68 & \verb|q200_a8_a0_th_60_ph_0| & 2 &-&-&-& 0.693 &-& 0.400 & 0.13 & 64.8 \\
125.68 & \verb|('Unbalanced',1,0.2,0.4,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.400 & 0.30 & 75.7 \\
125.67 & \verb|a8_th_60_ph_30| & 1.005 & -0.426 & 0.555 & 0.420 & - &-& - & 0.21 & 73.3 \\
125.64 & \verb|a8_q1_KoL_th135_ph_0| & 1.0 & -0.026 & 0.304 & 0.760 & -0.008 & 0.310 & -0.759 & 0.00 & 68.2 \\
125.61 & \verb|a8_q1_KoL_th45_ph_105| & 1.0 & -0.567 & -0.177 & 0.564 & -0.560 & -0.150 & -0.579 & -0.01 & 71.0 \\
125.61 & \verb|q200_a8_a0_th_135_ph_0| & 2 &-&-&-& 0.566 &-& -0.566 & -0.19 & 63.3 \\
125.61 & \verb|('Unbalanced',1,0.0,0.6,'M160','D11')| & 1 &-&-&-&-&-& 0.600 & 0.30 & 74.9 \\
125.61 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 64.6 \\
125.6 & \verb|a8_th_60_ph_0| & 1.005 & -0.058 & 0.692 & 0.429 &-& - & - & 0.21 & 73.0 \\
125.58 & \verb|hu_a7_th_120_ph_30| & 1.0 & -0.361 & 0.515 & -0.352 & 0.312 & -0.541 & -0.361 & -0.36 & 65.1 \\
125.55 & \verb|a8_q1_KoL_th45_ph_0| & 1.0 & -0.037 & 0.570 & 0.587 & -0.021 & 0.578 & -0.580 & 0.00 & 73.0 \\
125.55 & \verb|a8_q1_up_dn_th_45_ph_0| & 1.0 & -0.034 & 0.569 & 0.589 & 0.002 & -0.591 & -0.568 & 0.01 & 68.9 \\
125.55 & \verb|hu_a7_th_120_ph_0| & 1.0 & -0.055 & 0.621 & -0.362 &-& -0.625 & -0.361 & -0.36 & 63.9 \\
125.55 & \verb|q200_a8_a0_th_30_ph_0| & 2 &-&-&-& 0.400 &-& 0.693 & 0.23 & 66.6 \\
125.55 & \verb|hu_a7_th_135_ph_130| & 1.0 & -0.390 & -0.328 & -0.510 & 0.390 & 0.328 & -0.510 & -0.51 & 62.1 \\
125.52 & \verb|a8_q1_up_dn_th_45_ph_120| & 1.0 & -0.498 & -0.319 & 0.567 & 0.502 & 0.290 & -0.579 & -0.01 & 69.5 \\
125.51 & \verb|139| & 1.82 & 0.032 & -0.342 & 0.210 & -0.132 & -0.047 & -0.042 & 0.12 & 71.0 \\
125.5 & \verb|a8_th_60_ph_120| & 1.005 & -0.612 & -0.353 & 0.408 &-&-& - & 0.20 & 73.1 \\
125.49 & \verb|a8_th_45_ph_30| & 1.005 & -0.341 & 0.464 & 0.578 &-& - & - & 0.29 & 72.5 \\
125.49 & \verb|a8_q1_KoL_th45_ph_150| & 1.0 & -0.290 & -0.502 & 0.579 & -0.290 & -0.502 & -0.579 & -0.00 & 69.7 \\
125.48 & \verb|(0.0,2.5,'M200','D11')| & 2.5 &-&-&-&-&-&-& 0.00 & 64.7 \\
125.46 & \verb|a8_th_45_ph_40| & 1.005 & -0.417 & 0.401 & 0.575 &-& - & - & 0.29 & 74.5 \\
125.45 & \verb|a8_th_45_ph_120| & 1.005 & -0.500 & -0.289 & 0.577 &-& - & - & 0.29 & 74.6 \\
125.45 & \verb|a8_th_45_ph_50| & 1.005 & -0.485 & 0.328 & 0.568 & - &-&-& 0.28 & 74.2 \\
125.45 & \verb|a8_q1_KoL_th135_ph_60| & 1.0 & -0.297 & 0.138 & 0.751 & -0.272 & 0.157 & -0.757 & -0.00 & 69.6 \\
125.44 & \verb|a8_q1_KoL_th45_ph_30| & 1.0 & -0.355 & 0.443 & 0.590 & -0.290 & 0.502 & -0.579 & 0.01 & 73.1 \\
125.42 & \verb|a8_q1_up_dn_th_45_ph_150| & 1.0 & -0.290 & -0.502 & 0.579 & 0.290 & 0.502 & -0.579 & -0.00 & 69.4 \\
125.38 & \verb|a8_th_60_ph_60| & 1.005 & -0.656 & 0.274 & 0.401 &-& - & - & 0.20 & 73.5 \\
125.37 & \verb|q200_a8_a0_th_30_ph_90| & 2 &-&-&-&-& 0.400 & 0.693 & 0.23 & 66.8 \\
125.35 & \verb|a8_th_45_ph_75| & 1.005 & -0.582 & 0.097 & 0.564 &-& - & - & 0.28 & 76.0 \\
125.35 & \verb|a8_th_45_ph_1125| & 1.005 & -0.531 & -0.251 & 0.566 &-&-& - & 0.28 & 74.7 \\
125.34 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 69.0 \\
125.34 & \verb|hu_a7_th_135_ph_315| & 1.0 & 0.360 & 0.360 & -0.510 & -0.360 & -0.360 & -0.510 & -0.51 & 63.8 \\
125.34 & \verb|hu_a7_th_120_ph_210| & 1.0 & 0.361 & -0.512 & -0.358 & -0.312 & 0.541 & -0.361 & -0.36 & 64.6 \\
125.33 & \verb|a8_th_45_ph_60| & 1.005 & -0.536 & 0.241 & 0.566 & - &-&-& 0.28 & 75.3 \\
125.29 & \verb|a9_a0_q1_th_55_ph_150| & 1.012 & -0.373 & -0.646 & 0.523 &-&-& - & 0.26 & 75.2 \\
125.28 & \verb|a8_th_45_ph_0| & 1.005 & -0.034 & 0.568 & 0.584 &-& - & - & 0.29 & 74.8 \\
125.26 & \verb|q50_a0_a8_th_90_ph_60| & 2.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 67.9 \\
125.26 & \verb|hu_a7_th_135_ph_210| & 1.0 & 0.281 & -0.431 & -0.505 & -0.255 & 0.441 & -0.510 & -0.51 & 60.7 \\
125.26 & \verb|q50_a0_a8_th_90_ph_30| & 2.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 67.9 \\
125.25 & \verb|118| & 1.12 & -0.010 & 0.030 & 0.343 & -0.190 & -0.146 & 0.258 & 0.30 & 76.9 \\
125.25 & \verb|a8_th_30_ph_30| & 1.005 & -0.232 & 0.338 & 0.706 &-& - & - & 0.35 & 75.2 \\
125.23 & \verb|a8_q1_KoL_th45_ph_60| & 1.0 & -0.549 & 0.217 & 0.568 & -0.502 & 0.290 & -0.579 & -0.01 & 72.6 \\
125.23 & \verb|q200_a8_a0_th_30_ph_150| & 2 &-&-&-& -0.346 & 0.200 & 0.693 & 0.23 & 65.8 \\
125.22 & \verb|143| & 1.92 & -0.094 & -0.062 & 0.436 & -0.019 & -0.434 & -0.085 & 0.26 & 73.7 \\
125.22 & \verb|a8_th_45_ph_45| & 1.005 & -0.453 & 0.365 & 0.572 &-& - & - & 0.29 & 75.1 \\
125.21 & \verb|a9_a0_q1_th_55_ph_30| & 1.012 & -0.432 & 0.609 & 0.522 & - &-& - & 0.26 & 74.6 \\
125.18 & \verb|q50_a0_a8_th_90_ph_0| & 2.0 & 0.800 &-&-&-&-&-& 0.00 & 67.9 \\
125.14 & \verb|a8_th_45_ph_10| & 1.005 & -0.153 & 0.539 & 0.593 &-& - & - & 0.30 & 72.8 \\
125.12 & \verb|q66_a0_a8_th60_ph_30| & 3.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.30 & 75.7 \\
125.12 & \verb|a9_a0_q1_th_55_ph_0| & 1.012 & -0.062 & 0.725 & 0.549 & - &-& - & 0.28 & 74.1 \\
125.1 & \verb|136| & 1.68 & 0.118 & -0.114 & 0.326 & -0.145 & -0.071 & 0.145 & 0.26 & 72.9 \\
125.09 & \verb|a8_q1_KoL_th135_ph_30| & 1.0 & -0.185 & 0.257 & 0.756 & -0.157 & 0.272 & -0.757 & -0.00 & 68.7 \\
125.05 & \verb|a8_th_45_ph_20| & 1.005 & -0.251 & 0.511 & 0.584 &-& - & - & 0.29 & 74.8 \\
125.04 & \verb|a8_th_45_ph_150| & 1.005 & -0.289 & -0.500 & 0.577 &-&-&-& 0.29 & 72.5 \\
125.03 & \verb|hu_a7_th_135_ph_90| & 1.0 & -0.510 &-& -0.510 & 0.510 &-& -0.510 & -0.51 & 61.6 \\
125.01 & \verb|a9_a0_q1_th_55_ph_60| & 1.012 & -0.686 & 0.321 & 0.507 & - &-& - & 0.25 & 74.7 \\
125.01 & \verb|a8_q1_KoL_th45_ph_135| & 1.0 & -0.410 & -0.410 & 0.579 & -0.410 & -0.410 & -0.579 & -0.00 & 71.7 \\
125.0 & \verb|q33_a0_a8_th_100_ph_30| & 3 & 0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 62.7 \\
124.99 & \verb|q50_a0_a8_th_90_ph_120| & 2.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 70.5 \\
124.94 & \verb|a8_th_45_ph_1275| & 1.005 & -0.458 & -0.351 & 0.577 & - & - &-& 0.29 & 76.2 \\
124.93 & \verb|a9_a0_q1_th_55_ph_90| & 1.012 & -0.759 & -0.029 & 0.505 &-& - & - & 0.25 & 76.0 \\
124.91 & \verb|a8_th_30_ph_60| & 1.005 & -0.378 & 0.185 & 0.700 & - &-& - & 0.35 & 76.7 \\
124.87 & \verb|('Unbalanced',1,0.2,0.6,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.600 & 0.40 & 78.7 \\
124.85 & \verb|a8_th_30_ph_0| & 1.005 & -0.033 & 0.386 & 0.718 &-& - & - & 0.36 & 75.3 \\
124.83 & \verb|('Unbalanced',1,0.0,0.8,'M160','D11')| & 1 &-&-&-&-&-& 0.800 & 0.40 & 77.7 \\
124.83 & \verb|q66_a0_a8_th60_ph_0| & 3.0 & 0.693 &-& 0.400 &-&-&-& 0.30 & 75.7 \\
124.79 & \verb|BBH_SKS_d14.4_q1.19_sA_0_0_0.420_sB_0_0_0.380| & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.40 & 77.7 \\
124.77 & \verb|hu_a7_th_60_ph_130| & 1.0 & -0.467 & -0.427 & 0.354 & 0.481 & 0.404 & 0.363 & 0.36 & 74.6 \\
124.75 & \verb|164| & 1.0 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.33 & 79.4 \\
124.75 & \verb|q66_a0_a8_th60_ph_150| & 3.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.30 & 75.7 \\
124.75 & \verb|a8_th_30_ph_90| & 1.005 & -0.423 & -0.024 & 0.698 &-&-& - & 0.35 & 76.7 \\
124.72 & \verb|q50_a0_a8_th_90_ph_150| & 2.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 70.5 \\
124.72 & \verb|(0.4,1.0,'M200','D11')| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 77.3 \\
124.71 & \verb|a8_th_30_ph_150| & 1.005 & -0.204 & -0.353 & 0.707 & - &-& - & 0.35 & 76.4 \\
124.7 & \verb|a8_q1_KoL_th45_ph_120| & 1.0 & -0.502 & -0.290 & 0.579 & -0.502 & -0.290 & -0.579 & -0.00 & 72.9 \\
124.68 & \verb|hu_a7_th_60_ph_315| & 1.0 & 0.424 & 0.464 & 0.361 & -0.444 & -0.444 & 0.363 & 0.36 & 75.2 \\
124.67 & \verb|151| & 1.0 &-& - & -0.600 & - &-& -0.600 & -0.60 & 58.2 \\
124.67 & \verb|q33_a0_a8_th_100_ph_90| & 3 &-& 0.788 & -0.139 &-&-&-& -0.10 & 62.7 \\
124.67 & \verb|hu_a7_th_60_ph_0| & 1.0 & -0.053 & 0.616 & 0.379 & 0.028 & -0.624 & 0.368 & 0.37 & 73.7 \\
124.64 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 76.6 \\
124.63 & \verb|q50_a0_a8_th_135_ph_90| & 2.0 &-& 0.566 & -0.566 &-&-&-& -0.38 & 58.7 \\
124.63 & \verb|a8_th_30_ph_120| & 1.005 & -0.353 & -0.204 & 0.707 & - &-& - & 0.35 & 75.8 \\
124.62 & \verb|a8_th_15_ph_0| & 1.005 & -0.005 & 0.215 & 0.788 &-& - & - & 0.39 & 76.6 \\
124.61 & \verb|q66_a0_a8_th60_ph_120| & 3.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.30 & 75.7 \\
124.6 & \verb|a8_th_15_ph_120| & 1.005 & -0.183 & -0.106 & 0.789 & - & - & - & 0.40 & 76.3 \\
124.56 & \verb|q66_a0_a8_th60_ph_60| & 3.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.30 & 75.7 \\
124.55 & \verb|q33_a0_a8_th_100_ph_60| & 3 & 0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 62.7 \\
124.52 & \verb|q33_a0_a8_th_100_ph_0| & 3 & 0.788 &-& -0.139 &-&-&-& -0.10 & 62.7 \\
124.52 & \verb|hu_a7_th_60_ph_110| & 1.0 & -0.587 & -0.241 & 0.351 & 0.590 & 0.215 & 0.363 & 0.36 & 73.0 \\
124.51 & \verb|a8_th_15_ph_90| & 1.005 & -0.223 & -0.003 & 0.785 &-&-&-& 0.39 & 77.7 \\
124.5 & \verb|q50_a0_a8_th_135_ph_60| & 2.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 59.9 \\
124.49 & \verb|hu_a7_th_60_ph_30| & 1.0 & -0.376 & 0.493 & 0.376 & 0.339 & -0.532 & 0.356 & 0.37 & 73.4 \\
124.49 & \verb|a8_th_15_ph_30| & 1.005 & -0.106 & 0.183 & 0.789 &-& - & - & 0.40 & 76.6 \\
124.46 & \verb|(0.4,1.25,'M100')| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 78.8 \\
124.46 & \verb|a8_th_15_ph_150| & 1.005 & -0.106 & -0.183 & 0.789 & - &-& - & 0.40 & 78.4 \\
124.41 & \verb|q50_a0_a8_th_135_ph_30| & 2.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 60.6 \\
124.41 & \verb|q50_a0_a8_th_135_ph_120| & 2.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 59.9 \\
124.41 & \verb|a8_th_15_ph_60| & 1.005 & -0.185 & 0.106 & 0.788 &-&-& - & 0.40 & 76.4 \\
124.37 & \verb|(0.0,2.6,'M160','D9')| & 2.6 &-&-&-&-&-&-& 0.00 & 66.8 \\
124.34 & \verb|(0.4,1.75,'M100')| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 74.7 \\
124.33 & \verb|q50_a0_a8_th_135_ph_0| & 2.0 & 0.566 &-& -0.566 &-&-&-& -0.38 & 57.2 \\
124.32 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 74.3 \\
124.31 & \verb|q50_a0_a8_th_60_ph_150| & 2.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 75.7 \\
124.27 & \verb|th_315| & 1.0 & 0.565 & 0.565 & 0.462 & -0.565 & -0.565 & 0.462 & 0.46 & 77.3 \\
124.24 & \verb|q50_a0_a8_th_135_ph_150| & 2.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 58.9 \\
124.16 & \verb|hu_a7_th_60_ph_80| & 1.0 & -0.632 & 0.058 & 0.351 & 0.618 & -0.109 & 0.363 & 0.36 & 71.2 \\
124.1 & \verb|q50_a0_a8_th_60_ph_120| & 2.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 73.5 \\
124.03 & \verb|hu_a7_th_60_ph_10| & 1.0 & -0.161 & 0.600 & 0.373 & 0.137 & -0.612 & 0.364 & 0.37 & 74.7 \\
123.99 & \verb|hu_a7_th_60_ph_210| & 1.0 & 0.361 & -0.514 & 0.362 & -0.314 & 0.544 & 0.362 & 0.36 & 77.2 \\
123.98 & \verb|q66_a0_a8_th60_ph_90| & 3.0 &-& 0.693 & 0.400 &-&-&-& 0.30 & 75.7 \\
123.94 & \verb|th_90| & 1.0 & -0.809 & -0.030 & 0.443 & 0.808 & -0.006 & 0.446 & 0.44 & 78.3 \\
123.93 & \verb|q33_a0_a8_th_100_ph_120| & 3 & -0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 65.3 \\
123.91 & \verb|q33_a0_a8_th_135_ph_90| & 3 &-& 0.566 & -0.566 &-&-&-& -0.42 & 56.3 \\
123.88 & \verb|q50_a0_a8_th_60_ph_60| & 2.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 75.7 \\
123.85 & \verb|q50_a0_a8_th_60_ph_90| & 2.0 &-& 0.693 & 0.400 &-&-&-& 0.27 & 57.5 \\
123.78 & \verb|th_130| & 1.0 & -0.613 & -0.514 & 0.462 & 0.612 & 0.514 & 0.462 & 0.46 & 76.6 \\
123.75 & \verb|hu_a7_th_60_ph_90| & 1.0 & -0.632 & -0.052 & 0.351 & 0.628 &-& 0.363 & 0.36 & 75.0 \\
123.74 & \verb|hu_a7_th_60_ph_40| & 1.0 & -0.445 & 0.444 & 0.362 & 0.404 & -0.481 & 0.362 & 0.36 & 74.3 \\
123.73 & \verb|a8_q1_L_ph_0| & 1.0 & -0.064 & 0.817 & 0.013 & - & -0.010 & 0.820 & 0.42 & 79.2 \\
123.72 & \verb|th_0| & 1.0 & -0.043 & 0.791 & 0.474 & 0.023 & -0.797 & 0.465 & 0.47 & 78.0 \\
123.66 & \verb|a8_q1_L_ph_150| & 1.0 & -0.385 & -0.724 & 0.002 & 0.012 & 0.003 & 0.820 & 0.41 & 77.0 \\
123.64 & \verb|q33_a0_a8_th_135_ph_60| & 3 & 0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 56.0 \\
123.57 & \verb|q33_a0_a8_th_135_ph_30| & 3 & 0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 55.8 \\
123.57 & \verb|a8_q1_L_ph_120| & 1.0 & -0.703 & -0.422 & -0.009 & 0.016 & 0.006 & 0.820 & 0.41 & 76.9 \\
123.52 & \verb|q33_a0_a8_th_100_ph_150| & 3 & -0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 60.1 \\
123.5 & \verb|q33_a0_a8_th_75_ph_120| & 3 & -0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 67.9 \\
123.48 & \verb|q50_a0_a8_th_60_ph_0| & 2.0 & 0.693 &-& 0.400 &-&-&-& 0.27 & 75.1 \\
123.48 & \verb|162| & 2.0 &-& - & 0.600 &-&-&-& 0.40 & 77.2 \\
123.42 & \verb|q50_a0_a8_th_60_ph_30| & 2.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 75.7 \\
123.34 & \verb|q33_a0_a8_th_75_ph_150| & 3 & -0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 70.5 \\
123.33 & \verb|hu_a7_th_45_ph_315| & 1.0 & 0.344 & 0.384 & 0.510 & -0.363 & -0.363 & 0.513 & 0.51 & 78.1 \\
123.33 & \verb|117| & 1.08 & 0.118 & -0.069 & 0.070 & -0.302 & -0.298 & -0.200 & -0.06 & 64.1 \\
123.33 & \verb|('Unbalanced',1,0.2,0.8,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.800 & 0.50 & 80.2 \\
123.21 & \verb|a8_q1_L_ph_90| & 1.0 & -0.819 & -0.038 & -0.009 & 0.016 &-& 0.820 & 0.41 & 78.6 \\
123.13 & \verb|hu_a7_th_45_ph_90| & 1.0 & -0.518 & -0.054 & 0.505 & 0.513 &-& 0.513 & 0.51 & 78.6 \\
123.12 & \verb|q33_a0_a8_th_75_ph_90| & 3 &-& 0.773 & 0.207 &-&-&-& 0.16 & 57.5 \\
123.1 & \verb|q33_a0_a8_th_135_ph_0| & 3 & 0.566 &-& -0.566 &-&-&-& -0.42 & 55.4 \\
123.07 & \verb|q33_a0_a8_th_75_ph_30| & 3 & 0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 57.5 \\
122.93 & \verb|q33_a0_a8_th_75_ph_60| & 3 & 0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 73.1 \\
122.9 & \verb|hu_a7_th_45_ph_130| & 1.0 & -0.378 & -0.354 & 0.508 & 0.393 & 0.330 & 0.513 & 0.51 & 76.6 \\
122.89 & \verb|q33_a0_a8_th_135_ph_150| & 3 & -0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 52.3 \\
122.85 & \verb|a8_q1_L_ph_30| & 1.0 & -0.476 & 0.668 & 0.011 & 0.011 & 0.004 & 0.820 & 0.42 & 79.2 \\
122.83 & \verb|191| & 2.507 & - &-& - &-&-&-& -0.00 & 69.2 \\
122.79 & \verb|a8_q1_L_ph_60| & 1.0 & -0.746 & 0.341 & -0.002 & 0.016 & -0.002 & 0.820 & 0.41 & 78.9 \\
122.76 & \verb|q33_a0_a8_th_75_ph_0| & 3 & 0.773 &-& 0.207 &-&-&-& 0.16 & 73.1 \\
122.49 & \verb|q33_a0_a8_th_135_ph_120| & 3 & -0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 54.9 \\
122.25 & \verb|q50_a0_a8_th_30_ph_120| & 2.0 & -0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 80.2 \\
122.09 & \verb|hu_a7_th_45_ph_0| & 1.0 & -0.028 & 0.507 & 0.517 & 0.028 & -0.507 & 0.518 & 0.52 & 79.2 \\
122.01 & \verb|(0.0,2.7,'M160','D9')| & 2.7 &-&-&-&-&-&-& 0.00 & 68.9 \\
121.87 & \verb|th_30| & 1.0 & -0.455 & 0.653 & 0.468 & 0.400 & -0.692 & 0.462 & 0.46 & 78.4 \\
121.8 & \verb|152| & 1.0 &-& - & 0.600 & - &-& 0.600 & 0.60 & 82.4 \\
121.73 & \verb|hu_a7_th_45_ph_210| & 1.0 & 0.299 & -0.412 & 0.516 & -0.256 & 0.444 & 0.513 & 0.51 & 74.7 \\
121.72 & \verb|q50_a0_a8_th_30_ph_150| & 2.0 & -0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 79.8 \\
121.69 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 83.2 \\
121.66 & \verb|(0.6,1.25,'M100')| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 83.5 \\
121.58 & \verb|hu_a7_th_45_ph_30| & 1.0 & -0.299 & 0.411 & 0.518 & 0.256 & -0.444 & 0.513 & 0.52 & 77.1 \\
121.55 & \verb|q50_a0_a8_th_30_ph_90| & 2.0 &-& 0.400 & 0.693 &-&-&-& 0.46 & 80.3 \\
121.55 & \verb|(0.6,1.5,'M100')| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 82.0 \\
121.52 & \verb|q50_a0_a8_th_30_ph_0| & 2.0 & 0.400 &-& 0.693 &-&-&-& 0.46 & 80.3 \\
121.48 & \verb|(0.6,1.75,'M100')| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 81.2 \\
121.38 & \verb|th_210| & 1.0 & 0.458 & -0.653 & 0.465 & -0.400 & 0.692 & 0.462 & 0.46 & 77.0 \\
121.16 & \verb|q50_a0_a8_th_30_ph_30| & 2.0 & 0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 80.3 \\
121.11 & \verb|q50_a0_a8_th_30_ph_60| & 2.0 & 0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 80.3 \\
120.97 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 80.4 \\
120.89 & \verb|hu_a7_th_22.5_ph_210| & 1.0 & 0.139 & -0.240 & 0.670 & -0.139 & 0.240 & 0.670 & 0.67 & 82.5 \\
120.82 & \verb|hu_a7_th_22.5_ph_30| & 1.0 & -0.160 & 0.221 & 0.672 & 0.139 & -0.240 & 0.670 & 0.67 & 83.4 \\
120.82 & \verb|q33_a0_a8_th_45_ph_150| & 3 & -0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 75.7 \\
120.63 & \verb|hu_a7_th_22.5_ph_90| & 1.0 & -0.288 & -0.026 & 0.665 & 0.278 &-& 0.670 & 0.67 & 84.0 \\
120.42 & \verb|hu_a7_th_22.5_ph_0| & 1.0 &-& 0.278 & 0.670 &-& -0.278 & 0.670 & 0.67 & 84.4 \\
120.1 & \verb|q33_a0_a8_th_45_ph_120| & 3 & -0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 75.7 \\
120.04 & \verb|hu_a7_th_22.5_ph_315| & 1.0 & 0.196 & 0.196 & 0.670 & -0.196 & -0.196 & 0.670 & 0.67 & 83.2 \\
119.96 & \verb|46| & 3.0 &-&-& -0.500 & - &-& -0.499 & -0.50 & 61.4 \\
119.9 & \verb|hu_a7_th_22.5_ph_130| & 1.0 & -0.213 & -0.178 & 0.670 & 0.213 & 0.178 & 0.670 & 0.67 & 83.6 \\
119.78 & \verb|q33_a0_a8_th_45_ph_90| & 3 &-& 0.566 & 0.566 &-&-&-& 0.42 & 62.7 \\
119.75 & \verb|q33_a0_a8_th_45_ph_60| & 3 & 0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 66.4 \\
119.33 & \verb|q33_a0_a8_th_45_ph_30| & 3 & 0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 62.7 \\
119.13 & \verb|q33_a0_a8_th_45_ph_0| & 3 & 0.566 &-& 0.566 &-&-&-& 0.42 & 75.7 \\
118.94 & \verb|179| & 1.5 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.65 & 88.4 \\
118.8 & \verb|(0.0,2.8,'M160','D9')| & 2.8 &-&-&-&-&-&-& 0.00 & 71.1 \\
118.27 & \verb|hu_a9_th_30_ph_0| & 1.0 & -0.027 & 0.445 & 0.809 & -0.004 & -0.462 & 0.800 & 0.80 & 87.8 \\
118.1 & \verb|hu_a9_th_30_ph_210| & 1.0 & 0.231 & -0.400 & 0.800 & -0.231 & 0.400 & 0.800 & 0.80 & 86.8 \\
118.05 & \verb|175| & 1.0 &-& - & 0.750 & - &-& 0.750 & 0.75 & 88.4 \\
117.89 & \verb|hu_a9_th_30_ph_315| & 1.0 & 0.327 & 0.327 & 0.800 & -0.327 & -0.327 & 0.800 & 0.80 & 86.8 \\
117.67 & \verb|hu_a9_th_30_ph_30| & 1.0 & -0.262 & 0.381 & 0.799 & 0.231 & -0.400 & 0.800 & 0.80 & 87.0 \\
117.62 & \verb|hu_a9_th_30_ph_130| & 1.0 & -0.354 & -0.297 & 0.800 & 0.354 & 0.297 & 0.800 & 0.80 & 84.4 \\
116.8 & \verb|(0.8,1.0,'M200','D11')| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 89.9 \\
116.5 & \verb|155| & 1.0 & - & - & 0.800 &-&-& 0.800 & 0.80 & 90.6 \\
116.32 & \verb|hu_a9_th_30_ph_90| & 1.0 & -0.462 & -0.003 & 0.800 & 0.462 & 0.003 & 0.800 & 0.80 & 89.1 \\
115.27 & \verb|(0.0,2.9,'M160','D9')| & 2.9 &-&-&-&-&-&-& 0.00 & 73.3 \\
114.86 & \verb|hu_a9_th_15_ph_90| & 1.0 & -0.258 & 0.005 & 0.887 & 0.258 & -0.005 & 0.888 & 0.89 & 91.0 \\
114.79 & \verb|153| & 1.0 & - & - & 0.850 &-&-& 0.850 & 0.85 & 92.3 \\
114.48 & \verb|hu_a9_th_15_ph_210| & 1.0 & 0.120 & -0.207 & 0.892 & -0.120 & 0.207 & 0.893 & 0.89 & 90.4 \\
114.37 & \verb|hu_a9_th_15_ph_315| & 1.0 & 0.169 & 0.169 & 0.893 & -0.169 & -0.169 & 0.893 & 0.89 & 92.2 \\
114.23 & \verb|52| & 3.0 & 0.494 & 0.073 & 0.001 & 0.001 & 0.008 & -0.499 & -0.12 & 76.0 \\
114.12 & \verb|105| & 3.001 &-& - & -0.500 & - & - &-& -0.37 & 66.3 \\
114.05 & \verb|42| & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.32 & 68.2 \\
114.02 & \verb|hu_a9_th_15_ph_30| & 1.0 & -0.120 & 0.207 & 0.892 & 0.120 & -0.207 & 0.893 & 0.89 & 92.3 \\
113.73 & \verb|hu_a9_th_15_ph_0| & 1.0 &-& 0.239 & 0.893 &-& -0.239 & 0.893 & 0.89 & 92.0 \\
113.49 & \verb|hu_a9_th_15_ph_130| & 1.0 & -0.183 & -0.154 & 0.893 & 0.183 & 0.154 & 0.893 & 0.89 & 92.1 \\
112.82 & \verb|160| & 1.0 &-& - & 0.900 &-&-& 0.900 & 0.90 & 94.8 \\
112.69 & \verb|159| & 1.0 &-&-& -0.900 & - & - & -0.900 & -0.90 & 42.1 \\
111.65 & \verb|(0.0,3,'M200','D11')| & 3 &-&-&-&-&-&-& 0.00 & 75.6 \\
110.48 & \verb|157| & 1.0 & - &-& 0.950 &-& - & 0.950 & 0.95 & 96.9 \\
109.95 & \verb|176| & 1.0 &-& - & 0.960 & - &-& 0.960 & 0.96 & 97.3 \\
109.51 & \verb|158| & 1.0 &-& - & 0.970 & - &-& 0.970 & 0.97 & 97.8 \\
109.18 & \verb|44| & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.00 & 80.8 \\
108.96 & \verb|177| & 1.0 &-&-& 0.989 & - & - & 0.989 & 0.99 & 98.5 \\
108.89 & \verb|172| & 1.0 &-& - & 0.979 & - &-& 0.979 & 0.98 & 98.2 \\
108.87 & \verb|156| & 1.0 &-&-& -0.949 &-&-& -0.949 & -0.95 & 39.4 \\
108.58 & \verb|50| & 3.0 & 0.494 & 0.072 & 0.002 & 0.467 & 0.176 & 0.005 & 0.00 & 80.8 \\
108.19 & \verb|178| & 1.0 &-&-& 0.994 & - & - & 0.994 & 0.99 & 99.1 \\
107.94 & \verb|53| & 3.0 & 0.494 & 0.075 & 0.001 & -0.464 & -0.184 & -0.003 & 0.00 & 80.8 \\
107.87 & \verb|(0.0,3.1,'M160','D9')| & 3.1 &-&-&-&-&-&-& 0.00 & 77.9 \\
104.19 & \verb|30| & 3.0 &-&-&-& - &-&-& 0.00 & 80.8 \\
104.05 & \verb|49| & 3.0 & 0.494 & 0.073 & 0.001 & - & -0.008 & 0.499 & 0.13 & 85.6 \\
103.93 & \verb|(0.0,3.2,'M160','D9')| & 3.2 &-&-&-&-&-&-& 0.00 & 80.2 \\
100.29 & \verb|43| & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.32 & 93.4 \\
98.57 & \verb|48| & 3.0 & - & -0.001 & 0.500 & 0.471 & 0.165 & 0.001 & 0.37 & 95.3 \\
98.55 & \verb|51| & 3.0 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.37 & 95.3 \\
98.44 & \verb|174| & 3.001 &-& - & 0.500 & - &-&-& 0.37 & 95.3 \\
93.05 & \verb|47| & 3.0 &-&-& 0.500 & - & - & 0.499 & 0.50 & 100.1 \\
91.63 & \verb|a8_q1_KoL_th45_ph_90| & 1.0 & -0.595 & -0.035 & 0.562 & -0.591 & - & -0.568 & -0.00 & 66.1 \\
\end{longtable}


==> simulation-rankings_10_C01.tex <==
\begin{longtable}{l|l|lrrrrrr|rr|r}
\caption{\label{tab:SimulationRanks:AllSignal}\textbf{Peak Marginalized $\ln L$: Low frequency included}: Peak value of the marginalized log likelihood $\ln L$ evaluated using a lower frequency $f_{low}=10\unit{Hz}$ and all modes with $l \le 2$; the simulation key, described in Table \ref{tab:SimulationList} [an asterisk (*) denotes a new simulation motivated by \TheEvent{}, and a (+) denotes one of the simulations reported in \PaperDetection];  the \emph{initial} spins of the simulation (using $-$ to denote zero, to enhance readability); the initial $\xi$; and the total (redshifted) mass of the best fit.   This choice of low-frequency cutoff ensures that long simulations can make the best use of low-frequency information in the data, significantly improving our constraints on $M$ and spin precession.  } \\ \hline \hline $\ln L$ & Key & $q$ & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ & $\chi_{\rm eff}$ & $M_z/M_\odot$  \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot 
277.3 & \verb|SXS:BBH:0002| & 1.0 &-& - &-&-&-&-& 0.00 & 72.7 & 10.0 \\
277.2 & \verb|SXS:BBH:0313|(*) & 1.217 &-& - & 0.380 &-&-& -0.520 & -0.03 & 72.9 & 15.5 \\
276.9 & \verb|SXS:BBH:0305|(*+) & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.02 & 73.2 & 15.5 \\
276.6 & \verb|D11_q0.75_a0.0_0.0_n100|(*) & 1.333 &-&-& - &-&-& - & -0.00 & 72.6 & 22.9 \\
276.1 & \verb|SXS:BBH:0006| & 1.345 & 0.234 & 0.148 & -0.161 & 0.091 & 0.064 & -0.101 & -0.14 & 69.0 & 13.7 \\
275.4 & \verb|SXS:BBH:0096| & 1.501 & 0.497 & 0.051 & - &-&-&-& -0.00 & 72.7 & 13.3 \\
275.4 & \verb|SXS:BBH:0163| & 1.0 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.02 & 74.4 & 13.4 \\
275.2 & \verb|SXS:BBH:0131| & 1.55 & 0.042 & -0.014 & -0.070 & 0.105 & 0.017 & -0.175 & -0.11 & 70.8 & 14.8 \\
275.0 & \verb|GT:BBH:898|(*) & 1.2 &-&-&-&-&-&-& 0.00 & 74.2 & 18.0 \\
274.9 & \verb|SXS:BBH:0029| & 1.5 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.00 & 74.2 & 13.4 \\
274.8 & \verb|SXS:BBH:0100| & 1.5 & - & - &-&-& - &-& 0.00 & 72.9 & 11.0 \\
274.5 & \verb|SXS:BBH:0121| & 1.12 & -0.061 & -0.109 & 0.356 & -0.323 & -0.127 & -0.297 & 0.05 & 74.6 & 15.0 \\
274.1 & \verb|SXS:BBH:0117| & 1.08 & 0.118 & -0.069 & 0.070 & -0.302 & -0.298 & -0.200 & -0.06 & 72.5 & 14.8 \\
274.1 & \verb|SXS:BBH:0316|(*) & 1.186 & 0.241 & 0.170 & 0.299 & -0.203 & -0.172 & -0.271 & 0.04 & 73.8 & 15.3 \\
274.0 & \verb|SXS:BBH:0307|(*) & 1.228 & - & - & 0.320 &-& - & -0.580 & -0.08 & 69.3 & 17.8 \\
273.9 & \verb|SXS:BBH:0312|(*) & 1.203 &-& - & 0.390 &-&-& -0.480 & -0.00 & 71.3 & 15.7 \\
273.6 & \verb|SXS:BBH:0308[Lev3]|(*) & 1.228 & 0.072 & 0.072 & 0.325 & 0.201 & 0.285 & -0.571 & -0.08 & 69.4 & 17.9 \\
273.5 & \verb|D21.5_q1_a0.2_0.8_th104.4775_n100| & 1.001 &-&-& 0.200 & 0.775 &-& -0.200 & -0.00 & 74.3 & 9.7 \\
273.5 & \verb|SXS:BBH:0003| & 1.0 & 0.497 & 0.053 & - &-&-&-& -0.00 & 73.8 & 11.4 \\
273.4 & \verb|SXS:BBH:0103| & 1.501 & 0.496 & 0.058 &-&-&-&-& 0.00 & 73.2 & 10.8 \\
273.4 & \verb|SXS:BBH:0310|(*) & 1.221 & - &-&-& - & - &-& 0.00 & 74.3 & 15.0 \\
273.1 & \verb|SXS:BBH:0015| & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.00 & 74.5 & 10.5 \\
273.0 & \verb|SXS:BBH:0004| & 1.0 & - & - & -0.500 & - & - &-& -0.25 & 66.4 & 11.2 \\
273.0 & \verb|SXS:BBH:0024| & 1.501 & 0.496 & 0.051 & -0.001 & -0.077 & 0.489 & 0.002 & 0.00 & 73.2 & 12.5 \\
272.9 & \verb|SXS:BBH:0198| & 1.202 & - & - & - & - & - &-& 0.00 & 71.2 & 13.3 \\
272.8 & \verb|GT:BBH:900|(*) & 1.2 & 0.400 &-&-& 0.400 &-&-& 0.00 & 71.0 & 22.8 \\
272.8 & \verb|SXS:BBH:0123| & 1.1 & 0.267 & 0.020 & -0.415 & 0.038 & -0.054 & 0.126 & -0.16 & 69.9 & 15.9 \\
272.8 & \verb|SXS:BBH:0021| & 1.5 & 0.496 & 0.053 & - & - & 0.001 & -0.499 & -0.20 & 69.8 & 12.8 \\
272.7 & \verb|SXS:BBH:0147| & 1.0 & 0.404 & 0.294 & -0.001 & -0.404 & -0.294 & -0.001 & -0.00 & 71.5 & 24.4 \\
272.6 & \verb|SXS:BBH:0127| & 1.34 & 0.010 & -0.077 & -0.017 & -0.061 & -0.065 & -0.179 & -0.09 & 72.4 & 14.5 \\
272.6 & \verb|D11_q0.75_a0.6_0.6_PNr500_th1d_n100|(*) & 1.333 & 0.460 & 0.351 & 0.161 & 0.526 & 0.288 & -0.023 & 0.08 & 76.2 & 21.6 \\
272.5 & \verb|UD_D10.01_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& -0.400 & -0.00 & 74.6 & 26.2 \\
272.4 & \verb|D11_q0.75_a-0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& -0.500 & 0.07 & 74.8 & 22.1 \\
272.2 & \verb|SXS:BBH:0115| & 1.07 & 0.019 & 0.013 & -0.204 & 0.243 & -0.067 & 0.291 & 0.04 & 71.8 & 15.0 \\
272.2 & \verb|SXS:BBH:0308| & 1.228 & 0.094 & 0.056 & 0.322 & 0.266 & 0.213 & -0.576 & -0.08 & 72.9 & 17.0 \\
272.1 & \verb|SXS:BBH:0137| & 1.76 & -0.248 & -0.319 & -0.034 & -0.071 & 0.151 & -0.190 & -0.09 & 72.2 & 14.8 \\
272.0 & \verb|SXS:BBH:0125| & 1.27 & 0.012 & 0.045 & -0.058 & 0.389 & 0.241 & 0.070 & -0.00 & 71.6 & 13.9 \\
272.0 & \verb|D11_q0.75_a-0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& -0.500 & -0.21 & 68.7 & 24.1 \\
271.8 & \verb|SXS:BBH:0120| & 1.12 & 0.138 & -0.200 & -0.008 & -0.065 & -0.241 & -0.099 & -0.05 & 69.7 & 14.9 \\
271.8 & \verb|GT:BBH:448| & 1.0 &-&-&-&-&-&-& 0.00 & 75.6 & 21.6 \\
271.8 & \verb|GT:BBH:448| & 1.0 &-&-&-&-&-&-& 0.00 & 75.6 & 21.6 \\
271.8 & \verb|D12.00_q0.85_a0.0_0.0_n100|(*) & 1.176 &-&-& - &-&-& - & -0.00 & 71.3 & 21.1 \\
271.7 & \verb|D11_q0.75_a-0.8500_0.6375_n100| & 1.334 &-&-& 0.638 & 0.001 & 0.003 & -0.851 & -0.00 & 76.2 & 22.2 \\
271.6 & \verb|SXS:BBH:0138| & 1.7 & -0.044 & 0.425 & 0.042 & -0.012 & -0.008 & -0.111 & -0.01 & 72.5 & 14.4 \\
271.6 & \verb|D12_q1.00_a-0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& -0.250 & -0.00 & 70.9 & 21.2 \\
271.6 & \verb|D11_q0.75_a0.8_0.4_PNr500_th1d_n100|(*) & 1.334 & 0.074 & -0.374 & 0.123 & -0.420 & -0.531 & -0.427 & -0.11 & 70.3 & 24.0 \\
271.5 & \verb|SXS:BBH:0116| & 1.08 & -0.078 & 0.065 & 0.033 & 0.185 & 0.007 & 0.103 & 0.07 & 73.2 & 14.3 \\
271.3 & \verb|GT:BBH:370| & 1.15 &-&-&-&-&-&-& 0.00 & 75.5 & 25.3 \\
271.3 & \verb|GT:BBH:370| & 1.15 &-&-&-&-&-&-& 0.00 & 75.5 & 25.3 \\
271.2 & \verb|D10_q0.75_a-0.5_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.500 & -0.07 & 73.6 & 26.8 \\
271.2 & \verb|SXS:BBH:0010| & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.26 & 65.8 & 14.1 \\
271.1 & \verb|GT:BBH:476| & 1.0 &-&-& -0.200 &-&-& -0.200 & -0.20 & 69.2 & 23.8 \\
271.1 & \verb|GT:BBH:476| & 1.0 &-&-& -0.200 &-&-& -0.200 & -0.20 & 69.2 & 23.8 \\
271.1 & \verb|SXS:BBH:0133| & 1.63 & 0.098 & 0.042 & -0.134 & -0.107 & -0.110 & -0.021 & -0.09 & 72.3 & 13.9 \\
271.1 & \verb|D12_q1.00_a-0.25_0.00_n100|(*) & 1.0 &-&-& - &-&-& -0.250 & -0.12 & 67.6 & 22.4 \\
271.0 & \verb|SXS:BBH:0129| & 1.36 & -0.001 & - & 0.088 & 0.193 & -0.289 & -0.075 & 0.02 & 72.0 & 14.4 \\
270.7 & \verb|D10_q0.75_a-0.25_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.250 & 0.04 & 73.6 & 25.4 \\
270.7 & \verb|SXS:BBH:0140| & 1.82 & 0.115 & -0.367 & -0.209 & -0.066 & 0.062 & 0.087 & -0.10 & 71.0 & 14.4 \\
270.6 & \verb|SXS:BBH:0025| & 1.5 & - & - & 0.500 & - & - & -0.499 & 0.10 & 76.7 & 11.1 \\
270.6 & \verb|SXS:BBH:0194| & 1.518 &-& - &-& - &-& - & -0.00 & 72.1 & 14.1 \\
270.6 & \verb|S0_D10.04_q1.3333_a0.45_-0.80_n100| & 1.334 &-&-& 0.450 &-&-& -0.801 & -0.09 & 73.6 & 27.2 \\
270.5 & \verb|RIT:BBH:NQ200TH135PH150| & 2 &-&-&-& -0.490 & 0.283 & -0.566 & -0.19 & 69.4 & 21.7 \\
270.4 & \verb|SXS:BBH:0027| & 1.5 & 0.497 & 0.051 & - & -0.494 & -0.071 &-& 0.00 & 72.2 & 14.0 \\
270.3 & \verb|SXS:BBH:0173| & 1.5 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.14 & 71.3 & 13.3 \\
270.3 & \verb|GW15_D12_q1.22_a0.33_-0.44_m140|(*) & 1.22 & - &-& 0.330 & - &-& -0.440 & -0.02 & 71.5 & 19.7 \\
270.1 & \verb|SXS:BBH:0088| & 1.0 & 0.495 & 0.067 &-&-&-&-& 0.00 & 71.5 & 12.0 \\
270.0 & \verb|D12.25_q0.82_a-0.44_0.33_n100|(*+) & 1.22 &-&-& 0.330 &-&-& -0.440 & -0.02 & 70.8 & 20.8 \\
270.0 & \verb|D10_q0.75_a-0.8_xi0_n100|(*) & 1.333 & 0.538 & 0.056 & 0.590 &-&-& -0.801 & -0.01 & 76.9 & 25.9 \\
269.9 & \verb|GT:BBH:477| & 1.5 &-&-&-&-&-&-& 0.00 & 76.1 & 21.5 \\
269.9 & \verb|GT:BBH:477| & 1.5 &-&-&-&-&-&-& 0.00 & 76.1 & 21.5 \\
269.8 & \verb|D10_q0.75_a0.5_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.500 & 0.07 & 76.4 & 24.3 \\
269.8 & \verb|GT:BBH:372| & 1.45 &-&-&-&-&-&-& 0.00 & 75.8 & 25.3 \\
269.8 & \verb|GT:BBH:372| & 1.45 &-&-&-&-&-&-& 0.00 & 75.8 & 25.3 \\
269.7 & \verb|D10_q0.75_a0.25_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.250 & -0.04 & 73.6 & 25.6 \\
269.6 & \verb|D11_q0.75_a0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& 0.500 & -0.07 & 68.6 & 24.5 \\
269.6 & \verb|SXS:BBH:0119| & 1.12 & -0.012 & 0.068 & 0.260 & 0.078 & -0.003 & 0.006 & 0.14 & 78.4 & 13.5 \\
269.6 & \verb|GT:BBH:546| & 1.0 &-&-&-&-&-& 0.200 & 0.10 & 74.6 & 21.9 \\
269.6 & \verb|GT:BBH:546| & 1.0 &-&-&-&-&-& 0.200 & 0.10 & 74.6 & 21.9 \\
269.6 & \verb|D10_q0.75_a0.8_xi0_n100|(*) & 1.333 & 0.528 & 0.062 & -0.598 &-&-& 0.801 & 0.00 & 71.6 & 27.7 \\
269.6 & \verb|RIT:BBH:NQ200TH135PH0| & 2 &-&-&-& 0.566 &-& -0.566 & -0.19 & 69.4 & 19.4 \\
269.6 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 75.9 & 24.9 \\
269.6 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 75.9 & 24.9 \\
269.6 & \verb|SXS:BBH:0169| & 2.0 & - & - &-&-&-&-& 0.00 & 74.0 & 15.9 \\
269.5 & \verb|U0_D9.53_q1.00_a0.0_n100| & 1.0 &-&-& - &-&-& - & -0.00 & 74.3 & 28.3 \\
269.4 & \verb|D9_q1.3_a0.0_m160| & 1.3 &-&-& - & - & - & - & -0.00 & 73.1 & 31.6 \\
269.4 & \verb|SXS:BBH:0082| & 1.501 & 0.496 & 0.053 & - &-&-&-& -0.00 & 75.7 & 13.7 \\
269.2 & \verb|RIT:BBH:NQ200TH135PH120| & 2 &-&-&-& -0.283 & 0.490 & -0.566 & -0.19 & 69.4 & 21.4 \\
269.1 & \verb|SXS:BBH:0145| & 1.96 & 0.017 & 0.029 & -0.049 & 0.091 & -0.002 & 0.027 & -0.02 & 72.8 & 13.9 \\
269.0 & \verb|SXS:BBH:0134| & 1.63 & -0.230 & 0.184 & -0.012 & -0.001 & 0.032 & 0.176 & 0.06 & 73.5 & 13.7 \\
269.0 & \verb|D11_q0.75_a0.8500_-0.6375_n100|(*) & 1.334 &-&-& -0.638 & -0.001 & 0.003 & 0.851 & 0.00 & 73.7 & 23.1 \\
268.9 & \verb|d0_D10.52_q1.3333_a-0.25_n100| & 1.333 &-&-& -0.250 &-&-& - & -0.14 & 70.2 & 25.7 \\
268.8 & \verb|SXS:BBH:0019| & 1.5 & - & - & -0.500 & - & - & 0.499 & -0.10 & 68.4 & 13.6 \\
268.8 & \verb|SXS:BBH:0097| & 1.501 & 0.495 & 0.065 & 0.001 &-&-&-& 0.00 & 71.5 & 15.3 \\
268.7 & \verb|RIT:BBH:NQ200TH135PH60| & 2 &-&-&-& 0.283 & 0.490 & -0.566 & -0.19 & 69.4 & 19.6 \\
268.7 & \verb|SXS:BBH:0101| & 1.501 &-& - & -0.500 & - & - &-& -0.30 & 65.2 & 17.7 \\
268.7 & \verb|SXS:BBH:0023| & 1.501 & 0.497 & 0.051 & 0.001 & 0.077 & -0.489 &-& 0.00 & 75.7 & 13.1 \\
268.7 & \verb|SXS:BBH:0135| & 1.64 & -0.110 & 0.027 & 0.024 & 0.211 & -0.144 & -0.229 & -0.07 & 69.9 & 14.9 \\
268.7 & \verb|GT:BBH:876| & 1.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.05 & 73.8 & 30.4 \\
268.6 & \verb|SXS:BBH:0126| & 1.29 & -0.250 & -0.237 & 0.091 & -0.358 & 0.172 & 0.215 & 0.15 & 76.0 & 14.3 \\
268.5 & \verb|GW15_D12_q1.19_a0.42_-0.38_m140|(*) & 1.19 & - &-& 0.420 & - &-& -0.380 & 0.05 & 73.4 & 18.8 \\
268.5 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 73.1 & 30.7 \\
268.5 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 73.1 & 30.7 \\
268.4 & \verb|RIT:BBH:NQ200TH135PH90| & 2 &-&-&-&-& 0.566 & -0.566 & -0.19 & 71.3 & 20.4 \\
268.4 & \verb|SXS:BBH:0098| & 1.501 & 0.486 & 0.114 & 0.002 &-&-&-& 0.00 & 75.7 & 11.4 \\
268.3 & \verb|SXS:BBH:0149| & 1.0 &-& - & -0.200 & - &-& -0.200 & -0.20 & 65.7 & 15.3 \\
268.3 & \verb|D10_q0.75_a0.0_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& - & 0.14 & 76.6 & 24.0 \\
268.3 & \verb|D11_q0.75_a0.8_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.308 & 0.640 & 0.369 & -0.006 & 0.763 & -0.243 & 0.11 & 78.1 & 21.8 \\
268.2 & \verb|D11.50_q0.60_a0.0_0.0_n100|(*) & 1.667 &-&-& - &-&-& - & -0.00 & 72.1 & 21.6 \\
268.1 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 74.7 & 30.1 \\
268.1 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 74.7 & 30.1 \\
268.1 & \verb|RIT:BBH:NQ200TH135PH30| & 2 &-&-&-& 0.490 & 0.283 & -0.566 & -0.19 & 71.3 & 18.4 \\
268.1 & \verb|SXS:BBH:0130| & 1.38 & 0.164 & 0.037 & -0.014 & 0.293 & 0.060 & 0.343 & 0.14 & 76.0 & 13.0 \\
268.0 & \verb|D10_q0.75_a-0.8_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.801 & 0.11 & 80.3 & 24.7 \\
268.0 & \verb|D12_q1.00_a-0.25_-0.25_n100|(*) & 1.0 &-&-& -0.250 &-&-& -0.250 & -0.25 & 64.5 & 23.6 \\
267.8 & \verb|SXS:BBH:0078| & 1.501 & 0.497 & 0.049 & - &-&-&-& -0.00 & 75.7 & 11.2 \\
267.7 & \verb|RIT:BBH:NQ200TH90PH0| & 2 &-&-&-& 0.800 &-&-& 0.00 & 74.3 & 20.7 \\
267.7 & \verb|S0_D9.96_q1.3333_a-0.45_0.80_n100| & 1.334 &-&-& -0.450 &-&-& 0.801 & 0.09 & 73.6 & 27.0 \\
267.7 & \verb|UD_D9.52_q1.00_a0.6_rl10_opt3_n100| & 1.0 &-&-& 0.600 &-&-& -0.600 & -0.00 & 74.3 & 29.2 \\
267.6 & \verb|SXS:BBH:0124| & 1.26 & 0.250 & -0.058 & 0.071 & 0.075 & -0.095 & 0.286 & 0.17 & 76.5 & 13.2 \\
267.6 & \verb|SXS:BBH:0142| & 1.91 & -0.291 & -0.230 & -0.052 & 0.004 & 0.001 & 0.110 & 0.00 & 76.0 & 13.5 \\
267.5 & \verb|RIT:BBH:NQ200TH90PH30| & 2 &-&-&-& 0.693 & 0.400 &-& 0.00 & 74.3 & 21.5 \\
267.2 & \verb|SXS:BBH:0306|(*) & 1.31 & - &-& 0.961 & - & - & -0.899 & 0.16 & 80.6 & 16.2 \\
267.2 & \verb|RIT:BBH:NQ200TH90PH90| & 2 &-&-&-&-& 0.800 &-& 0.00 & 74.3 & 22.1 \\
267.1 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 75.0 & 30.9 \\
267.0 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 75.4 & 29.9 \\
267.0 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 75.4 & 29.9 \\
266.7 & \verb|D10_q0.50_a-0.8_xi0_n100|(*) & 2.0 & 0.696 & 0.059 & 0.392 &-& -0.006 & -0.801 & -0.01 & 77.5 & 24.7 \\
266.7 & \verb|GT:BBH:885| & 1.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.00 & 73.3 & 31.0 \\
266.7 & \verb|SXS:BBH:0146| & 1.97 & -0.156 & -0.102 & -0.037 & -0.098 & 0.027 & -0.357 & -0.14 & 69.9 & 15.0 \\
266.7 & \verb|UD_D9.51_q1.00_a0.8_rl10_opt1_n100| & 1.0 &-&-& 0.801 &-&-& -0.801 & -0.00 & 74.3 & 29.7 \\
266.7 & \verb|Rflop_r500_d11_q0.7_a0.8_m088|(*) & 1.428 & 0.603 & 0.445 & 0.283 & 0.747 & 0.278 & -0.079 & 0.13 & 80.7 & 20.8 \\
266.5 & \verb|GT:BBH:891| & 2.0 & 0.328 & -0.270 & -0.423 & -0.425 & -0.076 & 0.417 & -0.14 & 66.3 & 34.0 \\
266.4 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 76.7 & 25.0 \\
266.4 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 76.7 & 25.0 \\
266.3 & \verb|SXS:BBH:0161| & 1.0 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.29 & 64.7 & 14.6 \\
266.1 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 74.6 & 30.9 \\
266.1 & \verb|RIT:BBH:NQ50TH90PH90| & 2.0 &-& 0.800 &-&-&-&-& 0.00 & 75.9 & 16.2 \\
266.1 & \verb|RIT:BBH:NQ200TH90PH120| & 2 &-&-&-& -0.400 & 0.693 &-& 0.00 & 74.3 & 20.6 \\
266.0 & \verb|RIT:BBH:NQ200TH90PH60| & 2 &-&-&-& 0.400 & 0.693 &-& 0.00 & 75.9 & 22.2 \\
266.0 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 71.7 & 31.2 \\
266.0 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 71.7 & 31.2 \\
266.0 & \verb|SXS:BBH:0122| & 1.17 & -0.019 & 0.061 & -0.477 & 0.041 & 0.050 & -0.364 & -0.42 & 62.2 & 17.1 \\
265.8 & \verb|D12.50_q0.50_a-0.50_-0.10_n100|(*) & 2.0 &-&-& -0.100 &-&-& -0.500 & -0.23 & 67.5 & 20.9 \\
265.7 & \verb|RIT:BBH:NQ200TH90PH150| & 2 &-&-&-& -0.693 & 0.400 &-& 0.00 & 74.3 & 18.8 \\
265.5 & \verb|S0_D9.87_q2.00_a0.20_-0.80_n100| & 2.001 &-&-& 0.200 & -0.015 & -0.007 & -0.800 & -0.13 & 74.5 & 27.4 \\
265.4 & \verb|GT:BBH:866| & 1.0 & -0.354 & 0.233 & 0.424 & 0.494 & -0.341 & -0.001 & 0.21 & 79.5 & 34.1 \\
265.2 & \verb|DU_D10.86_q1.3333_a-0.8_opt1_n100| & 1.333 &-&-& -0.801 &-&-& 0.801 & -0.11 & 70.2 & 24.9 \\
265.1 & \verb|D11_q0.75_a0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& 0.500 & 0.21 & 78.1 & 20.3 \\
265.1 & \verb|GT:BBH:420| & 1.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.0 & 20.2 \\
265.1 & \verb|GT:BBH:420| & 1.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.0 & 20.2 \\
265.0 & \verb|D11_q0.50_a0.0_0.0_n100|(*) & 2.0 &-&-& - &-&-& - & -0.00 & 76.4 & 21.5 \\
265.0 & \verb|SXS:BBH:0141| & 1.84 & -0.182 & 0.052 & 0.086 & -0.093 & 0.124 & 0.040 & 0.07 & 78.7 & 12.9 \\
264.9 & \verb|SXS:BBH:0150| & 1.0 &-& - & 0.200 & - &-& 0.200 & 0.20 & 80.9 & 12.3 \\
264.7 & \verb|GT:BBH:893| & 2.0 & -0.328 & 0.270 & -0.423 & 0.425 & 0.076 & 0.417 & -0.14 & 63.8 & 36.7 \\
264.7 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 75.4 & 29.4 \\
264.7 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 75.4 & 29.4 \\
264.6 & \verb|D9_q1.6_a0.0_m160| & 1.6 &-&-& - & - & - & - & -0.00 & 72.0 & 31.8 \\
264.6 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 73.1 & 30.4 \\
264.6 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 73.1 & 30.4 \\
264.5 & \verb|D11_q1.00_a0.0_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& - & -0.25 & 67.8 & 25.2 \\
264.4 & \verb|SXS:BBH:0022| & 1.5 & 0.497 & 0.049 & - & 0.001 & -0.001 & 0.499 & 0.20 & 78.4 & 12.5 \\
264.4 & \verb|SXS:BBH:0144| & 1.94 & 0.061 & 0.104 & -0.288 & -0.050 & -0.022 & 0.215 & -0.12 & 69.0 & 14.4 \\
264.4 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 77.2 & 21.7 \\
264.4 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 77.2 & 21.7 \\
264.3 & \verb|RIT:BBH:NQ50TH90PH120| & 2.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 74.3 & 17.1 \\
264.3 & \verb|SXS:BBH:0132| & 1.63 & -0.005 & -0.114 & -0.007 & 0.041 & -0.087 & 0.310 & 0.11 & 75.0 & 13.0 \\
264.2 & \verb|GT:BBH:856| & 2.0 & 0.106 &-& 0.106 & -0.424 &-& -0.424 & -0.07 & 70.0 & 29.3 \\
264.0 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 75.3 & 30.3 \\
264.0 & \verb|EMu0_D9.16_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& - & 0.20 & 79.2 & 28.1 \\
264.0 & \verb|GT:BBH:378| & 2.05 &-&-&-&-&-&-& 0.00 & 77.3 & 24.7 \\
264.0 & \verb|GT:BBH:378| & 2.05 &-&-&-&-&-&-& 0.00 & 77.3 & 24.7 \\
264.0 & \verb|D11_q0.50_a0.50_-0.50_n100|(*) & 2.0 &-&-& -0.500 &-&-& 0.500 & -0.17 & 69.2 & 24.8 \\
263.9 & \verb|GT:BBH:547| & 1.0 &-&-&-&-&-& 0.400 & 0.20 & 78.2 & 20.7 \\
263.9 & \verb|GT:BBH:547| & 1.0 &-&-&-&-&-& 0.400 & 0.20 & 78.2 & 20.7 \\
263.9 & \verb|RIT:BBH:NQ50TH90PH150| & 2.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 78.6 & 17.3 \\
263.9 & \verb|GT:BBH:872| & 2.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.14 & 81.2 & 24.5 \\
263.8 & \verb|SXS:BBH:0005| & 1.0 &-&-& 0.499 & - & - &-& 0.25 & 81.0 & 10.6 \\
263.7 & \verb|D9_q2.0_a0.6_0.6_th180_r100_res140_CE| & 2.0 & - & - & -0.600 & - &-& 0.601 & -0.20 & 64.8 & 35.1 \\
263.4 & \verb|GT:BBH:405| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 78.9 & 23.8 \\
263.4 & \verb|GT:BBH:405| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 78.9 & 23.8 \\
263.4 & \verb|RIT:BBH:NQ50TH90PH0| & 2.0 & 0.800 &-&-&-&-&-& 0.00 & 76.1 & 15.3 \\
263.2 & \verb|GT:BBH:894| & 2.0 & -0.500 & 0.324 & -0.070 & 0.188 & 0.556 & 0.122 & -0.01 & 74.0 & 30.3 \\
263.2 & \verb|RIT:BBH:NQ50TH90PH60| & 2.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 74.3 & 15.5 \\
263.2 & \verb|D11_q0.75_a-0.8_0.0_n100|(*) & 1.334 &-&-&-&-&-& -0.801 & -0.34 & 63.6 & 27.4 \\
263.1 & \verb|SXS:BBH:0148| & 1.0 &-&-& -0.438 & - & - & -0.438 & -0.44 & 61.0 & 16.7 \\
263.0 & \verb|GT:BBH:873| & 1.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.08 & 75.0 & 28.5 \\
263.0 & \verb|D9_q1.9_a0.0_m160| & 1.9 &-&-& - &-&-& - & -0.00 & 74.6 & 30.6 \\
262.9 & \verb|D12_q1.00_a0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& 0.250 & 0.25 & 79.0 & 18.9 \\
262.9 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 72.1 & 31.7 \\
262.9 & \verb|GT:BBH:413| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 80.7 & 23.4 \\
262.9 & \verb|GT:BBH:413| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 80.7 & 23.4 \\
262.8 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 76.0 & 29.1 \\
262.8 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 76.0 & 29.1 \\
262.7 & \verb|D11_q1.00_a0.0_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& - & -0.40 & 61.2 & 28.8 \\
262.5 & \verb|SXS:BBH:0139| & 1.82 & 0.032 & -0.342 & 0.210 & -0.132 & -0.047 & -0.042 & 0.12 & 76.8 & 13.2 \\
262.4 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.8 & 23.1 \\
262.4 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.8 & 23.1 \\
262.4 & \verb|RIT:BBH:NQ50TH90PH30| & 2.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 74.3 & 15.8 \\
262.1 & \verb|GT:BBH:871| & 1.5 & -0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 77.4 & 25.3 \\
262.1 & \verb|D10_q0.50_a0.8_xi0_n100|(*) & 2.0 & 0.689 & 0.062 & -0.403 & 0.012 & 0.006 & 0.800 & -0.00 & 72.4 & 26.6 \\
262.1 & \verb|GT:BBH:877| & 1.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.12 & 77.5 & 26.6 \\
261.9 & \verb|RIT:BBH:NQ50TH135PH150| & 2.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 61.2 & 21.1 \\
261.9 & \verb|RIT:BBH:NQ66TH60PH120| & 1.5 & -0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 79.5 & 31.8 \\
261.7 & \verb|D11_q0.75_a-0.5_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.500 & 0.24 & 81.4 & 20.1 \\
261.6 & \verb|GT:BBH:564| & 1.0 &-&-& -0.400 &-&-& -0.400 & -0.40 & 64.7 & 26.2 \\
261.6 & \verb|GT:BBH:564| & 1.0 &-&-& -0.400 &-&-& -0.400 & -0.40 & 64.7 & 26.2 \\
261.6 & \verb|RIT:BBH:NQ50TH135PH120| & 2.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 63.8 & 19.5 \\
261.6 & \verb|GT:BBH:897| & 2.0 & 0.500 & -0.324 & -0.070 & -0.188 & -0.556 & 0.122 & -0.01 & 71.2 & 30.2 \\
261.5 & \verb|GT:BBH:865| & 1.0 & -0.096 & 0.467 & 0.364 & 0.208 & 0.562 & 0.033 & 0.20 & 79.2 & 35.0 \\
261.4 & \verb|GT:BBH:858| & 1.5 & -0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 76.6 & 26.6 \\
261.2 & \verb|RIT:BBH:NQ50TH135PH90| & 2.0 &-& 0.566 & -0.566 &-&-&-& -0.38 & 63.3 & 22.6 \\
261.1 & \verb|GT:BBH:848| & 1.5 & 0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 77.0 & 26.6 \\
260.9 & \verb|D11_q0.75_a0.0_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& - & -0.29 & 66.9 & 25.6 \\
260.9 & \verb|GT:BBH:896| & 2.0 & -0.511 & 0.009 & 0.314 & -0.565 & -0.025 & -0.200 & 0.14 & 82.0 & 25.4 \\
260.8 & \verb|GT:BBH:380| & 2.35 &-&-&-&-&-&-& 0.00 & 78.1 & 24.5 \\
260.8 & \verb|GT:BBH:380| & 2.35 &-&-&-&-&-&-& 0.00 & 78.1 & 24.5 \\
260.8 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 73.5 & 30.0 \\
260.8 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 73.5 & 30.0 \\
260.5 & \verb|RIT:BBH:NQ50TH135PH0| & 2.0 & 0.566 &-& -0.566 &-&-&-& -0.38 & 62.7 & 24.0 \\
260.4 & \verb|RIT:BBH:NQ200TH60PH60| & 2 &-&-&-& 0.346 & 0.600 & 0.400 & 0.13 & 76.2 & 34.0 \\
260.2 & \verb|RIT:BBH:NQ66TH60PH150| & 1.5 & -0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 83.5 & 31.3 \\
260.1 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 75.0 & 30.3 \\
260.1 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 74.8 & 29.3 \\
260.1 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 74.8 & 29.3 \\
260.1 & \verb|RIT:BBH:NQ66TH60PH30| & 1.5 & 0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 78.8 & 32.7 \\
260.0 & \verb|GT:BBH:847| & 1.5 & 0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 77.5 & 30.2 \\
259.9 & \verb|RIT:BBH:NQ200TH60PH150| & 2 &-&-&-& -0.600 & 0.346 & 0.400 & 0.13 & 75.7 & 35.2 \\
259.9 & \verb|SXS:BBH:0128| & 1.35 & 0.041 & 0.005 & 0.134 & -0.048 & 0.103 & 0.397 & 0.25 & 82.7 & 12.7 \\
259.9 & \verb|GT:BBH:870| & 1.5 &-& 0.600 &-& -0.424 &-& 0.424 & 0.17 & 80.5 & 25.8 \\
259.9 & \verb|RIT:BBH:NQ50TH135PH60| & 2.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 63.7 & 27.0 \\
259.8 & \verb|SXS:BBH:0191| & 2.507 & - &-& - &-&-&-& -0.00 & 78.1 & 12.7 \\
259.6 & \verb|SXS:BBH:0164| & 1.0 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.33 & 85.2 & 12.3 \\
259.6 & \verb|GT:BBH:895| & 2.0 & 0.511 & -0.009 & 0.314 & 0.565 & 0.025 & -0.200 & 0.14 & 80.0 & 28.8 \\
259.5 & \verb|RIT:BBH:NQ66TH60PH90| & 1.5 &-& 0.693 & 0.400 &-&-&-& 0.24 & 82.3 & 30.0 \\
259.4 & \verb|EMu0_D8.98_q1.00_a0.6_n100| & 1.0 &-&-& 0.600 &-&-& - & 0.30 & 85.7 & 26.6 \\
259.4 & \verb|GT:BBH:878| & 2.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.16 & 83.2 & 23.7 \\
259.2 & \verb|RIT:BBH:NQ66TH60PH60| & 1.5 & 0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 81.6 & 30.5 \\
259.2 & \verb|RIT:BBH:NQ200TH60PH90| & 2 &-&-&-&-& 0.693 & 0.400 & 0.13 & 74.2 & 34.8 \\
259.2 & \verb|D11_q0.75_a0.4_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.597 & -0.231 & 0.481 & -0.346 & 0.200 & 0.003 & 0.28 & 83.0 & 19.3 \\
259.1 & \verb|SXS:BBH:0028| & 1.501 & -0.001 & 0.001 & 0.500 & 0.078 & -0.489 & 0.001 & 0.30 & 83.6 & 11.4 \\
259.1 & \verb|Del0_D10.01_q2.00_a-0.4_-0.8_n100| & 2.001 &-&-& -0.400 & -0.011 & 0.003 & -0.800 & -0.53 & 58.8 & 36.8 \\
259.1 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 76.2 & 29.6 \\
259.0 & \verb|D9_q2.2_a0.0_m160| & 2.2 &-&-& - &-&-& - & -0.00 & 76.3 & 29.7 \\
258.8 & \verb|SXS:BBH:0011| & 1.501 & 0.248 & 0.026 & 0.433 &-&-&-& 0.26 & 84.4 & 11.1 \\
258.7 & \verb|RIT:BBH:NQ50TH135PH30| & 2.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 63.0 & 27.7 \\
258.7 & \verb|S0_D9.75_q2.00_a-0.20_0.80_n100| & 2.001 &-&-& -0.200 & 0.015 & -0.006 & 0.800 & 0.13 & 76.3 & 26.4 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH0| & 2 &-&-&-& 0.693 &-& 0.400 & 0.13 & 74.5 & 36.5 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH120| & 2 &-&-&-& -0.346 & 0.600 & 0.400 & 0.13 & 74.0 & 35.2 \\
258.5 & \verb|RIT:BBH:NQ33TH100PH120| & 3 & -0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 73.2 & 27.8 \\
258.5 & \verb|SXS:BBH:0026| & 1.5 & - &-& 0.500 & -0.494 & -0.071 & - & 0.30 & 83.7 & 11.7 \\
258.5 & \verb|RIT:BBH:NQ200TH60PH30| & 2 &-&-&-& 0.600 & 0.346 & 0.400 & 0.13 & 74.4 & 35.7 \\
258.4 & \verb|D10_q0.33_a-0.8_xi0_n100|(*) & 2.999 & 0.757 & 0.030 & 0.259 &-&-& -0.800 & -0.01 & 84.6 & 22.3 \\
258.4 & \verb|GT:BBH:859| & 2.0 & -0.106 &-& -0.106 & 0.424 &-& 0.424 & 0.07 & 76.8 & 27.4 \\
258.3 & \verb|D10_q0.50_a-0.50_0.50_n100|(*) & 2.0 &-&-& 0.500 &-&-& -0.500 & 0.17 & 85.0 & 21.6 \\
258.2 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.5 & 23.2 \\
258.2 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.5 & 23.2 \\
258.0 & \verb|SXS:BBH:0118| & 1.12 & -0.010 & 0.030 & 0.343 & -0.190 & -0.146 & 0.258 & 0.30 & 81.1 & 13.1 \\
257.7 & \verb|SXS:BBH:0136| & 1.68 & 0.118 & -0.114 & 0.326 & -0.145 & -0.071 & 0.145 & 0.26 & 84.2 & 11.8 \\
257.7 & \verb|GT:BBH:565| & 2.5 &-&-&-&-&-&-& 0.00 & 78.8 & 20.7 \\
257.7 & \verb|GT:BBH:565| & 2.5 &-&-&-&-&-&-& 0.00 & 78.8 & 20.7 \\
257.7 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 76.5 & 29.4 \\
257.6 & \verb|GT:BBH:867| & 1.0 & 0.599 & 0.030 & - & -0.599 & -0.030 & - & 0.00 & 72.1 & 40.1 \\
257.6 & \verb|SXS:BBH:0035| & 3.001 & 0.499 & 0.029 & - &-& - &-& -0.00 & 78.9 & 11.5 \\
257.4 & \verb|D11_q0.75_a0.0_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& - & 0.29 & 81.5 & 19.9 \\
257.3 & \verb|RIT:BBH:NQ66TH60PH0| & 1.5 & 0.693 &-& 0.400 &-&-&-& 0.24 & 77.5 & 33.7 \\
257.2 & \verb|GT:BBH:864| & 1.0 & -0.269 & -0.536 & -0.014 & -0.269 & -0.536 & -0.014 & -0.01 & 72.2 & 41.6 \\
257.1 & \verb|GT:BBH:549| & 1.0 &-&-& 0.200 &-&-& 0.400 & 0.30 & 82.9 & 19.5 \\
257.1 & \verb|GT:BBH:549| & 1.0 &-&-& 0.200 &-&-& 0.400 & 0.30 & 82.9 & 19.5 \\
257.0 & \verb|GT:BBH:548| & 1.0 &-&-&-&-&-& 0.600 & 0.30 & 82.5 & 19.4 \\
257.0 & \verb|GT:BBH:548| & 1.0 &-&-&-&-&-& 0.600 & 0.30 & 82.5 & 19.4 \\
256.9 & \verb|RIT:BBH:NQ33TH100PH0| & 3 & 0.788 &-& -0.139 &-&-&-& -0.10 & 73.2 & 24.6 \\
256.7 & \verb|D12.00_q0.50_a0.50_0.10_n100|(*) & 2.0 &-&-& 0.100 &-&-& 0.500 & 0.23 & 80.8 & 18.1 \\
256.6 & \verb|SXS:BBH:0053| & 3.0 & 0.494 & 0.075 & 0.001 & -0.464 & -0.184 & -0.003 & 0.00 & 78.9 & 14.6 \\
256.6 & \verb|D10_q0.33_a0.8_xi0_n120|(*) & 2.999 & 0.754 & 0.031 & -0.268 &-&-& 0.800 & -0.00 & 70.9 & 26.7 \\
256.5 & \verb|d0_D10.50_q2.00_a-0.5_n100| & 2.0 &-&-& -0.500 &-&-& - & -0.33 & 65.8 & 28.2 \\
256.4 & \verb|GT:BBH:636| & 3.0 & -0.500 & 0.019 & -0.001 &-&-&-& -0.00 & 76.3 & 33.4 \\
256.4 & \verb|GT:BBH:890| & 2.0 &-&-& 0.600 &-&-& -0.600 & 0.20 & 82.5 & 25.1 \\
256.3 & \verb|RIT:BBH:NQ33TH100PH90| & 3 &-& 0.788 & -0.139 &-&-&-& -0.10 & 73.4 & 27.5 \\
256.2 & \verb|RIT:BBH:NQ33TH75PH60| & 3 & 0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 86.0 & 24.2 \\
256.1 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 74.1 & 29.5 \\
256.1 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 74.1 & 29.5 \\
256.1 & \verb|SXS:BBH:0030| & 3.0 &-&-&-& - &-&-& 0.00 & 78.9 & 14.5 \\
255.9 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 78.3 & 27.8 \\
255.9 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 78.3 & 27.8 \\
255.9 & \verb|RIT:BBH:NQ33TH75PH30| & 3 & 0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 83.8 & 23.5 \\
255.8 & \verb|RIT:BBH:NQ33TH75PH0| & 3 & 0.773 &-& 0.207 &-&-&-& 0.16 & 85.5 & 23.2 \\
255.8 & \verb|RIT:BBH:NQ33TH100PH60| & 3 & 0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 75.3 & 26.8 \\
255.8 & \verb|GT:BBH:724| & 3.0 & -0.464 & 0.182 & 0.046 &-&-&-& 0.03 & 77.5 & 33.0 \\
255.7 & \verb|SXS:BBH:0020| & 1.5 &-& - & 0.500 & 0.494 & 0.071 & - & 0.30 & 85.8 & 11.3 \\
255.6 & \verb|RIT:BBH:NQ33TH100PH30| & 3 & 0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 72.2 & 26.2 \\
255.6 & \verb|RIT:BBH:NQ33TH75PH90| & 3 &-& 0.773 & 0.207 &-&-&-& 0.16 & 84.0 & 26.0 \\
255.4 & \verb|RIT:BBH:NQ33TH100PH150| & 3 & -0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 75.2 & 26.9 \\
255.3 & \verb|SXS:BBH:0052| & 3.0 & 0.494 & 0.073 & 0.001 & 0.001 & 0.008 & -0.499 & -0.12 & 74.2 & 15.5 \\
255.2 & \verb|D11_q0.75_a0.0_-0.8_n100|(*) & 1.333 &-&-& -0.801 &-&-& - & -0.46 & 58.8 & 30.0 \\
255.2 & \verb|DU_D10.90_q2.00_a-0.8_rl10_opt1_n100| & 2.0 &-&-& -0.801 & - & -0.004 & 0.801 & -0.27 & 63.9 & 27.8 \\
255.0 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 75.7 & 28.6 \\
255.0 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 75.7 & 28.6 \\
255.0 & \verb|GT:BBH:860| & 1.0 & 0.109 & 0.481 & 0.342 & 0.460 & -0.287 & 0.257 & 0.30 & 80.4 & 33.5 \\
254.9 & \verb|RIT:BBH:NQ200TH30PH0| & 2 &-&-&-& 0.400 &-& 0.693 & 0.23 & 80.8 & 33.5 \\
254.7 & \verb|RIT:BBH:NQ200TH30PH60| & 2 &-&-&-& 0.200 & 0.346 & 0.693 & 0.23 & 79.7 & 33.0 \\
254.6 & \verb|RIT:BBH:NQ200TH30PH30| & 2 &-&-&-& 0.346 & 0.200 & 0.693 & 0.23 & 80.7 & 33.0 \\
254.6 & \verb|SXS:BBH:0009| & 1.501 & - &-& 0.500 & - & - &-& 0.30 & 85.8 & 13.5 \\
254.6 & \verb|SXS:BBH:0042| & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.32 & 66.5 & 21.6 \\
254.5 & \verb|SXS:BBH:0143| & 1.92 & -0.094 & -0.062 & 0.436 & -0.019 & -0.434 & -0.085 & 0.26 & 85.8 & 11.2 \\
254.3 & \verb|RIT:BBH:NQ33TH135PH150| & 3 & -0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 60.6 & 37.7 \\
254.2 & \verb|RIT:BBH:NQ200TH30PH90| & 2 &-&-&-&-& 0.400 & 0.693 & 0.23 & 77.9 & 33.3 \\
254.1 & \verb|RIT:BBH:NQ33TH135PH60| & 3 & 0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 59.8 & 38.4 \\
254.0 & \verb|RIT:BBH:NQ200TH30PH120| & 2 &-&-&-& -0.200 & 0.346 & 0.693 & 0.23 & 78.0 & 33.2 \\
254.0 & \verb|SXS:BBH:0050| & 3.0 & 0.494 & 0.072 & 0.002 & 0.467 & 0.176 & 0.005 & 0.00 & 80.9 & 13.9 \\
253.9 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 77.2 & 28.9 \\
253.9 & \verb|D11_q0.75_a0.8_0.0_n100|(*) & 1.334 &-&-& - &-&-& 0.801 & 0.34 & 85.2 & 19.1 \\
253.7 & \verb|SXS:BBH:0034| & 3.001 & 0.497 & 0.047 & 0.001 &-& - &-& 0.00 & 80.9 & 14.1 \\
253.7 & \verb|RIT:BBH:NQ33TH135PH120| & 3 & -0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 57.0 & 39.3 \\
253.7 & \verb|RIT:BBH:NQ33TH135PH90| & 3 &-& 0.566 & -0.566 &-&-&-& -0.42 & 58.8 & 37.7 \\
253.6 & \verb|SXS:BBH:0200| & 3.272 & - &-& - &-&-& - & -0.00 & 78.7 & 14.1 \\
253.6 & \verb|SXS:BBH:0037| & 3.001 & 0.498 & 0.038 &-&-& - &-& 0.00 & 81.0 & 11.9 \\
253.5 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 79.1 & 27.3 \\
253.5 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 79.1 & 27.3 \\
253.4 & \verb|SXS:BBH:0044| & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.00 & 81.0 & 17.5 \\
253.3 & \verb|GT:BBH:609| & 3.0 & -0.335 & -0.317 & -0.192 &-&-&-& -0.14 & 63.9 & 42.5 \\
253.3 & \verb|RIT:BBH:NQ33TH135PH30| & 3 & 0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 58.8 & 37.9 \\
253.3 & \verb|RIT:BBH:NQ200TH30PH150| & 2 &-&-&-& -0.346 & 0.200 & 0.693 & 0.23 & 77.9 & 33.5 \\
253.2 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 78.9 & 27.0 \\
253.2 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 78.9 & 27.0 \\
253.2 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 78.0 & 28.3 \\
253.1 & \verb|GT:BBH:657| & 3.0 & -0.201 & 0.405 & 0.213 &-&-&-& 0.16 & 76.6 & 35.2 \\
253.1 & \verb|RIT:BBH:NQ33TH75PH120| & 3 & -0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 84.3 & 26.9 \\
253.0 & \verb|RIT:BBH:NQ33TH135PH0| & 3 & 0.566 &-& -0.566 &-&-&-& -0.42 & 58.8 & 37.6 \\
253.0 & \verb|GT:BBH:680| & 3.0 & 0.500 & -0.019 & -0.001 &-&-&-& -0.00 & 74.8 & 33.9 \\
252.8 & \verb|D11.25_q0.3333_a0.0_0.0_n100|(*) & 3.0 &-&-&-&-&-& - & 0.00 & 76.6 & 20.2 \\
252.8 & \verb|GT:BBH:605| & 3.0 & 0.464 & -0.182 & 0.046 &-&-&-& 0.03 & 77.0 & 31.5 \\
252.8 & \verb|SXS:BBH:0049| & 3.0 & 0.494 & 0.073 & 0.001 & - & -0.008 & 0.499 & 0.13 & 80.9 & 14.0 \\
252.5 & \verb|GT:BBH:881| & 2.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.18 & 85.3 & 23.9 \\
252.3 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 78.6 & 28.0 \\
252.2 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 76.3 & 28.1 \\
252.2 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 76.3 & 28.1 \\
251.8 & \verb|RIT:BBH:NQ25TH90PH150| & 4.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 74.7 & 25.2 \\
251.7 & \verb|DD_D10.99_q2.00_a-0.8_n100| & 2.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 53.4 & 35.4 \\
251.6 & \verb|GT:BBH:874| & 3.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.21 & 88.3 & 24.0 \\
251.6 & \verb|GT:BBH:453| & 3.0 &-&-&-&-&-&-& 0.00 & 80.5 & 20.0 \\
251.6 & \verb|GT:BBH:453| & 3.0 &-&-&-&-&-&-& 0.00 & 80.5 & 20.0 \\
251.5 & \verb|GT:BBH:882| & 2.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.20 & 87.3 & 23.7 \\
251.5 & \verb|D11_q0.75_a-0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& -0.500 & -0.50 & 57.8 & 30.6 \\
251.4 & \verb|GT:BBH:857| & 3.0 & 0.047 &-& 0.047 & -0.424 &-& -0.424 & -0.07 & 76.3 & 28.1 \\
251.3 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 75.6 & 29.4 \\
251.3 & \verb|GT:BBH:743| & 3.0 & 0.267 & -0.412 & -0.094 &-&-&-& -0.07 & 63.4 & 42.4 \\
251.2 & \verb|RIT:BBH:NQ16TH115PH150| & 6.0 & -0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 66.9 & 32.8 \\
251.2 & \verb|RIT:BBH:NQ50TH60PH120| & 2.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 87.4 & 28.4 \\
251.1 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 77.4 & 27.5 \\
251.1 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 77.4 & 27.5 \\
251.1 & \verb|SXS:BBH:0151| & 1.0 &-& - & -0.600 & - &-& -0.600 & -0.60 & 59.6 & 17.0 \\
251.0 & \verb|RIT:BBH:NQ50TH60PH90| & 2.0 &-& 0.693 & 0.400 &-&-&-& 0.27 & 87.0 & 28.4 \\
251.0 & \verb|GT:BBH:635| & 3.0 & 0.201 & -0.405 & 0.213 &-&-&-& 0.16 & 79.3 & 33.0 \\
250.8 & \verb|D11_q1.00_a-0.5_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& -0.500 & -0.50 & 57.6 & 30.7 \\
250.7 & \verb|RIT:BBH:NQ25TH90PH90| & 4.0 &-& 0.800 &-&-&-&-& 0.00 & 76.6 & 20.5 \\
250.6 & \verb|RIT:BBH:NQ50TH60PH0| & 2.0 & 0.693 &-& 0.400 &-&-&-& 0.27 & 85.7 & 29.5 \\
250.3 & \verb|RIT:BBH:NQ50TH60PH60| & 2.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 85.7 & 28.7 \\
250.1 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 79.0 & 27.6 \\
249.7 & \verb|EMu0_D8.80_q1.00_a0.8_n100| & 1.0 &-&-& 0.801 &-&-& - & 0.40 & 87.3 & 26.9 \\
249.7 & \verb|GT:BBH:746| & 3.0 & -0.267 & 0.412 & -0.094 &-&-&-& -0.07 & 65.7 & 41.9 \\
249.7 & \verb|GT:BBH:747| & 3.0 & 0.335 & 0.317 & -0.192 &-&-&-& -0.14 & 63.3 & 42.0 \\
249.7 & \verb|GT:BBH:726| & 3.0 & -0.197 & 0.385 & -0.251 &-&-&-& -0.19 & 65.8 & 42.8 \\
249.5 & \verb|RIT:BBH:NQ50TH60PH150| & 2.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 85.7 & 29.8 \\
249.2 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 79.2 & 27.3 \\
249.1 & \verb|RIT:BBH:NQ25TH135PH90| & 4.0 &-& 0.566 & -0.566 &-&-&-& -0.45 & 56.5 & 40.0 \\
249.0 & \verb|RIT:BBH:NQ50TH60PH30| & 2.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 85.7 & 28.8 \\
248.9 & \verb|Del0_D10.97_q1.3333_a-0.6_-0.8_n100| & 1.334 &-&-& -0.600 &-&-& -0.801 & -0.69 & 56.0 & 33.2 \\
248.9 & \verb|SXS:BBH:0105| & 3.001 &-& - & -0.500 & - & - &-& -0.37 & 66.5 & 11.4 \\
248.8 & \verb|GT:BBH:735| & 3.0 & -0.155 & -0.394 & -0.265 &-&-&-& -0.20 & 63.5 & 44.2 \\
248.8 & \verb|SXS:BBH:0032| & 3.001 & 0.248 & 0.037 & -0.432 &-& - &-& -0.32 & 68.8 & 16.7 \\
248.6 & \verb|RIT:BBH:NQ25TH90PH30| & 4.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 78.5 & 21.7 \\
248.6 & \verb|RIT:BBH:NQ25TH135PH150| & 4.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 58.0 & 41.2 \\
248.4 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 79.0 & 27.1 \\
248.3 & \verb|RIT:BBH:NQ25TH90PH60| & 4.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 77.1 & 20.4 \\
248.3 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 78.4 & 27.0 \\
248.3 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 78.4 & 27.0 \\
248.2 & \verb|SXS:BBH:0311|(*) & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.40 & 86.0 & 13.2 \\
247.8 & \verb|RIT:BBH:NQ33TH75PH150| & 3 & -0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 87.7 & 26.6 \\
247.3 & \verb|GT:BBH:741| & 3.0 & 0.162 & 0.326 & 0.343 &-&-&-& 0.26 & 85.7 & 25.9 \\
247.3 & \verb|GT:BBH:406| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.3 & 21.3 \\
247.3 & \verb|GT:BBH:406| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.3 & 21.3 \\
247.2 & \verb|RIT:BBH:NQ25TH135PH60| & 4.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 61.2 & 39.3 \\
247.2 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 77.6 & 27.4 \\
247.2 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 77.6 & 27.4 \\
247.1 & \verb|D11_q1.00_a-0.8_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 49.8 & 38.2 \\
246.9 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 81.0 & 26.0 \\
246.9 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 81.0 & 26.0 \\
246.8 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 79.8 & 26.6 \\
246.7 & \verb|RIT:BBH:NQ25TH135PH120| & 4.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 60.6 & 38.3 \\
246.5 & \verb|D13.00_q0.50_a0.00_-0.80_n100|(*) & 1.999 &-&-& -0.801 &-&-& - & -0.53 & 58.6 & 22.7 \\
246.4 & \verb|GT:BBH:606| & 3.0 & -0.411 & 0.149 & 0.242 &-&-&-& 0.18 & 86.0 & 24.7 \\
246.3 & \verb|SXS:BBH:0165| & 6.001 & 0.704 & 0.313 & -0.484 & -0.170 & -0.072 & -0.236 & -0.45 & 66.6 & 28.6 \\
246.2 & \verb|RIT:BBH:NQ25TH135PH30| & 4.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 59.9 & 38.3 \\
246.1 & \verb|GT:BBH:684| & 3.0 & 0.289 & -0.281 & -0.296 &-&-&-& -0.22 & 63.7 & 44.1 \\
245.9 & \verb|U0_D9.4_q2.00_a0.5_n100_am| & 2.0 &-&-& 0.500 &-&-& - & 0.33 & 87.8 & 22.6 \\
245.9 & \verb|UD_D8.76_q2.00_a0.8_rl10_opt1_n100| & 2.0 &-&-& 0.801 &-&-& -0.801 & 0.27 & 89.0 & 26.9 \\
245.9 & \verb|GT:BBH:554| & 1.0 &-&-& 0.200 &-&-& 0.600 & 0.40 & 88.2 & 18.1 \\
245.9 & \verb|GT:BBH:554| & 1.0 &-&-& 0.200 &-&-& 0.600 & 0.40 & 88.2 & 18.1 \\
245.9 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 80.1 & 26.4 \\
245.8 & \verb|SXS:BBH:0167| & 4.0 & - & - &-&-&-&-& 0.00 & 81.6 & 16.2 \\
245.8 & \verb|GT:BBH:551| & 1.0 &-&-&-&-&-& 0.800 & 0.40 & 88.4 & 18.1 \\
245.8 & \verb|GT:BBH:551| & 1.0 &-&-&-&-&-& 0.800 & 0.40 & 88.4 & 18.1 \\
245.7 & \verb|D13.00_q0.50_a-0.50_-0.60_n100|(*) & 2.0 &-&-& -0.600 &-&-& -0.500 & -0.57 & 58.7 & 22.5 \\
245.5 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 80.2 & 26.1 \\
245.3 & \verb|GT:BBH:422| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 86.6 & 18.3 \\
245.3 & \verb|GT:BBH:422| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 86.6 & 18.3 \\
245.3 & \verb|D13_q1.00_a-0.80_-0.40_n100|(*) & 1.0 &-&-& -0.400 &-&-& -0.801 & -0.60 & 56.5 & 25.6 \\
245.0 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.8 & 20.9 \\
245.0 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.8 & 20.9 \\
244.9 & \verb|RIT:BBH:NQ25TH90PH120| & 4.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 80.5 & 20.0 \\
244.7 & \verb|GT:BBH:778| & 3.7 &-&-&-&-&-&-& 0.00 & 80.5 & 25.9 \\
244.6 & \verb|RIT:BBH:NQ25TH135PH0| & 4.0 & 0.566 &-& -0.566 &-&-&-& -0.45 & 62.6 & 36.4 \\
244.6 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 81.8 & 25.6 \\
244.6 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 81.8 & 25.6 \\
244.4 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 79.5 & 26.3 \\
244.4 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 79.5 & 26.3 \\
244.0 & \verb|GT:BBH:861| & 1.0 & -0.159 & -0.414 & -0.404 & 0.297 & 0.521 & -0.020 & -0.21 & 65.8 & 48.6 \\
243.8 & \verb|GT:BBH:863| & 1.0 & -0.512 & 0.270 & -0.157 & -0.506 & -0.175 & -0.270 & -0.21 & 70.2 & 48.5 \\
243.3 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 78.8 & 26.6 \\
243.3 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 78.8 & 26.6 \\
243.2 & \verb|GT:BBH:780| & 3.8 &-&-&-&-&-&-& 0.00 & 80.8 & 25.6 \\
242.7 & \verb|D11.00_q0.2500_a0.0_0.0_n100|(*) & 4.0 &-&-&-&-&-& - & 0.00 & 80.0 & 20.2 \\
242.5 & \verb|RIT:BBH:NQ16TH90PH90| & 6.0 &-& 0.800 &-&-&-&-& 0.00 & 83.1 & 25.7 \\
242.3 & \verb|RIT:BBH:NQ16TH90PH60| & 6.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 83.5 & 26.3 \\
242.2 & \verb|RIT:BBH:NQ16TH135PH90| & 6.0 &-& 0.566 & -0.566 &-&-&-& -0.48 & 61.7 & 39.3 \\
242.2 & \verb|GT:BBH:744| & 3.0 & 0.411 & -0.149 & 0.242 &-&-&-& 0.18 & 84.3 & 24.5 \\
242.1 & \verb|(0,4,'MXX','D11')| & 4 &-&-&-&-&-&-& 0.00 & 80.5 & 20.2 \\
242.1 & \verb|(0,4,'MXX','D11')| & 4 &-&-&-&-&-&-& 0.00 & 80.5 & 20.2 \\
242.0 & \verb|GT:BBH:797| & 4.1 &-&-&-&-&-&-& 0.00 & 81.5 & 25.1 \\
242.0 & \verb|GT:BBH:777| & 3.9 &-&-&-&-&-&-& 0.00 & 80.9 & 25.5 \\
241.8 & \verb|GT:BBH:739| & 3.0 & -0.162 & -0.326 & 0.343 &-&-&-& 0.26 & 89.2 & 24.0 \\
241.8 & \verb|RIT:BBH:NQ16TH90PH0| & 6.0 & 0.800 &-&-&-&-&-& 0.00 & 83.0 & 24.4 \\
241.7 & \verb|GT:BBH:613| & 3.0 & 0.176 & -0.221 & 0.413 &-&-&-& 0.31 & 90.1 & 23.8 \\
241.6 & \verb|RIT:BBH:NQ16TH135PH60| & 6.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 60.1 & 35.8 \\
241.2 & \verb|RIT:BBH:NQ16TH135PH120| & 6.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 59.5 & 38.7 \\
241.1 & \verb|RIT:BBH:NQ16TH135PH30| & 6.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 59.5 & 38.0 \\
241.1 & \verb|RIT:BBH:NQ16TH90PH30| & 6.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 82.3 & 24.1 \\
241.0 & \verb|GT:BBH:883| & 3.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.22 & 93.1 & 21.6 \\
240.8 & \verb|RIT:BBH:NQ16TH135PH150| & 6.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 57.2 & 37.8 \\
240.7 & \verb|GT:BBH:798| & 4.2 &-&-&-&-&-&-& 0.00 & 81.7 & 24.9 \\
240.6 & \verb|d0_D10.52_q3.00_a-0.66667_n100| & 2.999 &-&-& -0.667 &-&-& - & -0.50 & 58.4 & 33.8 \\
240.6 & \verb|GT:BBH:791| & 4.3 &-&-&-&-&-&-& 0.00 & 81.8 & 24.8 \\
240.4 & \verb|SXS:BBH:0043| & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.32 & 94.0 & 15.2 \\
240.3 & \verb|GT:BBH:414| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.1 & 21.2 \\
240.3 & \verb|GT:BBH:414| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.1 & 21.2 \\
240.2 & \verb|RIT:BBH:NQ16TH90PH150| & 6.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 80.7 & 29.0 \\
240.0 & \verb|GT:BBH:884| & 3.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 94.2 & 21.8 \\
239.8 & \verb|GT:BBH:795| & 4.4 &-&-&-&-&-&-& 0.00 & 82.1 & 24.6 \\
239.7 & \verb|SXS:BBH:0046| & 3.0 &-&-& -0.500 & - &-& -0.499 & -0.50 & 62.4 & 18.4 \\
239.3 & \verb|EMuu_D8.82_q1.00_a0.2_n100| & 1.0 &-&-& 0.801 &-&-& 0.200 & 0.50 & 90.7 & 25.4 \\
239.1 & \verb|SXS:BBH:0033| & 3.001 & 0.248 & 0.030 & 0.432 & - & - &-& 0.32 & 91.0 & 12.6 \\
239.0 & \verb|GT:BBH:879| & 3.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.24 & 95.5 & 22.0 \\
238.5 & \verb|GT:BBH:626| & 3.0 & 0.179 & 0.254 & 0.392 &-&-&-& 0.29 & 93.8 & 21.7 \\
238.5 & \verb|RIT:BBH:NQ16TH115PH90| & 6.0 &-& 0.725 & -0.338 &-&-&-& -0.29 & 71.2 & 32.2 \\
238.3 & \verb|RIT:BBH:NQ16TH135PH0| & 6.0 & 0.566 &-& -0.566 &-&-&-& -0.48 & 61.8 & 36.7 \\
238.3 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.2 & 21.6 \\
238.3 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.2 & 21.6 \\
238.2 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 82.3 & 24.4 \\
238.1 & \verb|SXS:BBH:0057| & 5.002 & 0.402 & -0.177 & -0.201 & - &-&-& -0.17 & 73.3 & 28.2 \\
237.8 & \verb|GT:BBH:607| & 3.0 & -0.276 & 0.148 & 0.390 &-&-&-& 0.29 & 90.1 & 22.7 \\
237.6 & \verb|RIT:BBH:NQ50TH30PH120| & 2.0 & -0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 96.3 & 25.9 \\
237.6 & \verb|RIT:BBH:NQ16TH90PH120| & 6.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 80.5 & 27.6 \\
237.4 & \verb|RIT:BBH:NQ16TH115PH60| & 6.0 & 0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 66.5 & 33.2 \\
237.2 & \verb|RIT:BBH:NQ50TH30PH90| & 2.0 &-& 0.400 & 0.693 &-&-&-& 0.46 & 93.8 & 26.3 \\
237.1 & \verb|RIT:BBH:NQ16TH115PH120| & 6.0 & -0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 65.1 & 34.1 \\
237.0 & \verb|RIT:BBH:NQ16TH150PH90| & 6.0 &-& 0.400 & -0.693 &-&-&-& -0.59 & 57.2 & 36.9 \\
236.9 & \verb|D11_q0.75_a0.0_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& - & 0.46 & 93.3 & 17.2 \\
236.9 & \verb|D11_q1.00_a0.5_0.5_n100|(*) & 1.0 &-&-& 0.500 &-&-& 0.500 & 0.50 & 92.1 & 17.1 \\
236.5 & \verb|RIT:BBH:NQ16TH150PH150| & 6.0 & -0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 59.5 & 38.1 \\
236.0 & \verb|RIT:BBH:NQ50TH30PH0| & 2.0 & 0.400 &-& 0.693 &-&-&-& 0.46 & 87.5 & 29.8 \\
235.8 & \verb|SXS:BBH:0059| & 5.0 & 0.265 & -0.096 & -0.157 &-& - &-& -0.13 & 76.8 & 26.3 \\
235.7 & \verb|GT:BBH:875| & 4.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 93.6 & 23.1 \\
235.6 & \verb|DU_D10.60_q3.00_a-0.8_rl11_n120| & 2.999 &-&-& -0.801 &-&-& 0.800 & -0.40 & 59.2 & 32.6 \\
235.6 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 84.1 & 24.5 \\
235.6 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 84.1 & 24.5 \\
235.6 & \verb|RIT:BBH:NQ16TH150PH120| & 6.0 & -0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 61.9 & 35.2 \\
235.6 & \verb|GT:BBH:745| & 6.0 & -0.046 & 0.539 & 0.259 &-&-&-& 0.22 & 79.8 & 25.7 \\
235.5 & \verb|RIT:BBH:NQ16TH150PH0| & 6.0 & 0.400 &-& -0.693 &-&-&-& -0.59 & 57.2 & 40.0 \\
235.3 & \verb|SXS:BBH:0058| & 5.002 & 0.498 & 0.027 &-&-& - &-& 0.00 & 82.8 & 11.7 \\
235.1 & \verb|RIT:BBH:NQ16TH115PH0| & 6.0 & 0.725 &-& -0.338 &-&-&-& -0.29 & 73.4 & 29.2 \\
235.0 & \verb|SXS:BBH:0162| & 2.0 &-& - & 0.600 &-&-&-& 0.40 & 92.9 & 12.4 \\
234.9 & \verb|RIT:BBH:NQ16TH150PH30| & 6.0 & 0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 57.2 & 38.5 \\
234.9 & \verb|RIT:BBH:NQ16TH115PH30| & 6.0 & 0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 73.3 & 28.6 \\
234.9 & \verb|RIT:BBH:NQ25TH90PH0| & 4.0 & 0.800 &-&-&-&-&-& 0.00 & 84.6 & 21.7 \\
234.8 & \verb|D11_q0.75_a0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& 0.500 & 0.50 & 91.3 & 17.5 \\
234.7 & \verb|RIT:BBH:NQ16TH150PH60| & 6.0 & 0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 57.2 & 38.0 \\
234.7 & \verb|RIT:BBH:NQ25TH60PH0| & 4.0 & 0.693 &-& 0.400 &-&-&-& 0.32 & 97.6 & 23.3 \\
234.3 & \verb|SXS:BBH:0107| & 5.0 &-&-&-& - & - &-& 0.00 & 84.2 & 11.8 \\
234.2 & \verb|SXS:BBH:0190| & 4.499 & - &-& - &-&-&-& -0.00 & 80.8 & 14.9 \\
234.1 & \verb|RIT:BBH:NQ25TH60PH90| & 4.0 &-& 0.693 & 0.400 &-&-&-& 0.32 & 91.7 & 24.1 \\
234.0 & \verb|RIT:BBH:NQ50TH30PH30| & 2.0 & 0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 93.9 & 27.2 \\
233.9 & \verb|RIT:BBH:NQ50TH30PH150| & 2.0 & -0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 97.5 & 26.3 \\
233.8 & \verb|SXS:BBH:0062| & 5.003 & 0.384 & -0.236 & -0.218 &-& - &-& -0.18 & 70.7 & 0.0 \\
233.2 & \verb|RIT:BBH:NQ25TH60PH60| & 4.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 92.5 & 22.5 \\
232.9 & \verb|GT:BBH:555| & 1.0 &-&-& 0.200 &-&-& 0.800 & 0.50 & 92.0 & 17.4 \\
232.9 & \verb|GT:BBH:555| & 1.0 &-&-& 0.200 &-&-& 0.800 & 0.50 & 92.0 & 17.4 \\
231.8 & \verb|RIT:BBH:NQ25TH60PH30| & 4.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 93.8 & 23.8 \\
231.3 & \verb|RIT:BBH:NQ25TH60PH120| & 4.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 102.6 & 20.2 \\
231.3 & \verb|RIT:BBH:NQ25TH60PH150| & 4.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 94.4 & 24.2 \\
231.2 & \verb|SXS:BBH:0048| & 3.0 & - & -0.001 & 0.500 & 0.471 & 0.165 & 0.001 & 0.37 & 96.2 & 11.7 \\
231.2 & \verb|GT:BBH:603| & 3.0 &-&-& 0.500 &-&-&-& 0.38 & 96.7 & 21.3 \\
231.0 & \verb|RIT:BBH:NQ50TH30PH60| & 2.0 & 0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 95.3 & 26.2 \\
230.9 & \verb|RIT:BBH:NQ25TH60PH165| & 4.0 & -0.669 & 0.179 & 0.400 &-&-&-& 0.32 & 98.4 & 24.0 \\
230.3 & \verb|GT:BBH:862| & 1.0 & 0.542 & -0.255 & -0.034 & 0.053 & 0.188 & -0.567 & -0.30 & 66.0 & 51.9 \\
230.2 & \verb|SXS:BBH:0051| & 3.0 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.37 & 97.0 & 11.8 \\
230.1 & \verb|GT:BBH:742| & 7.0 & -0.028 & 0.599 & -0.008 &-&-&-& -0.01 & 86.9 & 22.9 \\
229.9 & \verb|d0_D11.03_q4.00_a-0.75_v2_n100| & 3.998 &-&-& -0.751 & - &-& - & -0.60 & 60.5 & 30.0 \\
229.4 & \verb|Del0_D8.87_q2.00_a0.4_0.8_n100| & 2.001 &-&-& 0.400 & 0.015 & -0.007 & 0.800 & 0.53 & 97.3 & 23.0 \\
229.3 & \verb|RIT:BBH:NQ25TH60PH135| & 4.0 & -0.490 & 0.490 & 0.400 &-&-&-& 0.32 & 93.0 & 23.5 \\
229.3 & \verb|SXS:BBH:0174| & 3.001 &-& - & 0.500 & - &-&-& 0.37 & 95.7 & 8.5 \\
228.9 & \verb|SXS:BBH:0197| & 5.522 & - &-& - &-&-& - & -0.00 & 85.5 & 14.8 \\
228.2 & \verb|RIT:BBH:NQ33TH45PH120| & 3 & -0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 103.6 & 21.8 \\
228.0 & \verb|RIT:BBH:NQ33TH45PH90| & 3 &-& 0.566 & 0.566 &-&-&-& 0.42 & 87.7 & 24.6 \\
227.9 & \verb|SXS:BBH:0187| & 5.039 &-& - &-& - & - & - & 0.00 & 82.2 & 15.4 \\
227.5 & \verb|GT:BBH:880| & 4.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.27 & 98.5 & 20.8 \\
227.0 & \verb|RIT:BBH:NQ33TH45PH150| & 3 & -0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 102.2 & 22.9 \\
225.5 & \verb|D10.50_q0.1667_a0.0_0.0_n100|(*) & 6.0 &-&-&-&-&-& - & 0.00 & 86.4 & 18.9 \\
225.1 & \verb|SXS:BBH:0159| & 1.0 &-&-& -0.900 & - & - & -0.900 & -0.90 & 54.5 & 18.7 \\
224.3 & \verb|RIT:BBH:NQ33TH45PH0| & 3 & 0.566 &-& 0.566 &-&-&-& 0.42 & 99.7 & 22.6 \\
224.1 & \verb|EMuu_D8.78_q1.00_a0.4_n100| & 1.0 &-&-& 0.801 &-&-& 0.400 & 0.60 & 97.9 & 23.5 \\
224.1 & \verb|SXS:BBH:0156| & 1.0 &-&-& -0.949 &-&-& -0.949 & -0.95 & 52.0 & 17.1 \\
223.9 & \verb|SXS:BBH:0166| & 6.0 & - & - &-&-&-&-& 0.00 & 87.1 & 14.3 \\
223.3 & \verb|DU_D10.61_q4.00_a-0.8_rl11_n100| & 3.999 &-&-& -0.801 &-&-& 0.800 & -0.48 & 56.5 & 34.6 \\
222.8 & \verb|RIT:BBH:NQ33TH45PH30| & 3 & 0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 101.6 & 21.7 \\
222.7 & \verb|GT:BBH:887| & 5.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.28 & 103.2 & 18.9 \\
222.2 & \verb|RIT:BBH:NQ33TH45PH60| & 3 & 0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 99.6 & 21.5 \\
219.9 & \verb|SXS:BBH:0192| & 6.58 & - &-&-& - & - & - & 0.00 & 87.8 & 14.9 \\
219.3 & \verb|d0_D11.35_q5.00_a-0.8_opt1_n100| & 4.997 &-&-& -0.801 &-&-& - & -0.67 & 63.1 & 27.3 \\
219.2 & \verb|SXS:BBH:0152| & 1.0 &-& - & 0.600 & - &-& 0.600 & 0.60 & 96.5 & 10.4 \\
218.4 & \verb|GT:BBH:889| & 6.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.30 & 108.8 & 17.7 \\
218.3 & \verb|SXS:BBH:0108| & 5.002 & - & - & -0.500 &-&-&-& -0.42 & 69.0 & 16.8 \\
218.1 & \verb|GT:BBH:407| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 100.3 & 18.1 \\
218.1 & \verb|GT:BBH:407| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 100.3 & 18.1 \\
217.5 & \verb|SXS:BBH:0047| & 3.0 &-&-& 0.500 & - & - & 0.499 & 0.50 & 102.6 & 11.1 \\
217.3 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 99.6 & 15.7 \\
217.3 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 99.6 & 15.7 \\
217.1 & \verb|D11.50_q0.50_a0.50_0.60_n100|(*) & 2.0 &-&-& 0.600 &-&-& 0.500 & 0.57 & 104.2 & 14.5 \\
215.3 & \verb|GT:BBH:411| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 99.7 & 18.3 \\
215.3 & \verb|GT:BBH:411| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 99.7 & 18.3 \\
215.3 & \verb|D10_q7.00_a0.0_m320| & 7.0 &-&-&-&-&-&-& 0.00 & 88.8 & 0.0 \\
214.1 & \verb|UD_D8.40_q3.00_a0.8_rl11_n120| & 2.999 &-&-& 0.801 &-&-& -0.800 & 0.40 & 105.7 & 23.2 \\
213.4 & \verb|GT:BBH:415| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 101.2 & 18.5 \\
213.4 & \verb|GT:BBH:415| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 101.2 & 18.5 \\
213.2 & \verb|GT:BBH:888| & 7.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.32 & 112.6 & 16.4 \\
212.3 & \verb|D11_q0.50_a0.00_0.80_n100|(*) & 1.999 &-&-& 0.801 &-&-& - & 0.53 & 104.0 & 15.3 \\
211.5 & \verb|SXS:BBH:0188| & 7.187 &-& - &-& - &-& - & -0.00 & 91.3 & 14.3 \\
211.2 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 103.7 & 18.6 \\
211.2 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 103.7 & 18.6 \\
211.2 & \verb|SXS:BBH:0061| & 5.002 &-& - & 0.500 & - &-&-& 0.42 & 107.5 & 9.6 \\
209.8 & \verb|SXS:BBH:0179| & 1.5 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.65 & 108.5 & 9.7 \\
209.4 & \verb|SXS:BBH:0195| & 7.761 & - & - &-& - &-& - & 0.00 & 90.1 & 14.9 \\
209.1 & \verb|U0_D9.07_q3.00_a0.66667_n100| & 2.999 &-&-& 0.667 &-&-& - & 0.50 & 107.2 & 19.5 \\
208.5 & \verb|d0_D10.53_q6.00_a-0.83333_n100| & 5.996 &-&-& -0.835 &-&-& - & -0.72 & 61.2 & 33.2 \\
207.4 & \verb|Del0_D8.83_q1.3333_a0.6_0.8_n100| & 1.334 &-&-& 0.600 &-&-& 0.801 & 0.69 & 102.9 & 22.0 \\
204.4 & \verb|RIT:BBH:NQ16TH45PH120| & 6.0 & -0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 117.1 & 20.0 \\
199.4 & \verb|RIT:BBH:NQ16TH45PH60| & 6.0 & 0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 111.2 & 19.7 \\
197.5 & \verb|RIT:BBH:NQ16TH45PH0| & 6.0 & 0.566 &-& 0.566 &-&-&-& 0.48 & 111.2 & 21.1 \\
197.4 & \verb|RIT:BBH:NQ16TH45PH90| & 6.0 &-& 0.566 & 0.566 &-&-&-& 0.48 & 111.9 & 20.6 \\
196.7 & \verb|RIT:BBH:NQ16TH45PH30| & 6.0 & 0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 120.0 & 19.5 \\
195.9 & \verb|SXS:BBH:0175| & 1.0 &-& - & 0.750 & - &-& 0.750 & 0.75 & 111.0 & 0.0 \\
195.0 & \verb|RIT:BBH:NQ16TH45PH150| & 6.0 & -0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 127.5 & 19.0 \\
190.2 & \verb|D10_q1.00_a0.8_0.8_n100|(*) & 1.0 &-&-& 0.801 &-&-& 0.801 & 0.80 & 114.8 & 15.7 \\
188.6 & \verb|SXS:BBH:0155| & 1.0 & - & - & 0.800 &-&-& 0.800 & 0.80 & 117.0 & 8.2 \\
186.2 & \verb|GT:BBH:424| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 111.8 & 14.6 \\
186.2 & \verb|GT:BBH:424| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 111.8 & 14.6 \\
184.0 & \verb|U0_D8.8_q4.00_a0.75_n100_am| & 3.999 &-&-& 0.751 &-&-& - & 0.60 & 128.9 & 16.8 \\
180.8 & \verb|SXS:BBH:0153| & 1.0 & - & - & 0.850 &-&-& 0.850 & 0.85 & 119.2 & 8.5 \\
180.6 & \verb|UU_D8.56_q2.00_a0.8_m100| & 2.0 &-&-& 0.801 & 0.016 & -0.004 & 0.800 & 0.80 & 123.5 & 18.9 \\
170.4 & \verb|SXS:BBH:0160| & 1.0 &-& - & 0.900 &-&-& 0.900 & 0.90 & 119.2 & 8.1 \\
168.2 & \verb|U0_D8.65_q5.00_a0.8_n100| & 4.997 &-&-& 0.801 &-&-&-& 0.67 & 139.7 & 15.5 \\
158.3 & \verb|SXS:BBH:0157| & 1.0 & - &-& 0.950 &-& - & 0.950 & 0.95 & 119.2 & 8.3 \\
155.8 & \verb|SXS:BBH:0176| & 1.0 &-& - & 0.960 & - &-& 0.960 & 0.96 & 119.2 & 8.2 \\
153.1 & \verb|SXS:BBH:0158| & 1.0 &-& - & 0.970 & - &-& 0.970 & 0.97 & 119.2 & 8.4 \\
150.3 & \verb|SXS:BBH:0172| & 1.0 &-& - & 0.979 & - &-& 0.979 & 0.98 & 119.2 & 8.6 \\
147.2 & \verb|SXS:BBH:0177| & 1.0 &-&-& 0.989 & - & - & 0.989 & 0.99 & 119.2 & 8.2 \\
146.2 & \verb|SXS:BBH:0178| & 1.0 &-&-& 0.994 & - & - & 0.994 & 0.99 & 119.2 & 8.2 \\
144.0 & \verb|U0_D8.51_q6.00_a0.83333_n100_am| & 5.996 & 0.003 & -0.023 & 0.834 & - & - & - & 0.71 & 156.9 & 14.0 \\
\end{longtable}


==> simulation-rankings_30.tex <==
\begin{longtable}{l|l|lrrrrrr|rr}
\caption{\label{tab:SimulationRanks:30}\textbf{Peak Marginalized $\ln L$ I: Consistency between simulations}: Peak value of the marginalized log likelihood $\ln L_*$ evaluated using a lowerfrequency $f_{low}=30\unit{Hz}$ and all modes with $l \le 2$; the simulation key, described inTable \ref{tab:SimulationList} [an asterisk (*) denotes a new simulation motivated by \TheEvent{}];  the \emph{initial} spins of the simulation (using $-$ to denote zero, to enhance readability); the initial $\xi$; and the total (redshifted) mass of the best fit.  Though omitting information accessible to the longestsimulations, this choice of low-frequency cutoff eliminates systematic biases associated with simulation duration,which differs across our archive.  } \\ \hline\hline $\ln L$ & Key & q & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ &  $\xi$ & $M_z/M_\odot$  \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot
271.79 & \verb|D12.25_q0.82_a-0.44_0.33_n100|(*) & 1.22 &-&-& 0.330 &-&-& -0.440 & -0.02 & 72.1 \\
271.64 & \verb|Ossokine_0233|(*) & 1.228 & - & - & 0.320 &-& - & -0.580 & -0.08 & 71.0 \\
271.42 & \verb|BBH_SKS_d14.3_q1.22_sA_0_0_0.330_sB_0_0_-0.440|(*) & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.02 & 73.3 \\
271.23 & \verb|BBH_SKS_d14.3_q1.22_sA_0_0_0_sB_0_0_0|(*) & 1.221 & - &-&-& - & - &-& 0.00 & 73.0 \\
271.13 & \verb|2| & 1.0 &-& - &-&-&-&-& 0.00 & 73.5 \\
271.07 & \verb|198| & 1.202 & - & - & - & - & - &-& 0.00 & 73.1 \\
271.03 & \verb|D11_q0.75_a0.0_0.0_n100|(*) & 1.333 &-&-& - &-&-& - & -0.00 & 71.7 \\
270.94 & \verb|D12_q1.00_a-0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& -0.250 & -0.00 & 73.1 \\
270.9 & \verb|S0_D10.04_q1.3333_a0.45_-0.80_n100| & 1.334 &-&-& 0.450 &-&-& -0.801 & -0.09 & 71.9 \\
270.49 & \verb|UD_D10.01_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& -0.400 & -0.00 & 73.5 \\
270.2 & \verb|(-0.2,1,'M200','D11')| & 1 & - & - & -0.200 & - & - & -0.200 & -0.20 & 67.0 \\
270.19 & \verb|D12.00_q0.85_a0.0_0.0_n100|(*) & 1.176 &-&-& - &-&-& - & -0.00 & 73.0 \\
269.94 & \verb|D10_q0.75_a-0.5_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.500 & -0.07 & 72.3 \\
269.94 & \verb|(0.0,1.15)| & 1.15 &-&-&-&-&-&-& 0.00 & 74.0 \\
269.88 & \verb|Ossokine_0234|(*) & 1.228 & 0.072 & 0.072 & 0.325 & 0.201 & 0.285 & -0.571 & -0.08 & 71.3 \\
269.8 & \verb|3| & 1.0 & 0.497 & 0.053 & - &-&-&-& -0.00 & 73.7 \\
269.71 & \verb|D12_q1.00_a-0.25_0.00_n100|(*) & 1.0 &-&-& - &-&-& -0.250 & -0.12 & 69.1 \\
269.67 & \verb|D11_q0.75_a-0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& -0.500 & 0.07 & 76.6 \\
269.66 & \verb|D10_q0.75_a-0.25_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.250 & 0.04 & 76.0 \\
269.63 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 73.9 \\
269.55 & \verb|D11_q0.75_a-0.8500_0.6375_n100| & 1.334 &-&-& 0.638 & 0.001 & 0.003 & -0.851 & -0.00 & 74.8 \\
269.53 & \verb|(0.0,1.0,'M240','D11')| & 1.0 &-&-&-&-&-&-& 0.00 & 73.9 \\
269.18 & \verb|D11_q0.75_a-0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& -0.500 & -0.21 & 67.6 \\
269.09 & \verb|D10_q0.75_a-0.8_xi0_n100|(*) & 1.333 & 0.538 & 0.056 & 0.590 &-&-& -0.801 & -0.01 & 75.3 \\
269.05 & \verb|('Unbalanced',1,0.0,0.2,'M160','D11')| & 1 &-&-&-&-&-& 0.200 & 0.10 & 76.6 \\
268.93 & \verb|(0.0,1.1,'M160','D9')| & 1.1 &-&-&-&-&-&-& 0.00 & 72.4 \\
268.91 & \verb|163| & 1.0 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.02 & 75.1 \\
268.89 & \verb|6| & 1.345 & 0.234 & 0.148 & -0.161 & 0.091 & 0.064 & -0.101 & -0.14 & 69.1 \\
268.66 & \verb|a8_q1_up_dn_th_45_ph_30| & 1.0 & -0.337 & 0.463 & 0.585 & 0.290 & -0.502 & -0.579 & 0.00 & 70.1 \\
268.62 & \verb|29| & 1.5 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.00 & 74.7 \\
268.55 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 72.3 \\
268.49 & \verb|194| & 1.518 &-& - &-& - &-& - & -0.00 & 73.8 \\
268.42 & \verb|(0.0,1.45)| & 1.45 &-&-&-&-&-&-& 0.00 & 73.5 \\
268.41 & \verb|D11_q0.75_a0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& 0.500 & -0.07 & 69.2 \\
268.38 & \verb|D10_q0.75_a0.25_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.250 & -0.04 & 72.2 \\
268.24 & \verb|a8_q1_up_dn_th_45_ph_60| & 1.0 & -0.537 & 0.242 & 0.570 & 0.502 & -0.290 & -0.579 & -0.00 & 70.0 \\
268.23 & \verb|100| & 1.5 & - & - &-&-& - &-& 0.00 & 74.1 \\
268.23 & \verb|D21.5_q1_a0.2_0.8_th104.4775_n100| & 1.001 &-&-& 0.200 & 0.775 &-& -0.200 & -0.00 & 75.1 \\
268.19 & \verb|U0_D9.53_q1.00_a0.0_n100| & 1.0 &-&-& - &-&-& - & -0.00 & 73.5 \\
267.86 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 72.5 \\
267.84 & \verb|D10_q0.75_a0.5_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.500 & 0.07 & 75.1 \\
267.69 & \verb|a8_q1_KoL_th45_ph_135| & 1.0 & -0.410 & -0.410 & 0.579 & -0.410 & -0.410 & -0.579 & -0.00 & 73.0 \\
267.67 & \verb|(0.0,1.5,'M200','D11')| & 1.5 &-&-&-&-&-&-& 0.00 & 74.2 \\
267.67 & \verb|96| & 1.501 & 0.497 & 0.051 & - &-&-&-& -0.00 & 73.8 \\
267.59 & \verb|a8_q1_up_dn_th_45_ph_90| & 1.0 & -0.591 & -0.053 & 0.565 & 0.568 & -0.003 & -0.591 & -0.01 & 70.0 \\
267.57 & \verb|a8_q1_KoL_th45_ph_150| & 1.0 & -0.290 & -0.502 & 0.579 & -0.290 & -0.502 & -0.579 & -0.00 & 72.8 \\
267.56 & \verb|a8_q1_KoL_th45_ph_60| & 1.0 & -0.549 & 0.217 & 0.568 & -0.502 & 0.290 & -0.579 & -0.01 & 73.3 \\
267.52 & \verb|24| & 1.501 & 0.496 & 0.051 & -0.001 & -0.077 & 0.489 & 0.002 & 0.00 & 74.3 \\
267.46 & \verb|a8_th_120_ph_120| & 1.005 & -0.611 & -0.353 & -0.407 &-&-& - & -0.20 & 65.1 \\
267.35 & \verb|a8_th_120_ph_90| & 1.005 & -0.706 & -0.033 & -0.403 & - &-& - & -0.20 & 65.0 \\
267.33 & \verb|D10_q0.75_a-0.8_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.801 & 0.11 & 79.6 \\
267.33 & \verb|23| & 1.501 & 0.497 & 0.051 & 0.001 & 0.077 & -0.489 &-& 0.00 & 72.4 \\
267.26 & \verb|27| & 1.5 & 0.497 & 0.051 & - & -0.494 & -0.071 &-& 0.00 & 73.7 \\
267.25 & \verb|D11_q0.75_a0.8500_-0.6375_n100|(*) & 1.334 &-&-& -0.638 & -0.001 & 0.003 & 0.851 & 0.00 & 71.9 \\
267.24 & \verb|25| & 1.5 & - & - & 0.500 & - & - & -0.499 & 0.10 & 78.7 \\
267.19 & \verb|D10_q0.75_a0.8_xi0_n100|(*) & 1.333 & 0.528 & 0.062 & -0.598 &-&-& 0.801 & 0.00 & 72.5 \\
267.18 & \verb|21| & 1.5 & 0.496 & 0.053 & - & - & 0.001 & -0.499 & -0.20 & 69.3 \\
267.1 & \verb|a8_q1_up_dn_th_45_ph_0| & 1.0 & -0.034 & 0.569 & 0.589 & 0.002 & -0.591 & -0.568 & 0.01 & 70.6 \\
267.1 & \verb|173| & 1.5 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.14 & 69.5 \\
267.09 & \verb|q200_a8_a0_th_135_ph_120| & 2 &-&-&-& -0.283 & 0.490 & -0.566 & -0.19 & 69.8 \\
267.07 & \verb|D10_q0.75_a0.0_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& - & 0.14 & 79.3 \\
267.04 & \verb|a8_q1_up_dn_th_45_ph_150| & 1.0 & -0.290 & -0.502 & 0.579 & 0.290 & 0.502 & -0.579 & -0.00 & 70.1 \\
267.04 & \verb|a8_q1_up_dn_th_45_ph_120| & 1.0 & -0.498 & -0.319 & 0.567 & 0.502 & 0.290 & -0.579 & -0.01 & 69.8 \\
266.98 & \verb|q200_a8_a0_th_135_ph_150| & 2 &-&-&-& -0.490 & 0.283 & -0.566 & -0.19 & 69.8 \\
266.94 & \verb|a8_q1_KoL_th135_ph_90| & 1.0 & -0.331 & -0.026 & 0.749 & -0.314 & -0.007 & -0.757 & -0.00 & 70.9 \\
266.94 & \verb|15| & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.00 & 74.1 \\
266.78 & \verb|(0.0,1.4,'M160','D9')| & 1.4 &-&-&-&-&-&-& 0.00 & 72.3 \\
266.72 & \verb|4| & 1.0 & - & - & -0.500 & - & - &-& -0.25 & 65.9 \\
266.72 & \verb|D11_q0.75_a0.6_0.6_PNr500_th1d_n100|(*) & 1.333 & 0.460 & 0.351 & 0.161 & 0.526 & 0.288 & -0.023 & 0.08 & 78.2 \\
266.66 & \verb|q200_a8_a0_th_135_ph_90| & 2 &-&-&-&-& 0.566 & -0.566 & -0.19 & 69.8 \\
266.55 & \verb|DU_D10.86_q1.3333_a-0.8_opt1_n100| & 1.333 &-&-& -0.801 &-&-& 0.801 & -0.11 & 68.0 \\
266.54 & \verb|a8_q1_KoL_th45_ph_105| & 1.0 & -0.567 & -0.177 & 0.564 & -0.560 & -0.150 & -0.579 & -0.01 & 72.8 \\
266.53 & \verb|a8_q1_KoL_th45_ph_165| & 1.0 & -0.119 & -0.558 & 0.588 & -0.150 & -0.560 & -0.579 & 0.00 & 74.7 \\
266.45 & \verb|a8_q1_KoL_th135_ph_60| & 1.0 & -0.297 & 0.138 & 0.751 & -0.272 & 0.157 & -0.757 & -0.00 & 69.6 \\
266.38 & \verb|d0_D10.52_q1.3333_a-0.25_n100| & 1.333 &-&-& -0.250 &-&-& - & -0.14 & 69.1 \\
266.31 & \verb|19| & 1.5 & - & - & -0.500 & - & - & 0.499 & -0.10 & 69.4 \\
266.31 & \verb|a8_q1_KoL_th45_ph_0| & 1.0 & -0.037 & 0.570 & 0.587 & -0.021 & 0.578 & -0.580 & 0.00 & 73.4 \\
266.3 & \verb|a8_q1_KoL_th45_ph_120| & 1.0 & -0.502 & -0.290 & 0.579 & -0.502 & -0.290 & -0.579 & -0.00 & 73.0 \\
266.24 & \verb|S0_D9.96_q1.3333_a-0.45_0.80_n100| & 1.334 &-&-& -0.450 &-&-& 0.801 & 0.09 & 75.2 \\
266.24 & \verb|S0_D9.87_q2.00_a0.20_-0.80_n100| & 2.001 &-&-& 0.200 & -0.015 & -0.007 & -0.800 & -0.13 & 73.2 \\
266.22 & \verb|a8_q1_KoL_th135_ph_120| & 1.0 & -0.272 & -0.157 & 0.757 & -0.272 & -0.157 & -0.757 & -0.00 & 71.3 \\
266.17 & \verb|a8_th_120_ph_60| & 1.005 & -0.643 & 0.299 & -0.399 &-& - & - & -0.20 & 65.1 \\
266.17 & \verb|D11.50_q0.60_a0.0_0.0_n100|(*) & 1.667 &-&-& - &-&-& - & -0.00 & 75.2 \\
266.17 & \verb|10| & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.26 & 65.5 \\
266.11 & \verb|a8_q1_KoL_th45_ph_30| & 1.0 & -0.355 & 0.443 & 0.590 & -0.290 & 0.502 & -0.579 & 0.01 & 74.7 \\
266.06 & \verb|UD_D9.52_q1.00_a0.6_rl10_opt3_n100| & 1.0 &-&-& 0.600 &-&-& -0.600 & -0.00 & 72.9 \\
266.02 & \verb|Rflop_r500_d11_q0.7_a0.8_m088|(*) & 1.428 & 0.603 & 0.445 & 0.283 & 0.747 & 0.278 & -0.079 & 0.13 & 81.1 \\
266.01 & \verb|a8_th_120_ph_150| & 1.005 & -0.322 & -0.617 & -0.422 & - & - &-& -0.21 & 65.8 \\
265.99 & \verb|BBH_SKS_d12.8_q1.31_sA_0_0_0.962_sB_0_0_-0.900|(*) & 1.31 & - &-& 0.961 & - & - & -0.899 & 0.16 & 80.9 \\
265.93 & \verb|a8_th_120_ph_30| & 1.005 & -0.408 & 0.580 & -0.399 & - &-& - & -0.20 & 65.0 \\
265.79 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 74.6 \\
265.66 & \verb|q200_a8_a0_th_135_ph_60| & 2 &-&-&-& 0.283 & 0.490 & -0.566 & -0.19 & 70.6 \\
265.63 & \verb|a8_q1_KoL_th135_ph_30| & 1.0 & -0.185 & 0.257 & 0.756 & -0.157 & 0.272 & -0.757 & -0.00 & 71.4 \\
265.51 & \verb|161| & 1.0 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.29 & 66.4 \\
265.46 & \verb|a8_q1_KoL_th135_ph_150| & 1.0 & -0.157 & -0.272 & 0.757 & -0.157 & -0.272 & -0.757 & -0.00 & 71.3 \\
265.29 & \verb|D10_q0.50_a-0.8_xi0_n100|(*) & 2.0 & 0.696 & 0.059 & 0.392 &-& -0.006 & -0.801 & -0.01 & 80.2 \\
265.27 & \verb|q200_a8_a0_th_135_ph_0| & 2 &-&-&-& 0.566 &-& -0.566 & -0.19 & 69.6 \\
265.23 & \verb|UD_D9.51_q1.00_a0.8_rl10_opt1_n100| & 1.0 &-&-& 0.801 &-&-& -0.801 & -0.00 & 74.1 \\
265.13 & \verb|('Unbalanced',1,0.0,0.4,'M160','D11')| & 1 &-&-&-&-&-& 0.400 & 0.20 & 80.2 \\
265.02 & \verb|a8_q1_KoL_th135_ph_0| & 1.0 & -0.026 & 0.304 & 0.760 & -0.008 & 0.310 & -0.759 & 0.00 & 72.9 \\
264.99 & \verb|q200_a8_a0_th_135_ph_30| & 2 &-&-&-& 0.490 & 0.283 & -0.566 & -0.19 & 69.6 \\
264.9 & \verb|a8_th_120_ph_0| & 1.005 & -0.062 & 0.702 & -0.407 &-&-&-& -0.20 & 64.0 \\
264.84 & \verb|169| & 2.0 & - & - &-&-&-&-& 0.00 & 74.5 \\
264.79 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 73.8 \\
264.76 & \verb|a8_th_60_ph_150| & 1.005 & -0.353 & -0.612 & 0.408 & - &-& - & 0.20 & 78.3 \\
264.75 & \verb|a8_th_60_ph_90| & 1.005 & -0.716 & -0.035 & 0.389 & - & - &-& 0.20 & 77.9 \\
264.35 & \verb|a8_th_60_ph_120| & 1.005 & -0.612 & -0.353 & 0.408 &-&-& - & 0.20 & 78.3 \\
264.2 & \verb|D11_q1.00_a0.0_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& - & -0.25 & 65.8 \\
264.19 & \verb|(0.2,1.0,'M200','D11')| & 1 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.4 \\
264.06 & \verb|q150_a8_a0_th_60_ph_120| & 1.492 & - & - &-& -0.595 & -0.380 & 0.405 & 0.16 & 76.0 \\
263.88 & \verb|a8_th_60_ph_0| & 1.005 & -0.058 & 0.692 & 0.429 &-& - & - & 0.21 & 78.1 \\
263.82 & \verb|q50_a0_a8_th_90_ph_120| & 2.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 76.1 \\
263.81 & \verb|EMu0_D9.16_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& - & 0.20 & 81.2 \\
263.79 & \verb|q50_a0_a8_th_90_ph_150| & 2.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 76.5 \\
263.67 & \verb|101| & 1.501 &-& - & -0.500 & - & - &-& -0.30 & 64.4 \\
263.6 & \verb|D11_q0.75_a0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& 0.500 & 0.21 & 80.2 \\
263.53 & \verb|(0.0,1.7,'M160','D9')| & 1.7 &-&-&-&-&-&-& 0.00 & 73.2 \\
263.48 & \verb|a8_th_60_ph_60| & 1.005 & -0.656 & 0.274 & 0.401 &-& - & - & 0.20 & 77.8 \\
263.47 & \verb|(0.0,2.05)| & 2.05 &-&-&-&-&-&-& 0.00 & 75.0 \\
263.41 & \verb|D11_q0.50_a0.0_0.0_n100|(*) & 2.0 &-&-& - &-&-& - & -0.00 & 74.5 \\
263.36 & \verb|D11_q0.50_a0.50_-0.50_n100|(*) & 2.0 &-&-& -0.500 &-&-& 0.500 & -0.17 & 67.3 \\
263.28 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 75.0 \\
263.26 & \verb|q50_a0_a8_th_90_ph_90| & 2.0 &-& 0.800 &-&-&-&-& 0.00 & 76.0 \\
262.99 & \verb|(0.0,1.8,'M160','D9')| & 1.8 &-&-&-&-&-&-& 0.00 & 73.7 \\
262.88 & \verb|(0.2,1.25,'M100')| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.8 \\
262.63 & \verb|q200_a8_a0_th_90_ph_0| & 2 &-&-&-& 0.800 &-&-& 0.00 & 74.6 \\
262.53 & \verb|q50_a0_a8_th_90_ph_0| & 2.0 & 0.800 &-&-&-&-&-& 0.00 & 77.5 \\
262.33 & \verb|a8_th_135_ph_90| & 1.005 & -0.579 & -0.025 & -0.572 & - &-& - & -0.29 & 61.6 \\
262.05 & \verb|q200_a8_a0_th_90_ph_60| & 2 &-&-&-& 0.400 & 0.693 &-& 0.00 & 75.4 \\
261.97 & \verb|a8_th_60_ph_30| & 1.005 & -0.426 & 0.555 & 0.420 & - &-& - & 0.21 & 76.8 \\
261.95 & \verb|D11_q1.00_a0.0_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& - & -0.40 & 62.1 \\
261.77 & \verb|hu_a7_th_120_ph_315| & 1.0 & 0.442 & 0.442 & -0.361 & -0.442 & -0.442 & -0.361 & -0.36 & 62.3 \\
261.68 & \verb|5| & 1.0 &-&-& 0.499 & - & - &-& 0.25 & 82.6 \\
261.65 & \verb|a8_th_135_ph_120| & 1.005 & -0.498 & -0.288 & -0.576 & - & - & - & -0.29 & 62.7 \\
261.63 & \verb|D11_q0.75_a0.0_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& - & -0.29 & 65.6 \\
261.48 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 81.4 \\
261.45 & \verb|q200_a8_a0_th_90_ph_30| & 2 &-&-&-& 0.693 & 0.400 &-& 0.00 & 75.1 \\
261.45 & \verb|(0.2,1.75,'M100')| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.8 \\
261.31 & \verb|q200_a8_a0_th_90_ph_90| & 2 &-&-&-&-& 0.800 &-& 0.00 & 74.8 \\
261.3 & \verb|q66_a0_a8_th60_ph_120| & 3.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.30 & 80.9 \\
261.29 & \verb|q50_a0_a8_th_90_ph_60| & 2.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 74.7 \\
261.2 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 73.9 \\
261.18 & \verb|RO3_D10_q2.00_a0.60_oth.135_M120| & 1.999 & 0.424 & 0.002 & -0.425 & - & - & 0.600 & -0.08 & 71.4 \\
260.97 & \verb|D11_q0.75_a-0.8_0.0_n100|(*) & 1.334 &-&-&-&-&-& -0.801 & -0.34 & 64.8 \\
260.9 & \verb|a8_th_135_ph_150| & 1.005 & -0.259 & -0.498 & -0.590 & - & - &-& -0.30 & 61.3 \\
260.83 & \verb|q200_a8_a0_th_90_ph_150| & 2 &-&-&-& -0.693 & 0.400 &-& 0.00 & 74.5 \\
260.68 & \verb|a8_th_135_ph_60| & 1.005 & -0.520 & 0.265 & -0.568 &-& - &-& -0.28 & 62.7 \\
260.56 & \verb|hu_a7_th_120_ph_0| & 1.0 & -0.055 & 0.621 & -0.362 &-& -0.625 & -0.361 & -0.36 & 62.8 \\
260.5 & \verb|q200_a8_a0_th_90_ph_120| & 2 &-&-&-& -0.400 & 0.693 &-& 0.00 & 74.8 \\
260.48 & \verb|q200_a8_a0_th_60_ph_60| & 2 &-&-&-& 0.346 & 0.600 & 0.400 & 0.13 & 75.7 \\
260.37 & \verb|q200_a8_a0_th_60_ph_30| & 2 &-&-&-& 0.600 & 0.346 & 0.400 & 0.13 & 75.4 \\
260.36 & \verb|q50_a0_a8_th_135_ph_120| & 2.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 58.8 \\
260.04 & \verb|q200_a8_a0_th_60_ph_0| & 2 &-&-&-& 0.693 &-& 0.400 & 0.13 & 75.7 \\
260.04 & \verb|a8_th_45_ph_60| & 1.005 & -0.536 & 0.241 & 0.566 & - &-&-& 0.28 & 81.5 \\
260.0 & \verb|D11_q0.75_a-0.5_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.500 & 0.24 & 84.6 \\
260.0 & \verb|Del0_D10.01_q2.00_a-0.4_-0.8_n100| & 2.001 &-&-& -0.400 & -0.011 & 0.003 & -0.800 & -0.53 & 57.9 \\
259.89 & \verb|(-0.4,1,'M200','D11')| & 1 & - & - & -0.400 & - & - & -0.400 & -0.40 & 62.3 \\
259.88 & \verb|a8_th_45_ph_150| & 1.005 & -0.289 & -0.500 & 0.577 &-&-&-& 0.29 & 81.6 \\
259.79 & \verb|q50_a0_a8_th_90_ph_30| & 2.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 76.1 \\
259.76 & \verb|164| & 1.0 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.33 & 85.3 \\
259.76 & \verb|q200_a8_a0_th_60_ph_150| & 2 &-&-&-& -0.600 & 0.346 & 0.400 & 0.13 & 75.6 \\
259.74 & \verb|a8_th_45_ph_50| & 1.005 & -0.485 & 0.328 & 0.568 & - &-&-& 0.28 & 80.2 \\
259.67 & \verb|q66_a0_a8_th60_ph_30| & 3.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.30 & 79.5 \\
259.64 & \verb|q200_a8_a0_th_60_ph_90| & 2 &-&-&-&-& 0.693 & 0.400 & 0.13 & 75.6 \\
259.59 & \verb|22| & 1.5 & 0.497 & 0.049 & - & 0.001 & -0.001 & 0.499 & 0.20 & 80.3 \\
259.58 & \verb|a8_th_45_ph_30| & 1.005 & -0.341 & 0.464 & 0.578 &-& - & - & 0.29 & 81.3 \\
259.56 & \verb|a8_th_45_ph_20| & 1.005 & -0.251 & 0.511 & 0.584 &-& - & - & 0.29 & 81.2 \\
259.54 & \verb|q66_a0_a8_th60_ph_150| & 3.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.30 & 81.6 \\
259.53 & \verb|q50_a0_a8_th_135_ph_90| & 2.0 &-& 0.566 & -0.566 &-&-&-& -0.38 & 62.4 \\
259.52 & \verb|a8_th_45_ph_40| & 1.005 & -0.417 & 0.401 & 0.575 &-& - & - & 0.29 & 79.9 \\
259.47 & \verb|q200_a8_a0_th_60_ph_120| & 2 &-&-&-& -0.346 & 0.600 & 0.400 & 0.13 & 75.1 \\
259.42 & \verb|a8_th_135_ph_30| & 1.005 & -0.343 & 0.468 & -0.571 & - & - & - & -0.29 & 64.3 \\
259.42 & \verb|a8_th_45_ph_0| & 1.005 & -0.034 & 0.568 & 0.584 &-& - & - & 0.29 & 80.8 \\
259.4 & \verb|(0.0,2.3499999999999996)| & 2.35 &-&-&-&-&-&-& 0.00 & 75.8 \\
259.22 & \verb|EMu0_D8.98_q1.00_a0.6_n100| & 1.0 &-&-& 0.600 &-&-& - & 0.30 & 85.1 \\
259.17 & \verb|hu_a7_th_120_ph_130| & 1.0 & -0.478 & -0.401 & -0.361 & 0.478 & 0.401 & -0.361 & -0.36 & 62.1 \\
259.12 & \verb|(0.0,2.1,'M160','D9')| & 2.1 &-&-&-&-&-&-& 0.00 & 74.9 \\
259.1 & \verb|a9_a0_q1_th_55_ph_30| & 1.012 & -0.432 & 0.609 & 0.522 & - &-& - & 0.26 & 80.7 \\
259.05 & \verb|a8_th_135_ph_0| & 1.005 & -0.034 & 0.576 & -0.574 &-&-&-& -0.29 & 62.8 \\
259.05 & \verb|RO3_D10_q2.50_a0.40_oth.090_M120| & 2.5 & 0.400 & 0.001 & - & - & - & 0.400 & 0.11 & 79.5 \\
259.05 & \verb|a8_th_45_ph_10| & 1.005 & -0.153 & 0.539 & 0.593 &-& - & - & 0.30 & 81.8 \\
259.05 & \verb|RO3_D10_q2.00_a0.60_oth.270_M120| & 1.999 & -0.600 & -0.002 & - &-&-& 0.600 & 0.20 & 82.2 \\
259.03 & \verb|q50_a0_a8_th_135_ph_150| & 2.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 61.9 \\
259.03 & \verb|a8_th_45_ph_1275| & 1.005 & -0.458 & -0.351 & 0.577 & - & - &-& 0.29 & 80.6 \\
258.93 & \verb|a8_th_45_ph_75| & 1.005 & -0.582 & 0.097 & 0.564 &-& - & - & 0.28 & 80.4 \\
258.86 & \verb|a8_th_45_ph_45| & 1.005 & -0.453 & 0.365 & 0.572 &-& - & - & 0.29 & 82.0 \\
258.83 & \verb|('Unbalanced',1,0.2,0.4,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.400 & 0.30 & 84.6 \\
258.77 & \verb|a8_th_45_ph_120| & 1.005 & -0.500 & -0.289 & 0.577 &-& - & - & 0.29 & 81.7 \\
258.76 & \verb|hu_a7_th_120_ph_90| & 1.0 & -0.629 & -0.027 & -0.353 & 0.625 &-& -0.361 & -0.36 & 62.3 \\
258.76 & \verb|a8_th_45_ph_1125| & 1.005 & -0.531 & -0.251 & 0.566 &-&-& - & 0.28 & 79.7 \\
258.6 & \verb|q66_a0_a8_th60_ph_90| & 3.0 &-& 0.693 & 0.400 &-&-&-& 0.30 & 81.1 \\
258.53 & \verb|hu_a7_th_120_ph_210| & 1.0 & 0.361 & -0.512 & -0.358 & -0.312 & 0.541 & -0.361 & -0.36 & 61.8 \\
258.43 & \verb|a9_a0_q1_th_55_ph_60| & 1.012 & -0.686 & 0.321 & 0.507 & - &-& - & 0.25 & 80.4 \\
258.42 & \verb|a9_a0_q1_th_55_ph_90| & 1.012 & -0.759 & -0.029 & 0.505 &-& - & - & 0.25 & 82.3 \\
258.38 & \verb|a9_a0_q1_th_55_ph_0| & 1.012 & -0.062 & 0.725 & 0.549 & - &-& - & 0.28 & 81.3 \\
258.35 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 81.3 \\
258.27 & \verb|('Unbalanced',1,0.0,0.6,'M160','D11')| & 1 &-&-&-&-&-& 0.600 & 0.30 & 83.6 \\
258.25 & \verb|hu_a7_th_120_ph_30| & 1.0 & -0.361 & 0.515 & -0.352 & 0.312 & -0.541 & -0.361 & -0.36 & 62.8 \\
258.12 & \verb|D10_q0.50_a0.8_xi0_n100|(*) & 2.0 & 0.689 & 0.062 & -0.403 & 0.012 & 0.006 & 0.800 & -0.00 & 72.5 \\
258.04 & \verb|q66_a0_a8_th60_ph_60| & 3.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.30 & 81.7 \\
257.99 & \verb|11| & 1.501 & 0.248 & 0.026 & 0.433 &-&-&-& 0.26 & 84.4 \\
257.98 & \verb|D11_q0.75_a0.0_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& - & 0.29 & 84.6 \\
257.75 & \verb|a9_a0_q1_th_55_ph_150| & 1.012 & -0.373 & -0.646 & 0.523 &-&-& - & 0.26 & 82.1 \\
257.55 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 75.0 \\
257.5 & \verb|S0_D9.75_q2.00_a-0.20_0.80_n100| & 2.001 &-&-& -0.200 & 0.015 & -0.006 & 0.800 & 0.13 & 78.7 \\
257.16 & \verb|191| & 2.507 & - &-& - &-&-&-& -0.00 & 76.3 \\
257.11 & \verb|(0.0,2.5,'M200','D11')| & 2.5 &-&-&-&-&-&-& 0.00 & 76.2 \\
257.0 & \verb|q50_a0_a8_th_135_ph_60| & 2.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 60.8 \\
256.72 & \verb|D10_q0.50_a-0.50_0.50_n100|(*) & 2.0 &-&-& 0.500 &-&-& -0.500 & 0.17 & 84.7 \\
256.64 & \verb|28| & 1.501 & -0.001 & 0.001 & 0.500 & 0.078 & -0.489 & 0.001 & 0.30 & 86.4 \\
256.64 & \verb|RO3_D10_q1.50_a0.60_oth.090_M120| & 1.5 & 0.600 & 0.002 & - & - & - & 0.601 & 0.24 & 83.1 \\
256.12 & \verb|q50_a0_a8_th_135_ph_0| & 2.0 & 0.566 &-& -0.566 &-&-&-& -0.38 & 62.7 \\
255.93 & \verb|q66_a0_a8_th60_ph_0| & 3.0 & 0.693 &-& 0.400 &-&-&-& 0.30 & 79.6 \\
255.89 & \verb|q50_a0_a8_th_135_ph_30| & 2.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 62.3 \\
255.83 & \verb|D11_q0.75_a0.4_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.597 & -0.231 & 0.481 & -0.346 & 0.200 & 0.003 & 0.28 & 85.7 \\
255.8 & \verb|q200_a8_a0_th_30_ph_120| & 2 &-&-&-& -0.200 & 0.346 & 0.693 & 0.23 & 79.4 \\
255.68 & \verb|q33_a0_a8_th_135_ph_120| & 3 & -0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 58.8 \\
255.67 & \verb|hu_a7_th_135_ph_0| & 1.0 & -0.028 & 0.512 & -0.506 &-& -0.510 & -0.510 & -0.51 & 59.6 \\
255.62 & \verb|RO3_D10_q2.00_a0.40_oth.060_M120| & 2.0 & 0.347 & 0.001 & 0.200 & - & - & 0.400 & 0.27 & 83.6 \\
255.43 & \verb|hu_a7_th_60_ph_10| & 1.0 & -0.161 & 0.600 & 0.373 & 0.137 & -0.612 & 0.364 & 0.37 & 83.5 \\
255.4 & \verb|20| & 1.5 &-& - & 0.500 & 0.494 & 0.071 & - & 0.30 & 86.5 \\
255.38 & \verb|a8_th_30_ph_90| & 1.005 & -0.423 & -0.024 & 0.698 &-&-& - & 0.35 & 82.9 \\
255.33 & \verb|(0.0,2.3,'M160','D9')| & 2.3 &-&-&-&-&-&-& 0.00 & 75.9 \\
255.31 & \verb|d0_D10.50_q2.00_a-0.5_n100| & 2.0 &-&-& -0.500 &-&-& - & -0.33 & 63.8 \\
255.3 & \verb|q33_a0_a8_th_100_ph_120| & 3 & -0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 71.9 \\
255.27 & \verb|DD_D10.99_q2.00_a-0.8_n100| & 2.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 51.3 \\
255.25 & \verb|26| & 1.5 & - &-& 0.500 & -0.494 & -0.071 & - & 0.30 & 86.4 \\
255.25 & \verb|RO3_D10_q1.50_a0.40_oth.060_M120| & 1.5 & 0.347 & 0.001 & 0.200 & - & - & 0.400 & 0.28 & 84.7 \\
255.21 & \verb|q200_a8_a0_th_30_ph_0| & 2 &-&-&-& 0.400 &-& 0.693 & 0.23 & 79.5 \\
255.15 & \verb|(0.0,2.4,'M160','D9')| & 2.4 &-&-&-&-&-&-& 0.00 & 76.1 \\
255.04 & \verb|q33_a0_a8_th_100_ph_0| & 3 & 0.788 &-& -0.139 &-&-&-& -0.10 & 74.3 \\
254.97 & \verb|q200_a8_a0_th_30_ph_30| & 2 &-&-&-& 0.346 & 0.200 & 0.693 & 0.23 & 79.0 \\
254.96 & \verb|q200_a8_a0_th_30_ph_60| & 2 &-&-&-& 0.200 & 0.346 & 0.693 & 0.23 & 79.3 \\
254.95 & \verb|a8_th_30_ph_30| & 1.005 & -0.232 & 0.338 & 0.706 &-& - & - & 0.35 & 83.7 \\
254.84 & \verb|a8_th_30_ph_60| & 1.005 & -0.378 & 0.185 & 0.700 & - &-& - & 0.35 & 84.5 \\
254.8 & \verb|q33_a0_a8_th_135_ph_150| & 3 & -0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 59.8 \\
254.73 & \verb|q200_a8_a0_th_30_ph_90| & 2 &-&-&-&-& 0.400 & 0.693 & 0.23 & 79.4 \\
254.72 & \verb|D11_q0.75_a0.0_-0.8_n100|(*) & 1.333 &-&-& -0.801 &-&-& - & -0.46 & 60.4 \\
254.7 & \verb|hu_a7_th_135_ph_30| & 1.0 & -0.281 & 0.434 & -0.502 & 0.255 & -0.441 & -0.510 & -0.51 & 59.5 \\
254.7 & \verb|a8_th_30_ph_0| & 1.005 & -0.033 & 0.386 & 0.718 &-& - & - & 0.36 & 82.8 \\
254.63 & \verb|q33_a0_a8_th_100_ph_30| & 3 & 0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 73.8 \\
254.55 & \verb|hu_a7_th_60_ph_40| & 1.0 & -0.445 & 0.444 & 0.362 & 0.404 & -0.481 & 0.362 & 0.36 & 82.9 \\
254.44 & \verb|a8_th_165_ph_90| & 1.005 & -0.211 &-& -0.786 & - &-& - & -0.39 & 61.7 \\
254.35 & \verb|a8_th_165_ph_0| & 1.005 & -0.009 & 0.195 & -0.790 & - & - & - & -0.40 & 61.4 \\
254.35 & \verb|q200_a8_a0_th_30_ph_150| & 2 &-&-&-& -0.346 & 0.200 & 0.693 & 0.23 & 79.5 \\
254.32 & \verb|D10_q0.33_a-0.8_xi0_n100|(*) & 2.999 & 0.757 & 0.030 & 0.259 &-&-& -0.800 & -0.01 & 82.7 \\
254.28 & \verb|a8_th_165_ph_120| & 1.005 & -0.187 & -0.098 & -0.786 & - &-& - & -0.39 & 60.5 \\
254.2 & \verb|a8_th_165_ph_30| & 1.005 & -0.103 & 0.188 & -0.785 & - &-& - & -0.39 & 60.5 \\
254.18 & \verb|hu_a7_th_135_ph_315| & 1.0 & 0.360 & 0.360 & -0.510 & -0.360 & -0.360 & -0.510 & -0.51 & 58.3 \\
254.16 & \verb|D10_q0.33_a0.8_xi0_n120|(*) & 2.999 & 0.754 & 0.031 & -0.268 &-&-& 0.800 & -0.00 & 71.7 \\
254.16 & \verb|DU_D10.90_q2.00_a-0.8_rl10_opt1_n100| & 2.0 &-&-& -0.801 & - & -0.004 & 0.801 & -0.27 & 64.8 \\
254.11 & \verb|9| & 1.501 & - &-& 0.500 & - & - &-& 0.30 & 86.9 \\
254.03 & \verb|q33_a0_a8_th_135_ph_90| & 3 &-& 0.566 & -0.566 &-&-&-& -0.42 & 56.4 \\
254.03 & \verb|q33_a0_a8_th_100_ph_60| & 3 & 0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 74.6 \\
253.98 & \verb|a8_th_165_ph_150| & 1.005 & -0.105 & -0.182 & -0.786 & - & - & - & -0.39 & 61.7 \\
253.93 & \verb|D11_q0.75_a0.8_0.0_n100|(*) & 1.334 &-&-& - &-&-& 0.801 & 0.34 & 85.3 \\
253.87 & \verb|hu_a7_th_60_ph_80| & 1.0 & -0.632 & 0.058 & 0.351 & 0.618 & -0.109 & 0.363 & 0.36 & 85.6 \\
253.82 & \verb|a8_th_30_ph_150| & 1.005 & -0.204 & -0.353 & 0.707 & - &-& - & 0.35 & 84.0 \\
253.82 & \verb|RO3_D10_q2.00_a0.60_oth.090_M120| & 1.999 & 0.600 & 0.002 & - & - & - & 0.600 & 0.20 & 82.6 \\
253.77 & \verb|q33_a0_a8_th_100_ph_150| & 3 & -0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 74.1 \\
253.65 & \verb|q33_a0_a8_th_135_ph_60| & 3 & 0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 58.3 \\
253.65 & \verb|q33_a0_a8_th_100_ph_90| & 3 &-& 0.788 & -0.139 &-&-&-& -0.10 & 67.6 \\
253.63 & \verb|hu_a7_th_135_ph_210| & 1.0 & 0.281 & -0.431 & -0.505 & -0.255 & 0.441 & -0.510 & -0.51 & 58.9 \\
253.57 & \verb|q33_a0_a8_th_75_ph_30| & 3 & 0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 85.3 \\
253.42 & \verb|a8_q1_L_ph_120| & 1.0 & -0.703 & -0.422 & -0.009 & 0.016 & 0.006 & 0.820 & 0.41 & 87.6 \\
253.36 & \verb|a8_th_30_ph_120| & 1.005 & -0.353 & -0.204 & 0.707 & - &-& - & 0.35 & 84.5 \\
253.32 & \verb|hu_a7_th_60_ph_315| & 1.0 & 0.424 & 0.464 & 0.361 & -0.444 & -0.444 & 0.363 & 0.36 & 85.2 \\
253.24 & \verb|a8_th_165_ph_60| & 1.005 & -0.182 & 0.105 & -0.786 &-& - &-& -0.39 & 60.5 \\
253.2 & \verb|RO3_D10_q2.00_a0.60_oth.180_M120| & 1.999 & - & - & -0.600 & - & - & 0.600 & -0.20 & 65.6 \\
253.19 & \verb|q33_a0_a8_th_135_ph_30| & 3 & 0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 60.8 \\
253.19 & \verb|q33_a0_a8_th_75_ph_60| & 3 & 0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 85.1 \\
253.14 & \verb|q33_a0_a8_th_75_ph_90| & 3 &-& 0.773 & 0.207 &-&-&-& 0.16 & 85.1 \\
253.09 & \verb|RO3_D10_q2.50_a0.60_oth.090_M120| & 2.499 & 0.600 & 0.001 & - & - & - & 0.600 & 0.17 & 81.4 \\
252.98 & \verb|(0.0,2.6,'M160','D9')| & 2.6 &-&-&-&-&-&-& 0.00 & 76.7 \\
252.78 & \verb|hu_a7_th_60_ph_0| & 1.0 & -0.053 & 0.616 & 0.379 & 0.028 & -0.624 & 0.368 & 0.37 & 85.6 \\
252.71 & \verb|q33_a0_a8_th_135_ph_0| & 3 & 0.566 &-& -0.566 &-&-&-& -0.42 & 59.7 \\
252.63 & \verb|hu_a7_th_135_ph_90| & 1.0 & -0.510 &-& -0.510 & 0.510 &-& -0.510 & -0.51 & 59.5 \\
252.19 & \verb|q33_a0_a8_th_75_ph_0| & 3 & 0.773 &-& 0.207 &-&-&-& 0.16 & 84.3 \\
252.08 & \verb|hu_a7_th_60_ph_30| & 1.0 & -0.376 & 0.493 & 0.376 & 0.339 & -0.532 & 0.356 & 0.37 & 85.2 \\
251.99 & \verb|hu_a7_th_60_ph_110| & 1.0 & -0.587 & -0.241 & 0.351 & 0.590 & 0.215 & 0.363 & 0.36 & 86.1 \\
251.76 & \verb|hu_a7_th_135_ph_130| & 1.0 & -0.390 & -0.328 & -0.510 & 0.390 & 0.328 & -0.510 & -0.51 & 59.5 \\
251.64 & \verb|hu_a7_th_60_ph_130| & 1.0 & -0.467 & -0.427 & 0.354 & 0.481 & 0.404 & 0.363 & 0.36 & 84.9 \\
251.34 & \verb|a8_th_15_ph_90| & 1.005 & -0.223 & -0.003 & 0.785 &-&-&-& 0.39 & 86.0 \\
251.31 & \verb|D11_q0.75_a-0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& -0.500 & -0.50 & 59.1 \\
251.15 & \verb|hu_a7_th_60_ph_90| & 1.0 & -0.632 & -0.052 & 0.351 & 0.628 &-& 0.363 & 0.36 & 86.6 \\
251.15 & \verb|Del0_D10.97_q1.3333_a-0.6_-0.8_n100| & 1.334 &-&-& -0.600 &-&-& -0.801 & -0.69 & 54.0 \\
250.98 & \verb|(0.0,2.7,'M160','D9')| & 2.7 &-&-&-&-&-&-& 0.00 & 77.7 \\
250.78 & \verb|(0.4,1.25,'M100')| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.4 \\
250.69 & \verb|30| & 3.0 &-&-&-& - &-&-& 0.00 & 77.9 \\
250.6 & \verb|a8_q1_L_ph_150| & 1.0 & -0.385 & -0.724 & 0.002 & 0.012 & 0.003 & 0.820 & 0.41 & 88.0 \\
250.55 & \verb|a8_th_15_ph_0| & 1.005 & -0.005 & 0.215 & 0.788 &-& - & - & 0.39 & 87.6 \\
250.53 & \verb|(0.0,2.8,'M160','D9')| & 2.8 &-&-&-&-&-&-& 0.00 & 77.9 \\
250.47 & \verb|a8_th_15_ph_60| & 1.005 & -0.185 & 0.106 & 0.788 &-&-& - & 0.40 & 87.7 \\
250.41 & \verb|(0.0,3,'M200','D11')| & 3 &-&-&-&-&-&-& 0.00 & 77.8 \\
250.19 & \verb|D11.25_q0.3333_a0.0_0.0_n100|(*) & 3.0 &-&-&-&-&-& - & 0.00 & 77.4 \\
250.14 & \verb|a8_th_15_ph_150| & 1.005 & -0.106 & -0.183 & 0.789 & - &-& - & 0.40 & 86.5 \\
250.14 & \verb|a8_th_15_ph_30| & 1.005 & -0.106 & 0.183 & 0.789 &-& - & - & 0.40 & 87.4 \\
250.12 & \verb|D11_q1.00_a-0.5_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& -0.500 & -0.50 & 58.9 \\
250.06 & \verb|a8_th_15_ph_120| & 1.005 & -0.183 & -0.106 & 0.789 & - & - & - & 0.40 & 86.2 \\
250.06 & \verb|EMu0_D8.80_q1.00_a0.8_n100| & 1.0 &-&-& 0.801 &-&-& - & 0.40 & 89.5 \\
249.96 & \verb|D11_q1.00_a-0.8_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 51.3 \\
249.75 & \verb|q33_a0_a8_th_75_ph_120| & 3 & -0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 85.5 \\
249.71 & \verb|hu_a7_th_60_ph_210| & 1.0 & 0.361 & -0.514 & 0.362 & -0.314 & 0.544 & 0.362 & 0.36 & 86.1 \\
249.66 & \verb|(0.0,2.9,'M160','D9')| & 2.9 &-&-&-&-&-&-& 0.00 & 78.0 \\
249.61 & \verb|q50_a0_a8_th_60_ph_120| & 2.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 84.6 \\
249.58 & \verb|35| & 3.001 & 0.499 & 0.029 & - &-& - &-& -0.00 & 80.8 \\
249.54 & \verb|q50_a0_a8_th_60_ph_90| & 2.0 &-& 0.693 & 0.400 &-&-&-& 0.27 & 89.1 \\
249.46 & \verb|a8_q1_L_ph_60| & 1.0 & -0.746 & 0.341 & -0.002 & 0.016 & -0.002 & 0.820 & 0.41 & 87.1 \\
249.44 & \verb|37| & 3.001 & 0.498 & 0.038 &-&-& - &-& 0.00 & 80.8 \\
249.4 & \verb|a8_q1_L_ph_30| & 1.0 & -0.476 & 0.668 & 0.011 & 0.011 & 0.004 & 0.820 & 0.42 & 87.1 \\
249.29 & \verb|q50_a0_a8_th_60_ph_0| & 2.0 & 0.693 &-& 0.400 &-&-&-& 0.27 & 87.2 \\
249.28 & \verb|('Unbalanced',1,0.2,0.6,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.600 & 0.40 & 89.2 \\
249.26 & \verb|(0.4,1.0,'M200','D11')| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 88.8 \\
249.16 & \verb|q25_a0_a8_th_135_ph_120| & 4.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 58.6 \\
249.1 & \verb|q25_a0_a8_th_135_ph_150| & 4.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 60.9 \\
249.01 & \verb|34| & 3.001 & 0.497 & 0.047 & 0.001 &-& - &-& 0.00 & 80.8 \\
248.96 & \verb|('Unbalanced',1,0.0,0.8,'M160','D11')| & 1 &-&-&-&-&-& 0.800 & 0.40 & 89.3 \\
248.91 & \verb|a8_q1_L_ph_90| & 1.0 & -0.819 & -0.038 & -0.009 & 0.016 &-& 0.820 & 0.41 & 88.5 \\
248.88 & \verb|q16_a0_a8_th115_ph_150| & 6.0 & -0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 66.7 \\
248.79 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.2 \\
248.72 & \verb|q50_a0_a8_th_60_ph_30| & 2.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 87.7 \\
248.66 & \verb|q25_a0_a8_th_135_ph_90| & 4.0 &-& 0.566 & -0.566 &-&-&-& -0.45 & 57.3 \\
248.63 & \verb|q25_a0_a8_th_90_ph_150| & 4.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 74.3 \\
248.51 & \verb|q50_a0_a8_th_60_ph_60| & 2.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 88.4 \\
248.46 & \verb|BBH_SKS_d14.4_q1.19_sA_0_0_0.420_sB_0_0_0.380|(*) & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.40 & 90.1 \\
248.09 & \verb|q50_a0_a8_th_60_ph_150| & 2.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 88.1 \\
248.01 & \verb|44| & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.00 & 80.8 \\
247.86 & \verb|200| & 3.272 & - &-& - &-&-& - & -0.00 & 78.3 \\
247.85 & \verb|a8_q1_L_ph_0| & 1.0 & -0.064 & 0.817 & 0.013 & - & -0.010 & 0.820 & 0.42 & 79.2 \\
247.49 & \verb|(0.0,3.1,'M160','D9')| & 3.1 &-&-&-&-&-&-& 0.00 & 78.5 \\
246.97 & \verb|q25_a0_a8_th_90_ph_30| & 4.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 78.6 \\
246.9 & \verb|q25_a0_a8_th_90_ph_120| & 4.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 77.8 \\
246.88 & \verb|q25_a0_a8_th_135_ph_60| & 4.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 56.6 \\
246.17 & \verb|q25_a0_a8_th_135_ph_30| & 4.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 56.2 \\
245.89 & \verb|RO3_D10_q2.50_a0.40_oth.060_M120| & 2.5 & 0.347 &-& 0.200 & - & - & 0.400 & 0.26 & 86.8 \\
245.58 & \verb|q25_a0_a8_th_135_ph_0| & 4.0 & 0.566 &-& -0.566 &-&-&-& -0.45 & 58.9 \\
245.53 & \verb|32| & 3.001 & 0.248 & 0.037 & -0.432 &-& - &-& -0.32 & 68.2 \\
245.42 & \verb|UD_D8.76_q2.00_a0.8_rl10_opt1_n100| & 2.0 &-&-& 0.801 &-&-& -0.801 & 0.27 & 91.6 \\
245.38 & \verb|42| & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.32 & 68.2 \\
245.28 & \verb|th_90| & 1.0 & -0.809 & -0.030 & 0.443 & 0.808 & -0.006 & 0.446 & 0.44 & 91.0 \\
245.28 & \verb|q25_a0_a8_th_90_ph_60| & 4.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 75.5 \\
245.17 & \verb|(0.0,3.2,'M160','D9')| & 3.2 &-&-&-&-&-&-& 0.00 & 80.2 \\
245.17 & \verb|RO3_D10_q1.50_a0.60_oth.060_M120| & 1.5 & 0.520 & 0.002 & 0.300 & - & - & 0.601 & 0.42 & 88.3 \\
245.1 & \verb|105| & 3.001 &-& - & -0.500 & - & - &-& -0.37 & 66.3 \\
244.87 & \verb|U0_D9.4_q2.00_a0.5_n100_am| & 2.0 &-&-& 0.500 &-&-& - & 0.33 & 91.2 \\
244.31 & \verb|q25_a0_a8_th_90_ph_90| & 4.0 &-& 0.800 &-&-&-&-& 0.00 & 75.3 \\
244.3 & \verb|th_130| & 1.0 & -0.613 & -0.514 & 0.462 & 0.612 & 0.514 & 0.462 & 0.46 & 92.0 \\
244.11 & \verb|RO3_D10_q2.50_a0.40_oth.045_M120| & 2.5 & 0.283 &-& 0.283 & - & - & 0.400 & 0.32 & 89.3 \\
244.08 & \verb|165| & 6.001 & 0.704 & 0.313 & -0.484 & -0.170 & -0.072 & -0.236 & -0.45 & 64.5 \\
243.49 & \verb|d0_D10.53_q6.00_a-0.83333_n100| & 5.996 &-&-& -0.835 &-&-& - & -0.72 & 53.6 \\
243.26 & \verb|q33_a0_a8_th_75_ph_150| & 3 & -0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 86.8 \\
242.52 & \verb|(0.4,1.75,'M100')| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 92.2 \\
242.34 & \verb|hu_a7_th_45_ph_130| & 1.0 & -0.378 & -0.354 & 0.508 & 0.393 & 0.330 & 0.513 & 0.51 & 93.4 \\
242.01 & \verb|th_315| & 1.0 & 0.565 & 0.565 & 0.462 & -0.565 & -0.565 & 0.462 & 0.46 & 92.9 \\
241.96 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 91.6 \\
241.5 & \verb|167| & 4.0 & - & - &-&-&-&-& 0.00 & 79.8 \\
241.47 & \verb|th_210| & 1.0 & 0.458 & -0.653 & 0.465 & -0.400 & 0.692 & 0.462 & 0.46 & 94.0 \\
241.43 & \verb|q16_a0_a8_th135_ph_150| & 6.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 56.4 \\
240.98 & \verb|q16_a0_a8_th135_ph_60| & 6.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 57.8 \\
240.97 & \verb|q16_a0_a8_th135_ph_30| & 6.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 57.8 \\
240.61 & \verb|q16_a0_a8_th90_ph_30| & 6.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 82.1 \\
240.6 & \verb|RO3_D10_q2.00_a0.60_oth.060_M120| & 1.999 & 0.520 & 0.001 & 0.300 & - & - & 0.600 & 0.40 & 91.2 \\
240.58 & \verb|hu_a7_th_45_ph_315| & 1.0 & 0.344 & 0.384 & 0.510 & -0.363 & -0.363 & 0.513 & 0.51 & 93.5 \\
240.57 & \verb|q16_a0_a8_th135_ph_90| & 6.0 &-& 0.566 & -0.566 &-&-&-& -0.48 & 61.7 \\
240.13 & \verb|q16_a0_a8_th135_ph_120| & 6.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 61.1 \\
240.06 & \verb|th_0| & 1.0 & -0.043 & 0.791 & 0.474 & 0.023 & -0.797 & 0.465 & 0.47 & 93.8 \\
239.92 & \verb|th_30| & 1.0 & -0.455 & 0.653 & 0.468 & 0.400 & -0.692 & 0.462 & 0.46 & 93.8 \\
239.9 & \verb|q16_a0_a8_th150_ph_0| & 6.0 & 0.400 &-& -0.693 &-&-&-& -0.59 & 55.4 \\
239.82 & \verb|RO3_D10_q2.50_a0.60_oth.060_M120| & 2.499 & 0.520 & 0.001 & 0.300 & - & - & 0.600 & 0.39 & 87.3 \\
239.8 & \verb|hu_a7_th_45_ph_90| & 1.0 & -0.518 & -0.054 & 0.505 & 0.513 &-& 0.513 & 0.51 & 93.3 \\
239.66 & \verb|d0_D10.52_q3.00_a-0.66667_n100| & 2.999 &-&-& -0.667 &-&-& - & -0.50 & 59.2 \\
239.56 & \verb|hu_a7_th_45_ph_210| & 1.0 & 0.299 & -0.412 & 0.516 & -0.256 & 0.444 & 0.513 & 0.51 & 93.6 \\
239.47 & \verb|D11.00_q0.2500_a0.0_0.0_n100|(*) & 4.0 &-&-&-&-&-& - & 0.00 & 80.1 \\
239.39 & \verb|D11_q0.75_a0.0_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& - & 0.46 & 94.3 \\
239.31 & \verb|q16_a0_a8_th150_ph_120| & 6.0 & -0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 54.0 \\
239.29 & \verb|q16_a0_a8_th90_ph_90| & 6.0 &-& 0.800 &-&-&-&-& 0.00 & 82.5 \\
239.14 & \verb|q16_a0_a8_th135_ph_0| & 6.0 & 0.566 &-& -0.566 &-&-&-& -0.48 & 59.5 \\
239.05 & \verb|RO3_D10_q2.00_a0.60_oth.045_M120| & 2.0 & 0.425 &-& 0.424 & - & - & 0.600 & 0.48 & 95.3 \\
238.97 & \verb|EMuu_D8.82_q1.00_a0.2_n100| & 1.0 &-&-& 0.801 &-&-& 0.200 & 0.50 & 95.0 \\
238.91 & \verb|q16_a0_a8_th90_ph_150| & 6.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 79.4 \\
238.85 & \verb|q16_a0_a8_th115_ph_120| & 6.0 & -0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 67.1 \\
238.83 & \verb|q16_a0_a8_th90_ph_120| & 6.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 81.7 \\
238.74 & \verb|D11_q1.00_a0.5_0.5_n100|(*) & 1.0 &-&-& 0.500 &-&-& 0.500 & 0.50 & 94.7 \\
238.67 & \verb|q16_a0_a8_th90_ph_0| & 6.0 & 0.800 &-&-&-&-&-& 0.00 & 82.2 \\
238.48 & \verb|q16_a0_a8_th90_ph_60| & 6.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 82.9 \\
238.41 & \verb|hu_a7_th_45_ph_0| & 1.0 & -0.028 & 0.507 & 0.517 & 0.028 & -0.507 & 0.518 & 0.52 & 94.3 \\
238.2 & \verb|q16_a0_a8_th150_ph_60| & 6.0 & 0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 54.7 \\
238.11 & \verb|q16_a0_a8_th115_ph_60| & 6.0 & 0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 68.0 \\
237.85 & \verb|RO3_D10_q1.50_a0.60_oth.045_M120| & 1.499 & 0.424 & 0.034 & 0.425 & 0.003 & 0.004 & 0.604 & 0.50 & 95.2 \\
237.64 & \verb|('Unbalanced',1,0.2,0.8,'M160','D11')| & 1 &-&-& 0.200 &-&-& 0.800 & 0.50 & 94.7 \\
237.57 & \verb|q16_a0_a8_th150_ph_90| & 6.0 &-& 0.400 & -0.693 &-&-&-& -0.59 & 54.8 \\
237.26 & \verb|q16_a0_a8_th150_ph_30| & 6.0 & 0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 54.8 \\
237.23 & \verb|hu_a7_th_45_ph_30| & 1.0 & -0.299 & 0.411 & 0.518 & 0.256 & -0.444 & 0.513 & 0.52 & 94.6 \\
236.8 & \verb|q16_a0_a8_th150_ph_150| & 6.0 & -0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 53.3 \\
236.68 & \verb|162| & 2.0 &-& - & 0.600 &-&-&-& 0.40 & 95.3 \\
236.58 & \verb|D11_q0.75_a0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& 0.500 & 0.50 & 95.2 \\
236.06 & \verb|q16_a0_a8_th115_ph_90| & 6.0 &-& 0.725 & -0.338 &-&-&-& -0.29 & 64.2 \\
236.0 & \verb|DU_D10.60_q3.00_a-0.8_rl11_n120| & 2.999 &-&-& -0.801 &-&-& 0.800 & -0.40 & 60.5 \\
235.28 & \verb|q50_a0_a8_th_30_ph_120| & 2.0 & -0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 95.2 \\
234.19 & \verb|q16_a0_a8_th115_ph_0| & 6.0 & 0.725 &-& -0.338 &-&-&-& -0.29 & 72.3 \\
234.13 & \verb|q25_a0_a8_th_90_ph_0| & 4.0 & 0.800 &-&-&-&-&-& 0.00 & 86.2 \\
233.96 & \verb|43| & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.32 & 95.5 \\
233.91 & \verb|190| & 4.499 & - &-& - &-&-&-& -0.00 & 81.1 \\
233.85 & \verb|q16_a0_a8_th115_ph_30| & 6.0 & 0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 72.3 \\
233.43 & \verb|q50_a0_a8_th_30_ph_150| & 2.0 & -0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 96.7 \\
233.42 & \verb|q50_a0_a8_th_30_ph_30| & 2.0 & 0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 97.4 \\
233.41 & \verb|33| & 3.001 & 0.248 & 0.030 & 0.432 & - & - &-& 0.32 & 94.8 \\
233.19 & \verb|q50_a0_a8_th_30_ph_90| & 2.0 &-& 0.400 & 0.693 &-&-&-& 0.46 & 91.1 \\
231.37 & \verb|q50_a0_a8_th_30_ph_60| & 2.0 & 0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 93.3 \\
231.29 & \verb|q50_a0_a8_th_30_ph_0| & 2.0 & 0.400 &-& 0.693 &-&-&-& 0.46 & 89.6 \\
231.13 & \verb|q25_a0_a8_th_60_ph_60| & 4.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 94.0 \\
231.04 & \verb|a8_q1_KoL_th45_ph_90| & 1.0 & -0.595 & -0.035 & 0.562 & -0.591 & - & -0.568 & -0.00 & 79.1 \\
230.5 & \verb|q25_a0_a8_th_60_ph_90| & 4.0 &-& 0.693 & 0.400 &-&-&-& 0.32 & 92.5 \\
229.89 & \verb|159| & 1.0 &-&-& -0.900 & - & - & -0.900 & -0.90 & 51.1 \\
229.77 & \verb|d0_D11.03_q4.00_a-0.75_v2_n100| & 3.998 &-&-& -0.751 & - &-& - & -0.60 & 54.1 \\
229.42 & \verb|q25_a0_a8_th_60_ph_0| & 4.0 & 0.693 &-& 0.400 &-&-&-& 0.32 & 91.7 \\
229.17 & \verb|187| & 5.039 &-& - &-& - & - & - & 0.00 & 82.8 \\
228.78 & \verb|Del0_D8.87_q2.00_a0.4_0.8_n100| & 2.001 &-&-& 0.400 & 0.015 & -0.007 & 0.800 & 0.53 & 98.6 \\
228.65 & \verb|q25_a0_a8_th_60_ph_165| & 4.0 & -0.669 & 0.179 & 0.400 &-&-&-& 0.32 & 94.0 \\
228.48 & \verb|RO3_D10_q2.50_a0.60_oth.045_M120| & 2.499 & 0.424 &-& 0.424 & - & - & 0.600 & 0.47 & 99.0 \\
228.45 & \verb|q25_a0_a8_th_60_ph_30| & 4.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 92.8 \\
227.91 & \verb|174| & 3.001 &-& - & 0.500 & - &-&-& 0.37 & 99.4 \\
227.55 & \verb|156| & 1.0 &-&-& -0.949 &-&-& -0.949 & -0.95 & 50.5 \\
227.15 & \verb|q25_a0_a8_th_60_ph_150| & 4.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 94.8 \\
226.91 & \verb|q25_a0_a8_th_60_ph_120| & 4.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 103.0 \\
225.54 & \verb|EMuu_D8.78_q1.00_a0.4_n100| & 1.0 &-&-& 0.801 &-&-& 0.400 & 0.60 & 101.0 \\
225.28 & \verb|197| & 5.522 & - &-& - &-&-& - & -0.00 & 83.6 \\
224.78 & \verb|(0.6,1.25,'M100')| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 100.4 \\
224.76 & \verb|DU_D10.61_q4.00_a-0.8_rl11_n100| & 3.999 &-&-& -0.801 &-&-& 0.800 & -0.48 & 56.3 \\
224.25 & \verb|q25_a0_a8_th_60_ph_135| & 4.0 & -0.490 & 0.490 & 0.400 &-&-&-& 0.32 & 94.7 \\
223.95 & \verb|152| & 1.0 &-& - & 0.600 & - &-& 0.600 & 0.60 & 101.4 \\
223.9 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 101.1 \\
223.8 & \verb|q33_a0_a8_th_45_ph_120| & 3 & -0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 94.6 \\
223.02 & \verb|q33_a0_a8_th_45_ph_150| & 3 & -0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 105.7 \\
222.95 & \verb|q33_a0_a8_th_45_ph_0| & 3 & 0.566 &-& 0.566 &-&-&-& 0.42 & 103.0 \\
222.51 & \verb|166| & 6.0 & - & - &-&-&-&-& 0.00 & 84.2 \\
222.47 & \verb|(0.6,1.5,'M100')| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 101.8 \\
221.74 & \verb|D10.50_q0.1667_a0.0_0.0_n100|(*) & 6.0 &-&-&-&-&-& - & 0.00 & 84.1 \\
221.04 & \verb|hu_a7_th_22.5_ph_90| & 1.0 & -0.288 & -0.026 & 0.665 & 0.278 &-& 0.670 & 0.67 & 102.1 \\
220.99 & \verb|hu_a7_th_22.5_ph_315| & 1.0 & 0.196 & 0.196 & 0.670 & -0.196 & -0.196 & 0.670 & 0.67 & 102.3 \\
220.89 & \verb|q33_a0_a8_th_45_ph_30| & 3 & 0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 103.5 \\
220.75 & \verb|q33_a0_a8_th_45_ph_90| & 3 &-& 0.566 & 0.566 &-&-&-& 0.42 & 104.3 \\
220.51 & \verb|d0_D11.35_q5.00_a-0.8_opt1_n100| & 4.997 &-&-& -0.801 &-&-& - & -0.67 & 60.9 \\
220.42 & \verb|hu_a7_th_22.5_ph_30| & 1.0 & -0.160 & 0.221 & 0.672 & 0.139 & -0.240 & 0.670 & 0.67 & 103.0 \\
220.2 & \verb|hu_a7_th_22.5_ph_130| & 1.0 & -0.213 & -0.178 & 0.670 & 0.213 & 0.178 & 0.670 & 0.67 & 103.5 \\
220.14 & \verb|q33_a0_a8_th_45_ph_60| & 3 & 0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 103.0 \\
220.03 & \verb|(0.6,1.75,'M100')| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 103.6 \\
219.69 & \verb|D11.50_q0.50_a0.50_0.60_n100|(*) & 2.0 &-&-& 0.600 &-&-& 0.500 & 0.57 & 103.5 \\
218.22 & \verb|hu_a7_th_22.5_ph_0| & 1.0 &-& 0.278 & 0.670 &-& -0.278 & 0.670 & 0.67 & 102.2 \\
218.06 & \verb|192| & 6.58 & - &-&-& - & - & - & 0.00 & 85.6 \\
217.76 & \verb|hu_a7_th_22.5_ph_210| & 1.0 & 0.139 & -0.240 & 0.670 & -0.139 & 0.240 & 0.670 & 0.67 & 104.2 \\
216.7 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 106.2 \\
213.8 & \verb|UD_D8.40_q3.00_a0.8_rl11_n120| & 2.999 &-&-& 0.801 &-&-& -0.800 & 0.40 & 108.8 \\
213.31 & \verb|188| & 7.187 &-& - &-& - &-& - & -0.00 & 86.5 \\
212.86 & \verb|hu_a9_th_30_ph_210| & 1.0 & 0.231 & -0.400 & 0.800 & -0.231 & 0.400 & 0.800 & 0.80 & 113.9 \\
212.62 & \verb|Del0_D8.83_q1.3333_a0.6_0.8_n100| & 1.334 &-&-& 0.600 &-&-& 0.801 & 0.69 & 107.3 \\
211.64 & \verb|179| & 1.5 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.65 & 104.3 \\
211.56 & \verb|hu_a9_th_30_ph_0| & 1.0 & -0.027 & 0.445 & 0.809 & -0.004 & -0.462 & 0.800 & 0.80 & 108.1 \\
210.33 & \verb|195| & 7.761 & - & - &-& - &-& - & 0.00 & 88.0 \\
209.98 & \verb|U0_D9.07_q3.00_a0.66667_n100| & 2.999 &-&-& 0.667 &-&-& - & 0.50 & 108.9 \\
209.23 & \verb|hu_a9_th_30_ph_90| & 1.0 & -0.462 & -0.003 & 0.800 & 0.462 & 0.003 & 0.800 & 0.80 & 113.1 \\
206.76 & \verb|hu_a9_th_30_ph_130| & 1.0 & -0.354 & -0.297 & 0.800 & 0.354 & 0.297 & 0.800 & 0.80 & 113.9 \\
206.46 & \verb|hu_a9_th_30_ph_30| & 1.0 & -0.262 & 0.381 & 0.799 & 0.231 & -0.400 & 0.800 & 0.80 & 114.7 \\
205.75 & \verb|hu_a9_th_30_ph_315| & 1.0 & 0.327 & 0.327 & 0.800 & -0.327 & -0.327 & 0.800 & 0.80 & 115.1 \\
202.73 & \verb|175| & 1.0 &-& - & 0.750 & - &-& 0.750 & 0.75 & 112.6 \\
198.55 & \verb|q16_a0_a8_th45_ph_120| & 6.0 & -0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 128.9 \\
198.08 & \verb|q16_a0_a8_th45_ph_150| & 6.0 & -0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 119.2 \\
196.51 & \verb|D10_q1.00_a0.8_0.8_n100|(*) & 1.0 &-&-& 0.801 &-&-& 0.801 & 0.80 & 118.0 \\
195.8 & \verb|(0.8,1.0,'M200','D11')| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 116.2 \\
194.98 & \verb|q16_a0_a8_th45_ph_60| & 6.0 & 0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 114.1 \\
194.87 & \verb|q16_a0_a8_th45_ph_90| & 6.0 &-& 0.566 & 0.566 &-&-&-& 0.48 & 110.3 \\
194.67 & \verb|q16_a0_a8_th45_ph_0| & 6.0 & 0.566 &-& 0.566 &-&-&-& 0.48 & 122.9 \\
194.59 & \verb|155| & 1.0 & - & - & 0.800 &-&-& 0.800 & 0.80 & 117.3 \\
192.34 & \verb|q16_a0_a8_th45_ph_30| & 6.0 & 0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 112.5 \\
191.76 & \verb|hu_a9_th_15_ph_315| & 1.0 & 0.169 & 0.169 & 0.893 & -0.169 & -0.169 & 0.893 & 0.89 & 124.1 \\
191.36 & \verb|hu_a9_th_15_ph_0| & 1.0 &-& 0.239 & 0.893 &-& -0.239 & 0.893 & 0.89 & 121.5 \\
190.86 & \verb|hu_a9_th_15_ph_130| & 1.0 & -0.183 & -0.154 & 0.893 & 0.183 & 0.154 & 0.893 & 0.89 & 124.1 \\
190.22 & \verb|hu_a9_th_15_ph_30| & 1.0 & -0.120 & 0.207 & 0.892 & 0.120 & -0.207 & 0.893 & 0.89 & 122.7 \\
189.69 & \verb|U0_D8.8_q4.00_a0.75_n100_am| & 3.999 &-&-& 0.751 &-&-& - & 0.60 & 130.1 \\
189.66 & \verb|hu_a9_th_15_ph_210| & 1.0 & 0.120 & -0.207 & 0.892 & -0.120 & 0.207 & 0.893 & 0.89 & 122.1 \\
187.36 & \verb|153| & 1.0 & - & - & 0.850 &-&-& 0.850 & 0.85 & 121.4 \\
186.5 & \verb|hu_a9_th_15_ph_90| & 1.0 & -0.258 & 0.005 & 0.887 & 0.258 & -0.005 & 0.888 & 0.89 & 123.8 \\
185.87 & \verb|UU_D8.56_q2.00_a0.8_m100| & 2.0 &-&-& 0.801 & 0.016 & -0.004 & 0.800 & 0.80 & 123.8 \\
181.58 & \verb|151| & 1.0 &-& - & -0.600 & - &-& -0.600 & -0.60 & 67.0 \\
178.52 & \verb|160| & 1.0 &-& - & 0.900 &-&-& 0.900 & 0.90 & 126.1 \\
169.9 & \verb|157| & 1.0 & - &-& 0.950 &-& - & 0.950 & 0.95 & 128.1 \\
169.84 & \verb|U0_D8.65_q5.00_a0.8_n100| & 4.997 &-&-& 0.801 &-&-&-& 0.67 & 141.9 \\
168.26 & \verb|176| & 1.0 &-& - & 0.960 & - &-& 0.960 & 0.96 & 130.6 \\
166.67 & \verb|158| & 1.0 &-& - & 0.970 & - &-& 0.970 & 0.97 & 131.0 \\
165.46 & \verb|172| & 1.0 &-& - & 0.979 & - &-& 0.979 & 0.98 & 131.5 \\
163.03 & \verb|177| & 1.0 &-&-& 0.989 & - & - & 0.989 & 0.99 & 132.8 \\
162.08 & \verb|178| & 1.0 &-&-& 0.994 & - & - & 0.994 & 0.99 & 133.8 \\
147.44 & \verb|U0_D8.51_q6.00_a0.83333_n100_am| & 5.996 & 0.003 & -0.023 & 0.834 & - & - & - & 0.71 & 164.8 \\
\end{longtable}


==> simulation-rankings_30_C01.tex <==
\begin{longtable}{l|l|lrrrrrr|rr|r}
\caption{\label{tab:SimulationRanks:30}\textbf{Peak Marginalized $\ln L$ I: Consistency between simulations}: Peak value of the marginalized log likelihood $\ln L$ [Eq. (\ref{eq:lnL})] evaluated using a lower frequency $f_{\rm low}=30\unit{Hz}$ and all modes with $l \le 2$; the simulation key, described in Table \ref{tab:SimulationList} [an asterisk (*) denotes a new simulation motivated by \TheEvent{}, and a (+) denotes one of the simulations reported in \PaperDetection];  the \emph{initial} spins of the simulation (using $-$ to denote zero, to enhance readability); the initial $\chi_{\rm eff}$; the total (redshifted) mass of the best fit; and the starting frequency (in Hz) of the best fit.  Though omitting information accessible to the longest simulations, this choice of low-frequency cutoff eliminates systematic biases associated with simulation duration, which differs across our archive, as seen by the last column.  } \\ \hline \hline $\ln L$ & Key & $q$ & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ & $\chi_{\rm eff}$ & $M_z/M_\odot$  & $f_{\rm start} ({\rm Hz})$ \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot 
272.2 & \verb|SXS:BBH:0310|(*) & 1.221 & - &-&-& - & - &-& 0.00 & 73.0 & 15.3 \\
272.1 & \verb|D12_q1.00_a-0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& -0.250 & -0.00 & 73.2 & 20.5 \\
272.1 & \verb|SXS:BBH:0002| & 1.0 &-& - &-&-&-&-& 0.00 & 73.2 & 9.9 \\
271.8 & \verb|D11_q0.75_a0.0_0.0_n100|(*) & 1.333 &-&-& - &-&-& - & -0.00 & 72.1 & 23.1 \\
271.8 & \verb|SXS:BBH:0305|(*+) & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.02 & 74.2 & 15.3 \\
271.6 & \verb|SXS:BBH:0218| & 1.0 &-& - & -0.500 & - & - & 0.500 & 0.00 & 73.3 & 10.7 \\
271.6 & \verb|SXS:BBH:0198| & 1.202 & - & - & - & - & - &-& 0.00 & 73.4 & 12.9 \\
271.6 & \verb|SXS:BBH:0307|(*) & 1.228 & - & - & 0.320 &-& - & -0.580 & -0.08 & 70.0 & 17.6 \\
271.6 & \verb|GT:BBH:476| & 1.0 &-&-& -0.200 &-&-& -0.200 & -0.20 & 67.9 & 24.3 \\
271.6 & \verb|S0_D10.04_q1.3333_a0.45_-0.80_n100| & 1.334 &-&-& 0.450 &-&-& -0.801 & -0.09 & 71.9 & 27.9 \\
271.5 & \verb|D12.00_q0.85_a0.0_0.0_n100|(*) & 1.176 &-&-& - &-&-& - & -0.00 & 73.0 & 20.6 \\
271.5 & \verb|D12.25_q0.82_a-0.44_0.33_n100|(*+) & 1.22 &-&-& 0.330 &-&-& -0.440 & -0.02 & 72.9 & 20.2 \\
271.5 & \verb|SXS:BBH:0312|(*) & 1.203 &-& - & 0.390 &-&-& -0.480 & -0.00 & 73.9 & 15.2 \\
271.4 & \verb|SXS:BBH:0127| & 1.34 & 0.010 & -0.077 & -0.017 & -0.061 & -0.065 & -0.179 & -0.09 & 71.5 & 14.7 \\
271.4 & \verb|SXS:BBH:0115| & 1.07 & 0.019 & 0.013 & -0.204 & 0.243 & -0.067 & 0.291 & 0.04 & 74.1 & 14.6 \\
271.3 & \verb|SXS:BBH:0213| & 1.0 &-& - & -0.800 & - &-& 0.800 & 0.00 & 73.2 & 12.4 \\
271.3 & \verb|UD_D10.01_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& -0.400 & -0.00 & 73.4 & 26.7 \\
271.2 & \verb|D12_q1.00_a-0.25_0.00_n100|(*) & 1.0 &-&-& - &-&-& -0.250 & -0.12 & 69.4 & 21.8 \\
271.2 & \verb|SXS:BBH:0222| & 1.0 &-&-& -0.300 &-&-&-& -0.15 & 69.1 & 12.5 \\
271.2 & \verb|SXS:BBH:0217| & 1.0 &-& - & -0.600 & - &-& 0.600 & 0.00 & 73.2 & 12.4 \\
271.1 & \verb|D10_q0.75_a-0.5_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.500 & -0.07 & 71.9 & 27.4 \\
271.0 & \verb|BAM150914:24|(*) & 1.2 & 0.151 & 0.396 & 0.017 & -0.278 & -0.605 & -0.085 & -0.03 & 72.2 & 17.8 \\
270.9 & \verb|GW15_D12_q1.22_a0.33_-0.44_m140|(*) & 1.22 & - &-& 0.330 & - &-& -0.440 & -0.02 & 71.7 & 19.7 \\
270.9 & \verb|SXS:BBH:0308[Lev3]|(*) & 1.228 & 0.072 & 0.072 & 0.325 & 0.201 & 0.285 & -0.571 & -0.08 & 70.5 & 17.7 \\
270.9 & \verb|SXS:BBH:0120| & 1.12 & 0.138 & -0.200 & -0.008 & -0.065 & -0.241 & -0.099 & -0.05 & 70.3 & 14.8 \\
270.8 & \verb|SXS:BBH:0006| & 1.345 & 0.234 & 0.148 & -0.161 & 0.091 & 0.064 & -0.101 & -0.14 & 69.6 & 13.6 \\
270.8 & \verb|SXS:BBH:0313|(*) & 1.217 &-& - & 0.380 &-&-& -0.520 & -0.03 & 72.5 & 15.6 \\
270.7 & \verb|GT:BBH:370| & 1.15 &-&-&-&-&-&-& 0.00 & 74.0 & 25.8 \\
270.7 & \verb|SXS:BBH:0308| & 1.228 & 0.094 & 0.056 & 0.322 & 0.266 & 0.213 & -0.576 & -0.08 & 71.8 & 17.2 \\
270.6 & \verb|SXS:BBH:0123| & 1.1 & 0.267 & 0.020 & -0.415 & 0.038 & -0.054 & 0.126 & -0.16 & 68.0 & 16.3 \\
270.6 & \verb|D11_q0.75_a-0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& -0.500 & 0.07 & 76.7 & 21.6 \\
270.5 & \verb|SXS:BBH:0129| & 1.36 & -0.001 & - & 0.088 & 0.193 & -0.289 & -0.075 & 0.02 & 74.0 & 14.0 \\
270.5 & \verb|SXS:BBH:0117| & 1.08 & 0.118 & -0.069 & 0.070 & -0.302 & -0.298 & -0.200 & -0.06 & 72.8 & 14.7 \\
270.4 & \verb|SXS:BBH:0003| & 1.0 & 0.497 & 0.053 & - &-&-&-& -0.00 & 72.5 & 11.6 \\
270.4 & \verb|D10_q0.75_a-0.25_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.250 & 0.04 & 75.7 & 24.7 \\
270.4 & \verb|SXS:BBH:0224| & 1.0 & - &-& 0.400 & - & - & -0.800 & -0.20 & 67.3 & 13.0 \\
270.3 & \verb|D11_q0.75_a-0.8500_0.6375_n100| & 1.334 &-&-& 0.638 & 0.001 & 0.003 & -0.851 & -0.00 & 74.8 & 22.6 \\
270.3 & \verb|U0_D9.53_q1.00_a0.0_n100| & 1.0 &-&-& - &-&-& - & -0.00 & 73.7 & 28.6 \\
270.2 & \verb|SXS:BBH:0211| & 1.0 &-&-& -0.900 &-&-& 0.900 & 0.00 & 73.5 & 12.3 \\
270.2 & \verb|SXS:BBH:0116| & 1.08 & -0.078 & 0.065 & 0.033 & 0.185 & 0.007 & 0.103 & 0.07 & 76.4 & 13.7 \\
270.2 & \verb|D11_q0.75_a0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& 0.500 & -0.07 & 70.2 & 23.9 \\
270.2 & \verb|GW15_D12_q1.19_a0.42_-0.38_m140|(*) & 1.19 & - &-& 0.420 & - &-& -0.380 & 0.05 & 74.0 & 18.6 \\
270.1 & \verb|GT:BBH:900|(*) & 1.2 & 0.400 &-&-& 0.400 &-&-& 0.00 & 74.3 & 21.8 \\
270.1 & \verb|D11_q0.75_a-0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& -0.500 & -0.21 & 67.8 & 24.4 \\
270.0 & \verb|GT:BBH:898|(*) & 1.2 &-&-&-&-&-&-& 0.00 & 74.2 & 18.0 \\
269.9 & \verb|aa_b5_a0.6_M77| & 1 &-&-& 0.600 &-&-& -0.600 & 0.00 & 73.7 & 25.2 \\
269.9 & \verb|SXS:BBH:0125| & 1.27 & 0.012 & 0.045 & -0.058 & 0.389 & 0.241 & 0.070 & -0.00 & 75.1 & 13.3 \\
269.9 & \verb|D21.5_q1_a0.2_0.8_th104.4775_n100| & 1.001 &-&-& 0.200 & 0.775 &-& -0.200 & -0.00 & 74.2 & 9.7 \\
269.9 & \verb|SXS:BBH:0131| & 1.55 & 0.042 & -0.014 & -0.070 & 0.105 & 0.017 & -0.175 & -0.11 & 71.0 & 14.8 \\
269.8 & \verb|SXS:BBH:0096| & 1.501 & 0.497 & 0.051 & - &-&-&-& -0.00 & 73.0 & 13.2 \\
269.8 & \verb|SXS:BBH:0088| & 1.0 & 0.495 & 0.067 &-&-&-&-& 0.00 & 74.3 & 11.6 \\
269.7 & \verb|D10_q0.75_a-0.8_xi0_n100|(*) & 1.333 & 0.538 & 0.056 & 0.590 &-&-& -0.801 & -0.01 & 75.2 & 26.5 \\
269.7 & \verb|SXS:BBH:0029| & 1.5 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.00 & 74.3 & 13.4 \\
269.6 & \verb|BAM150914:25|(*) & 1.2 & 0.119 & -0.407 & 0.017 & 0.125 & 0.656 & -0.064 & -0.02 & 72.3 & 22.3 \\
269.6 & \verb|SXS:BBH:0163| & 1.0 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.02 & 73.5 & 13.6 \\
269.6 & \verb|SXS:BBH:0226| & 1.0 &-&-& 0.500 & - &-& -0.900 & -0.20 & 67.4 & 12.9 \\
269.5 & \verb|D10_q0.75_a0.25_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.250 & -0.04 & 71.8 & 26.2 \\
269.5 & \verb|BAM150914:9|(*) & 1.2 & 0.554 & -0.314 & 0.212 & 0.008 & 0.643 & -0.191 & 0.03 & 72.7 & 27.9 \\
269.4 & \verb|SXS:BBH:0316|(*) & 1.186 & 0.241 & 0.170 & 0.299 & -0.203 & -0.172 & -0.271 & 0.04 & 75.2 & 15.0 \\
269.4 & \verb|SXS:BBH:0121| & 1.12 & -0.061 & -0.109 & 0.356 & -0.323 & -0.127 & -0.297 & 0.05 & 76.5 & 14.7 \\
269.4 & \verb|SXS:BBH:0097| & 1.501 & 0.495 & 0.065 & 0.001 &-&-&-& 0.00 & 72.7 & 15.0 \\
269.4 & \verb|BAM150914:31|(*) & 1.2 & 0.384 & -0.135 & -0.119 & -0.354 & 0.218 & 0.086 & -0.03 & 71.5 & 23.9 \\
269.4 & \verb|SXS:BBH:0100| & 1.5 & - & - &-&-& - &-& 0.00 & 74.4 & 10.7 \\
269.2 & \verb|D10_q0.75_a0.5_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.500 & 0.07 & 75.2 & 24.7 \\
269.2 & \verb|GT:BBH:448| & 1.0 &-&-&-&-&-&-& 0.00 & 76.0 & 21.5 \\
269.1 & \verb|SXS:BBH:0135| & 1.64 & -0.110 & 0.027 & 0.024 & 0.211 & -0.144 & -0.229 & -0.07 & 71.5 & 14.5 \\
269.1 & \verb|SXS:BBH:0149| & 1.0 &-& - & -0.200 & - &-& -0.200 & -0.20 & 68.3 & 14.8 \\
269.0 & \verb|BAM150914:6|(*) & 1.2 & 0.662 & -0.070 & 0.083 & -0.358 & 0.201 & -0.106 & -0.00 & 72.7 & 23.8 \\
269.0 & \verb|BAM150914:14|(*) & 1.2 & 0.662 & -0.015 & 0.106 & -0.384 & 0.113 & -0.141 & -0.01 & 71.0 & 23.9 \\
268.9 & \verb|RIT:BBH:STH45PH30| & 1.0 & -0.337 & 0.463 & 0.585 & 0.290 & -0.502 & -0.579 & 0.00 & 71.0 & 37.6 \\
268.9 & \verb|SXS:BBH:0147| & 1.0 & 0.404 & 0.294 & -0.001 & -0.404 & -0.294 & -0.001 & -0.00 & 71.0 & 24.6 \\
268.9 & \verb|SXS:BBH:0194| & 1.518 &-& - &-& - &-& - & -0.00 & 73.0 & 13.9 \\
268.9 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 74.0 & 31.3 \\
268.8 & \verb|D11_q0.75_a0.8_0.4_PNr500_th1d_n100|(*) & 1.334 & 0.074 & -0.374 & 0.123 & -0.420 & -0.531 & -0.427 & -0.11 & 71.8 & 23.5 \\
268.8 & \verb|SXS:BBH:0138| & 1.7 & -0.044 & 0.425 & 0.042 & -0.012 & -0.008 & -0.111 & -0.01 & 73.9 & 14.1 \\
268.8 & \verb|SXS:BBH:0119| & 1.12 & -0.012 & 0.068 & 0.260 & 0.078 & -0.003 & 0.006 & 0.14 & 78.8 & 13.4 \\
268.6 & \verb|BAM150914:15|(*) & 1.2 & 0.276 & -0.106 & 0.052 & 0.144 & 0.268 & 0.295 & 0.16 & 77.4 & 18.4 \\
268.6 & \verb|SXS:BBH:0133| & 1.63 & 0.098 & 0.042 & -0.134 & -0.107 & -0.110 & -0.021 & -0.09 & 71.7 & 14.0 \\
268.6 & \verb|BAM150914:2|(*) & 1.2 & -0.099 & -0.377 & -0.167 & -0.108 & 0.484 & 0.452 & 0.11 & 76.3 & 21.6 \\
268.5 & \verb|SXS:BBH:0098| & 1.501 & 0.486 & 0.114 & 0.002 &-&-&-& 0.00 & 75.1 & 11.5 \\
268.4 & \verb|aa_b5_a0.8_M77| & 1 &-&-& 0.800 &-&-& -0.800 & 0.00 & 75.3 & 26.5 \\
268.4 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 73.0 & 30.8 \\
268.4 & \verb|D11.50_q0.60_a0.0_0.0_n100|(*) & 1.667 &-&-& - &-&-& - & -0.00 & 73.6 & 21.2 \\
268.4 & \verb|d0_D10.52_q1.3333_a-0.25_n100| & 1.333 &-&-& -0.250 &-&-& - & -0.14 & 69.1 & 26.2 \\
268.3 & \verb|SXS:BBH:0223| & 1.0 &-&-& 0.300 & - &-&-& 0.15 & 78.8 & 11.7 \\
268.3 & \verb|SXS:BBH:0082| & 1.501 & 0.496 & 0.053 & - &-&-&-& -0.00 & 75.5 & 13.7 \\
268.3 & \verb|RIT:BBH:STH45PH60| & 1.0 & -0.537 & 0.242 & 0.570 & 0.502 & -0.290 & -0.579 & -0.00 & 68.9 & 37.9 \\
268.3 & \verb|SXS:BBH:0027| & 1.5 & 0.497 & 0.051 & - & -0.494 & -0.071 &-& 0.00 & 72.8 & 13.9 \\
268.2 & \verb|BAM150914:5|(*) & 1.2 & 0.649 & 0.149 & 0.086 & -0.385 & -0.130 & -0.124 & -0.01 & 71.0 & 22.1 \\
268.2 & \verb|D12_q1.00_a-0.25_-0.25_n100|(*) & 1.0 &-&-& -0.250 &-&-& -0.250 & -0.25 & 65.7 & 23.1 \\
268.2 & \verb|aa_b5_a0.2_M77| & 1 &-&-& 0.200 &-&-& -0.200 & 0.00 & 75.3 & 23.2 \\
268.2 & \verb|SXS:BBH:0173| & 1.5 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.14 & 68.9 & 13.8 \\
268.2 & \verb|aa_b5_a0.4_M77| & 1 &-&-& 0.400 &-&-& -0.400 & 0.00 & 75.3 & 23.8 \\
268.1 & \verb|RIT:BBH:NTH120PH150| & 1.005 & -0.322 & -0.617 & -0.422 & - & - &-& -0.21 & 65.2 & 36.6 \\
268.1 & \verb|SXS:BBH:0103| & 1.501 & 0.496 & 0.058 &-&-&-&-& 0.00 & 75.5 & 10.5 \\
268.1 & \verb|GT:BBH:885| & 1.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.00 & 72.8 & 31.2 \\
268.1 & \verb|SXS:BBH:0004| & 1.0 & - & - & -0.500 & - & - &-& -0.25 & 66.2 & 11.3 \\
268.1 & \verb|SXS:BBH:0023| & 1.501 & 0.497 & 0.051 & 0.001 & 0.077 & -0.489 &-& 0.00 & 73.0 & 13.5 \\
268.0 & \verb|BAM150914:3|(*) & 1.2 & 0.299 & 0.028 & 0.008 & 0.192 & 0.092 & 0.367 & 0.17 & 77.3 & 18.2 \\
268.0 & \verb|BAM150914:4|(*) & 1.2 & 0.159 & -0.393 & -0.016 & 0.149 & 0.654 & -0.014 & -0.02 & 70.1 & 23.0 \\
268.0 & \verb|SXS:BBH:0021| & 1.5 & 0.496 & 0.053 & - & - & 0.001 & -0.499 & -0.20 & 70.3 & 12.7 \\
268.0 & \verb|SXS:BBH:0015| & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.00 & 75.0 & 10.4 \\
268.0 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 76.4 & 24.7 \\
267.9 & \verb|RIT:BBH:KTH45PH60| & 1.0 & -0.549 & 0.217 & 0.568 & -0.502 & 0.290 & -0.579 & -0.01 & 73.9 & 34.9 \\
267.9 & \verb|GT:BBH:546| & 1.0 &-&-&-&-&-& 0.200 & 0.10 & 78.0 & 20.9 \\
267.9 & \verb|D11_q0.75_a0.6_0.6_PNr500_th1d_n100|(*) & 1.333 & 0.460 & 0.351 & 0.161 & 0.526 & 0.288 & -0.023 & 0.08 & 78.0 & 21.0 \\
267.9 & \verb|D10_q0.75_a-0.8_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.801 & 0.11 & 79.2 & 25.1 \\
267.8 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 72.2 & 31.1 \\
267.7 & \verb|RIT:BBH:KTH45PH165| & 1.0 & -0.119 & -0.558 & 0.588 & -0.150 & -0.560 & -0.579 & 0.00 & 72.7 & 37.7 \\
267.7 & \verb|RIT:BBH:STH45PH150| & 1.0 & -0.290 & -0.502 & 0.579 & 0.290 & 0.502 & -0.579 & -0.00 & 71.4 & 36.8 \\
267.7 & \verb|RIT:BBH:KTH45PH0| & 1.0 & -0.037 & 0.570 & 0.587 & -0.021 & 0.578 & -0.580 & 0.00 & 73.7 & 36.0 \\
267.7 & \verb|SXS:BBH:0024| & 1.501 & 0.496 & 0.051 & -0.001 & -0.077 & 0.489 & 0.002 & 0.00 & 73.2 & 12.5 \\
267.6 & \verb|SXS:BBH:0019| & 1.5 & - & - & -0.500 & - & - & 0.499 & -0.10 & 69.3 & 13.5 \\
267.6 & \verb|RIT:BBH:STH45PH90| & 1.0 & -0.591 & -0.053 & 0.565 & 0.568 & -0.003 & -0.591 & -0.01 & 71.5 & 36.5 \\
267.6 & \verb|RIT:BBH:KTH22.5PH90| & 1.0 & -0.331 & -0.026 & 0.749 & -0.314 & -0.007 & -0.757 & -0.00 & 71.2 & 38.3 \\
267.6 & \verb|D11_q0.75_a0.8500_-0.6375_n100|(*) & 1.334 &-&-& -0.638 & -0.001 & 0.003 & 0.851 & 0.00 & 71.8 & 23.6 \\
267.6 & \verb|DU_D10.86_q1.3333_a-0.8_opt1_n100| & 1.333 &-&-& -0.801 &-&-& 0.801 & -0.11 & 68.3 & 25.7 \\
267.5 & \verb|BAM150914:19|(*) & 1.5 & 0.318 & 0.087 & -0.266 & 0.219 & 0.004 & 0.363 & -0.01 & 72.4 & 20.3 \\
267.4 & \verb|GT:BBH:893| & 2.0 & -0.328 & 0.270 & -0.423 & 0.425 & 0.076 & 0.417 & -0.14 & 66.2 & 35.4 \\
267.4 & \verb|RIT:BBH:KTH45PH120| & 1.0 & -0.502 & -0.290 & 0.579 & -0.502 & -0.290 & -0.579 & -0.00 & 74.7 & 35.3 \\
267.4 & \verb|D9_q1.3_a0.0_m160| & 1.3 &-&-& - & - & - & - & -0.00 & 72.7 & 31.8 \\
267.3 & \verb|RIT:BBH:KTH45PH30| & 1.0 & -0.355 & 0.443 & 0.590 & -0.290 & 0.502 & -0.579 & 0.01 & 74.9 & 35.4 \\
267.3 & \verb|SXS:BBH:0078| & 1.501 & 0.497 & 0.049 & - &-&-&-& -0.00 & 74.4 & 11.4 \\
267.3 & \verb|S0_D9.87_q2.00_a0.20_-0.80_n100| & 2.001 &-&-& 0.200 & -0.015 & -0.007 & -0.800 & -0.13 & 71.9 & 28.4 \\
267.3 & \verb|RIT:BBH:NTH120PH120| & 1.005 & -0.611 & -0.353 & -0.407 &-&-& - & -0.20 & 63.7 & 36.7 \\
267.3 & \verb|RIT:BBH:KTH45PH105| & 1.0 & -0.567 & -0.177 & 0.564 & -0.560 & -0.150 & -0.579 & -0.01 & 74.6 & 34.7 \\
267.2 & \verb|D10_q0.75_a0.0_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& - & 0.14 & 78.8 & 23.3 \\
267.2 & \verb|SXS:BBH:0252| & 1.999 &-& - & 0.371 &-& - & -0.849 & -0.04 & 76.6 & 12.4 \\
267.2 & \verb|RIT:BBH:NTH120PH60| & 1.005 & -0.643 & 0.299 & -0.399 &-& - & - & -0.20 & 64.1 & 37.4 \\
267.2 & \verb|BAM150914:30|(*) & 1.2 & 0.391 & 0.100 & -0.131 & -0.392 & -0.130 & 0.097 & -0.03 & 70.0 & 19.3 \\
267.1 & \verb|RIT:BBH:STH45PH120| & 1.0 & -0.498 & -0.319 & 0.567 & 0.502 & 0.290 & -0.579 & -0.01 & 71.0 & 37.1 \\
267.1 & \verb|SXS:BBH:0025| & 1.5 & - & - & 0.500 & - & - & -0.499 & 0.10 & 79.5 & 10.7 \\
267.1 & \verb|GT:BBH:891| & 2.0 & 0.328 & -0.270 & -0.423 & -0.425 & -0.076 & 0.417 & -0.14 & 66.3 & 34.0 \\
267.0 & \verb|Rflop_r500_d11_q0.7_a0.8_m088|(*) & 1.428 & 0.603 & 0.445 & 0.283 & 0.747 & 0.278 & -0.079 & 0.13 & 80.8 & 20.8 \\
267.0 & \verb|RIT:BBH:STH45PH0| & 1.0 & -0.034 & 0.569 & 0.589 & 0.002 & -0.591 & -0.568 & 0.01 & 71.4 & 37.8 \\
267.0 & \verb|UD_D9.52_q1.00_a0.6_rl10_opt3_n100| & 1.0 &-&-& 0.600 &-&-& -0.600 & -0.00 & 74.3 & 29.2 \\
267.0 & \verb|SXS:BBH:0150| & 1.0 &-& - & 0.200 & - &-& 0.200 & 0.20 & 80.2 & 12.4 \\
267.0 & \verb|D10_q0.75_a0.8_xi0_n100|(*) & 1.333 & 0.528 & 0.062 & -0.598 &-&-& 0.801 & 0.00 & 72.8 & 27.3 \\
266.9 & \verb|BAM150914:10|(*) & 1.2 & 0.587 & 0.102 & 0.074 & 0.120 & 0.087 & 0.398 & 0.22 & 79.5 & 19.3 \\
266.9 & \verb|SXS:BBH:0137| & 1.76 & -0.248 & -0.319 & -0.034 & -0.071 & 0.151 & -0.190 & -0.09 & 73.0 & 14.7 \\
266.9 & \verb|RIT:BBH:NQ200TH135PH60| & 2 &-&-&-& 0.283 & 0.490 & -0.566 & -0.19 & 69.8 & 19.5 \\
266.9 & \verb|RIT:BBH:NTH120PH90| & 1.005 & -0.706 & -0.033 & -0.403 & - &-& - & -0.20 & 63.7 & 37.1 \\
266.9 & \verb|BAM150914:8|(*) & 1.2 & -0.395 & 0.100 & -0.116 & 0.381 & -0.167 & 0.083 & -0.03 & 74.0 & 19.4 \\
266.9 & \verb|S0_D9.96_q1.3333_a-0.45_0.80_n100| & 1.334 &-&-& -0.450 &-&-& 0.801 & 0.09 & 75.1 & 26.4 \\
266.9 & \verb|SXS:BBH:0010| & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.26 & 64.8 & 14.3 \\
266.9 & \verb|RIT:BBH:KTH22.5PH150| & 1.0 & -0.157 & -0.272 & 0.757 & -0.157 & -0.272 & -0.757 & -0.00 & 70.8 & 39.6 \\
266.8 & \verb|BAM150914:20|(*) & 1.5 & -0.259 & -0.236 & -0.238 & -0.470 & 0.317 & 0.358 & 0.00 & 70.7 & 25.2 \\
266.8 & \verb|BAM150914:29|(*) & 1.2 & 0.123 & 0.366 & -0.175 & 0.136 & -0.460 & 0.469 & 0.12 & 78.1 & 22.5 \\
266.7 & \verb|SXS:BBH:0216| & 1.0 &-& - & -0.600 & - & - &-& -0.30 & 64.8 & 13.1 \\
266.7 & \verb|GT:BBH:477| & 1.5 &-&-&-&-&-&-& 0.00 & 76.3 & 21.4 \\
266.6 & \verb|BAM150914:13|(*) & 1.2 & -0.360 & 0.181 & -0.131 & 0.277 & -0.304 & 0.105 & -0.02 & 74.0 & 18.5 \\
266.6 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 75.0 & 29.9 \\
266.6 & \verb|UD_D9.51_q1.00_a0.8_rl10_opt1_n100| & 1.0 &-&-& 0.801 &-&-& -0.801 & -0.00 & 74.0 & 29.8 \\
266.6 & \verb|SXS:BBH:0134| & 1.63 & -0.230 & 0.184 & -0.012 & -0.001 & 0.032 & 0.176 & 0.06 & 74.8 & 13.4 \\
266.6 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 74.0 & 31.1 \\
266.5 & \verb|GT:BBH:866| & 1.0 & -0.354 & 0.233 & 0.424 & 0.494 & -0.341 & -0.001 & 0.21 & 79.0 & 34.3 \\
266.5 & \verb|RIT:BBH:NTH120PH30| & 1.005 & -0.408 & 0.580 & -0.399 & - &-& - & -0.20 & 65.8 & 37.0 \\
266.5 & \verb|RIT:BBH:KTH45PH150| & 1.0 & -0.290 & -0.502 & 0.579 & -0.290 & -0.502 & -0.579 & -0.00 & 74.5 & 36.4 \\
266.4 & \verb|RIT:BBH:KTH22.5PH30| & 1.0 & -0.185 & 0.257 & 0.756 & -0.157 & 0.272 & -0.757 & -0.00 & 71.0 & 38.0 \\
266.4 & \verb|BAM150914:23|(*) & 1.5 & 0.306 & 0.140 & -0.259 & 0.216 & -0.127 & 0.342 & -0.02 & 72.4 & 25.0 \\
266.4 & \verb|BAM150914:17|(*) & 1.2 & -0.297 & 0.031 & 0.028 & -0.176 & -0.184 & 0.340 & 0.17 & 79.3 & 16.8 \\
266.3 & \verb|SXS:BBH:0126| & 1.29 & -0.250 & -0.237 & 0.091 & -0.358 & 0.172 & 0.215 & 0.15 & 77.3 & 14.1 \\
266.3 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 74.0 & 30.2 \\
266.3 & \verb|BAM150914:7|(*) & 1.5 & 0.293 & 0.173 & -0.253 & 0.178 & -0.218 & 0.317 & -0.03 & 72.4 & 19.4 \\
266.3 & \verb|RIT:BBH:KTH22.5PH120| & 1.0 & -0.272 & -0.157 & 0.757 & -0.272 & -0.157 & -0.757 & -0.00 & 69.4 & 39.9 \\
266.3 & \verb|GT:BBH:876| & 1.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.05 & 76.0 & 29.5 \\
266.3 & \verb|BAM150914:28|(*) & 1.2 & -0.168 & -0.322 & -0.218 & -0.171 & 0.364 & 0.537 & 0.13 & 74.5 & 22.3 \\
266.2 & \verb|D10_q0.50_a-0.8_xi0_n100|(*) & 2.0 & 0.696 & 0.059 & 0.392 &-& -0.006 & -0.801 & -0.01 & 78.6 & 24.4 \\
266.2 & \verb|GT:BBH:372| & 1.45 &-&-&-&-&-&-& 0.00 & 76.1 & 25.2 \\
266.1 & \verb|RIT:BBH:KTH45PH135| & 1.0 & -0.410 & -0.410 & 0.579 & -0.410 & -0.410 & -0.579 & -0.00 & 74.4 & 36.1 \\
266.1 & \verb|BAM150914:22|(*) & 1.5 & -0.337 & 0.011 & -0.258 & -0.093 & -0.207 & 0.632 & 0.10 & 72.6 & 23.5 \\
266.0 & \verb|SXS:BBH:0146| & 1.97 & -0.156 & -0.102 & -0.037 & -0.098 & 0.027 & -0.357 & -0.14 & 70.5 & 14.8 \\
266.0 & \verb|SXS:BBH:0245| & 2.0 & - & - &-&-& - & -0.300 & -0.10 & 72.5 & 12.9 \\
265.9 & \verb|BAM150914:26|(*) & 1.2 & -0.095 & 0.404 & -0.088 & 0.605 & -0.442 & 0.399 & 0.13 & 75.9 & 24.5 \\
265.9 & \verb|RIT:BBH:KTH45PH90| & 1.0 & -0.595 & -0.035 & 0.562 & -0.591 & - & -0.568 & -0.00 & 73.9 & 34.6 \\
265.9 & \verb|SXS:BBH:0244| & 2.0 &-& - & - &-&-& -0.600 & -0.20 & 69.3 & 13.0 \\
265.9 & \verb|SXS:BBH:0306|(*) & 1.31 & - &-& 0.961 & - & - & -0.899 & 0.16 & 79.7 & 16.4 \\
265.9 & \verb|SXS:BBH:0140| & 1.82 & 0.115 & -0.367 & -0.209 & -0.066 & 0.062 & 0.087 & -0.10 & 70.0 & 14.6 \\
265.8 & \verb|RIT:BBH:NTH120PH0| & 1.005 & -0.062 & 0.702 & -0.407 &-&-&-& -0.20 & 63.7 & 39.7 \\
265.8 & \verb|RIT:BBH:KTH22.5PH0| & 1.0 & -0.026 & 0.304 & 0.760 & -0.008 & 0.310 & -0.759 & 0.00 & 71.0 & 38.3 \\
265.8 & \verb|RIT:BBH:KTH22.5PH60| & 1.0 & -0.297 & 0.138 & 0.751 & -0.272 & 0.157 & -0.757 & -0.00 & 73.2 & 37.0 \\
265.8 & \verb|SXS:BBH:0124| & 1.26 & 0.250 & -0.058 & 0.071 & 0.075 & -0.095 & 0.286 & 0.17 & 79.4 & 12.7 \\
265.7 & \verb|D11_q0.75_a0.8_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.308 & 0.640 & 0.369 & -0.006 & 0.763 & -0.243 & 0.11 & 80.8 & 21.1 \\
265.7 & \verb|SXS:BBH:0161| & 1.0 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.29 & 65.2 & 14.4 \\
265.6 & \verb|RIT:BBH:NQ200TH135PH150| & 2 &-&-&-& -0.490 & 0.283 & -0.566 & -0.19 & 68.7 & 21.9 \\
265.6 & \verb|SXS:BBH:0219| & 1.0 & - &-& -0.500 &-&-& 0.900 & 0.20 & 80.2 & 11.5 \\
265.5 & \verb|D11_q1.00_a0.0_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& - & -0.25 & 66.0 & 25.8 \\
265.4 & \verb|SXS:BBH:0221| & 1.0 &-&-& -0.400 & - &-& 0.800 & 0.20 & 80.6 & 11.7 \\
265.4 & \verb|D9_q2.0_a0.6_0.6_th180_r100_res140_CE| & 2.0 & - & - & -0.600 & - &-& 0.601 & -0.20 & 62.2 & 36.6 \\
265.4 & \verb|SXS:BBH:0145| & 1.96 & 0.017 & 0.029 & -0.049 & 0.091 & -0.002 & 0.027 & -0.02 & 73.8 & 13.7 \\
265.3 & \verb|SXS:BBH:0169| & 2.0 & - & - &-&-&-&-& 0.00 & 74.0 & 15.8 \\
265.3 & \verb|BAM150914:12|(*) & 1.5 & -0.624 & -0.197 & -0.148 & -0.143 & 0.185 & 0.354 & 0.05 & 70.8 & 29.1 \\
265.2 & \verb|SXS:BBH:0130| & 1.38 & 0.164 & 0.037 & -0.014 & 0.293 & 0.060 & 0.343 & 0.14 & 79.3 & 12.5 \\
265.2 & \verb|fr_b4_a0.6_oth.255_M77| & 1.0 & -0.580 & -0.001 & -0.155 & -0.600 & -0.001 &-& -0.08 & 72.8 & 32.8 \\
265.2 & \verb|RIT:BBH:NQ200TH135PH120| & 2 &-&-&-& -0.283 & 0.490 & -0.566 & -0.19 & 71.0 & 21.0 \\
265.0 & \verb|BAM150914:16|(*) & 1.2 & 0.272 & -0.108 & 0.063 & 0.424 & 0.370 & 0.366 & 0.20 & 75.9 & 19.8 \\
265.0 & \verb|RIT:BBH:NQ200TH135PH90| & 2 &-&-&-&-& 0.566 & -0.566 & -0.19 & 71.0 & 20.5 \\
264.9 & \verb|BAM150914:21|(*) & 1.5 & -0.272 & 0.107 & 0.069 & 0.079 & -0.347 & 0.230 & 0.13 & 77.3 & 23.1 \\
264.7 & \verb|RIT:BBH:NQ200TH135PH30| & 2 &-&-&-& 0.490 & 0.283 & -0.566 & -0.19 & 70.9 & 18.5 \\
264.7 & \verb|SXS:BBH:0141| & 1.84 & -0.182 & 0.052 & 0.086 & -0.093 & 0.124 & 0.040 & 0.07 & 77.8 & 13.1 \\
264.7 & \verb|RIT:BBH:NTH60PH150| & 1.005 & -0.353 & -0.612 & 0.408 & - &-& - & 0.20 & 80.0 & 36.6 \\
264.7 & \verb|RIT:BBH:NTH60PH90| & 1.005 & -0.716 & -0.035 & 0.389 & - & - &-& 0.20 & 78.3 & 36.4 \\
264.6 & \verb|BAM150914:11|(*) & 1.2 & -0.463 & -0.481 & 0.069 & 0.217 & 0.608 & 0.181 & 0.12 & 74.7 & 25.5 \\
264.6 & \verb|GT:BBH:856| & 2.0 & 0.106 &-& 0.106 & -0.424 &-& -0.424 & -0.07 & 69.2 & 29.7 \\
264.5 & \verb|RIT:BBH:NTH60PH120| & 1.005 & -0.612 & -0.353 & 0.408 &-&-& - & 0.20 & 79.7 & 36.5 \\
264.5 & \verb|SXS:BBH:0101| & 1.501 &-& - & -0.500 & - & - &-& -0.30 & 63.9 & 18.0 \\
264.5 & \verb|D9_q1.6_a0.0_m160| & 1.6 &-&-& - & - & - & - & -0.00 & 74.8 & 30.6 \\
264.4 & \verb|SXS:BBH:0144| & 1.94 & 0.061 & 0.104 & -0.288 & -0.050 & -0.022 & 0.215 & -0.12 & 69.8 & 14.3 \\
264.4 & \verb|D11_q0.50_a0.0_0.0_n100|(*) & 2.0 &-&-& - &-&-& - & -0.00 & 74.6 & 22.0 \\
264.3 & \verb|q150_a8_a0_th_60_ph_120| & 1.492 & - & - &-& -0.595 & -0.380 & 0.405 & 0.16 & 76.7 & 35.0 \\
264.3 & \verb|GT:BBH:865| & 1.0 & -0.096 & 0.467 & 0.364 & 0.208 & 0.562 & 0.033 & 0.20 & 80.6 & 34.4 \\
264.3 & \verb|SXS:BBH:0132| & 1.63 & -0.005 & -0.114 & -0.007 & 0.041 & -0.087 & 0.310 & 0.11 & 77.1 & 12.7 \\
264.3 & \verb|RIT:BBH:NTH60PH0| & 1.005 & -0.058 & 0.692 & 0.429 &-& - & - & 0.21 & 78.6 & 36.7 \\
264.2 & \verb|RIT:BBH:NTH60PH60| & 1.005 & -0.656 & 0.274 & 0.401 &-& - & - & 0.20 & 77.5 & 36.5 \\
264.2 & \verb|RIT:BBH:NTH60PH30| & 1.005 & -0.426 & 0.555 & 0.420 & - &-& - & 0.21 & 78.3 & 36.4 \\
264.0 & \verb|EMu0_D9.16_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& - & 0.20 & 81.0 & 27.5 \\
264.0 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 75.0 & 30.5 \\
263.9 & \verb|SXS:BBH:0142| & 1.91 & -0.291 & -0.230 & -0.052 & 0.004 & 0.001 & 0.110 & 0.00 & 73.5 & 14.0 \\
263.9 & \verb|GT:BBH:873| & 1.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.08 & 75.6 & 28.3 \\
263.9 & \verb|SXS:BBH:0241| & 2.0 &-&-& -0.300 &-&-&-& -0.20 & 67.8 & 13.2 \\
263.8 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 76.8 & 24.9 \\
263.7 & \verb|SXS:BBH:0242| & 2.0 & - & - & -0.300 &-&-& 0.300 & -0.10 & 70.5 & 13.0 \\
263.5 & \verb|GT:BBH:547| & 1.0 &-&-&-&-&-& 0.400 & 0.20 & 79.6 & 20.4 \\
263.4 & \verb|D11_q1.00_a0.0_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& - & -0.40 & 62.9 & 28.0 \\
263.4 & \verb|D11_q0.75_a0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& 0.500 & 0.21 & 80.9 & 19.6 \\
263.4 & \verb|D12.50_q0.50_a-0.50_-0.10_n100|(*) & 2.0 &-&-& -0.100 &-&-& -0.500 & -0.23 & 67.7 & 20.8 \\
263.4 & \verb|D11_q0.50_a0.50_-0.50_n100|(*) & 2.0 &-&-& -0.500 &-&-& 0.500 & -0.17 & 67.5 & 25.5 \\
263.3 & \verb|RIT:BBH:NQ200TH135PH0| & 2 &-&-&-& 0.566 &-& -0.566 & -0.19 & 68.5 & 19.6 \\
263.2 & \verb|GT:BBH:420| & 1.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 79.2 & 20.2 \\
263.0 & \verb|GT:BBH:877| & 1.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.12 & 80.6 & 25.6 \\
263.0 & \verb|RIT:BBH:NQ50TH90PH120| & 2.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 73.5 & 17.3 \\
263.0 & \verb|GT:BBH:378| & 2.05 &-&-&-&-&-&-& 0.00 & 74.3 & 25.6 \\
262.9 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 72.9 & 30.5 \\
262.9 & \verb|SXS:BBH:0240| & 2.0 & - & - & -0.300 &-&-& -0.300 & -0.30 & 65.8 & 13.0 \\
262.9 & \verb|SXS:BBH:0005| & 1.0 &-&-& 0.499 & - & - &-& 0.25 & 82.4 & 10.4 \\
262.7 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 73.3 & 31.2 \\
262.7 & \verb|RIT:BBH:NQ200TH90PH0| & 2 &-&-&-& 0.800 &-&-& 0.00 & 74.9 & 20.5 \\
262.6 & \verb|D11_q0.75_a-0.8_0.0_n100|(*) & 1.334 &-&-&-&-&-& -0.801 & -0.34 & 64.0 & 27.2 \\
262.3 & \verb|q150_a8_a0_th_60_ph_0| & 1.492 & - &-& - & -0.087 & 0.682 & 0.435 & 0.17 & 74.6 & 36.7 \\
262.3 & \verb|RIT:BBH:NTH135PH90| & 1.005 & -0.579 & -0.025 & -0.572 & - &-& - & -0.29 & 63.6 & 37.7 \\
262.3 & \verb|SXS:BBH:0243| & 2.0 & - &-& -0.129 &-&-& -0.850 & -0.37 & 64.6 & 13.5 \\
262.3 & \verb|GT:BBH:871| & 1.5 & -0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 78.8 & 24.8 \\
262.2 & \verb|SXS:BBH:0214| & 1.0 &-&-& -0.625 & - & - & -0.250 & -0.44 & 61.5 & 13.1 \\
262.2 & \verb|D12_q1.00_a0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& 0.250 & 0.25 & 81.7 & 18.2 \\
262.2 & \verb|RIT:BBH:NQ50TH90PH90| & 2.0 &-& 0.800 &-&-&-&-& 0.00 & 76.8 & 16.0 \\
262.1 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 74.3 & 22.5 \\
262.0 & \verb|RIT:BBH:NQ50TH90PH150| & 2.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 75.7 & 18.0 \\
262.0 & \verb|fr_b4_a0.6_oth.240_M77| & 1.0 & -0.520 & -0.001 & -0.300 & -0.600 & -0.001 &-& -0.15 & 69.2 & 35.1 \\
262.0 & \verb|SXS:BBH:0139| & 1.82 & 0.032 & -0.342 & 0.210 & -0.132 & -0.047 & -0.042 & 0.12 & 79.1 & 12.8 \\
262.0 & \verb|RIT:BBH:NTH135PH120| & 1.005 & -0.498 & -0.288 & -0.576 & - & - & - & -0.29 & 63.3 & 37.9 \\
262.0 & \verb|GT:BBH:872| & 2.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.14 & 82.0 & 24.3 \\
261.9 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 76.3 & 29.0 \\
261.9 & \verb|D11_q0.75_a0.0_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& - & -0.29 & 65.0 & 26.3 \\
261.8 & \verb|GT:BBH:405| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 81.4 & 23.1 \\
261.8 & \verb|RIT:BBH:NTH135PH60| & 1.005 & -0.520 & 0.265 & -0.568 &-& - &-& -0.28 & 63.7 & 38.0 \\
261.8 & \verb|GT:BBH:858| & 1.5 & -0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 79.3 & 25.7 \\
261.6 & \verb|RIT:BBH:A7TH120PH315| & 1.0 & 0.442 & 0.442 & -0.361 & -0.442 & -0.442 & -0.361 & -0.36 & 61.7 & 23.1 \\
261.6 & \verb|RIT:BBH:NQ200TH90PH30| & 2 &-&-&-& 0.693 & 0.400 &-& 0.00 & 74.1 & 21.5 \\
261.6 & \verb|GT:BBH:894| & 2.0 & -0.500 & 0.324 & -0.070 & 0.188 & 0.556 & 0.122 & -0.01 & 73.0 & 30.7 \\
261.6 & \verb|Del0_D10.01_q2.00_a-0.4_-0.8_n100| & 2.001 &-&-& -0.400 & -0.011 & 0.003 & -0.800 & -0.53 & 58.3 & 37.0 \\
261.6 & \verb|SXS:BBH:0249| & 2.0 & - & - & 0.300 & - & - & -0.300 & 0.10 & 80.1 & 11.9 \\
261.6 & \verb|RIT:BBH:NQ50TH90PH60| & 2.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 73.5 & 15.7 \\
261.6 & \verb|SXS:BBH:0122| & 1.17 & -0.019 & 0.061 & -0.477 & 0.041 & 0.050 & -0.364 & -0.42 & 60.9 & 17.5 \\
261.6 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 76.0 & 29.1 \\
261.6 & \verb|RIT:BBH:NQ66TH60PH120| & 1.5 & -0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 81.3 & 31.1 \\
261.4 & \verb|RIT:BBH:NTH45PH10| & 1.005 & -0.153 & 0.539 & 0.593 &-& - & - & 0.30 & 80.0 & 35.7 \\
261.2 & \verb|RIT:BBH:NTH45PH40| & 1.005 & -0.417 & 0.401 & 0.575 &-& - & - & 0.29 & 79.3 & 35.9 \\
261.1 & \verb|RIT:BBH:NTH135PH150| & 1.005 & -0.259 & -0.498 & -0.590 & - & - &-& -0.30 & 60.4 & 40.3 \\
261.1 & \verb|SXS:BBH:0246| & 2.0 &-&-&-&-& - & 0.300 & 0.10 & 77.9 & 12.4 \\
261.1 & \verb|BAM150914:18|(*) & 1.2 & -0.161 & -0.207 & 0.145 & 0.378 & 0.352 & 0.428 & 0.27 & 81.0 & 18.4 \\
261.0 & \verb|RIT:BBH:NQ200TH90PH60| & 2 &-&-&-& 0.400 & 0.693 &-& 0.00 & 76.5 & 22.0 \\
261.0 & \verb|RIT:BBH:NQ200TH90PH90| & 2 &-&-&-&-& 0.800 &-& 0.00 & 76.9 & 21.4 \\
260.9 & \verb|RIT:BBH:NQ200TH90PH120| & 2 &-&-&-& -0.400 & 0.693 &-& 0.00 & 74.1 & 20.6 \\
260.9 & \verb|GT:BBH:550| & 2.0 & 0.424 &-& -0.424 &-&-& 0.600 & -0.08 & 72.1 & 29.1 \\
260.8 & \verb|fr_b4_a0.6_oth.090_M77| & 1.0 & 0.600 & 0.001 &-& -0.600 & -0.001 &-& 0.00 & 74.5 & 32.2 \\
260.8 & \verb|RIT:BBH:NQ50TH90PH30| & 2.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 76.2 & 15.4 \\
260.7 & \verb|SXS:BBH:0148| & 1.0 &-&-& -0.438 & - & - & -0.438 & -0.44 & 60.8 & 16.8 \\
260.7 & \verb|SXS:BBH:0128| & 1.35 & 0.041 & 0.005 & 0.134 & -0.048 & 0.103 & 0.397 & 0.25 & 82.8 & 12.7 \\
260.6 & \verb|D11_q0.75_a-0.5_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.500 & 0.24 & 84.4 & 19.4 \\
260.6 & \verb|RIT:BBH:NQ200TH90PH150| & 2 &-&-&-& -0.693 & 0.400 &-& 0.00 & 74.1 & 18.8 \\
260.6 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.6 & 22.3 \\
260.6 & \verb|GT:BBH:897| & 2.0 & 0.500 & -0.324 & -0.070 & -0.188 & -0.556 & 0.122 & -0.01 & 69.9 & 30.8 \\
260.5 & \verb|SXS:BBH:0239| & 1.999 &-& - & -0.371 & - & - & 0.850 & 0.04 & 73.7 & 12.8 \\
260.4 & \verb|RIT:BBH:NQ200TH60PH0| & 2 &-&-&-& 0.693 &-& 0.400 & 0.13 & 75.9 & 35.8 \\
260.3 & \verb|D9_q1.9_a0.0_m160| & 1.9 &-&-& - &-&-& - & -0.00 & 75.6 & 30.2 \\
260.3 & \verb|RIT:BBH:NQ50TH90PH0| & 2.0 & 0.800 &-&-&-&-&-& 0.00 & 77.3 & 15.0 \\
260.2 & \verb|RIT:BBH:A7TH120PH90| & 1.0 & -0.629 & -0.027 & -0.353 & 0.625 &-& -0.361 & -0.36 & 62.7 & 23.6 \\
260.2 & \verb|RIT:BBH:NQ200TH60PH150| & 2 &-&-&-& -0.600 & 0.346 & 0.400 & 0.13 & 75.8 & 35.2 \\
260.2 & \verb|SXS:BBH:0022| & 1.5 & 0.497 & 0.049 & - & 0.001 & -0.001 & 0.499 & 0.20 & 81.9 & 12.0 \\
260.2 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 75.0 & 29.4 \\
260.2 & \verb|RIT:BBH:N9TH55PH60| & 1.012 & -0.686 & 0.321 & 0.507 & - &-& - & 0.25 & 80.0 & 33.0 \\
260.0 & \verb|RIT:BBH:NTH45PH50| & 1.005 & -0.485 & 0.328 & 0.568 & - &-&-& 0.28 & 81.0 & 35.2 \\
260.0 & \verb|GT:BBH:847| & 1.5 & 0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 79.4 & 29.5 \\
260.0 & \verb|RIT:BBH:NTH135PH30| & 1.005 & -0.343 & 0.468 & -0.571 & - & - & - & -0.29 & 61.4 & 40.2 \\
259.9 & \verb|RIT:BBH:NTH135PH0| & 1.005 & -0.034 & 0.576 & -0.574 &-&-&-& -0.29 & 60.9 & 41.6 \\
259.9 & \verb|RIT:BBH:NTH45PH1275| & 1.005 & -0.458 & -0.351 & 0.577 & - & - &-& 0.29 & 81.1 & 36.3 \\
259.8 & \verb|SXS:BBH:0118| & 1.12 & -0.010 & 0.030 & 0.343 & -0.190 & -0.146 & 0.258 & 0.30 & 83.3 & 12.7 \\
259.8 & \verb|RIT:BBH:NQ200TH60PH30| & 2 &-&-&-& 0.600 & 0.346 & 0.400 & 0.13 & 74.8 & 35.5 \\
259.8 & \verb|RIT:BBH:NTH45PH120| & 1.005 & -0.500 & -0.289 & 0.577 &-& - & - & 0.29 & 78.5 & 37.4 \\
259.8 & \verb|RIT:BBH:NQ50TH135PH120| & 2.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 58.6 & 21.2 \\
259.8 & \verb|RIT:BBH:NTH45PH150| & 1.005 & -0.289 & -0.500 & 0.577 &-&-&-& 0.29 & 80.9 & 36.3 \\
259.8 & \verb|GT:BBH:413| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 80.7 & 23.4 \\
259.7 & \verb|GT:BBH:895| & 2.0 & 0.511 & -0.009 & 0.314 & 0.565 & 0.025 & -0.200 & 0.14 & 83.7 & 27.6 \\
259.7 & \verb|RIT:BBH:NQ200TH60PH60| & 2 &-&-&-& 0.346 & 0.600 & 0.400 & 0.13 & 74.5 & 34.8 \\
259.4 & \verb|RIT:BBH:NTH45PH60| & 1.005 & -0.536 & 0.241 & 0.566 & - &-&-& 0.28 & 81.7 & 34.9 \\
259.4 & \verb|D10_q0.50_a0.8_xi0_n100|(*) & 2.0 & 0.689 & 0.062 & -0.403 & 0.012 & 0.006 & 0.800 & -0.00 & 72.5 & 26.6 \\
259.3 & \verb|RIT:BBH:NQ66TH60PH150| & 1.5 & -0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 83.7 & 31.2 \\
259.3 & \verb|RIT:BBH:NTH45PH75| & 1.005 & -0.582 & 0.097 & 0.564 &-& - & - & 0.28 & 79.9 & 35.8 \\
259.3 & \verb|RIT:BBH:NTH45PH30| & 1.005 & -0.341 & 0.464 & 0.578 &-& - & - & 0.29 & 79.2 & 36.0 \\
259.3 & \verb|RIT:BBH:A7TH120PH0| & 1.0 & -0.055 & 0.621 & -0.362 &-& -0.625 & -0.361 & -0.36 & 64.5 & 20.1 \\
259.2 & \verb|SXS:BBH:0011| & 1.501 & 0.248 & 0.026 & 0.433 &-&-&-& 0.26 & 85.1 & 11.0 \\
259.2 & \verb|GT:BBH:848| & 1.5 & 0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 80.4 & 25.5 \\
259.2 & \verb|RIT:BBH:A7TH120PH210| & 1.0 & 0.361 & -0.512 & -0.358 & -0.312 & 0.541 & -0.361 & -0.36 & 62.6 & 28.3 \\
259.2 & \verb|GT:BBH:380| & 2.35 &-&-&-&-&-&-& 0.00 & 74.9 & 25.5 \\
259.2 & \verb|GT:BBH:870| & 1.5 &-& 0.600 &-& -0.424 &-& 0.424 & 0.17 & 79.9 & 26.0 \\
259.2 & \verb|RIT:BBH:A7TH120PH130| & 1.0 & -0.478 & -0.401 & -0.361 & 0.478 & 0.401 & -0.361 & -0.36 & 61.5 & 24.0 \\
259.1 & \verb|RIT:BBH:N9TH55PH30| & 1.012 & -0.432 & 0.609 & 0.522 & - &-& - & 0.26 & 82.1 & 31.9 \\
259.1 & \verb|SXS:BBH:0210| & 1.0 &-& - & -0.900 &-& - & - & -0.45 & 62.1 & 12.9 \\
259.1 & \verb|RIT:BBH:NQ66TH60PH60| & 1.5 & 0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 81.2 & 30.7 \\
259.1 & \verb|GT:BBH:867| & 1.0 & 0.599 & 0.030 & - & -0.599 & -0.030 & - & 0.00 & 72.0 & 40.2 \\
259.1 & \verb|RIT:BBH:N9TH55PH0| & 1.012 & -0.062 & 0.725 & 0.549 & - &-& - & 0.28 & 82.1 & 31.6 \\
259.1 & \verb|GT:BBH:564| & 1.0 &-&-& -0.400 &-&-& -0.400 & -0.40 & 64.7 & 26.2 \\
259.0 & \verb|SXS:BBH:0227| & 1.0 &-& - & 0.600 &-& - &-& 0.30 & 84.9 & 11.0 \\
259.0 & \verb|SXS:BBH:0164| & 1.0 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.33 & 86.6 & 12.1 \\
259.0 & \verb|fr_b4_a0.6_oth.225_M77| & 1.0 & -0.424 & -0.001 & -0.424 & -0.600 & -0.001 & - & -0.21 & 67.8 & 36.6 \\
258.9 & \verb|RIT:BBH:NQ50TH135PH150| & 2.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 60.1 & 21.4 \\
258.9 & \verb|q150_a8_a0_th_60_ph_30| & 1.492 &-& - & - & -0.430 & 0.556 & 0.410 & 0.16 & 77.4 & 35.5 \\
258.7 & \verb|RIT:BBH:NTH45PH0| & 1.005 & -0.034 & 0.568 & 0.584 &-& - & - & 0.29 & 83.5 & 34.3 \\
258.7 & \verb|SXS:BBH:0237| & 2.0 & - &-& -0.600 & - &-& 0.600 & -0.20 & 67.9 & 13.5 \\
258.6 & \verb|RIT:BBH:NTH45PH45| & 1.005 & -0.453 & 0.365 & 0.572 &-& - & - & 0.29 & 83.2 & 34.2 \\
258.6 & \verb|GT:BBH:548| & 1.0 &-&-&-&-&-& 0.600 & 0.30 & 86.4 & 18.5 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH90| & 2 &-&-&-&-& 0.693 & 0.400 & 0.13 & 77.9 & 33.1 \\
258.6 & \verb|RIT:BBH:NTH45PH20| & 1.005 & -0.251 & 0.511 & 0.584 &-& - & - & 0.29 & 79.2 & 36.0 \\
258.6 & \verb|fr_b4_a0.6_oth.315_M77| & 1.0 & -0.424 & - & 0.424 & -0.600 & -0.001 &-& 0.21 & 82.0 & 30.4 \\
258.5 & \verb|RIT:BBH:A7TH120PH30| & 1.0 & -0.361 & 0.515 & -0.352 & 0.312 & -0.541 & -0.361 & -0.36 & 61.5 & 21.7 \\
258.5 & \verb|RIT:BBH:NQ66TH60PH30| & 1.5 & 0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 78.5 & 32.8 \\
258.4 & \verb|RIT:BBH:NTH45PH1125| & 1.005 & -0.531 & -0.251 & 0.566 &-&-& - & 0.28 & 82.9 & 35.1 \\
258.4 & \verb|RIT:BBH:NQ50TH135PH60| & 2.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 60.5 & 28.5 \\
258.4 & \verb|S0_D9.75_q2.00_a-0.20_0.80_n100| & 2.001 &-&-& -0.200 & 0.015 & -0.006 & 0.800 & 0.13 & 77.9 & 25.8 \\
258.4 & \verb|GT:BBH:859| & 2.0 & -0.106 &-& -0.106 & 0.424 &-& 0.424 & 0.07 & 76.5 & 27.5 \\
258.4 & \verb|EMu0_D8.98_q1.00_a0.6_n100| & 1.0 &-&-& 0.600 &-&-& - & 0.30 & 85.2 & 26.8 \\
258.2 & \verb|RIT:BBH:NQ200TH60PH120| & 2 &-&-&-& -0.346 & 0.600 & 0.400 & 0.13 & 77.9 & 33.5 \\
258.2 & \verb|RIT:BBH:N9TH55PH120| & 1.012 & -0.373 & -0.647 & 0.523 &-&-& - & 0.26 & 83.9 & 31.7 \\
258.2 & \verb|D11_q0.75_a0.0_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& - & 0.29 & 84.4 & 19.2 \\
258.2 & \verb|SXS:BBH:0259| & 2.5 &-& - &-& - &-&-& 0.00 & 76.2 & 11.3 \\
258.0 & \verb|GT:BBH:896| & 2.0 & -0.511 & 0.009 & 0.314 & -0.565 & -0.025 & -0.200 & 0.14 & 82.4 & 25.3 \\
257.9 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 77.2 & 29.4 \\
257.8 & \verb|GT:BBH:864| & 1.0 & -0.269 & -0.536 & -0.014 & -0.269 & -0.536 & -0.014 & -0.01 & 73.8 & 40.7 \\
257.8 & \verb|RIT:BBH:NTH45PH975| & 1.005 & -0.580 & -0.104 & 0.565 & - & - &-& 0.28 & 82.2 & 35.2 \\
257.8 & \verb|SXS:BBH:0191| & 2.507 & - &-& - &-&-&-& -0.00 & 77.2 & 12.8 \\
257.7 & \verb|D10_q0.50_a-0.50_0.50_n100|(*) & 2.0 &-&-& 0.500 &-&-& -0.500 & 0.17 & 84.0 & 21.9 \\
257.7 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 74.6 & 29.3 \\
257.7 & \verb|RIT:BBH:N9TH55PH90| & 1.012 & -0.759 & -0.029 & 0.505 &-& - & - & 0.25 & 84.3 & 31.6 \\
257.6 & \verb|RIT:BBH:NQ50TH135PH0| & 2.0 & 0.566 &-& -0.566 &-&-&-& -0.38 & 60.8 & 24.8 \\
257.5 & \verb|SXS:BBH:0028| & 1.501 & -0.001 & 0.001 & 0.500 & 0.078 & -0.489 & 0.001 & 0.30 & 86.5 & 11.0 \\
257.5 & \verb|GT:BBH:860| & 1.0 & 0.109 & 0.481 & 0.342 & 0.460 & -0.287 & 0.257 & 0.30 & 79.4 & 33.9 \\
257.5 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 75.7 & 28.9 \\
257.4 & \verb|SXS:BBH:0136| & 1.68 & 0.118 & -0.114 & 0.326 & -0.145 & -0.071 & 0.145 & 0.26 & 85.5 & 11.6 \\
257.3 & \verb|GT:BBH:549| & 1.0 &-&-& 0.200 &-&-& 0.400 & 0.30 & 83.4 & 19.4 \\
257.3 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 80.8 & 23.7 \\
257.2 & \verb|GT:BBH:636| & 3.0 & -0.500 & 0.019 & -0.001 &-&-&-& -0.00 & 75.8 & 33.6 \\
257.2 & \verb|RIT:BBH:NQ50TH135PH90| & 2.0 &-& 0.566 & -0.566 &-&-&-& -0.38 & 63.2 & 22.7 \\
257.1 & \verb|RIT:BBH:NQ50TH135PH30| & 2.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 62.1 & 28.1 \\
257.1 & \verb|GT:BBH:565| & 2.5 &-&-&-&-&-&-& 0.00 & 76.6 & 21.3 \\
257.0 & \verb|SXS:BBH:0247| & 2.0 &-& - & - &-& - & 0.600 & 0.20 & 81.1 & 11.9 \\
257.0 & \verb|SXS:BBH:0236| & 2.0 & - & - & -0.600 & - &-& - & -0.40 & 62.2 & 13.8 \\
256.9 & \verb|RIT:BBH:NTH165PH30| & 1.005 & -0.103 & 0.188 & -0.785 & - &-& - & -0.39 & 61.4 & 38.8 \\
256.9 & \verb|RIT:BBH:NTH165PH60| & 1.005 & -0.182 & 0.105 & -0.786 &-& - &-& -0.39 & 61.4 & 38.5 \\
256.8 & \verb|RIT:BBH:NTH165PH0| & 1.005 & -0.009 & 0.195 & -0.790 & - & - & - & -0.40 & 61.4 & 39.3 \\
256.7 & \verb|GT:BBH:890| & 2.0 &-&-& 0.600 &-&-& -0.600 & 0.20 & 84.8 & 24.4 \\
256.6 & \verb|GT:BBH:764| & 1.5 & 0.600 &-&-&-&-& 0.600 & 0.24 & 83.1 & 24.2 \\
256.6 & \verb|SXS:BBH:0233| & 2.0 &-&-& -0.871 &-& - & 0.850 & -0.30 & 63.7 & 14.3 \\
256.6 & \verb|GT:BBH:878| & 2.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.16 & 83.6 & 23.6 \\
256.5 & \verb|RIT:BBH:NQ66TH60PH90| & 1.5 &-& 0.693 & 0.400 &-&-&-& 0.24 & 84.3 & 29.3 \\
256.4 & \verb|SXS:BBH:0052| & 3.0 & 0.494 & 0.073 & 0.001 & 0.001 & 0.008 & -0.499 & -0.12 & 75.2 & 15.3 \\
256.4 & \verb|RIT:BBH:NTH45PH90| & 1.005 & -0.590 & -0.050 & 0.562 &-& - & - & 0.28 & 81.7 & 35.2 \\
256.4 & \verb|D9_q2.2_a0.0_m160| & 2.2 &-&-& - &-&-& - & -0.00 & 76.8 & 29.5 \\
256.4 & \verb|D11_q0.75_a0.4_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.597 & -0.231 & 0.481 & -0.346 & 0.200 & 0.003 & 0.28 & 86.3 & 18.5 \\
256.3 & \verb|RIT:BBH:NTH165PH120| & 1.005 & -0.187 & -0.098 & -0.786 & - &-& - & -0.39 & 59.0 & 39.8 \\
256.1 & \verb|GT:BBH:764| & 1.5 & 0.600 &-&-&-&-& 0.600 & 0.24 & 81.5 & 16.3 \\
256.1 & \verb|SXS:BBH:0250| & 2.0 &-& - & 0.300 &-&-&-& 0.20 & 83.8 & 11.5 \\
256.1 & \verb|d0_D10.50_q2.00_a-0.5_n100| & 2.0 &-&-& -0.500 &-&-& - & -0.33 & 64.1 & 29.0 \\
256.1 & \verb|RIT:BBH:NQ66TH60PH0| & 1.5 & 0.693 &-& 0.400 &-&-&-& 0.24 & 79.0 & 33.1 \\
256.0 & \verb|SXS:BBH:0026| & 1.5 & - &-& 0.500 & -0.494 & -0.071 & - & 0.30 & 84.6 & 11.6 \\
255.9 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 77.5 & 28.1 \\
255.8 & \verb|D11_q0.75_a0.0_-0.8_n100|(*) & 1.333 &-&-& -0.801 &-&-& - & -0.46 & 60.5 & 29.2 \\
255.8 & \verb|RIT:BBH:NQ200TH30PH120| & 2 &-&-&-& -0.200 & 0.346 & 0.693 & 0.23 & 80.1 & 32.4 \\
255.7 & \verb|RIT:BBH:A7TH60PH10| & 1.0 & -0.161 & 0.600 & 0.373 & 0.137 & -0.612 & 0.364 & 0.37 & 85.2 & 31.8 \\
255.7 & \verb|DD_D10.99_q2.00_a-0.8_n100| & 2.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 51.6 & 36.7 \\
255.7 & \verb|RIT:BBH:NQ33TH135PH150| & 3 & -0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 60.7 & 37.6 \\
255.6 & \verb|SXS:BBH:0238| & 2.0 &-&-& -0.500 &-&-& -0.499 & -0.50 & 60.4 & 12.9 \\
255.6 & \verb|GT:BBH:458| & 2.0 & 0.346 &-& 0.200 &-&-& 0.400 & 0.27 & 83.6 & 24.0 \\
255.6 & \verb|RIT:BBH:NQ200TH30PH30| & 2 &-&-&-& 0.346 & 0.200 & 0.693 & 0.23 & 79.6 & 33.4 \\
255.6 & \verb|RIT:BBH:NQ33TH135PH120| & 3 & -0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 57.4 & 39.1 \\
255.6 & \verb|SXS:BBH:0020| & 1.5 &-& - & 0.500 & 0.494 & 0.071 & - & 0.30 & 86.4 & 11.2 \\
255.5 & \verb|RIT:BBH:NTH165PH90| & 1.005 & -0.211 &-& -0.786 & - &-& - & -0.39 & 60.3 & 39.0 \\
255.4 & \verb|SXS:BBH:0275| & 3.0 & - &-& - &-&-& -0.600 & -0.15 & 73.5 & 13.5 \\
255.4 & \verb|RIT:BBH:NTH165PH150| & 1.005 & -0.105 & -0.182 & -0.786 & - & - & - & -0.39 & 60.1 & 39.4 \\
255.4 & \verb|SXS:BBH:0279| & 2.999 & - &-& 0.231 & - & - & -0.849 & -0.04 & 78.4 & 13.0 \\
255.4 & \verb|RIT:BBH:NQ200TH30PH60| & 2 &-&-&-& 0.200 & 0.346 & 0.693 & 0.23 & 79.8 & 32.9 \\
255.3 & \verb|GT:BBH:458| & 2.0 & 0.346 &-& 0.200 &-&-& 0.400 & 0.27 & 83.8 & 17.6 \\
255.3 & \verb|RIT:BBH:NQ33TH100PH120| & 3 & -0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 74.1 & 27.4 \\
255.2 & \verb|GT:BBH:456| & 1.5 & 0.346 &-& 0.200 &-&-& 0.400 & 0.28 & 85.3 & 23.2 \\
255.2 & \verb|RIT:BBH:NTH30PH0| & 1.005 & -0.033 & 0.386 & 0.718 &-& - & - & 0.36 & 85.3 & 33.7 \\
255.2 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 78.2 & 28.8 \\
255.1 & \verb|RIT:BBH:A7TH60PH40| & 1.0 & -0.445 & 0.444 & 0.362 & 0.404 & -0.481 & 0.362 & 0.36 & 84.3 & 31.9 \\
255.1 & \verb|D10_q0.33_a-0.8_xi0_n100|(*) & 2.999 & 0.757 & 0.030 & 0.259 &-&-& -0.800 & -0.01 & 82.8 & 22.8 \\
255.0 & \verb|GT:BBH:724| & 3.0 & -0.464 & 0.182 & 0.046 &-&-&-& 0.03 & 74.2 & 34.5 \\
255.0 & \verb|D11_q0.75_a0.8_0.0_n100|(*) & 1.334 &-&-& - &-&-& 0.801 & 0.34 & 86.0 & 18.9 \\
255.0 & \verb|GT:BBH:456| & 1.5 & 0.346 &-& 0.200 &-&-& 0.400 & 0.28 & 83.2 & 18.4 \\
254.9 & \verb|GT:BBH:556| & 2.0 & -0.600 &-& - &-&-& 0.600 & 0.20 & 81.6 & 25.3 \\
254.9 & \verb|D10_q0.33_a0.8_xi0_n120|(*) & 2.999 & 0.754 & 0.031 & -0.268 &-&-& 0.800 & -0.00 & 71.9 & 26.3 \\
254.8 & \verb|RIT:BBH:A7TH135PH0| & 1.0 & -0.028 & 0.512 & -0.506 &-& -0.510 & -0.510 & -0.51 & 60.7 & 16.7 \\
254.8 & \verb|SXS:BBH:0254| & 2.0 &-& - & 0.600 &-&-& -0.600 & 0.20 & 86.3 & 11.4 \\
254.8 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 78.4 & 28.7 \\
254.8 & \verb|SXS:BBH:0009| & 1.501 & - &-& 0.500 & - & - &-& 0.30 & 86.8 & 13.4 \\
254.8 & \verb|RIT:BBH:NQ33TH100PH0| & 3 & 0.788 &-& -0.139 &-&-&-& -0.10 & 72.7 & 24.8 \\
254.8 & \verb|D12.00_q0.50_a0.50_0.10_n100|(*) & 2.0 &-&-& 0.100 &-&-& 0.500 & 0.23 & 83.0 & 17.6 \\
254.8 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 76.9 & 28.2 \\
254.7 & \verb|SXS:BBH:0042| & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.32 & 64.8 & 22.2 \\
254.6 & \verb|GT:BBH:680| & 3.0 & 0.500 & -0.019 & -0.001 &-&-&-& -0.00 & 76.2 & 33.2 \\
254.6 & \verb|RIT:BBH:NTH30PH90| & 1.005 & -0.423 & -0.024 & 0.698 &-&-& - & 0.35 & 81.8 & 35.5 \\
254.6 & \verb|RIT:BBH:A7TH135PH315| & 1.0 & 0.360 & 0.360 & -0.510 & -0.360 & -0.360 & -0.510 & -0.51 & 60.8 & 18.6 \\
254.5 & \verb|RIT:BBH:NQ33TH135PH90| & 3 &-& 0.566 & -0.566 &-&-&-& -0.42 & 57.6 & 38.4 \\
254.5 & \verb|GT:BBH:657| & 3.0 & -0.201 & 0.405 & 0.213 &-&-&-& 0.16 & 77.0 & 35.0 \\
254.4 & \verb|RIT:BBH:NQ200TH30PH0| & 2 &-&-&-& 0.400 &-& 0.693 & 0.23 & 81.4 & 33.2 \\
254.4 & \verb|RIT:BBH:A7TH135PH30| & 1.0 & -0.281 & 0.434 & -0.502 & 0.255 & -0.441 & -0.510 & -0.51 & 58.6 & 17.8 \\
254.4 & \verb|RIT:BBH:NTH30PH30| & 1.005 & -0.232 & 0.338 & 0.706 &-& - & - & 0.35 & 86.5 & 33.2 \\
254.3 & \verb|RIT:BBH:NQ33TH75PH0| & 3 & 0.773 &-& 0.207 &-&-&-& 0.16 & 82.6 & 24.0 \\
254.3 & \verb|DU_D10.90_q2.00_a-0.8_rl10_opt1_n100| & 2.0 &-&-& -0.801 & - & -0.004 & 0.801 & -0.27 & 64.5 & 27.5 \\
254.3 & \verb|RIT:BBH:NQ200TH30PH150| & 2 &-&-&-& -0.346 & 0.200 & 0.693 & 0.23 & 80.4 & 32.5 \\
254.2 & \verb|RIT:BBH:NTH30PH60| & 1.005 & -0.378 & 0.185 & 0.700 & - &-& - & 0.35 & 81.9 & 35.1 \\
254.2 & \verb|RIT:BBH:LPH120| & 1.0 & -0.703 & -0.422 & -0.009 & 0.016 & 0.006 & 0.820 & 0.41 & 87.2 & 29.1 \\
254.1 & \verb|SXS:BBH:0035| & 3.001 & 0.499 & 0.029 & - &-& - &-& -0.00 & 76.1 & 11.9 \\
254.0 & \verb|SXS:BBH:0276| & 3.0 & - & - &-& - & - & -0.300 & -0.07 & 75.2 & 13.0 \\
254.0 & \verb|RIT:BBH:NQ33TH100PH30| & 3 & 0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 74.1 & 25.5 \\
254.0 & \verb|GT:BBH:463| & 2.0 & 0.600 &-&-&-&-& 0.600 & 0.20 & 80.8 & 9.1 \\
253.7 & \verb|GT:BBH:609| & 3.0 & -0.335 & -0.317 & -0.192 &-&-&-& -0.14 & 65.9 & 41.2 \\
253.7 & \verb|RIT:BBH:A7TH60PH80| & 1.0 & -0.632 & 0.058 & 0.351 & 0.618 & -0.109 & 0.363 & 0.36 & 87.0 & 31.6 \\
253.7 & \verb|GT:BBH:605| & 3.0 & 0.464 & -0.182 & 0.046 &-&-&-& 0.03 & 76.7 & 31.6 \\
253.7 & \verb|RIT:BBH:NQ33TH135PH60| & 3 & 0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 57.9 & 39.7 \\
253.7 & \verb|GT:BBH:464| & 2.5 & 0.400 &-&-&-&-& 0.400 & 0.11 & 79.7 & 25.5 \\
253.6 & \verb|RIT:BBH:A7TH135PH210| & 1.0 & 0.281 & -0.431 & -0.505 & -0.255 & 0.441 & -0.510 & -0.51 & 57.4 & 27.6 \\
253.6 & \verb|GT:BBH:467| & 2.5 & 0.600 &-&-&-&-& 0.600 & 0.17 & 83.2 & 26.0 \\
253.5 & \verb|RIT:BBH:NQ33TH135PH30| & 3 & 0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 58.8 & 37.9 \\
253.4 & \verb|RIT:BBH:NQ200TH30PH90| & 2 &-&-&-&-& 0.400 & 0.693 & 0.23 & 78.1 & 33.2 \\
253.3 & \verb|RIT:BBH:NQ33TH100PH60| & 3 & 0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 72.4 & 27.8 \\
253.3 & \verb|RIT:BBH:NQ33TH100PH150| & 3 & -0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 75.1 & 27.0 \\
253.2 & \verb|RIT:BBH:NQ33TH100PH90| & 3 &-& 0.788 & -0.139 &-&-&-& -0.10 & 75.1 & 26.9 \\
253.2 & \verb|RIT:BBH:NTH30PH120| & 1.005 & -0.353 & -0.204 & 0.707 & - &-& - & 0.35 & 82.0 & 35.8 \\
253.2 & \verb|RIT:BBH:A7TH60PH315| & 1.0 & 0.424 & 0.464 & 0.361 & -0.444 & -0.444 & 0.363 & 0.36 & 84.3 & 31.6 \\
253.1 & \verb|RIT:BBH:NTH30PH150| & 1.005 & -0.204 & -0.353 & 0.707 & - &-& - & 0.35 & 81.0 & 36.3 \\
253.1 & \verb|RIT:BBH:NQ33TH75PH90| & 3 &-& 0.773 & 0.207 &-&-&-& 0.16 & 84.5 & 25.9 \\
253.0 & \verb|GT:BBH:463| & 2.0 & 0.600 &-&-&-&-& 0.600 & 0.20 & 81.7 & 25.0 \\
253.0 & \verb|SXS:BBH:0032| & 3.001 & 0.248 & 0.037 & -0.432 &-& - &-& -0.32 & 64.7 & 17.7 \\
252.9 & \verb|GT:BBH:464| & 2.5 & 0.400 &-&-&-&-& 0.400 & 0.11 & 78.0 & 15.3 \\
252.9 & \verb|RIT:BBH:A7TH135PH130| & 1.0 & -0.390 & -0.328 & -0.510 & 0.390 & 0.328 & -0.510 & -0.51 & 59.6 & 26.7 \\
252.8 & \verb|GT:BBH:743| & 3.0 & 0.267 & -0.412 & -0.094 &-&-&-& -0.07 & 65.0 & 41.4 \\
252.8 & \verb|GT:BBH:545| & 2.0 &-&-& -0.600 &-&-& 0.600 & -0.20 & 64.6 & 33.5 \\
252.8 & \verb|D11_q0.75_a-0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& -0.500 & -0.50 & 59.4 & 29.8 \\
252.7 & \verb|RIT:BBH:NQ33TH135PH0| & 3 & 0.566 &-& -0.566 &-&-&-& -0.42 & 60.5 & 36.5 \\
252.7 & \verb|RIT:BBH:NQ33TH75PH60| & 3 & 0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 86.3 & 24.1 \\
252.6 & \verb|GT:BBH:467| & 2.5 & 0.600 &-&-&-&-& 0.600 & 0.17 & 80.1 & 25.3 \\
252.6 & \verb|fr_b4_a0.6_oth.000_M77| & 1.0 &-&-& 0.600 & -0.600 & -0.001 &-& 0.30 & 83.8 & 29.0 \\
252.6 & \verb|RIT:BBH:A7TH135PH90| & 1.0 & -0.510 &-& -0.510 & 0.510 &-& -0.510 & -0.51 & 58.3 & 22.9 \\
252.6 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 76.7 & 29.1 \\
252.6 & \verb|RIT:BBH:NQ33TH75PH30| & 3 & 0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 86.5 & 22.8 \\
252.6 & \verb|Del0_D10.97_q1.3333_a-0.6_-0.8_n100| & 1.334 &-&-& -0.600 &-&-& -0.801 & -0.69 & 54.2 & 34.3 \\
252.5 & \verb|D13_q1.00_a-0.80_-0.40_n100|(*) & 1.0 &-&-& -0.400 &-&-& -0.801 & -0.60 & 57.8 & 25.1 \\
252.5 & \verb|SXS:BBH:0044| & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.00 & 77.9 & 18.2 \\
252.5 & \verb|D11_q1.00_a-0.8_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 51.3 & 37.1 \\
252.4 & \verb|D11_q1.00_a-0.5_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& -0.500 & -0.50 & 59.2 & 29.9 \\
252.3 & \verb|GT:BBH:635| & 3.0 & 0.201 & -0.405 & 0.213 &-&-&-& 0.16 & 79.1 & 33.1 \\
252.3 & \verb|RIT:BBH:A7TH60PH0| & 1.0 & -0.053 & 0.616 & 0.379 & 0.028 & -0.624 & 0.368 & 0.37 & 87.4 & 30.4 \\
252.3 & \verb|RIT:BBH:A7TH60PH30| & 1.0 & -0.376 & 0.493 & 0.376 & 0.339 & -0.532 & 0.356 & 0.37 & 85.7 & 30.5 \\
252.1 & \verb|SXS:BBH:0037| & 3.001 & 0.498 & 0.038 &-&-& - &-& 0.00 & 79.6 & 12.1 \\
252.1 & \verb|RIT:BBH:A7TH60PH110| & 1.0 & -0.587 & -0.241 & 0.351 & 0.590 & 0.215 & 0.363 & 0.36 & 87.6 & 32.5 \\
251.9 & \verb|SXS:BBH:0271| & 3.0 &-&-& -0.300 & - & - &-& -0.22 & 69.4 & 13.6 \\
251.9 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 77.0 & 28.0 \\
251.9 & \verb|SXS:BBH:0270| & 3.0 &-& - & -0.300 & - & - & -0.300 & -0.30 & 67.1 & 13.9 \\
251.8 & \verb|SXS:BBH:0143| & 1.92 & -0.094 & -0.062 & 0.436 & -0.019 & -0.434 & -0.085 & 0.26 & 86.8 & 11.1 \\
251.7 & \verb|SXS:BBH:0030| & 3.0 &-&-&-& - &-&-& 0.00 & 78.3 & 14.6 \\
251.7 & \verb|D11.25_q0.3333_a0.0_0.0_n100|(*) & 3.0 &-&-&-&-&-& - & 0.00 & 77.3 & 20.1 \\
251.7 & \verb|SXS:BBH:0151| & 1.0 &-& - & -0.600 & - &-& -0.600 & -0.60 & 57.9 & 17.5 \\
251.7 & \verb|SXS:BBH:0273| & 2.999 &-&-& -0.269 & - & - & -0.849 & -0.41 & 65.2 & 14.5 \\
251.6 & \verb|SXS:BBH:0272| & 3.0 & - & - & -0.300 &-&-& 0.300 & -0.15 & 70.5 & 13.7 \\
251.6 & \verb|SXS:BBH:0034| & 3.001 & 0.497 & 0.047 & 0.001 &-& - &-& 0.00 & 77.7 & 14.7 \\
251.5 & \verb|SXS:BBH:0220| & 1.0 &-& - & -0.400 & - &-& -0.800 & -0.60 & 57.5 & 13.5 \\
251.5 & \verb|SXS:BBH:0050| & 3.0 & 0.494 & 0.072 & 0.002 & 0.467 & 0.176 & 0.005 & 0.00 & 78.4 & 14.3 \\
251.5 & \verb|RIT:BBH:A7TH60PH130| & 1.0 & -0.467 & -0.427 & 0.354 & 0.481 & 0.404 & 0.363 & 0.36 & 83.8 & 33.7 \\
251.3 & \verb|GT:BBH:747| & 3.0 & 0.335 & 0.317 & -0.192 &-&-&-& -0.14 & 64.0 & 41.5 \\
251.2 & \verb|RIT:BBH:LPH150| & 1.0 & -0.385 & -0.724 & 0.002 & 0.012 & 0.003 & 0.820 & 0.41 & 89.5 & 28.6 \\
251.1 & \verb|SXS:BBH:0053| & 3.0 & 0.494 & 0.075 & 0.001 & -0.464 & -0.184 & -0.003 & 0.00 & 78.9 & 14.6 \\
251.0 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 78.8 & 28.2 \\
250.9 & \verb|RIT:BBH:NTH15PH120| & 1.005 & -0.183 & -0.106 & 0.789 & - & - & - & 0.40 & 86.5 & 33.9 \\
250.9 & \verb|RIT:BBH:LPH90| & 1.0 & -0.819 & -0.038 & -0.009 & 0.016 &-& 0.820 & 0.41 & 88.8 & 28.6 \\
250.8 & \verb|RIT:BBH:A7TH60PH90| & 1.0 & -0.632 & -0.052 & 0.351 & 0.628 &-& 0.363 & 0.36 & 88.2 & 30.7 \\
250.8 & \verb|GT:BBH:746| & 3.0 & -0.267 & 0.412 & -0.094 &-&-&-& -0.07 & 66.8 & 41.2 \\
250.8 & \verb|SXS:BBH:0235| & 2.0 & - & - & -0.600 & - & - & -0.600 & -0.60 & 58.6 & 13.8 \\
250.7 & \verb|RIT:BBH:NTH15PH60| & 1.005 & -0.185 & 0.106 & 0.788 &-&-& - & 0.40 & 88.4 & 32.9 \\
250.7 & \verb|RIT:BBH:NQ25TH90PH150| & 4.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 73.8 & 25.5 \\
250.7 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 79.4 & 27.0 \\
250.7 & \verb|RIT:BBH:NTH15PH30| & 1.005 & -0.106 & 0.183 & 0.789 &-& - & - & 0.40 & 85.7 & 33.8 \\
250.5 & \verb|RIT:BBH:NTH15PH90| & 1.005 & -0.223 & -0.003 & 0.785 &-&-&-& 0.39 & 88.5 & 33.1 \\
250.5 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 78.3 & 27.3 \\
250.5 & \verb|RIT:BBH:NTH15PH0| & 1.005 & -0.005 & 0.215 & 0.788 &-& - & - & 0.39 & 88.4 & 32.7 \\
250.3 & \verb|D13.00_q0.50_a-0.50_-0.60_n100|(*) & 2.0 &-&-& -0.600 &-&-& -0.500 & -0.57 & 58.5 & 22.6 \\
250.3 & \verb|RIT:BBH:NQ50TH60PH120| & 2.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 86.0 & 28.8 \\
250.2 & \verb|GT:BBH:857| & 3.0 & 0.047 &-& 0.047 & -0.424 &-& -0.424 & -0.07 & 74.6 & 28.7 \\
250.2 & \verb|GT:BBH:406| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 87.9 & 21.2 \\
249.9 & \verb|EMu0_D8.80_q1.00_a0.8_n100| & 1.0 &-&-& 0.801 &-&-& - & 0.40 & 89.0 & 26.4 \\
249.9 & \verb|RIT:BBH:NTH15PH150| & 1.005 & -0.106 & -0.183 & 0.789 & - &-& - & 0.40 & 88.5 & 33.2 \\
249.8 & \verb|D13.00_q0.50_a0.00_-0.80_n100|(*) & 1.999 &-&-& -0.801 &-&-& - & -0.53 & 58.4 & 22.8 \\
249.8 & \verb|SXS:BBH:0277| & 3.0 & - & - &-& - &-& 0.300 & 0.07 & 79.7 & 12.7 \\
249.8 & \verb|SXS:BBH:0269| & 3.0 &-& - & -0.400 & - &-& 0.600 & -0.15 & 69.5 & 14.2 \\
249.8 & \verb|RIT:BBH:A7TH60PH210| & 1.0 & 0.361 & -0.514 & 0.362 & -0.314 & 0.544 & 0.362 & 0.36 & 87.9 & 29.9 \\
249.8 & \verb|RIT:BBH:NQ50TH60PH0| & 2.0 & 0.693 &-& 0.400 &-&-&-& 0.27 & 88.3 & 28.7 \\
249.6 & \verb|GT:BBH:551| & 1.0 &-&-&-&-&-& 0.800 & 0.40 & 87.7 & 18.2 \\
249.4 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 77.1 & 28.5 \\
249.4 & \verb|SXS:BBH:0311|(*) & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.40 & 92.2 & 12.3 \\
249.4 & \verb|RIT:BBH:LPH30| & 1.0 & -0.476 & 0.668 & 0.011 & 0.011 & 0.004 & 0.820 & 0.42 & 84.0 & 30.8 \\
249.3 & \verb|RIT:BBH:NQ25TH135PH150| & 4.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 57.4 & 41.7 \\
249.3 & \verb|RIT:BBH:NQ50TH60PH90| & 2.0 &-& 0.693 & 0.400 &-&-&-& 0.27 & 83.0 & 29.7 \\
249.3 & \verb|RIT:BBH:NQ33TH75PH120| & 3 & -0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 84.9 & 26.7 \\
249.2 & \verb|RIT:BBH:NQ25TH135PH120| & 4.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 57.7 & 40.3 \\
249.2 & \verb|SXS:BBH:0105| & 3.001 &-& - & -0.500 & - & - &-& -0.37 & 64.9 & 11.7 \\
249.2 & \verb|GT:BBH:881| & 2.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.18 & 87.5 & 23.3 \\
249.1 & \verb|RIT:BBH:LPH60| & 1.0 & -0.746 & 0.341 & -0.002 & 0.016 & -0.002 & 0.820 & 0.41 & 85.5 & 29.7 \\
249.1 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 76.9 & 28.7 \\
248.9 & \verb|SXS:BBH:0268| & 3.0 & - &-& -0.400 & - & - & -0.600 & -0.45 & 64.1 & 14.4 \\
248.9 & \verb|SXS:BBH:0251| & 2.0 & - & - & 0.300 & - & - & 0.300 & 0.30 & 87.4 & 11.0 \\
248.9 & \verb|GT:BBH:554| & 1.0 &-&-& 0.200 &-&-& 0.600 & 0.40 & 90.8 & 17.6 \\
248.8 & \verb|SXS:BBH:0049| & 3.0 & 0.494 & 0.073 & 0.001 & - & -0.008 & 0.499 & 0.13 & 81.6 & 13.9 \\
248.8 & \verb|GT:BBH:453| & 3.0 &-&-&-&-&-&-& 0.00 & 80.0 & 20.1 \\
248.8 & \verb|RIT:BBH:NQ25TH135PH90| & 4.0 &-& 0.566 & -0.566 &-&-&-& -0.45 & 59.1 & 38.2 \\
248.8 & \verb|SXS:BBH:0200| & 3.272 & - &-& - &-&-& - & -0.00 & 77.4 & 14.4 \\
248.7 & \verb|GT:BBH:422| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 90.8 & 17.4 \\
248.6 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 88.4 & 20.7 \\
248.6 & \verb|RIT:BBH:LPH0| & 1.0 & -0.064 & 0.817 & 0.013 & - & -0.010 & 0.820 & 0.42 & 80.8 & 32.5 \\
248.6 & \verb|RIT:BBH:NQ50TH60PH60| & 2.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 89.0 & 27.6 \\
248.5 & \verb|RIT:BBH:NQ50TH60PH150| & 2.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 87.0 & 29.3 \\
248.5 & \verb|SXS:BBH:0274| & 2.999 & - &-& -0.231 & - & - & 0.850 & 0.04 & 76.2 & 13.4 \\
248.4 & \verb|RIT:BBH:NQ50TH60PH30| & 2.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 86.4 & 28.6 \\
248.3 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 79.8 & 26.6 \\
248.3 & \verb|GT:BBH:882| & 2.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.20 & 88.3 & 23.4 \\
248.2 & \verb|GT:BBH:874| & 3.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.21 & 87.7 & 24.2 \\
247.6 & \verb|RIT:BBH:NQ25TH135PH60| & 4.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 60.7 & 39.6 \\
247.6 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 79.9 & 26.7 \\
247.3 & \verb|GT:BBH:726| & 3.0 & -0.197 & 0.385 & -0.251 &-&-&-& -0.19 & 61.8 & 45.5 \\
247.3 & \verb|SXS:BBH:0165| & 6.001 & 0.704 & 0.313 & -0.484 & -0.170 & -0.072 & -0.236 & -0.45 & 64.3 & 29.6 \\
247.1 & \verb|RIT:BBH:NQ25TH135PH30| & 4.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 56.2 & 40.8 \\
247.1 & \verb|SXS:BBH:0278| & 3.0 &-&-&-& - &-& 0.600 & 0.15 & 81.9 & 12.7 \\
247.1 & \verb|SXS:BBH:0281| & 3.0 &-& - & 0.300 & - & - & -0.300 & 0.15 & 86.5 & 12.0 \\
246.8 & \verb|RIT:BBH:NQ16TH115PH150| & 6.0 & -0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 65.9 & 33.3 \\
246.8 & \verb|RIT:BBH:NQ25TH90PH60| & 4.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 75.9 & 20.7 \\
246.7 & \verb|SXS:BBH:0046| & 3.0 &-&-& -0.500 & - &-& -0.499 & -0.50 & 62.8 & 18.3 \\
246.6 & \verb|SXS:BBH:0284| & 3.0 &-& - & 0.400 &-&-& -0.600 & 0.15 & 87.8 & 12.0 \\
246.6 & \verb|SXS:BBH:0248| & 2.0 &-& - & 0.129 &-& - & 0.850 & 0.37 & 88.9 & 11.4 \\
246.4 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 77.9 & 28.0 \\
246.3 & \verb|SXS:BBH:0266| & 3.0 &-&-& -0.600 &-&-& 0.400 & -0.35 & 65.4 & 14.6 \\
246.3 & \verb|SXS:BBH:0263| & 3.0 & - &-& -0.600 & - &-& 0.600 & -0.30 & 65.4 & 14.8 \\
246.3 & \verb|UD_D8.76_q2.00_a0.8_rl10_opt1_n100| & 2.0 &-&-& 0.801 &-&-& -0.801 & 0.27 & 91.7 & 26.2 \\
246.1 & \verb|SXS:BBH:0261| & 2.999 &-&-& -0.731 &-& - & 0.850 & -0.34 & 63.8 & 14.9 \\
245.9 & \verb|GT:BBH:684| & 3.0 & 0.289 & -0.281 & -0.296 &-&-&-& -0.22 & 65.0 & 43.2 \\
245.9 & \verb|GT:BBH:462| & 2.5 & 0.346 &-& 0.200 &-&-& 0.400 & 0.26 & 86.8 & 22.9 \\
245.8 & \verb|RIT:BBH:NQ25TH135PH0| & 4.0 & 0.566 &-& -0.566 &-&-&-& -0.45 & 60.8 & 37.5 \\
245.7 & \verb|RIT:BBH:NQ25TH90PH0| & 4.0 & 0.800 &-&-&-&-&-& 0.00 & 80.3 & 22.9 \\
245.7 & \verb|GT:BBH:606| & 3.0 & -0.411 & 0.149 & 0.242 &-&-&-& 0.18 & 84.8 & 25.1 \\
245.7 & \verb|GT:BBH:735| & 3.0 & -0.155 & -0.394 & -0.265 &-&-&-& -0.20 & 61.9 & 45.4 \\
245.6 & \verb|GT:BBH:462| & 2.5 & 0.346 &-& 0.200 &-&-& 0.400 & 0.26 & 84.8 & 24.3 \\
245.5 & \verb|RIT:BBH:NQ25TH90PH30| & 4.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 79.6 & 21.5 \\
245.4 & \verb|SXS:BBH:0262| & 3.0 &-&-& -0.600 &-&-& - & -0.45 & 61.9 & 15.0 \\
245.4 & \verb|GT:BBH:741| & 3.0 & 0.162 & 0.326 & 0.343 &-&-&-& 0.26 & 85.3 & 26.0 \\
245.2 & \verb|SXS:BBH:0209| & 1.0 & - & - & -0.900 & - & - & -0.500 & -0.70 & 55.4 & 12.6 \\
245.2 & \verb|SXS:BBH:0193| & 3.498 & - &-& - &-&-& - & -0.00 & 80.0 & 14.3 \\
245.2 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 77.5 & 27.9 \\
245.1 & \verb|GT:BBH:457| & 1.5 & 0.520 &-& 0.300 &-&-& 0.600 & 0.42 & 88.9 & 22.3 \\
245.0 & \verb|U0_D9.4_q2.00_a0.5_n100_am| & 2.0 &-&-& 0.500 &-&-& - & 0.33 & 90.9 & 21.8 \\
245.0 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 80.2 & 26.7 \\
244.9 & \verb|d0_D10.53_q6.00_a-0.83333_n100| & 5.996 &-&-& -0.835 &-&-& - & -0.72 & 53.7 & 37.9 \\
244.7 & \verb|RIT:BBH:NQ33TH75PH150| & 3 & -0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 86.9 & 26.8 \\
244.3 & \verb|SXS:BBH:0265| & 3.0 &-&-& -0.600 &-&-& -0.400 & -0.55 & 60.5 & 15.0 \\
244.2 & \verb|SXS:BBH:0229| & 1.0 &-& - & 0.650 & - &-& 0.250 & 0.45 & 92.4 & 10.5 \\
244.0 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 80.7 & 26.3 \\
243.9 & \verb|RIT:BBH:NQ25TH90PH90| & 4.0 &-& 0.800 &-&-&-&-& 0.00 & 75.4 & 20.8 \\
243.8 & \verb|SXS:BBH:0231| & 1.0 &-& - & 0.900 & - &-&-& 0.45 & 92.8 & 10.4 \\
243.8 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 78.9 & 26.9 \\
243.6 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 81.5 & 25.9 \\
243.5 & \verb|GT:BBH:457| & 1.5 & 0.520 &-& 0.300 &-&-& 0.600 & 0.42 & 92.0 & 14.6 \\
243.4 & \verb|GT:BBH:861| & 1.0 & -0.159 & -0.414 & -0.404 & 0.297 & 0.521 & -0.020 & -0.21 & 70.0 & 45.7 \\
243.4 & \verb|GT:BBH:863| & 1.0 & -0.512 & 0.270 & -0.157 & -0.506 & -0.175 & -0.270 & -0.21 & 69.1 & 49.3 \\
243.2 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 79.7 & 26.3 \\
243.2 & \verb|GT:BBH:459| & 2.5 & 0.283 &-& 0.283 &-&-& 0.400 & 0.32 & 90.4 & 21.9 \\
243.2 & \verb|SXS:BBH:0264| & 3.0 & - & - & -0.600 & - &-& -0.600 & -0.60 & 59.8 & 15.0 \\
242.9 & \verb|GT:BBH:459| & 2.5 & 0.283 &-& 0.283 &-&-& 0.400 & 0.32 & 87.7 & 24.2 \\
242.8 & \verb|RIT:BBH:NQ16TH135PH60| & 6.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 58.2 & 37.0 \\
242.8 & \verb|SXS:BBH:0282| & 3.0 &-&-& 0.300 & - & - &-& 0.22 & 89.1 & 12.1 \\
242.6 & \verb|RIT:BBH:NQ25TH90PH120| & 4.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 79.8 & 20.1 \\
242.5 & \verb|RIT:BBH:NQ16TH135PH150| & 6.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 56.9 & 38.0 \\
242.2 & \verb|GT:BBH:744| & 3.0 & 0.411 & -0.149 & 0.242 &-&-&-& 0.18 & 85.3 & 24.2 \\
242.2 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 80.2 & 26.1 \\
242.2 & \verb|Sq4_d9_a0.6_oth.270_rr_M100| & 4.0 & -0.601 & - &-& -0.601 & - &-& 0.00 & 84.8 & 37.3 \\
241.9 & \verb|SXS:BBH:0167| & 4.0 & - & - &-&-&-&-& 0.00 & 80.2 & 16.5 \\
241.8 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 81.8 & 25.6 \\
241.7 & \verb|RIT:BBH:A7TH45PH130| & 1.0 & -0.378 & -0.354 & 0.508 & 0.393 & 0.330 & 0.513 & 0.51 & 95.3 & 30.2 \\
241.7 & \verb|ro_b5_a0.6_oth.120_M077| & 1 & -0.212 & 0.367 & 0.424 &-&-& 0.600 & 0.51 & 94.5 & 18.5 \\
241.5 & \verb|RIT:BBH:NQ16TH135PH90| & 6.0 &-& 0.566 & -0.566 &-&-&-& -0.48 & 58.9 & 41.2 \\
241.3 & \verb|RIT:BBH:A7TH45PH315| & 1.0 & 0.344 & 0.384 & 0.510 & -0.363 & -0.363 & 0.513 & 0.51 & 93.0 & 29.4 \\
241.3 & \verb|GT:BBH:739| & 3.0 & -0.162 & -0.326 & 0.343 &-&-&-& 0.26 & 88.8 & 24.1 \\
241.2 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 78.3 & 27.0 \\
241.2 & \verb|RIT:BBH:NQ16TH135PH30| & 6.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 58.2 & 38.8 \\
241.1 & \verb|SXS:BBH:0258| & 2.0 & - &-& 0.871 & - & - & -0.849 & 0.30 & 94.2 & 10.6 \\
240.8 & \verb|RIT:BBH:NQ16TH115PH120| & 6.0 & -0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 66.0 & 33.7 \\
240.7 & \verb|GT:BBH:778| & 3.7 &-&-&-&-&-&-& 0.00 & 80.4 & 26.0 \\
240.7 & \verb|d0_D10.52_q3.00_a-0.66667_n100| & 2.999 &-&-& -0.667 &-&-& - & -0.50 & 57.5 & 34.3 \\
240.6 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 93.1 & 20.7 \\
240.6 & \verb|GT:BBH:461| & 2.0 & 0.520 &-& 0.300 &-&-& 0.600 & 0.40 & 91.2 & 22.0 \\
240.5 & \verb|GT:BBH:461| & 2.0 & 0.520 &-& 0.300 &-&-& 0.600 & 0.40 & 87.2 & 15.6 \\
240.5 & \verb|GT:BBH:414| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 91.1 & 20.8 \\
240.3 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 82.2 & 25.4 \\
240.2 & \verb|RIT:BBH:NQ16TH135PH120| & 6.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 61.1 & 37.6 \\
240.2 & \verb|D11.00_q0.2500_a0.0_0.0_n100|(*) & 4.0 &-&-&-&-&-& - & 0.00 & 80.3 & 20.2 \\
240.0 & \verb|RIT:BBH:NQ16TH90PH60| & 6.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 82.7 & 26.5 \\
239.9 & \verb|RIT:BBH:A7TH45PH0| & 1.0 & -0.028 & 0.507 & 0.517 & 0.028 & -0.507 & 0.518 & 0.52 & 93.9 & 28.8 \\
239.8 & \verb|GT:BBH:466| & 2.5 & 0.520 &-& 0.300 &-&-& 0.600 & 0.39 & 87.3 & 22.6 \\
239.8 & \verb|D11_q0.75_a0.0_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& - & 0.46 & 95.2 & 16.9 \\
239.8 & \verb|RIT:BBH:NQ16TH90PH30| & 6.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 79.7 & 24.9 \\
239.7 & \verb|GT:BBH:460| & 2.0 & 0.424 &-& 0.424 &-&-& 0.600 & 0.48 & 96.2 & 15.6 \\
239.6 & \verb|GT:BBH:613| & 3.0 & 0.176 & -0.221 & 0.413 &-&-&-& 0.31 & 90.7 & 23.7 \\
239.6 & \verb|RIT:BBH:NQ16TH150PH60| & 6.0 & 0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 55.2 & 39.4 \\
239.4 & \verb|RIT:BBH:NQ16TH150PH0| & 6.0 & 0.400 &-& -0.693 &-&-&-& -0.59 & 54.8 & 41.8 \\
239.4 & \verb|RIT:BBH:A7TH45PH210| & 1.0 & 0.299 & -0.412 & 0.516 & -0.256 & 0.444 & 0.513 & 0.51 & 92.9 & 29.5 \\
239.4 & \verb|EMuu_D8.82_q1.00_a0.2_n100| & 1.0 &-&-& 0.801 &-&-& 0.200 & 0.50 & 94.7 & 24.3 \\
239.2 & \verb|RIT:BBH:A7TH45PH90| & 1.0 & -0.518 & -0.054 & 0.505 & 0.513 &-& 0.513 & 0.51 & 92.9 & 29.9 \\
239.2 & \verb|RIT:BBH:NQ16TH90PH0| & 6.0 & 0.800 &-&-&-&-&-& 0.00 & 83.5 & 24.3 \\
239.1 & \verb|D11_q1.00_a0.5_0.5_n100|(*) & 1.0 &-&-& 0.500 &-&-& 0.500 & 0.50 & 94.3 & 16.7 \\
239.1 & \verb|GT:BBH:460| & 2.0 & 0.424 &-& 0.424 &-&-& 0.600 & 0.48 & 95.3 & 20.9 \\
239.0 & \verb|RIT:BBH:NQ16TH135PH0| & 6.0 & 0.566 &-& -0.566 &-&-&-& -0.48 & 57.7 & 39.3 \\
239.0 & \verb|GT:BBH:777| & 3.9 &-&-&-&-&-&-& 0.00 & 81.5 & 25.3 \\
238.9 & \verb|RIT:BBH:NQ16TH150PH120| & 6.0 & -0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 53.7 & 40.6 \\
238.8 & \verb|ro_b5_a0.6_oth.240_M077| & 1 & -0.212 & -0.367 & 0.424 &-&-& 0.600 & 0.51 & 93.6 & 18.6 \\
238.7 & \verb|ro_b5_a0.6_oth.000_M077| & 1 & 0.424 &-& 0.424 &-&-& 0.600 & 0.51 & 94.8 & 17.9 \\
238.6 & \verb|RIT:BBH:A7TH45PH30| & 1.0 & -0.299 & 0.411 & 0.518 & 0.256 & -0.444 & 0.513 & 0.52 & 95.7 & 28.0 \\
238.6 & \verb|SXS:BBH:0154| & 1.0 & - & - & -0.800 &-& - & -0.800 & -0.80 & 54.2 & 19.3 \\
238.6 & \verb|RIT:BBH:NQ16TH150PH30| & 6.0 & 0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 55.7 & 39.5 \\
238.4 & \verb|GT:BBH:780| & 3.8 &-&-&-&-&-&-& 0.00 & 82.1 & 25.2 \\
238.2 & \verb|SXS:BBH:0283| & 3.0 &-& - & 0.300 &-&-& 0.300 & 0.30 & 91.9 & 11.9 \\
238.2 & \verb|SXS:BBH:0062| & 5.003 & 0.384 & -0.236 & -0.218 &-& - &-& -0.18 & 67.8 & 0.0 \\
238.2 & \verb|(0,4,'MXX','D11')| & 4 &-&-&-&-&-&-& 0.00 & 78.5 & 20.7 \\
238.1 & \verb|RIT:BBH:NQ16TH115PH90| & 6.0 &-& 0.725 & -0.338 &-&-&-& -0.29 & 68.0 & 33.7 \\
238.0 & \verb|RIT:BBH:NQ16TH90PH90| & 6.0 &-& 0.800 &-&-&-&-& 0.00 & 80.6 & 26.5 \\
237.9 & \verb|GT:BBH:466| & 2.5 & 0.520 &-& 0.300 &-&-& 0.600 & 0.39 & 93.6 & 37.6 \\
237.9 & \verb|GT:BBH:879| & 3.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.24 & 89.0 & 23.6 \\
237.8 & \verb|GT:BBH:626| & 3.0 & 0.179 & 0.254 & 0.392 &-&-&-& 0.29 & 93.0 & 21.9 \\
237.8 & \verb|RIT:BBH:NQ16TH150PH90| & 6.0 &-& 0.400 & -0.693 &-&-&-& -0.59 & 56.8 & 37.2 \\
237.5 & \verb|RIT:BBH:NQ16TH115PH60| & 6.0 & 0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 66.4 & 33.3 \\
237.3 & \verb|GT:BBH:455| & 1.5 & 0.424 &-& 0.424 &-&-& 0.600 & 0.49 & 96.4 & 20.3 \\
237.2 & \verb|DU_D10.60_q3.00_a-0.8_rl11_n120| & 2.999 &-&-& -0.801 &-&-& 0.800 & -0.40 & 60.0 & 32.1 \\
237.1 & \verb|D11_q0.75_a0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& 0.500 & 0.50 & 95.5 & 16.7 \\
237.1 & \verb|GT:BBH:455| & 1.5 & 0.424 &-& 0.424 &-&-& 0.600 & 0.49 & 94.9 & 13.6 \\
236.7 & \verb|SXS:BBH:0058| & 5.002 & 0.498 & 0.027 &-&-& - &-& 0.00 & 79.0 & 12.2 \\
236.7 & \verb|RIT:BBH:NQ16TH90PH120| & 6.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 83.7 & 26.5 \\
236.5 & \verb|RIT:BBH:NQ16TH150PH150| & 6.0 & -0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 52.9 & 42.9 \\
236.4 & \verb|SXS:BBH:0057| & 5.002 & 0.402 & -0.177 & -0.201 & - &-&-& -0.17 & 75.9 & 27.3 \\
236.4 & \verb|GT:BBH:883| & 3.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.22 & 91.0 & 22.1 \\
236.3 & \verb|SXS:BBH:0162| & 2.0 &-& - & 0.600 &-&-&-& 0.40 & 94.3 & 12.2 \\
236.3 & \verb|GT:BBH:798| & 4.2 &-&-&-&-&-&-& 0.00 & 80.3 & 25.3 \\
236.3 & \verb|GT:BBH:470| & 4.0 & 0.600 &-&-&-&-& 0.600 & 0.12 & 80.0 & 29.9 \\
236.2 & \verb|RIT:BBH:NQ50TH30PH120| & 2.0 & -0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 93.8 & 26.6 \\
236.1 & \verb|GT:BBH:607| & 3.0 & -0.276 & 0.148 & 0.390 &-&-&-& 0.29 & 90.0 & 22.8 \\
235.8 & \verb|RIT:BBH:NQ16TH90PH150| & 6.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 81.2 & 28.8 \\
235.8 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 81.7 & 24.6 \\
235.8 & \verb|GT:BBH:884| & 3.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 96.2 & 21.3 \\
235.8 & \verb|GT:BBH:797| & 4.1 &-&-&-&-&-&-& 0.00 & 79.6 & 25.7 \\
235.6 & \verb|GT:BBH:795| & 4.4 &-&-&-&-&-&-& 0.00 & 82.7 & 24.4 \\
235.5 & \verb|SXS:BBH:0234| & 2.0 &-& - & -0.850 &-&-& -0.850 & -0.85 & 53.7 & 13.6 \\
235.5 & \verb|SXS:BBH:0059| & 5.0 & 0.265 & -0.096 & -0.157 &-& - &-& -0.13 & 75.1 & 26.9 \\
235.3 & \verb|SXS:BBH:0190| & 4.499 & - &-& - &-&-&-& -0.00 & 81.9 & 14.7 \\
235.3 & \verb|SXS:BBH:0043| & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.32 & 95.0 & 15.0 \\
235.3 & \verb|GT:BBH:555| & 1.0 &-&-& 0.200 &-&-& 0.800 & 0.50 & 98.6 & 16.2 \\
235.1 & \verb|GT:BBH:791| & 4.3 &-&-&-&-&-&-& 0.00 & 82.8 & 24.5 \\
234.4 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 81.9 & 25.1 \\
234.3 & \verb|RIT:BBH:NQ16TH115PH0| & 6.0 & 0.725 &-& -0.338 &-&-&-& -0.29 & 71.7 & 29.9 \\
234.2 & \verb|SXS:BBH:0033| & 3.001 & 0.248 & 0.030 & 0.432 & - & - &-& 0.32 & 96.2 & 11.9 \\
233.9 & \verb|RIT:BBH:NQ50TH30PH90| & 2.0 &-& 0.400 & 0.693 &-&-&-& 0.46 & 93.9 & 26.3 \\
233.7 & \verb|GT:BBH:400| & 1.0 & -0.693 &-& 0.400 & -0.800 &-&-& 0.20 & 81.4 & 40.6 \\
233.6 & \verb|RIT:BBH:NQ16TH115PH30| & 6.0 & 0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 73.5 & 28.6 \\
233.5 & \verb|RIT:BBH:NQ50TH30PH30| & 2.0 & 0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 94.9 & 26.9 \\
233.3 & \verb|GT:BBH:745| & 6.0 & -0.046 & 0.539 & 0.259 &-&-&-& 0.22 & 77.5 & 26.4 \\
233.1 & \verb|RIT:BBH:NQ50TH30PH0| & 2.0 & 0.400 &-& 0.693 &-&-&-& 0.46 & 88.2 & 29.5 \\
233.0 & \verb|RIT:BBH:NQ50TH30PH150| & 2.0 & -0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 95.1 & 26.9 \\
231.7 & \verb|SXS:BBH:0287| & 3.0 & - & - & 0.600 &-&-& -0.600 & 0.30 & 98.3 & 11.0 \\
231.7 & \verb|SXS:BBH:0159| & 1.0 &-&-& -0.900 & - & - & -0.900 & -0.90 & 52.1 & 19.6 \\
231.4 & \verb|RIT:BBH:NQ25TH60PH90| & 4.0 &-& 0.693 & 0.400 &-&-&-& 0.32 & 93.7 & 23.6 \\
231.3 & \verb|SXS:BBH:0280| & 2.999 & - & - & 0.269 &-& - & 0.850 & 0.41 & 95.3 & 11.4 \\
231.3 & \verb|SXS:BBH:0107| & 5.0 &-&-&-& - & - &-& 0.00 & 82.3 & 12.1 \\
231.1 & \verb|RIT:BBH:NQ25TH60PH60| & 4.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 93.2 & 22.3 \\
230.8 & \verb|d0_D11.03_q4.00_a-0.75_v2_n100| & 3.998 &-&-& -0.751 & - &-& - & -0.60 & 56.3 & 32.2 \\
230.6 & \verb|RIT:BBH:NQ25TH60PH0| & 4.0 & 0.693 &-& 0.400 &-&-&-& 0.32 & 92.7 & 24.5 \\
230.5 & \verb|GT:BBH:742| & 7.0 & -0.028 & 0.599 & -0.008 &-&-&-& -0.01 & 81.5 & 24.4 \\
230.3 & \verb|RIT:BBH:NQ50TH30PH60| & 2.0 & 0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 96.8 & 25.8 \\
230.3 & \verb|RIT:BBH:NQ25TH60PH165| & 4.0 & -0.669 & 0.179 & 0.400 &-&-&-& 0.32 & 93.6 & 25.2 \\
230.2 & \verb|GT:BBH:862| & 1.0 & 0.542 & -0.255 & -0.034 & 0.053 & 0.188 & -0.567 & -0.30 & 65.0 & 52.7 \\
230.2 & \verb|fr_b3.1_a0.6_oth.330_M77| & 1 & -0.300 &-& 0.520 & -0.600 &-&-& 0.26 & 79.8 & 45.5 \\
230.2 & \verb|SXS:BBH:0051| & 3.0 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.37 & 100.4 & 11.4 \\
230.0 & \verb|SXS:BBH:0187| & 5.039 &-& - &-& - & - & - & 0.00 & 83.7 & 15.2 \\
229.5 & \verb|SXS:BBH:0253| & 2.0 & - & - & 0.500 & - &-& 0.499 & 0.50 & 100.2 & 9.1 \\
229.5 & \verb|GT:BBH:875| & 4.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 87.5 & 24.7 \\
229.4 & \verb|GT:BBH:603| & 3.0 &-&-& 0.500 &-&-&-& 0.38 & 97.7 & 21.0 \\
229.2 & \verb|Del0_D8.87_q2.00_a0.4_0.8_n100| & 2.001 &-&-& 0.400 & 0.015 & -0.007 & 0.800 & 0.53 & 99.8 & 22.4 \\
229.1 & \verb|GT:BBH:469| & 4.0 & 0.520 &-& 0.300 &-&-& 0.600 & 0.36 & 101.5 & 9.9 \\
229.1 & \verb|GT:BBH:465| & 2.5 & 0.424 &-& 0.424 &-&-& 0.600 & 0.47 & 98.2 & 41.0 \\
229.0 & \verb|fr_b3.1_a0.6_oth.345_M77| & 1 & -0.155 &-& 0.580 & -0.600 &-&-& 0.29 & 80.9 & 45.3 \\
228.7 & \verb|SXS:BBH:0174| & 3.001 &-& - & 0.500 & - &-&-& 0.37 & 99.6 & 8.2 \\
228.6 & \verb|SXS:BBH:0048| & 3.0 & - & -0.001 & 0.500 & 0.471 & 0.165 & 0.001 & 0.37 & 100.1 & 11.3 \\
228.4 & \verb|GT:BBH:465| & 2.5 & 0.424 &-& 0.424 &-&-& 0.600 & 0.47 & 98.2 & 20.3 \\
228.1 & \verb|SXS:BBH:0156| & 1.0 &-&-& -0.949 &-&-& -0.949 & -0.95 & 49.9 & 17.8 \\
227.7 & \verb|SXS:BBH:0288| & 3.0 & - &-& 0.600 & - &-& -0.400 & 0.35 & 102.0 & 10.7 \\
227.6 & \verb|RIT:BBH:NQ25TH60PH120| & 4.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 102.6 & 20.2 \\
227.4 & \verb|RIT:BBH:NQ25TH60PH30| & 4.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 92.7 & 24.1 \\
227.3 & \verb|fr_b3.1_a0.6_oth.030_M77| & 1 & 0.300 &-& 0.520 & -0.600 &-&-& 0.26 & 82.9 & 45.1 \\
227.2 & \verb|fr_b3.1_a0.6_oth.015_M77| & 1 & 0.155 &-& 0.580 & -0.600 &-&-& 0.29 & 83.4 & 44.6 \\
226.9 & \verb|SXS:BBH:0197| & 5.522 & - &-& - &-&-& - & -0.00 & 84.4 & 15.0 \\
226.6 & \verb|fr_b3.1_a0.6_oth.300_M77| & 1 & -0.520 &-& 0.300 & -0.600 &-&-& 0.15 & 81.3 & 44.3 \\
226.6 & \verb|RIT:BBH:NQ25TH60PH150| & 4.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 93.9 & 24.3 \\
226.4 & \verb|EMuu_D8.78_q1.00_a0.4_n100| & 1.0 &-&-& 0.801 &-&-& 0.400 & 0.60 & 102.1 & 22.5 \\
226.1 & \verb|GT:BBH:401| & 1.0 & -0.400 &-& 0.693 & -0.800 &-&-& 0.35 & 88.7 & 39.4 \\
225.4 & \verb|SXS:BBH:0285| & 3.0 & - & - & 0.400 &-&-& 0.600 & 0.45 & 100.2 & 10.9 \\
225.2 & \verb|GT:BBH:398| & 1.0 & -0.800 &-& - & -0.800 &-&-& -0.00 & 76.3 & 43.0 \\
225.0 & \verb|GT:BBH:384| & 1.0 & 0.400 &-& 0.693 & -0.800 &-&-& 0.35 & 87.1 & 41.6 \\
224.6 & \verb|SXS:BBH:0225| & 1.0 &-& - & 0.400 & - &-& 0.800 & 0.60 & 101.7 & 9.6 \\
224.5 & \verb|GT:BBH:407| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 99.9 & 18.2 \\
224.5 & \verb|SXS:BBH:0152| & 1.0 &-& - & 0.600 & - &-& 0.600 & 0.60 & 101.2 & 9.9 \\
224.4 & \verb|DU_D10.61_q4.00_a-0.8_rl11_n100| & 3.999 &-&-& -0.801 &-&-& 0.800 & -0.48 & 56.5 & 34.7 \\
224.4 & \verb|fr_b3.1_a0.6_oth.285_M77| & 1 & -0.580 &-& 0.155 & -0.600 &-&-& 0.08 & 73.9 & 48.0 \\
224.3 & \verb|SXS:BBH:0108| & 5.002 & - & - & -0.500 &-&-&-& -0.42 & 66.2 & 17.5 \\
224.3 & \verb|GT:BBH:385| & 1.0 & 0.693 &-& 0.400 & -0.800 &-&-& 0.20 & 73.2 & 48.2 \\
223.8 & \verb|GT:BBH:880| & 4.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.27 & 100.1 & 20.5 \\
223.4 & \verb|RIT:BBH:NQ33TH45PH0| & 3 & 0.566 &-& 0.566 &-&-&-& 0.42 & 105.2 & 21.4 \\
223.3 & \verb|SXS:BBH:0292| & 2.999 &-& - & 0.731 &-& - & -0.849 & 0.34 & 103.6 & 10.7 \\
223.3 & \verb|RIT:BBH:NQ33TH45PH120| & 3 & -0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 103.8 & 21.8 \\
223.2 & \verb|SXS:BBH:0166| & 6.0 & - & - &-&-&-&-& 0.00 & 84.2 & 14.8 \\
223.1 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 101.0 & 15.5 \\
223.1 & \verb|D10.50_q0.1667_a0.0_0.0_n100|(*) & 6.0 &-&-&-&-&-& - & 0.00 & 84.6 & 19.3 \\
223.1 & \verb|RIT:BBH:NQ33TH45PH150| & 3 & -0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 108.6 & 21.6 \\
223.1 & \verb|GT:BBH:500| & 1.0 & 0.336 &-& 0.497 & -0.336 &-& 0.497 & 0.50 & 98.6 & 39.1 \\
223.0 & \verb|GT:BBH:507| & 1.0 & -0.336 &-& 0.497 & 0.336 & - & 0.497 & 0.50 & 97.6 & 39.5 \\
223.0 & \verb|fr_b3.1_a0.6_oth.045_M77| & 1 & 0.424 &-& 0.424 & -0.600 &-&-& 0.21 & 75.1 & 50.1 \\
222.9 & \verb|GT:BBH:411| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 104.1 & 17.5 \\
222.8 & \verb|GT:BBH:508| & 1.0 & -0.291 & -0.168 & 0.497 & 0.291 & 0.168 & 0.497 & 0.50 & 98.6 & 39.2 \\
222.8 & \verb|RIT:BBH:NQ25TH60PH135| & 4.0 & -0.490 & 0.490 & 0.400 &-&-&-& 0.32 & 92.7 & 23.6 \\
222.7 & \verb|GT:BBH:503| & 1.0 & 0.168 & 0.291 & 0.497 & -0.168 & -0.291 & 0.497 & 0.50 & 98.9 & 39.2 \\
222.6 & \verb|RIT:BBH:NQ33TH45PH90| & 3 &-& 0.566 & 0.566 &-&-&-& 0.42 & 88.8 & 24.3 \\
222.5 & \verb|GT:BBH:502| & 1.0 & 0.237 & 0.237 & 0.497 & -0.237 & -0.237 & 0.497 & 0.50 & 98.7 & 39.3 \\
222.1 & \verb|GT:BBH:512| & 1.0 & 0.291 & -0.168 & 0.497 & -0.291 & 0.168 & 0.497 & 0.50 & 98.6 & 39.1 \\
222.0 & \verb|d0_D11.35_q5.00_a-0.8_opt1_n100| & 4.997 &-&-& -0.801 &-&-& - & -0.67 & 61.3 & 28.2 \\
222.0 & \verb|GT:BBH:501| & 1.0 & 0.291 & 0.168 & 0.497 & -0.291 & -0.168 & 0.497 & 0.50 & 96.3 & 40.2 \\
221.6 & \verb|GT:BBH:509| & 1.0 & -0.168 & -0.291 & 0.497 & 0.168 & 0.291 & 0.497 & 0.50 & 100.8 & 38.5 \\
221.5 & \verb|GT:BBH:510| & 1.0 & - & -0.336 & 0.497 &-& 0.336 & 0.497 & 0.50 & 99.3 & 39.0 \\
221.5 & \verb|GT:BBH:506| & 1.0 & -0.291 & 0.168 & 0.497 & 0.291 & -0.168 & 0.497 & 0.50 & 98.6 & 39.1 \\
221.3 & \verb|GT:BBH:511| & 1.0 & 0.168 & -0.291 & 0.497 & -0.168 & 0.291 & 0.497 & 0.50 & 99.6 & 38.8 \\
221.2 & \verb|RIT:BBH:NQ33TH45PH60| & 3 & 0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 103.4 & 20.7 \\
221.2 & \verb|GT:BBH:504| & 1.0 &-& 0.336 & 0.497 & - & -0.336 & 0.497 & 0.50 & 99.9 & 38.8 \\
221.0 & \verb|RIT:BBH:A7TH22.5PH315| & 1.0 & 0.196 & 0.196 & 0.670 & -0.196 & -0.196 & 0.670 & 0.67 & 101.9 & 27.4 \\
220.8 & \verb|RIT:BBH:NQ33TH45PH30| & 3 & 0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 101.1 & 21.8 \\
220.7 & \verb|RIT:BBH:A7TH22.5PH90| & 1.0 & -0.288 & -0.026 & 0.665 & 0.278 &-& 0.670 & 0.67 & 102.9 & 27.6 \\
220.7 & \verb|D11.50_q0.50_a0.50_0.60_n100|(*) & 2.0 &-&-& 0.600 &-&-& 0.500 & 0.57 & 104.4 & 14.5 \\
220.5 & \verb|RIT:BBH:A7TH22.5PH130| & 1.0 & -0.213 & -0.178 & 0.670 & 0.213 & 0.178 & 0.670 & 0.67 & 104.3 & 27.6 \\
220.3 & \verb|RIT:BBH:A7TH22.5PH0| & 1.0 &-& 0.278 & 0.670 &-& -0.278 & 0.670 & 0.67 & 101.4 & 27.5 \\
220.3 & \verb|GT:BBH:513| & 1.0 & 0.548 &-& 0.244 & -0.548 &-& 0.244 & 0.24 & 81.8 & 50.0 \\
220.2 & \verb|RIT:BBH:A7TH22.5PH30| & 1.0 & -0.160 & 0.221 & 0.672 & 0.139 & -0.240 & 0.670 & 0.67 & 100.2 & 27.8 \\
220.0 & \verb|fr_b3.1_a0.6_oth.060_M77| & 1 & 0.520 &-& 0.300 & -0.600 &-&-& 0.15 & 75.6 & 50.3 \\
219.7 & \verb|GT:BBH:514| & 1.0 & 0.475 & 0.274 & 0.244 & -0.475 & -0.274 & 0.244 & 0.24 & 78.6 & 52.2 \\
219.4 & \verb|GT:BBH:505| & 1.0 & -0.168 & 0.291 & 0.497 & 0.168 & -0.291 & 0.497 & 0.50 & 97.8 & 39.6 \\
219.3 & \verb|SXS:BBH:0297| & 6.5 &-&-&-& - & - &-& 0.00 & 85.8 & 15.6 \\
219.3 & \verb|GT:BBH:518| & 1.0 & -0.475 & 0.274 & 0.244 & 0.475 & -0.274 & 0.244 & 0.24 & 79.2 & 52.3 \\
219.1 & \verb|GT:BBH:415| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 104.6 & 17.9 \\
218.9 & \verb|SXS:BBH:0289| & 3.0 &-&-& 0.600 &-&-& - & 0.45 & 105.4 & 10.4 \\
218.8 & \verb|SXS:BBH:0192| & 6.58 & - &-&-& - & - & - & 0.00 & 85.2 & 15.4 \\
218.6 & \verb|GT:BBH:517| & 1.0 & -0.274 & 0.475 & 0.244 & 0.274 & -0.475 & 0.244 & 0.24 & 81.4 & 51.3 \\
218.4 & \verb|SXS:BBH:0047| & 3.0 &-&-& 0.500 & - & - & 0.499 & 0.50 & 105.0 & 10.9 \\
218.0 & \verb|GT:BBH:515| & 1.0 & 0.274 & 0.475 & 0.244 & -0.274 & -0.475 & 0.244 & 0.24 & 80.8 & 51.5 \\
217.9 & \verb|fr_b3.1_a0.6_oth.270_M77| & 1 & -0.600 &-& - & -0.600 &-&-& -0.00 & 77.5 & 46.4 \\
217.7 & \verb|GT:BBH:516| & 1.0 &-& 0.548 & 0.244 & - & -0.548 & 0.244 & 0.24 & 81.2 & 51.7 \\
217.4 & \verb|RIT:BBH:A7TH22.5PH210| & 1.0 & 0.139 & -0.240 & 0.670 & -0.139 & 0.240 & 0.670 & 0.67 & 103.2 & 27.4 \\
217.4 & \verb|GT:BBH:887| & 5.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.28 & 105.2 & 18.5 \\
217.1 & \verb|SXS:BBH:0260| & 2.999 & - & - & -0.850 & - & - & -0.849 & -0.85 & 54.9 & 14.8 \\
217.1 & \verb|D11_q0.50_a0.00_0.80_n100|(*) & 1.999 &-&-& 0.801 &-&-& - & 0.53 & 106.9 & 14.8 \\
216.9 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 106.2 & 18.2 \\
216.8 & \verb|fr_b3.1_a0.6_oth.265_M77| & 1 & -0.598 &-& -0.052 & -0.600 &-&-& -0.03 & 69.9 & 51.3 \\
216.6 & \verb|SXS:BBH:0256| & 2.0 & - &-& 0.600 & - &-& 0.600 & 0.60 & 106.4 & 9.8 \\
216.2 & \verb|fr_b3.1_a0.6_oth.260_M77| & 1 & -0.591 &-& -0.104 & -0.600 &-&-& -0.05 & 70.3 & 51.5 \\
216.1 & \verb|GT:BBH:468| & 4.0 & 0.424 &-& 0.424 &-&-& 0.600 & 0.46 & 92.2 & 15.5 \\
215.4 & \verb|SXS:BBH:0188| & 7.187 &-& - &-& - &-& - & -0.00 & 87.0 & 15.0 \\
215.3 & \verb|SXS:BBH:0298| & 7.0 & - &-&-& - & - &-& 0.00 & 86.4 & 15.9 \\
215.0 & \verb|fr_b3.1_a0.6_oth.075_M77| & 1 & 0.580 &-& 0.155 & -0.600 &-&-& 0.08 & 70.9 & 54.7 \\
214.9 & \verb|GT:BBH:397| & 1.0 & -0.773 &-& -0.207 & -0.800 &-&-& -0.10 & 76.8 & 43.1 \\
214.7 & \verb|GT:BBH:889| & 6.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.30 & 109.3 & 17.7 \\
214.3 & \verb|UD_D8.40_q3.00_a0.8_rl11_n120| & 2.999 &-&-& 0.801 &-&-& -0.800 & 0.40 & 108.1 & 22.7 \\
213.9 & \verb|GT:BBH:720| & 3.0 & -0.424 & - & 0.424 & -0.600 &-&-& 0.32 & 94.9 & 27.2 \\
213.8 & \verb|GT:BBH:689| & 3.0 & 0.300 &-& 0.520 & -0.600 &-&-& 0.39 & 104.3 & 32.6 \\
213.3 & \verb|GT:BBH:388| & 1.0 & 0.800 &-&-& -0.800 &-&-& 0.00 & 72.3 & 52.2 \\
212.9 & \verb|SXS:BBH:0299| & 7.5 & - &-&-&-&-&-& 0.00 & 87.3 & 15.9 \\
212.8 & \verb|Del0_D8.83_q1.3333_a0.6_0.8_n100| & 1.334 &-&-& 0.600 &-&-& 0.801 & 0.69 & 107.8 & 21.0 \\
212.8 & \verb|GT:BBH:698| & 3.0 & 0.155 &-& 0.580 & -0.600 &-&-& 0.43 & 101.0 & 35.8 \\
212.6 & \verb|GT:BBH:666| & 2.5 & -0.300 & - & 0.520 & -0.600 &-&-& 0.37 & 99.0 & 29.6 \\
212.5 & \verb|GT:BBH:721| & 3.0 & -0.300 & - & 0.520 & -0.600 &-&-& 0.39 & 98.8 & 30.1 \\
212.0 & \verb|RIT:BBH:A9TH30PH210| & 1.0 & 0.231 & -0.400 & 0.800 & -0.231 & 0.400 & 0.800 & 0.80 & 112.4 & 23.0 \\
211.9 & \verb|D10_q7.00_a0.0_m320| & 7.0 &-&-&-&-&-&-& 0.00 & 88.9 & 0.0 \\
211.6 & \verb|GT:BBH:630| & 2.5 & -0.424 & - & 0.424 & -0.600 &-&-& 0.30 & 92.3 & 34.5 \\
211.5 & \verb|GT:BBH:723| & 3.0 & -0.520 & - & 0.300 & -0.600 &-&-& 0.22 & 92.5 & 33.3 \\
211.4 & \verb|SXS:BBH:0195| & 7.761 & - & - &-& - &-& - & 0.00 & 87.9 & 15.3 \\
210.8 & \verb|SXS:BBH:0061| & 5.002 &-& - & 0.500 & - &-&-& 0.42 & 111.4 & 9.2 \\
210.8 & \verb|SXS:BBH:0179| & 1.5 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.65 & 110.3 & 9.5 \\
210.6 & \verb|U0_D9.07_q3.00_a0.66667_n100| & 2.999 &-&-& 0.667 &-&-& - & 0.50 & 108.9 & 19.2 \\
210.1 & \verb|GT:BBH:648| & 2.5 & 0.155 &-& 0.580 & -0.600 &-&-& 0.41 & 97.9 & 37.6 \\
209.8 & \verb|RIT:BBH:A9TH30PH90| & 1.0 & -0.462 & -0.003 & 0.800 & 0.462 & 0.003 & 0.800 & 0.80 & 114.5 & 23.6 \\
209.7 & \verb|SXS:BBH:0232| & 1.0 &-& - & 0.900 &-& - & 0.500 & 0.70 & 109.5 & 8.8 \\
209.5 & \verb|GT:BBH:647| & 2.5 &-&-& 0.600 & -0.600 &-&-& 0.43 & 107.0 & 34.2 \\
209.2 & \verb|SXS:BBH:0290| & 3.0 &-& - & 0.600 & - &-& 0.400 & 0.55 & 111.7 & 9.9 \\
209.1 & \verb|GT:BBH:649| & 2.5 & 0.300 &-& 0.520 & -0.600 &-&-& 0.37 & 101.5 & 35.7 \\
209.1 & \verb|GT:BBH:668| & 2.5 & -0.155 & - & 0.580 & -0.600 &-&-& 0.41 & 100.7 & 33.5 \\
208.9 & \verb|GT:BBH:694| & 3.0 &-&-& 0.600 & -0.600 &-&-& 0.45 & 108.2 & 34.8 \\
208.5 & \verb|GT:BBH:888| & 7.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.32 & 110.2 & 16.8 \\
208.5 & \verb|RIT:BBH:A9TH30PH30| & 1.0 & -0.262 & 0.381 & 0.799 & 0.231 & -0.400 & 0.800 & 0.80 & 109.7 & 23.7 \\
208.4 & \verb|GT:BBH:722| & 3.0 & -0.155 & - & 0.580 & -0.600 &-&-& 0.43 & 109.7 & 33.3 \\
208.2 & \verb|GT:BBH:396| & 1.0 & -0.693 &-& -0.400 & -0.800 &-&-& -0.20 & 75.1 & 46.4 \\
208.0 & \verb|GT:BBH:690| & 3.0 & 0.424 &-& 0.424 & -0.600 &-&-& 0.32 & 100.3 & 32.2 \\
208.0 & \verb|RIT:BBH:A9TH30PH130| & 1.0 & -0.354 & -0.297 & 0.800 & 0.354 & 0.297 & 0.800 & 0.80 & 113.7 & 23.6 \\
207.6 & \verb|RIT:BBH:A9TH30PH0| & 1.0 & -0.027 & 0.445 & 0.809 & -0.004 & -0.462 & 0.800 & 0.80 & 117.0 & 21.8 \\
207.4 & \verb|RIT:BBH:A9TH30PH315| & 1.0 & 0.327 & 0.327 & 0.800 & -0.327 & -0.327 & 0.800 & 0.80 & 114.9 & 22.0 \\
205.6 & \verb|GT:BBH:382| & 1.0 &-&-& 0.800 & -0.800 &-&-& 0.40 & 98.0 & 37.4 \\
205.1 & \verb|SXS:BBH:0291| & 3.0 & - & - & 0.600 &-&-& 0.600 & 0.60 & 115.0 & 9.6 \\
204.6 & \verb|GT:BBH:646| & 2.5 & 0.424 &-& 0.424 & -0.600 &-&-& 0.30 & 100.1 & 34.3 \\
203.5 & \verb|GT:BBH:628| & 2.5 & -0.520 & - & 0.300 & -0.600 &-&-& 0.21 & 85.3 & 41.6 \\
202.7 & \verb|fr_b3.1_a0.6_oth.105_M77| & 1 & 0.580 &-& -0.155 & -0.600 &-&-& -0.08 & 74.8 & 55.1 \\
202.4 & \verb|SXS:BBH:0175| & 1.0 &-& - & 0.750 & - &-& 0.750 & 0.75 & 113.0 & 0.0 \\
202.2 & \verb|EK_D6.2_a0.6_th180_M77| & 1.0 & -0.584 & -0.143 & 0.002 & 0.584 & 0.143 & 0.002 & 0.00 & 70.7 & 65.3 \\
201.9 & \verb|GT:BBH:487| & 1.0 & -0.520 & 0.300 &-& 0.520 & -0.300 &-& 0.00 & 72.7 & 63.5 \\
201.5 & \verb|GT:BBH:691| & 3.0 & 0.520 &-& 0.300 & -0.600 &-&-& 0.22 & 90.0 & 33.5 \\
200.9 & \verb|EK_D6.2_a0.6_th000_M77| & 1.0 & 0.584 & 0.143 & 0.002 & -0.584 & -0.143 & 0.002 & 0.00 & 72.9 & 62.3 \\
200.4 & \verb|GT:BBH:489| & 1.0 & -0.520 & -0.300 &-& 0.520 & 0.300 &-& 0.00 & 70.7 & 65.9 \\
199.6 & \verb|GT:BBH:482| & 1.0 & 0.520 & 0.300 &-& -0.520 & -0.300 &-& 0.00 & 72.2 & 63.4 \\
199.5 & \verb|GT:BBH:486| & 1.0 & -0.300 & 0.520 &-& 0.300 & -0.520 &-& 0.00 & 72.5 & 64.0 \\
199.5 & \verb|GT:BBH:493| & 1.0 & 0.520 & -0.300 &-& -0.520 & 0.300 &-& 0.00 & 71.0 & 64.3 \\
198.5 & \verb|GT:BBH:490| & 1.0 & -0.300 & -0.520 &-& 0.300 & 0.520 &-& 0.00 & 72.9 & 64.1 \\
198.5 & \verb|RIT:BBH:NQ16TH45PH150| & 6.0 & -0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 118.9 & 20.4 \\
198.4 & \verb|GT:BBH:492| & 1.0 & 0.300 & -0.520 &-& -0.300 & 0.520 &-& 0.00 & 70.0 & 66.1 \\
198.3 & \verb|GT:BBH:645| & 2.5 & 0.520 &-& 0.300 & -0.600 &-&-& 0.21 & 83.4 & 37.2 \\
198.2 & \verb|GT:BBH:483| & 1.0 & 0.424 & 0.424 &-& -0.424 & -0.424 &-& 0.00 & 72.7 & 63.5 \\
198.1 & \verb|RIT:BBH:NQ16TH45PH120| & 6.0 & -0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 131.0 & 17.9 \\
198.0 & \verb|fr_b3.1_a0.6_oth.120_M77| & 1 & 0.520 &-& -0.300 & -0.600 &-&-& -0.15 & 69.1 & 61.8 \\
197.2 & \verb|GT:BBH:484| & 1.0 & 0.300 & 0.520 &-& -0.300 & -0.520 &-& 0.00 & 72.7 & 63.9 \\
197.1 & \verb|GT:BBH:491| & 1.0 & - & -0.600 &-&-& 0.600 &-& 0.00 & 75.0 & 62.1 \\
197.0 & \verb|GT:BBH:485| & 1.0 &-& 0.600 &-& - & -0.600 &-& 0.00 & 71.0 & 65.7 \\
196.6 & \verb|D10_q1.00_a0.8_0.8_n100|(*) & 1.0 &-&-& 0.801 &-&-& 0.801 & 0.80 & 117.2 & 15.4 \\
196.6 & \verb|GT:BBH:390| & 1.0 & 0.693 &-& -0.400 & -0.800 &-&-& -0.20 & 69.7 & 59.9 \\
196.5 & \verb|RIT:BBH:NQ16TH45PH90| & 6.0 &-& 0.566 & 0.566 &-&-&-& 0.48 & 111.0 & 20.8 \\
195.7 & \verb|GT:BBH:692| & 3.0 & 0.580 &-& 0.155 & -0.600 &-&-& 0.12 & 72.3 & 38.6 \\
195.6 & \verb|RIT:BBH:NQ16TH45PH60| & 6.0 & 0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 114.0 & 19.2 \\
195.6 & \verb|RIT:BBH:A9TH15PH130| & 1.0 & -0.183 & -0.154 & 0.893 & 0.183 & 0.154 & 0.893 & 0.89 & 123.5 & 21.9 \\
195.2 & \verb|GT:BBH:424| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 116.0 & 14.1 \\
195.1 & \verb|fr_b3.1_a0.6_oth.210_M77| & 1 & -0.300 &-& -0.520 & -0.600 &-&-& -0.26 & 72.0 & 60.0 \\
194.6 & \verb|SXS:BBH:0155| & 1.0 & - & - & 0.800 &-&-& 0.800 & 0.80 & 116.8 & 8.3 \\
194.5 & \verb|fr_b3.1_a0.6_oth.135_M77| & 1 & 0.424 &-& -0.424 & -0.600 &-&-& -0.21 & 73.4 & 60.2 \\
193.7 & \verb|RIT:BBH:A9TH15PH315| & 1.0 & 0.169 & 0.169 & 0.893 & -0.169 & -0.169 & 0.893 & 0.89 & 116.9 & 22.7 \\
193.6 & \verb|GT:BBH:395| & 1.0 & -0.400 &-& -0.693 & -0.800 &-&-& -0.35 & 72.7 & 56.8 \\
192.8 & \verb|RIT:BBH:NQ16TH45PH0| & 6.0 & 0.566 &-& 0.566 &-&-&-& 0.48 & 112.5 & 20.9 \\
192.8 & \verb|RIT:BBH:NQ16TH45PH30| & 6.0 & 0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 115.9 & 20.2 \\
191.3 & \verb|RIT:BBH:A9TH15PH0| & 1.0 &-& 0.239 & 0.893 &-& -0.239 & 0.893 & 0.89 & 124.1 & 21.4 \\
190.9 & \verb|RIT:BBH:A9TH15PH30| & 1.0 & -0.120 & 0.207 & 0.892 & 0.120 & -0.207 & 0.893 & 0.89 & 124.1 & 21.5 \\
190.3 & \verb|U0_D8.8_q4.00_a0.75_n100_am| & 3.999 &-&-& 0.751 &-&-& - & 0.60 & 129.8 & 16.7 \\
190.2 & \verb|RIT:BBH:A9TH15PH210| & 1.0 & 0.120 & -0.207 & 0.892 & -0.120 & 0.207 & 0.893 & 0.89 & 124.1 & 21.5 \\
190.1 & \verb|fr_b3.1_a0.6_oth.150_M77| & 1 & 0.300 &-& -0.520 & -0.600 &-&-& -0.26 & 73.5 & 61.7 \\
189.9 & \verb|fr_b3.1_a0.6_oth.195_M77| & 1 & -0.155 &-& -0.580 & -0.600 &-&-& -0.29 & 74.9 & 59.8 \\
189.5 & \verb|RIT:BBH:A9TH15PH90| & 1.0 & -0.258 & 0.005 & 0.887 & 0.258 & -0.005 & 0.888 & 0.89 & 116.3 & 23.3 \\
188.1 & \verb|GT:BBH:644| & 2.5 & 0.580 &-& 0.155 & -0.600 &-&-& 0.11 & 80.2 & 37.0 \\
187.6 & \verb|UU_D8.56_q2.00_a0.8_m100| & 2.0 &-&-& 0.801 & 0.016 & -0.004 & 0.800 & 0.80 & 123.1 & 18.9 \\
187.6 & \verb|fr_b3.1_a0.6_oth.165_M77| & 1 & 0.155 &-& -0.580 & -0.600 &-&-& -0.29 & 77.6 & 59.2 \\
187.5 & \verb|fr_b3.1_a0.6_oth.180_M77| & 1 &-&-& -0.600 & -0.600 &-&-& -0.30 & 75.5 & 60.6 \\
186.8 & \verb|SXS:BBH:0153| & 1.0 & - & - & 0.850 &-&-& 0.850 & 0.85 & 124.5 & 8.2 \\
183.6 & \verb|GT:BBH:391| & 1.0 & 0.400 &-& -0.693 & -0.800 &-&-& -0.35 & 80.2 & 55.9 \\
182.5 & \verb|GT:BBH:714| & 3.0 & -0.600 & - & - & -0.600 &-&-& 0.00 & 71.3 & 36.5 \\
180.7 & \verb|GT:BBH:393| & 1.0 &-&-& -0.800 & -0.800 &-&-& -0.40 & 69.4 & 65.9 \\
179.4 & \verb|GT:BBH:662| & 2.5 & -0.600 & - & - & -0.600 &-&-& 0.00 & 72.5 & 42.6 \\
178.5 & \verb|SXS:BBH:0160| & 1.0 &-& - & 0.900 &-&-& 0.900 & 0.90 & 125.9 & 7.7 \\
175.0 & \verb|SXS:BBH:0257| & 2.0 &-& - & 0.850 & - & - & 0.850 & 0.85 & 131.3 & 8.1 \\
170.3 & \verb|U0_D8.65_q5.00_a0.8_n100| & 4.997 &-&-& 0.801 &-&-&-& 0.67 & 142.6 & 15.2 \\
170.2 & \verb|SXS:BBH:0157| & 1.0 & - &-& 0.950 &-& - & 0.950 & 0.95 & 130.5 & 7.6 \\
170.1 & \verb|SXS:BBH:0293| & 2.999 &-& - & 0.850 & - &-& 0.849 & 0.85 & 146.6 & 7.7 \\
168.5 & \verb|SXS:BBH:0176| & 1.0 &-& - & 0.960 & - &-& 0.960 & 0.96 & 132.1 & 7.4 \\
168.2 & \verb|GT:BBH:693| & 3.0 & 0.600 &-&-& -0.600 &-&-& 0.00 & 73.5 & 40.4 \\
166.3 & \verb|SXS:BBH:0158| & 1.0 &-& - & 0.970 & - &-& 0.970 & 0.97 & 133.2 & 7.5 \\
165.0 & \verb|SXS:BBH:0172| & 1.0 &-& - & 0.979 & - &-& 0.979 & 0.98 & 132.7 & 7.7 \\
163.2 & \verb|Sq_D6.2_q2.50_a0.6_th090_m140| & 2.499 & 0.600 & 0.005 & -0.001 & -0.600 & -0.030 & -0.002 & -0.00 & 81.2 & 39.8 \\
162.8 & \verb|SXS:BBH:0177| & 1.0 &-&-& 0.989 & - & - & 0.989 & 0.99 & 133.2 & 7.4 \\
162.0 & \verb|SXS:BBH:0178| & 1.0 &-&-& 0.994 & - & - & 0.994 & 0.99 & 132.6 & 7.4 \\
148.2 & \verb|U0_D8.51_q6.00_a0.83333_n100_am| & 5.996 & 0.003 & -0.023 & 0.834 & - & - & - & 0.71 & 168.4 & 13.0 \\
128.0 & \verb|GT:BBH:663| & 2.5 & -0.520 & - & -0.300 & -0.600 &-&-& -0.21 & 66.0 & 58.4 \\
127.5 & \verb|GT:BBH:713| & 3.0 & -0.520 & - & -0.300 & -0.600 &-&-& -0.22 & 76.5 & 45.7 \\
116.8 & \verb|GT:BBH:685| & 3.0 & 0.520 &-& -0.300 & -0.600 &-&-& -0.22 & 69.6 & 50.4 \\
116.0 & \verb|GT:BBH:642| & 2.5 & 0.520 &-& -0.300 & -0.600 &-&-& -0.21 & 69.7 & 50.7 \\
\end{longtable}


==> simulation-rankings_30_C01_Lmax3.tex <==
\begin{longtable}{l|l|lrrrrrr|rr|r}
\caption{\label{tab:SimulationRanks:30:Lmax3}\textbf{Peak Marginalized $\ln L$ I: Consistency between simulations}: Peak value of the marginalized log likelihood $\ln L$ evaluated using a lower frequency $f_{low}=30\unit{Hz}$ [Eq. (\ref{eq:lnL})]  and all modes with $l \le 3$; the simulation key, described in Table \ref{tab:SimulationList} [an asterisk (*) denotes a new simulation motivated by \TheEvent{}]; the \emph{initial} spins of the simulation (using $-$ to denote zero, to enhance readability); the initial $\chi_{\rm eff}$; the total (redshifted) mass of the best fit; and the starting frequency (in Hz) of the best fit.   Though omitting information accessible to the longest simulations, this choice of low-frequency cutoff eliminates systematic biases associated with simulation duration, which differs across our archive.  } \\ \hline \hline $\ln L$ & Key & $q$ & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ & $\chi_{\rm eff}$ & $M_z/M_\odot$  & $f_{\rm start} (Hz)$  \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot 
272.0 & \verb|SXS:BBH:0307|(*) & 1.228 & - & - & 0.320 &-& - & -0.580 & -0.08 & 70.9 & 17.3 \\
271.8 & \verb|SXS:BBH:0115| & 1.07 & 0.019 & 0.013 & -0.204 & 0.243 & -0.067 & 0.291 & 0.04 & 74.0 & 14.6 \\
271.8 & \verb|SXS:BBH:0305|(*+) & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.02 & 73.5 & 15.4 \\
271.8 & \verb|D12_q1.00_a-0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& -0.250 & -0.00 & 73.6 & 20.4 \\
271.5 & \verb|SXS:BBH:0310|(*) & 1.221 & - &-&-& - & - &-& 0.00 & 72.4 & 15.4 \\
271.0 & \verb|GW15_D12_q1.22_a0.33_-0.44_m140|(*) & 1.22 & - &-& 0.330 & - &-& -0.440 & -0.02 & 72.8 & 19.4 \\
270.8 & \verb|SXS:BBH:0116| & 1.08 & -0.078 & 0.065 & 0.033 & 0.185 & 0.007 & 0.103 & 0.07 & 75.8 & 13.9 \\
270.7 & \verb|SXS:BBH:0002| & 1.0 &-& - &-&-&-&-& 0.00 & 75.1 & 9.7 \\
270.6 & \verb|SXS:BBH:0316|(*) & 1.186 & 0.241 & 0.170 & 0.299 & -0.203 & -0.172 & -0.271 & 0.04 & 74.1 & 15.2 \\
270.4 & \verb|D12.00_q0.85_a0.0_0.0_n100|(*) & 1.176 &-&-& - &-&-& - & -0.00 & 74.5 & 20.2 \\
270.4 & \verb|SXS:BBH:0120| & 1.12 & 0.138 & -0.200 & -0.008 & -0.065 & -0.241 & -0.099 & -0.05 & 70.0 & 14.9 \\
270.4 & \verb|SXS:BBH:0198| & 1.202 & - & - & - & - & - &-& 0.00 & 74.7 & 12.7 \\
270.3 & \verb|SXS:BBH:0125| & 1.27 & 0.012 & 0.045 & -0.058 & 0.389 & 0.241 & 0.070 & -0.00 & 73.5 & 13.6 \\
270.3 & \verb|GT:BBH:900|(*) & 1.2 & 0.400 &-&-& 0.400 &-&-& 0.00 & 72.7 & 22.3 \\
270.2 & \verb|D10_q0.75_a-0.5_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.500 & -0.07 & 73.7 & 26.7 \\
270.1 & \verb|GT:BBH:898|(*) & 1.2 &-&-&-&-&-&-& 0.00 & 74.8 & 17.9 \\
270.0 & \verb|SXS:BBH:0149| & 1.0 &-& - & -0.200 & - &-& -0.200 & -0.20 & 67.1 & 15.0 \\
269.9 & \verb|UD_D10.01_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& -0.400 & -0.00 & 72.7 & 26.9 \\
269.9 & \verb|S0_D10.04_q1.3333_a0.45_-0.80_n100| & 1.334 &-&-& 0.450 &-&-& -0.801 & -0.09 & 73.9 & 27.1 \\
269.9 & \verb|D12.25_q0.82_a-0.44_0.33_n100|(*+) & 1.22 &-&-& 0.330 &-&-& -0.440 & -0.02 & 71.8 & 20.6 \\
269.8 & \verb|aa_b5_a0.8_M77| & 1 &-&-& 0.800 &-&-& -0.800 & 0.00 & 74.7 & 26.7 \\
269.8 & \verb|D11_q0.75_a0.0_0.0_n100|(*) & 1.333 &-&-& - &-&-& - & -0.00 & 70.6 & 23.5 \\
269.8 & \verb|GW15_D12_q1.19_a0.42_-0.38_m140|(*) & 1.19 & - &-& 0.420 & - &-& -0.380 & 0.05 & 76.3 & 18.0 \\
269.8 & \verb|SXS:BBH:0308[Lev3]|(*) & 1.228 & 0.072 & 0.072 & 0.325 & 0.201 & 0.285 & -0.571 & -0.08 & 69.5 & 17.9 \\
269.8 & \verb|D10_q0.75_a-0.25_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& -0.250 & 0.04 & 76.6 & 24.4 \\
269.7 & \verb|U0_D9.53_q1.00_a0.0_n100| & 1.0 &-&-& - &-&-& - & -0.00 & 73.1 & 28.8 \\
269.7 & \verb|SXS:BBH:0308| & 1.228 & 0.094 & 0.056 & 0.322 & 0.266 & 0.213 & -0.576 & -0.08 & 71.0 & 17.4 \\
269.5 & \verb|SXS:BBH:0003| & 1.0 & 0.497 & 0.053 & - &-&-&-& -0.00 & 71.5 & 11.8 \\
269.5 & \verb|GT:BBH:476| & 1.0 &-&-& -0.200 &-&-& -0.200 & -0.20 & 66.6 & 24.8 \\
269.4 & \verb|GT:BBH:370| & 1.15 &-&-&-&-&-&-& 0.00 & 73.3 & 26.1 \\
269.4 & \verb|D12_q1.00_a-0.25_0.00_n100|(*) & 1.0 &-&-& - &-&-& -0.250 & -0.12 & 70.6 & 21.4 \\
269.2 & \verb|SXS:BBH:0131| & 1.55 & 0.042 & -0.014 & -0.070 & 0.105 & 0.017 & -0.175 & -0.11 & 70.9 & 14.8 \\
269.2 & \verb|GT:BBH:448| & 1.0 &-&-&-&-&-&-& 0.00 & 75.7 & 21.6 \\
269.1 & \verb|SXS:BBH:0147| & 1.0 & 0.404 & 0.294 & -0.001 & -0.404 & -0.294 & -0.001 & -0.00 & 71.6 & 24.4 \\
269.0 & \verb|SXS:BBH:0100| & 1.5 & - & - &-&-& - &-& 0.00 & 74.2 & 10.8 \\
269.0 & \verb|SXS:BBH:0127| & 1.34 & 0.010 & -0.077 & -0.017 & -0.061 & -0.065 & -0.179 & -0.09 & 73.0 & 14.4 \\
269.0 & \verb|SXS:BBH:0163| & 1.0 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.02 & 75.6 & 13.2 \\
268.9 & \verb|GT:BBH:885| & 1.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.00 & 70.2 & 32.4 \\
268.9 & \verb|RIT:BBH:KTH45PH90| & 1.0 & -0.595 & -0.035 & 0.562 & -0.591 & - & -0.568 & -0.00 & 73.3 & 34.9 \\
268.9 & \verb|SXS:BBH:0129| & 1.36 & -0.001 & - & 0.088 & 0.193 & -0.289 & -0.075 & 0.02 & 75.8 & 13.7 \\
268.9 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 73.6 & 31.4 \\
268.7 & \verb|(0,1.25,'M100')| & 1.25 &-&-&-&-&-&-& 0.00 & 76.0 & 24.9 \\
268.7 & \verb|SXS:BBH:0096| & 1.501 & 0.497 & 0.051 & - &-&-&-& -0.00 & 74.7 & 12.9 \\
268.6 & \verb|SXS:BBH:0117| & 1.08 & 0.118 & -0.069 & 0.070 & -0.302 & -0.298 & -0.200 & -0.06 & 73.6 & 14.5 \\
268.6 & \verb|RIT:BBH:NTH120PH120| & 1.005 & -0.611 & -0.353 & -0.407 &-&-& - & -0.20 & 65.8 & 35.6 \\
268.6 & \verb|RIT:BBH:KTH45PH120| & 1.0 & -0.502 & -0.290 & 0.579 & -0.502 & -0.290 & -0.579 & -0.00 & 72.4 & 36.4 \\
268.6 & \verb|SXS:BBH:0123| & 1.1 & 0.267 & 0.020 & -0.415 & 0.038 & -0.054 & 0.126 & -0.16 & 66.9 & 16.6 \\
268.6 & \verb|RIT:BBH:STH45PH60| & 1.0 & -0.537 & 0.242 & 0.570 & 0.502 & -0.290 & -0.579 & -0.00 & 68.7 & 38.1 \\
268.5 & \verb|RIT:BBH:STH45PH150| & 1.0 & -0.290 & -0.502 & 0.579 & 0.290 & 0.502 & -0.579 & -0.00 & 68.9 & 38.2 \\
268.5 & \verb|SXS:BBH:0082| & 1.501 & 0.496 & 0.053 & - &-&-&-& -0.00 & 74.3 & 13.9 \\
268.4 & \verb|(0.0,1.2,'M160','D9')| & 1.2 &-&-&-&-&-&-& 0.00 & 73.4 & 30.6 \\
268.4 & \verb|SXS:BBH:0121| & 1.12 & -0.061 & -0.109 & 0.356 & -0.323 & -0.127 & -0.297 & 0.05 & 74.0 & 15.1 \\
268.4 & \verb|RIT:BBH:STH45PH30| & 1.0 & -0.337 & 0.463 & 0.585 & 0.290 & -0.502 & -0.579 & 0.00 & 68.8 & 38.8 \\
268.4 & \verb|SXS:BBH:0098| & 1.501 & 0.486 & 0.114 & 0.002 &-&-&-& 0.00 & 74.4 & 11.6 \\
268.4 & \verb|D11_q0.75_a-0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& -0.500 & 0.07 & 78.3 & 21.2 \\
268.3 & \verb|RIT:BBH:STH45PH90| & 1.0 & -0.591 & -0.053 & 0.565 & 0.568 & -0.003 & -0.591 & -0.01 & 68.7 & 37.9 \\
268.3 & \verb|D11_q0.75_a0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& 0.500 & -0.07 & 68.8 & 24.4 \\
268.2 & \verb|SXS:BBH:0119| & 1.12 & -0.012 & 0.068 & 0.260 & 0.078 & -0.003 & 0.006 & 0.14 & 78.0 & 13.5 \\
268.2 & \verb|D11_q0.75_a0.8_0.4_PNr500_th1d_n100|(*) & 1.334 & 0.074 & -0.374 & 0.123 & -0.420 & -0.531 & -0.427 & -0.11 & 73.0 & 23.1 \\
268.0 & \verb|RIT:BBH:STH45PH0| & 1.0 & -0.034 & 0.569 & 0.589 & 0.002 & -0.591 & -0.568 & 0.01 & 71.0 & 38.0 \\
267.9 & \verb|RIT:BBH:KTH45PH135| & 1.0 & -0.410 & -0.410 & 0.579 & -0.410 & -0.410 & -0.579 & -0.00 & 72.3 & 37.2 \\
267.9 & \verb|GT:BBH:876| & 1.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.05 & 73.0 & 30.7 \\
267.8 & \verb|SXS:BBH:0029| & 1.5 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.00 & 73.7 & 13.5 \\
267.8 & \verb|SXS:BBH:0078| & 1.501 & 0.497 & 0.049 & - &-&-&-& -0.00 & 74.2 & 11.5 \\
267.8 & \verb|UD_D9.52_q1.00_a0.6_rl10_opt3_n100| & 1.0 &-&-& 0.600 &-&-& -0.600 & -0.00 & 73.8 & 29.4 \\
267.7 & \verb|SXS:BBH:0097| & 1.501 & 0.495 & 0.065 & 0.001 &-&-&-& 0.00 & 75.1 & 14.5 \\
267.7 & \verb|RIT:BBH:KTH45PH105| & 1.0 & -0.567 & -0.177 & 0.564 & -0.560 & -0.150 & -0.579 & -0.01 & 72.7 & 35.6 \\
267.7 & \verb|RIT:BBH:NTH120PH90| & 1.005 & -0.706 & -0.033 & -0.403 & - &-& - & -0.20 & 63.6 & 37.1 \\
267.7 & \verb|D21.5_q1_a0.2_0.8_th104.4775_n100| & 1.001 &-&-& 0.200 & 0.775 &-& -0.200 & -0.00 & 72.3 & 9.9 \\
267.6 & \verb|D11_q0.75_a-0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& -0.500 & -0.21 & 68.7 & 24.1 \\
267.5 & \verb|D10_q0.75_a0.8_xi0_n100|(*) & 1.333 & 0.528 & 0.062 & -0.598 &-&-& 0.801 & 0.00 & 72.1 & 27.5 \\
267.5 & \verb|RIT:BBH:KTH22.5PH60| & 1.0 & -0.297 & 0.138 & 0.751 & -0.272 & 0.157 & -0.757 & -0.00 & 71.1 & 38.0 \\
267.4 & \verb|RIT:BBH:KTH45PH150| & 1.0 & -0.290 & -0.502 & 0.579 & -0.290 & -0.502 & -0.579 & -0.00 & 71.0 & 38.2 \\
267.4 & \verb|GT:BBH:546| & 1.0 &-&-&-&-&-& 0.200 & 0.10 & 79.3 & 20.6 \\
267.4 & \verb|D10_q0.75_a0.25_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.250 & -0.04 & 73.6 & 25.6 \\
267.4 & \verb|RIT:BBH:KTH45PH0| & 1.0 & -0.037 & 0.570 & 0.587 & -0.021 & 0.578 & -0.580 & 0.00 & 72.7 & 36.5 \\
267.4 & \verb|D10_q0.75_a0.5_-0.25_n100|(*) & 1.333 &-&-& -0.250 &-&-& 0.500 & 0.07 & 76.9 & 24.2 \\
267.3 & \verb|D11_q0.75_a0.6_0.6_PNr500_th1d_n100|(*) & 1.333 & 0.460 & 0.351 & 0.161 & 0.526 & 0.288 & -0.023 & 0.08 & 78.1 & 21.0 \\
267.3 & \verb|RIT:BBH:KTH45PH60| & 1.0 & -0.549 & 0.217 & 0.568 & -0.502 & 0.290 & -0.579 & -0.01 & 74.9 & 34.5 \\
267.2 & \verb|SXS:BBH:0088| & 1.0 & 0.495 & 0.067 &-&-&-&-& 0.00 & 72.0 & 11.9 \\
267.2 & \verb|RIT:BBH:KTH22.5PH120| & 1.0 & -0.272 & -0.157 & 0.757 & -0.272 & -0.157 & -0.757 & -0.00 & 70.9 & 39.0 \\
267.1 & \verb|SXS:BBH:0173| & 1.5 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.14 & 69.2 & 13.7 \\
267.1 & \verb|RIT:BBH:KTH22.5PH30| & 1.0 & -0.185 & 0.257 & 0.756 & -0.157 & 0.272 & -0.757 & -0.00 & 71.0 & 38.1 \\
267.1 & \verb|SXS:BBH:0103| & 1.501 & 0.496 & 0.058 &-&-&-&-& 0.00 & 74.5 & 10.6 \\
267.0 & \verb|(0.0,1.3,'M160','D9')| & 1.3 &-&-&-&-&-&-& 0.00 & 73.4 & 30.5 \\
267.0 & \verb|SXS:BBH:0006| & 1.345 & 0.234 & 0.148 & -0.161 & 0.091 & 0.064 & -0.101 & -0.14 & 67.8 & 13.9 \\
267.0 & \verb|SXS:BBH:0010| & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.26 & 65.1 & 14.2 \\
267.0 & \verb|SXS:BBH:0024| & 1.501 & 0.496 & 0.051 & -0.001 & -0.077 & 0.489 & 0.002 & 0.00 & 72.6 & 12.6 \\
267.0 & \verb|RIT:BBH:KTH45PH30| & 1.0 & -0.355 & 0.443 & 0.590 & -0.290 & 0.502 & -0.579 & 0.01 & 75.9 & 34.9 \\
266.9 & \verb|RIT:BBH:NTH120PH150| & 1.005 & -0.322 & -0.617 & -0.422 & - & - &-& -0.21 & 67.3 & 35.4 \\
266.9 & \verb|SXS:BBH:0027| & 1.5 & 0.497 & 0.051 & - & -0.494 & -0.071 &-& 0.00 & 74.5 & 13.6 \\
266.9 & \verb|SXS:BBH:0021| & 1.5 & 0.496 & 0.053 & - & - & 0.001 & -0.499 & -0.20 & 68.7 & 13.0 \\
266.9 & \verb|RIT:BBH:NTH120PH30| & 1.005 & -0.408 & 0.580 & -0.399 & - &-& - & -0.20 & 65.6 & 37.2 \\
266.8 & \verb|D11_q0.75_a-0.8500_0.6375_n100| & 1.334 &-&-& 0.638 & 0.001 & 0.003 & -0.851 & -0.00 & 77.0 & 22.0 \\
266.8 & \verb|D12_q1.00_a-0.25_-0.25_n100|(*) & 1.0 &-&-& -0.250 &-&-& -0.250 & -0.25 & 64.5 & 23.6 \\
266.7 & \verb|SXS:BBH:0194| & 1.518 &-& - &-& - &-& - & -0.00 & 74.8 & 13.6 \\
266.6 & \verb|D10_q0.75_a-0.8_xi0_n100|(*) & 1.333 & 0.538 & 0.056 & 0.590 &-&-& -0.801 & -0.01 & 74.1 & 26.9 \\
266.6 & \verb|SXS:BBH:0133| & 1.63 & 0.098 & 0.042 & -0.134 & -0.107 & -0.110 & -0.021 & -0.09 & 72.1 & 14.0 \\
266.6 & \verb|Rflop_r500_d11_q0.7_a0.8_m088|(*) & 1.428 & 0.603 & 0.445 & 0.283 & 0.747 & 0.278 & -0.079 & 0.13 & 79.7 & 21.1 \\
266.6 & \verb|D11_q0.75_a0.8_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.308 & 0.640 & 0.369 & -0.006 & 0.763 & -0.243 & 0.11 & 82.1 & 20.8 \\
266.5 & \verb|SXS:BBH:0126| & 1.29 & -0.250 & -0.237 & 0.091 & -0.358 & 0.172 & 0.215 & 0.15 & 79.8 & 13.7 \\
266.5 & \verb|SXS:BBH:0137| & 1.76 & -0.248 & -0.319 & -0.034 & -0.071 & 0.151 & -0.190 & -0.09 & 73.6 & 14.5 \\
266.4 & \verb|SXS:BBH:0138| & 1.7 & -0.044 & 0.425 & 0.042 & -0.012 & -0.008 & -0.111 & -0.01 & 73.2 & 14.3 \\
266.4 & \verb|RIT:BBH:NQ200TH135PH30| & 2 &-&-&-& 0.490 & 0.283 & -0.566 & -0.19 & 69.8 & 18.8 \\
266.3 & \verb|GT:BBH:866| & 1.0 & -0.354 & 0.233 & 0.424 & 0.494 & -0.341 & -0.001 & 0.21 & 77.1 & 35.1 \\
266.2 & \verb|RIT:BBH:STH45PH120| & 1.0 & -0.498 & -0.319 & 0.567 & 0.502 & 0.290 & -0.579 & -0.01 & 68.8 & 38.3 \\
266.2 & \verb|SXS:BBH:0023| & 1.501 & 0.497 & 0.051 & 0.001 & 0.077 & -0.489 &-& 0.00 & 75.2 & 13.1 \\
266.2 & \verb|RIT:BBH:KTH22.5PH0| & 1.0 & -0.026 & 0.304 & 0.760 & -0.008 & 0.310 & -0.759 & 0.00 & 71.1 & 38.3 \\
266.2 & \verb|SXS:BBH:0025| & 1.5 & - & - & 0.500 & - & - & -0.499 & 0.10 & 80.5 & 10.6 \\
266.2 & \verb|SXS:BBH:0004| & 1.0 & - & - & -0.500 & - & - &-& -0.25 & 64.9 & 11.5 \\
266.1 & \verb|d0_D10.52_q1.3333_a-0.25_n100| & 1.333 &-&-& -0.250 &-&-& - & -0.14 & 70.2 & 25.7 \\
266.1 & \verb|SXS:BBH:0135| & 1.64 & -0.110 & 0.027 & 0.024 & 0.211 & -0.144 & -0.229 & -0.07 & 72.8 & 14.3 \\
266.1 & \verb|RIT:BBH:KTH22.5PH90| & 1.0 & -0.331 & -0.026 & 0.749 & -0.314 & -0.007 & -0.757 & -0.00 & 73.3 & 37.3 \\
266.1 & \verb|RIT:BBH:NTH120PH60| & 1.005 & -0.643 & 0.299 & -0.399 &-& - & - & -0.20 & 63.5 & 37.7 \\
266.1 & \verb|SXS:BBH:0019| & 1.5 & - & - & -0.500 & - & - & 0.499 & -0.10 & 71.0 & 13.1 \\
266.0 & \verb|aa_b5_a0.6_M77| & 1 &-&-& 0.600 &-&-& -0.600 & 0.00 & 72.7 & 25.6 \\
266.0 & \verb|aa_b5_a0.4_M77| & 1 &-&-& 0.400 &-&-& -0.400 & 0.00 & 72.7 & 24.7 \\
265.9 & \verb|D10_q0.75_a0.0_0.25_n100|(*) & 1.333 &-&-& 0.250 &-&-& - & 0.14 & 80.2 & 22.9 \\
265.9 & \verb|GT:BBH:372| & 1.45 &-&-&-&-&-&-& 0.00 & 75.8 & 25.3 \\
265.9 & \verb|aa_b5_a0.2_M77| & 1 &-&-& 0.200 &-&-& -0.200 & 0.00 & 72.7 & 24.1 \\
265.9 & \verb|RIT:BBH:KTH45PH165| & 1.0 & -0.119 & -0.558 & 0.588 & -0.150 & -0.560 & -0.579 & 0.00 & 70.6 & 38.8 \\
265.8 & \verb|SXS:BBH:0140| & 1.82 & 0.115 & -0.367 & -0.209 & -0.066 & 0.062 & 0.087 & -0.10 & 71.7 & 14.3 \\
265.8 & \verb|RIT:BBH:NQ200TH135PH150| & 2 &-&-&-& -0.490 & 0.283 & -0.566 & -0.19 & 69.8 & 21.6 \\
265.8 & \verb|SXS:BBH:0161| & 1.0 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.29 & 65.7 & 14.3 \\
265.7 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 73.2 & 31.4 \\
265.6 & \verb|D10_q0.75_a-0.8_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.801 & 0.11 & 77.6 & 25.6 \\
265.5 & \verb|S0_D9.96_q1.3333_a-0.45_0.80_n100| & 1.334 &-&-& -0.450 &-&-& 0.801 & 0.09 & 73.8 & 26.9 \\
265.5 & \verb|GT:BBH:717| & 1.1 &-&-&-&-&-&-& 0.00 & 72.0 & 31.3 \\
265.5 & \verb|GT:BBH:477| & 1.5 &-&-&-&-&-&-& 0.00 & 76.1 & 21.5 \\
265.5 & \verb|D11.50_q0.60_a0.0_0.0_n100|(*) & 1.667 &-&-& - &-&-& - & -0.00 & 75.7 & 20.6 \\
265.3 & \verb|D9_q1.3_a0.0_m160| & 1.3 &-&-& - & - & - & - & -0.00 & 75.5 & 30.6 \\
265.3 & \verb|GT:BBH:730| & 1.4 &-&-&-&-&-&-& 0.00 & 75.0 & 29.8 \\
265.1 & \verb|SXS:BBH:0015| & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.00 & 76.1 & 10.3 \\
265.1 & \verb|GT:BBH:891| & 2.0 & 0.328 & -0.270 & -0.423 & -0.425 & -0.076 & 0.417 & -0.14 & 65.4 & 34.4 \\
265.1 & \verb|D11_q0.75_a0.8500_-0.6375_n100|(*) & 1.334 &-&-& -0.638 & -0.001 & 0.003 & 0.851 & 0.00 & 70.5 & 24.1 \\
265.1 & \verb|RIT:BBH:NTH120PH0| & 1.005 & -0.062 & 0.702 & -0.407 &-&-&-& -0.20 & 63.5 & 39.9 \\
265.1 & \verb|DU_D10.86_q1.3333_a-0.8_opt1_n100| & 1.333 &-&-& -0.801 &-&-& 0.801 & -0.11 & 66.9 & 26.2 \\
265.0 & \verb|RIT:BBH:KTH22.5PH150| & 1.0 & -0.157 & -0.272 & 0.757 & -0.157 & -0.272 & -0.757 & -0.00 & 72.8 & 38.5 \\
265.0 & \verb|UD_D9.51_q1.00_a0.8_rl10_opt1_n100| & 1.0 &-&-& 0.801 &-&-& -0.801 & -0.00 & 71.2 & 30.9 \\
264.8 & \verb|RIT:BBH:NTH60PH150| & 1.005 & -0.353 & -0.612 & 0.408 & - &-& - & 0.20 & 76.4 & 38.3 \\
264.8 & \verb|SXS:BBH:0134| & 1.63 & -0.230 & 0.184 & -0.012 & -0.001 & 0.032 & 0.176 & 0.06 & 77.0 & 13.0 \\
264.7 & \verb|GT:BBH:893| & 2.0 & -0.328 & 0.270 & -0.423 & 0.425 & 0.076 & 0.417 & -0.14 & 65.0 & 36.1 \\
264.7 & \verb|D9_q2.0_a0.6_0.6_th180_r100_res140_CE| & 2.0 & - & - & -0.600 & - &-& 0.601 & -0.20 & 62.3 & 36.6 \\
264.7 & \verb|GT:BBH:865| & 1.0 & -0.096 & 0.467 & 0.364 & 0.208 & 0.562 & 0.033 & 0.20 & 80.3 & 34.5 \\
264.5 & \verb|RIT:BBH:NQ200TH135PH90| & 2 &-&-&-&-& 0.566 & -0.566 & -0.19 & 68.5 & 21.2 \\
264.4 & \verb|SXS:BBH:0146| & 1.97 & -0.156 & -0.102 & -0.037 & -0.098 & 0.027 & -0.357 & -0.14 & 70.5 & 14.8 \\
264.2 & \verb|SXS:BBH:0306|(*) & 1.31 & - &-& 0.961 & - & - & -0.899 & 0.16 & 82.7 & 15.8 \\
264.1 & \verb|SXS:BBH:0150| & 1.0 &-& - & 0.200 & - &-& 0.200 & 0.20 & 82.2 & 12.1 \\
264.0 & \verb|RIT:BBH:NQ200TH135PH0| & 2 &-&-&-& 0.566 &-& -0.566 & -0.19 & 70.9 & 18.9 \\
264.0 & \verb|SXS:BBH:0130| & 1.38 & 0.164 & 0.037 & -0.014 & 0.293 & 0.060 & 0.343 & 0.14 & 79.8 & 12.4 \\
263.9 & \verb|D11_q1.00_a0.0_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& - & -0.25 & 66.1 & 25.8 \\
263.8 & \verb|(0.0,1.75,'M100')| & 1.75 &-&-&-&-&-&-& 0.00 & 76.5 & 25.0 \\
263.7 & \verb|RIT:BBH:NQ200TH135PH120| & 2 &-&-&-& -0.283 & 0.490 & -0.566 & -0.19 & 68.7 & 21.7 \\
263.7 & \verb|RIT:BBH:NTH60PH0| & 1.005 & -0.058 & 0.692 & 0.429 &-& - & - & 0.21 & 78.6 & 36.7 \\
263.7 & \verb|RIT:BBH:NTH60PH120| & 1.005 & -0.612 & -0.353 & 0.408 &-&-& - & 0.20 & 79.8 & 36.5 \\
263.6 & \verb|GT:BBH:873| & 1.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.08 & 77.1 & 27.7 \\
263.6 & \verb|SXS:BBH:0169| & 2.0 & - & - &-&-&-&-& 0.00 & 73.9 & 15.9 \\
263.6 & \verb|GT:BBH:856| & 2.0 & 0.106 &-& 0.106 & -0.424 &-& -0.424 & -0.07 & 71.2 & 28.8 \\
263.6 & \verb|D12_q1.00_a0.25_0.25_n100|(*) & 1.0 &-&-& 0.250 &-&-& 0.250 & 0.25 & 82.1 & 18.1 \\
263.5 & \verb|D11_q0.75_a0.5_0.0_n100|(*) & 1.333 &-&-& - &-&-& 0.500 & 0.21 & 80.5 & 19.7 \\
263.5 & \verb|RIT:BBH:NTH60PH90| & 1.005 & -0.716 & -0.035 & 0.389 & - & - &-& 0.20 & 79.2 & 36.0 \\
263.4 & \verb|EMu0_D9.16_q1.00_a0.4_n100| & 1.0 &-&-& 0.400 &-&-& - & 0.20 & 80.2 & 27.8 \\
263.3 & \verb|SXS:BBH:0124| & 1.26 & 0.250 & -0.058 & 0.071 & 0.075 & -0.095 & 0.286 & 0.17 & 80.8 & 12.5 \\
263.3 & \verb|q150_a8_a0_th_60_ph_120| & 1.492 & - & - &-& -0.595 & -0.380 & 0.405 & 0.16 & 78.2 & 34.3 \\
263.2 & \verb|RIT:BBH:NQ200TH135PH60| & 2 &-&-&-& 0.283 & 0.490 & -0.566 & -0.19 & 71.0 & 19.2 \\
263.1 & \verb|RIT:BBH:NTH60PH60| & 1.005 & -0.656 & 0.274 & 0.401 &-& - & - & 0.20 & 77.9 & 36.4 \\
263.1 & \verb|GT:BBH:547| & 1.0 &-&-&-&-&-& 0.400 & 0.20 & 82.7 & 19.6 \\
262.8 & \verb|D9_q1.6_a0.0_m160| & 1.6 &-&-& - & - & - & - & -0.00 & 74.8 & 30.6 \\
262.8 & \verb|SXS:BBH:0132| & 1.63 & -0.005 & -0.114 & -0.007 & 0.041 & -0.087 & 0.310 & 0.11 & 79.1 & 12.4 \\
262.5 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 75.1 & 30.4 \\
262.5 & \verb|(0.0,1.6,'M160','D9')| & 1.6 &-&-&-&-&-&-& 0.00 & 76.2 & 29.1 \\
262.4 & \verb|GT:BBH:877| & 1.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.12 & 80.9 & 25.5 \\
262.3 & \verb|RIT:BBH:NTH135PH120| & 1.005 & -0.498 & -0.288 & -0.576 & - & - & - & -0.29 & 61.2 & 39.1 \\
262.3 & \verb|RIT:BBH:NTH135PH60| & 1.005 & -0.520 & 0.265 & -0.568 &-& - &-& -0.28 & 62.5 & 38.8 \\
262.3 & \verb|SXS:BBH:0142| & 1.91 & -0.291 & -0.230 & -0.052 & 0.004 & 0.001 & 0.110 & 0.00 & 76.1 & 13.5 \\
262.3 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 75.7 & 29.3 \\
262.2 & \verb|S0_D9.87_q2.00_a0.20_-0.80_n100| & 2.001 &-&-& 0.200 & -0.015 & -0.007 & -0.800 & -0.13 & 74.9 & 27.2 \\
262.2 & \verb|D12.50_q0.50_a-0.50_-0.10_n100|(*) & 2.0 &-&-& -0.100 &-&-& -0.500 & -0.23 & 67.3 & 21.0 \\
262.2 & \verb|GT:BBH:420| & 1.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.7 & 19.3 \\
262.1 & \verb|SXS:BBH:0005| & 1.0 &-&-& 0.499 & - & - &-& 0.25 & 81.9 & 10.5 \\
262.1 & \verb|RIT:BBH:NQ50TH90PH150| & 2.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 75.8 & 17.9 \\
262.0 & \verb|SXS:BBH:0145| & 1.96 & 0.017 & 0.029 & -0.049 & 0.091 & -0.002 & 0.027 & -0.02 & 75.1 & 13.4 \\
262.0 & \verb|D10_q0.50_a-0.8_xi0_n100|(*) & 2.0 & 0.696 & 0.059 & 0.392 &-& -0.006 & -0.801 & -0.01 & 77.7 & 24.6 \\
261.9 & \verb|(0.0,2.0,'M180','D11')| & 2.0 &-&-&-&-&-&-& 0.00 & 75.8 & 22.1 \\
261.9 & \verb|RIT:BBH:NTH135PH90| & 1.005 & -0.579 & -0.025 & -0.572 & - &-& - & -0.29 & 60.4 & 39.7 \\
261.9 & \verb|SXS:BBH:0139| & 1.82 & 0.032 & -0.342 & 0.210 & -0.132 & -0.047 & -0.042 & 0.12 & 79.7 & 12.7 \\
261.8 & \verb|SXS:BBH:0101| & 1.501 &-& - & -0.500 & - & - &-& -0.30 & 66.1 & 17.4 \\
261.8 & \verb|SXS:BBH:0144| & 1.94 & 0.061 & 0.104 & -0.288 & -0.050 & -0.022 & 0.215 & -0.12 & 72.0 & 13.8 \\
261.7 & \verb|GT:BBH:615| & 1.7 &-&-&-&-&-&-& 0.00 & 75.7 & 30.2 \\
261.4 & \verb|RIT:BBH:NTH60PH30| & 1.005 & -0.426 & 0.555 & 0.420 & - &-& - & 0.21 & 76.3 & 37.4 \\
261.2 & \verb|RIT:BBH:NTH135PH150| & 1.005 & -0.259 & -0.498 & -0.590 & - & - &-& -0.30 & 63.8 & 38.2 \\
261.0 & \verb|D11_q0.75_a0.0_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& - & -0.29 & 66.2 & 25.8 \\
260.9 & \verb|D11_q0.50_a0.0_0.0_n100|(*) & 2.0 &-&-& - &-&-& - & -0.00 & 76.4 & 21.5 \\
260.9 & \verb|RIT:BBH:NQ50TH90PH120| & 2.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 74.7 & 17.0 \\
260.8 & \verb|GT:BBH:564| & 1.0 &-&-& -0.400 &-&-& -0.400 & -0.40 & 64.1 & 26.4 \\
260.8 & \verb|RIT:BBH:NQ200TH90PH120| & 2 &-&-&-& -0.400 & 0.693 &-& 0.00 & 74.2 & 20.6 \\
260.8 & \verb|GT:BBH:405| & 1.25 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.2 & 22.8 \\
260.7 & \verb|D9_q1.9_a0.0_m160| & 1.9 &-&-& - &-&-& - & -0.00 & 74.3 & 30.7 \\
260.6 & \verb|RIT:BBH:NTH135PH30| & 1.005 & -0.343 & 0.468 & -0.571 & - & - & - & -0.29 & 62.2 & 39.6 \\
260.6 & \verb|RIT:BBH:NQ200TH90PH30| & 2 &-&-&-& 0.693 & 0.400 &-& 0.00 & 76.0 & 21.0 \\
260.4 & \verb|SXS:BBH:0141| & 1.84 & -0.182 & 0.052 & 0.086 & -0.093 & 0.124 & 0.040 & 0.07 & 79.4 & 12.8 \\
260.4 & \verb|SXS:BBH:0122| & 1.17 & -0.019 & 0.061 & -0.477 & 0.041 & 0.050 & -0.364 & -0.42 & 61.1 & 17.5 \\
260.4 & \verb|RIT:BBH:NQ200TH90PH0| & 2 &-&-&-& 0.800 &-&-& 0.00 & 74.3 & 20.7 \\
260.3 & \verb|RIT:BBH:NTH45PH0| & 1.005 & -0.034 & 0.568 & 0.584 &-& - & - & 0.29 & 80.3 & 35.7 \\
260.2 & \verb|RIT:BBH:NTH45PH40| & 1.005 & -0.417 & 0.401 & 0.575 &-& - & - & 0.29 & 81.3 & 35.0 \\
260.2 & \verb|RIT:BBH:NQ66TH60PH150| & 1.5 & -0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 82.3 & 31.7 \\
260.2 & \verb|GT:BBH:897| & 2.0 & 0.500 & -0.324 & -0.070 & -0.188 & -0.556 & 0.122 & -0.01 & 73.8 & 29.2 \\
260.1 & \verb|SXS:BBH:0128| & 1.35 & 0.041 & 0.005 & 0.134 & -0.048 & 0.103 & 0.397 & 0.25 & 82.9 & 12.7 \\
260.1 & \verb|RIT:BBH:NQ200TH90PH90| & 2 &-&-&-&-& 0.800 &-& 0.00 & 74.3 & 22.1 \\
260.1 & \verb|RIT:BBH:NQ200TH90PH60| & 2 &-&-&-& 0.400 & 0.693 &-& 0.00 & 76.3 & 22.1 \\
260.0 & \verb|RIT:BBH:NTH45PH30| & 1.005 & -0.341 & 0.464 & 0.578 &-& - & - & 0.29 & 79.5 & 35.8 \\
260.0 & \verb|RIT:BBH:NQ66TH60PH120| & 1.5 & -0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 81.7 & 31.0 \\
259.9 & \verb|RIT:BBH:NTH45PH50| & 1.005 & -0.485 & 0.328 & 0.568 & - &-&-& 0.28 & 79.5 & 35.9 \\
259.9 & \verb|SXS:BBH:0022| & 1.5 & 0.497 & 0.049 & - & 0.001 & -0.001 & 0.499 & 0.20 & 79.9 & 12.3 \\
259.8 & \verb|D11_q0.50_a0.50_-0.50_n100|(*) & 2.0 &-&-& -0.500 &-&-& 0.500 & -0.17 & 69.2 & 24.8 \\
259.7 & \verb|RIT:BBH:NTH45PH10| & 1.005 & -0.153 & 0.539 & 0.593 &-& - & - & 0.30 & 79.4 & 36.0 \\
259.7 & \verb|RIT:BBH:NQ200TH60PH120| & 2 &-&-&-& -0.346 & 0.600 & 0.400 & 0.13 & 75.9 & 34.3 \\
259.7 & \verb|GT:BBH:618| & 1.8 &-&-&-&-&-&-& 0.00 & 75.8 & 29.2 \\
259.6 & \verb|RIT:BBH:NQ200TH90PH150| & 2 &-&-&-& -0.693 & 0.400 &-& 0.00 & 74.7 & 18.7 \\
259.6 & \verb|GT:BBH:378| & 2.05 &-&-&-&-&-&-& 0.00 & 77.0 & 24.8 \\
259.6 & \verb|(0.0,1.9,'M160','D9')| & 1.9 &-&-&-&-&-&-& 0.00 & 74.6 & 29.5 \\
259.6 & \verb|SXS:BBH:0118| & 1.12 & -0.010 & 0.030 & 0.343 & -0.190 & -0.146 & 0.258 & 0.30 & 83.7 & 12.6 \\
259.5 & \verb|RIT:BBH:NTH135PH0| & 1.005 & -0.034 & 0.576 & -0.574 &-&-&-& -0.29 & 62.4 & 40.6 \\
259.4 & \verb|RIT:BBH:NTH45PH1275| & 1.005 & -0.458 & -0.351 & 0.577 & - & - &-& 0.29 & 79.2 & 37.2 \\
259.4 & \verb|D11_q1.00_a0.0_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& - & -0.40 & 60.9 & 28.9 \\
259.3 & \verb|GT:BBH:894| & 2.0 & -0.500 & 0.324 & -0.070 & 0.188 & 0.556 & 0.122 & -0.01 & 72.6 & 30.9 \\
259.3 & \verb|RIT:BBH:NQ50TH90PH0| & 2.0 & 0.800 &-&-&-&-&-& 0.00 & 79.3 & 14.7 \\
259.3 & \verb|GT:BBH:895| & 2.0 & 0.511 & -0.009 & 0.314 & 0.565 & 0.025 & -0.200 & 0.14 & 81.5 & 28.3 \\
259.2 & \verb|RIT:BBH:A7TH120PH0| & 1.0 & -0.055 & 0.621 & -0.362 &-& -0.625 & -0.361 & -0.36 & 61.2 & 21.1 \\
259.2 & \verb|D11_q0.75_a-0.5_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& -0.500 & 0.24 & 86.2 & 19.0 \\
259.2 & \verb|RIT:BBH:NQ50TH90PH30| & 2.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 75.7 & 15.5 \\
259.2 & \verb|RIT:BBH:NTH45PH45| & 1.005 & -0.453 & 0.365 & 0.572 &-& - & - & 0.29 & 82.5 & 34.6 \\
259.1 & \verb|GT:BBH:847| & 1.5 & 0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 80.6 & 29.1 \\
259.1 & \verb|RIT:BBH:NTH45PH120| & 1.005 & -0.500 & -0.289 & 0.577 &-& - & - & 0.29 & 80.9 & 36.3 \\
259.1 & \verb|GT:BBH:848| & 1.5 & 0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 80.7 & 25.4 \\
259.0 & \verb|GT:BBH:867| & 1.0 & 0.599 & 0.030 & - & -0.599 & -0.030 & - & 0.00 & 69.4 & 41.6 \\
258.9 & \verb|D11_q0.75_a-0.8_0.0_n100|(*) & 1.334 &-&-&-&-&-& -0.801 & -0.34 & 66.0 & 26.4 \\
258.9 & \verb|RIT:BBH:NQ50TH90PH60| & 2.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 76.1 & 15.1 \\
258.9 & \verb|RIT:BBH:A7TH120PH90| & 1.0 & -0.629 & -0.027 & -0.353 & 0.625 &-& -0.361 & -0.36 & 61.1 & 24.3 \\
258.9 & \verb|GT:BBH:871| & 1.5 & -0.600 &-&-& -0.424 &-& 0.424 & 0.17 & 79.0 & 24.7 \\
258.9 & \verb|SXS:BBH:0164| & 1.0 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.33 & 85.1 & 12.3 \\
258.9 & \verb|RIT:BBH:NTH45PH20| & 1.005 & -0.251 & 0.511 & 0.584 &-& - & - & 0.29 & 79.2 & 36.0 \\
258.8 & \verb|RIT:BBH:A7TH120PH210| & 1.0 & 0.361 & -0.512 & -0.358 & -0.312 & 0.541 & -0.361 & -0.36 & 61.7 & 28.6 \\
258.7 & \verb|Del0_D10.01_q2.00_a-0.4_-0.8_n100| & 2.001 &-&-& -0.400 & -0.011 & 0.003 & -0.800 & -0.53 & 59.5 & 36.3 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH30| & 2 &-&-&-& 0.600 & 0.346 & 0.400 & 0.13 & 77.5 & 34.2 \\
258.6 & \verb|RIT:BBH:N9TH55PH150| & 1.012 & -0.373 & -0.646 & 0.523 &-&-& - & 0.26 & 82.1 & 32.4 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH90| & 2 &-&-&-&-& 0.693 & 0.400 & 0.13 & 74.6 & 34.6 \\
258.6 & \verb|RIT:BBH:NQ200TH60PH60| & 2 &-&-&-& 0.346 & 0.600 & 0.400 & 0.13 & 77.1 & 33.6 \\
258.6 & \verb|RIT:BBH:NTH45PH60| & 1.005 & -0.536 & 0.241 & 0.566 & - &-&-& 0.28 & 79.2 & 36.0 \\
258.5 & \verb|RIT:BBH:A7TH120PH130| & 1.0 & -0.478 & -0.401 & -0.361 & 0.478 & 0.401 & -0.361 & -0.36 & 61.2 & 24.1 \\
258.5 & \verb|RIT:BBH:A7TH120PH315| & 1.0 & 0.442 & 0.442 & -0.361 & -0.442 & -0.442 & -0.361 & -0.36 & 61.2 & 23.3 \\
258.4 & \verb|RIT:BBH:NTH45PH75| & 1.005 & -0.582 & 0.097 & 0.564 &-& - & - & 0.28 & 82.5 & 34.7 \\
258.4 & \verb|RIT:BBH:NTH45PH150| & 1.005 & -0.289 & -0.500 & 0.577 &-&-&-& 0.29 & 79.5 & 36.9 \\
258.3 & \verb|RIT:BBH:NTH45PH90| & 1.005 & -0.590 & -0.050 & 0.562 &-& - & - & 0.28 & 82.5 & 34.9 \\
258.2 & \verb|SXS:BBH:0011| & 1.501 & 0.248 & 0.026 & 0.433 &-&-&-& 0.26 & 86.2 & 10.9 \\
258.2 & \verb|RIT:BBH:NTH45PH975| & 1.005 & -0.580 & -0.104 & 0.565 & - & - &-& 0.28 & 82.5 & 35.1 \\
258.2 & \verb|RIT:BBH:NQ50TH90PH90| & 2.0 &-& 0.800 &-&-&-&-& 0.00 & 74.7 & 16.4 \\
258.1 & \verb|RIT:BBH:N9TH55PH0| & 1.012 & -0.062 & 0.725 & 0.549 & - &-& - & 0.28 & 84.1 & 30.9 \\
258.1 & \verb|RIT:BBH:N9TH55PH30| & 1.012 & -0.432 & 0.609 & 0.522 & - &-& - & 0.26 & 80.8 & 32.4 \\
258.1 & \verb|RIT:BBH:N9TH55PH60| & 1.012 & -0.686 & 0.321 & 0.507 & - &-& - & 0.25 & 84.2 & 31.4 \\
258.1 & \verb|RIT:BBH:NTH45PH1125| & 1.005 & -0.531 & -0.251 & 0.566 &-&-& - & 0.28 & 78.5 & 37.1 \\
258.1 & \verb|SXS:BBH:0148| & 1.0 &-&-& -0.438 & - & - & -0.438 & -0.44 & 62.3 & 16.4 \\
257.9 & \verb|(0.2,1.5,'M100')| & 1.5 &-&-& 0.200 &-&-& 0.200 & 0.20 & 83.6 & 22.1 \\
257.9 & \verb|GT:BBH:413| & 1.75 &-&-& 0.200 &-&-& 0.200 & 0.20 & 81.3 & 23.3 \\
257.8 & \verb|RIT:BBH:NQ200TH60PH150| & 2 &-&-&-& -0.600 & 0.346 & 0.400 & 0.13 & 74.7 & 35.7 \\
257.7 & \verb|RIT:BBH:A7TH120PH30| & 1.0 & -0.361 & 0.515 & -0.352 & 0.312 & -0.541 & -0.361 & -0.36 & 61.2 & 21.8 \\
257.7 & \verb|RIT:BBH:NQ66TH60PH90| & 1.5 &-& 0.693 & 0.400 &-&-&-& 0.24 & 81.0 & 30.5 \\
257.6 & \verb|RIT:BBH:NQ200TH60PH0| & 2 &-&-&-& 0.693 &-& 0.400 & 0.13 & 77.5 & 35.0 \\
257.5 & \verb|GT:BBH:858| & 1.5 & -0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.17 & 77.7 & 26.2 \\
257.5 & \verb|GT:BBH:864| & 1.0 & -0.269 & -0.536 & -0.014 & -0.269 & -0.536 & -0.014 & -0.01 & 73.2 & 41.0 \\
257.5 & \verb|GT:BBH:859| & 2.0 & -0.106 &-& -0.106 & 0.424 &-& 0.424 & 0.07 & 74.3 & 28.3 \\
257.4 & \verb|GT:BBH:872| & 2.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.14 & 80.2 & 24.8 \\
257.4 & \verb|RIT:BBH:N9TH55PH90| & 1.012 & -0.759 & -0.029 & 0.505 &-& - & - & 0.25 & 84.1 & 31.7 \\
257.2 & \verb|GT:BBH:860| & 1.0 & 0.109 & 0.481 & 0.342 & 0.460 & -0.287 & 0.257 & 0.30 & 81.9 & 32.9 \\
257.1 & \verb|D11_q0.75_a0.0_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& - & 0.29 & 86.2 & 18.8 \\
257.0 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 76.7 & 28.6 \\
256.7 & \verb|RIT:BBH:NQ50TH135PH90| & 2.0 &-& 0.566 & -0.566 &-&-&-& -0.38 & 67.0 & 21.4 \\
256.6 & \verb|GT:BBH:896| & 2.0 & -0.511 & 0.009 & 0.314 & -0.565 & -0.025 & -0.200 & 0.14 & 83.5 & 24.9 \\
256.5 & \verb|RIT:BBH:NTH165PH0| & 1.005 & -0.009 & 0.195 & -0.790 & - & - & - & -0.40 & 62.5 & 38.6 \\
256.5 & \verb|RIT:BBH:NQ50TH135PH0| & 2.0 & 0.566 &-& -0.566 &-&-&-& -0.38 & 62.6 & 24.0 \\
256.5 & \verb|EMu0_D8.98_q1.00_a0.6_n100| & 1.0 &-&-& 0.600 &-&-& - & 0.30 & 83.2 & 27.4 \\
256.4 & \verb|RIT:BBH:NTH165PH30| & 1.005 & -0.103 & 0.188 & -0.785 & - &-& - & -0.39 & 60.7 & 39.2 \\
256.4 & \verb|RIT:BBH:NTH165PH90| & 1.005 & -0.211 &-& -0.786 & - &-& - & -0.39 & 60.7 & 38.8 \\
256.2 & \verb|S0_D9.75_q2.00_a-0.20_0.80_n100| & 2.001 &-&-& -0.200 & 0.015 & -0.006 & 0.800 & 0.13 & 77.6 & 25.9 \\
256.1 & \verb|GT:BBH:870| & 1.5 &-& 0.600 &-& -0.424 &-& 0.424 & 0.17 & 79.0 & 26.3 \\
256.1 & \verb|RIT:BBH:NTH165PH150| & 1.005 & -0.105 & -0.182 & -0.786 & - & - & - & -0.39 & 62.4 & 37.9 \\
256.0 & \verb|RIT:BBH:NTH30PH30| & 1.005 & -0.232 & 0.338 & 0.706 &-& - & - & 0.35 & 84.0 & 34.1 \\
256.0 & \verb|D9_q2.2_a0.0_m160| & 2.2 &-&-& - &-&-& - & -0.00 & 76.9 & 29.5 \\
255.9 & \verb|RIT:BBH:NTH165PH120| & 1.005 & -0.187 & -0.098 & -0.786 & - &-& - & -0.39 & 62.5 & 37.6 \\
255.8 & \verb|GT:BBH:548| & 1.0 &-&-&-&-&-& 0.600 & 0.30 & 84.1 & 19.0 \\
255.8 & \verb|RIT:BBH:A7TH60PH10| & 1.0 & -0.161 & 0.600 & 0.373 & 0.137 & -0.612 & 0.364 & 0.37 & 81.5 & 33.3 \\
255.7 & \verb|GT:BBH:549| & 1.0 &-&-& 0.200 &-&-& 0.400 & 0.30 & 84.4 & 19.2 \\
255.7 & \verb|D11_q0.75_a0.4_0.8_PNr500_th1d_n100|(*) & 1.333 & -0.597 & -0.231 & 0.481 & -0.346 & 0.200 & 0.003 & 0.28 & 84.3 & 19.0 \\
255.7 & \verb|RIT:BBH:NQ66TH60PH30| & 1.5 & 0.600 & 0.346 & 0.400 &-&-&-& 0.24 & 78.6 & 32.8 \\
255.7 & \verb|RIT:BBH:NTH30PH0| & 1.005 & -0.033 & 0.386 & 0.718 &-& - & - & 0.36 & 86.0 & 33.4 \\
255.6 & \verb|RIT:BBH:NQ50TH135PH60| & 2.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 66.9 & 25.8 \\
255.5 & \verb|RIT:BBH:A7TH60PH40| & 1.0 & -0.445 & 0.444 & 0.362 & 0.404 & -0.481 & 0.362 & 0.36 & 85.9 & 31.3 \\
255.5 & \verb|D10_q0.50_a-0.50_0.50_n100|(*) & 2.0 &-&-& 0.500 &-&-& -0.500 & 0.17 & 82.9 & 22.1 \\
255.5 & \verb|RIT:BBH:A7TH135PH0| & 1.0 & -0.028 & 0.512 & -0.506 &-& -0.510 & -0.510 & -0.51 & 60.4 & 16.7 \\
255.5 & \verb|RIT:BBH:NTH30PH60| & 1.005 & -0.378 & 0.185 & 0.700 & - &-& - & 0.35 & 83.7 & 34.4 \\
255.4 & \verb|GT:BBH:890| & 2.0 &-&-& 0.600 &-&-& -0.600 & 0.20 & 86.1 & 24.1 \\
255.4 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 77.4 & 29.2 \\
255.4 & \verb|RIT:BBH:NQ66TH60PH60| & 1.5 & 0.346 & 0.600 & 0.400 &-&-&-& 0.24 & 83.7 & 29.8 \\
255.4 & \verb|RIT:BBH:NQ50TH135PH30| & 2.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 62.1 & 28.0 \\
255.3 & \verb|D10_q0.50_a0.8_xi0_n100|(*) & 2.0 & 0.689 & 0.062 & -0.403 & 0.012 & 0.006 & 0.800 & -0.00 & 71.2 & 27.0 \\
255.3 & \verb|SXS:BBH:0191| & 2.507 & - &-& - &-&-&-& -0.00 & 76.6 & 12.9 \\
255.3 & \verb|GT:BBH:380| & 2.35 &-&-&-&-&-&-& 0.00 & 77.8 & 24.6 \\
255.3 & \verb|RIT:BBH:NQ50TH135PH150| & 2.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.38 & 61.0 & 21.1 \\
255.2 & \verb|RIT:BBH:NTH30PH90| & 1.005 & -0.423 & -0.024 & 0.698 &-&-& - & 0.35 & 82.5 & 35.2 \\
255.1 & \verb|d0_D10.50_q2.00_a-0.5_n100| & 2.0 &-&-& -0.500 &-&-& - & -0.33 & 62.7 & 29.7 \\
255.1 & \verb|(0.0,2.2,'M160','D9')| & 2.2 &-&-&-&-&-&-& 0.00 & 75.6 & 28.9 \\
255.0 & \verb|RIT:BBH:NQ33TH135PH150| & 3 & -0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 58.4 & 39.1 \\
254.8 & \verb|RIT:BBH:NQ50TH135PH120| & 2.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.38 & 66.5 & 18.7 \\
254.7 & \verb|RIT:BBH:NTH165PH60| & 1.005 & -0.182 & 0.105 & -0.786 &-& - &-& -0.39 & 62.6 & 37.8 \\
254.6 & \verb|(0.2,2.0,'M100')| & 2.0 &-&-& 0.200 &-&-& 0.200 & 0.20 & 82.7 & 23.1 \\
254.5 & \verb|SXS:BBH:0028| & 1.501 & -0.001 & 0.001 & 0.500 & 0.078 & -0.489 & 0.001 & 0.30 & 88.1 & 10.8 \\
254.5 & \verb|SXS:BBH:0136| & 1.68 & 0.118 & -0.114 & 0.326 & -0.145 & -0.071 & 0.145 & 0.26 & 84.8 & 11.7 \\
254.4 & \verb|RIT:BBH:NQ33TH135PH60| & 3 & 0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 62.6 & 36.7 \\
254.3 & \verb|RIT:BBH:NTH30PH120| & 1.005 & -0.353 & -0.204 & 0.707 & - &-& - & 0.35 & 84.6 & 34.7 \\
254.1 & \verb|DD_D10.99_q2.00_a-0.8_n100| & 2.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 52.1 & 36.3 \\
254.0 & \verb|GT:BBH:617| & 2.1 &-&-&-&-&-&-& 0.00 & 78.4 & 29.0 \\
254.0 & \verb|SXS:BBH:0009| & 1.501 & - &-& 0.500 & - & - &-& 0.30 & 86.6 & 13.4 \\
253.9 & \verb|RIT:BBH:A7TH60PH315| & 1.0 & 0.424 & 0.464 & 0.361 & -0.444 & -0.444 & 0.363 & 0.36 & 84.6 & 31.5 \\
253.8 & \verb|RIT:BBH:A7TH60PH0| & 1.0 & -0.053 & 0.616 & 0.379 & 0.028 & -0.624 & 0.368 & 0.37 & 85.1 & 31.3 \\
253.7 & \verb|RIT:BBH:A7TH135PH210| & 1.0 & 0.281 & -0.431 & -0.505 & -0.255 & 0.441 & -0.510 & -0.51 & 57.7 & 27.4 \\
253.6 & \verb|RIT:BBH:A7TH60PH80| & 1.0 & -0.632 & 0.058 & 0.351 & 0.618 & -0.109 & 0.363 & 0.36 & 84.1 & 32.7 \\
253.6 & \verb|RIT:BBH:NQ33TH135PH30| & 3 & 0.490 & 0.283 & -0.566 &-&-&-& -0.42 & 61.3 & 36.3 \\
253.5 & \verb|RIT:BBH:A7TH135PH315| & 1.0 & 0.360 & 0.360 & -0.510 & -0.360 & -0.360 & -0.510 & -0.51 & 61.2 & 18.5 \\
253.5 & \verb|RIT:BBH:LPH120| & 1.0 & -0.703 & -0.422 & -0.009 & 0.016 & 0.006 & 0.820 & 0.41 & 89.0 & 28.5 \\
253.4 & \verb|RIT:BBH:NQ66TH60PH0| & 1.5 & 0.693 &-& 0.400 &-&-&-& 0.24 & 79.2 & 33.0 \\
253.1 & \verb|RIT:BBH:NQ33TH135PH90| & 3 &-& 0.566 & -0.566 &-&-&-& -0.42 & 64.5 & 34.3 \\
253.0 & \verb|GT:BBH:565| & 2.5 &-&-&-&-&-&-& 0.00 & 78.2 & 20.8 \\
252.9 & \verb|RIT:BBH:NTH30PH150| & 1.005 & -0.204 & -0.353 & 0.707 & - &-& - & 0.35 & 84.8 & 34.7 \\
252.9 & \verb|RIT:BBH:LPH150| & 1.0 & -0.385 & -0.724 & 0.002 & 0.012 & 0.003 & 0.820 & 0.41 & 87.2 & 29.3 \\
252.9 & \verb|D11_q0.75_a0.8_0.0_n100|(*) & 1.334 &-&-& - &-&-& 0.801 & 0.34 & 88.1 & 18.4 \\
252.8 & \verb|GT:BBH:636| & 3.0 & -0.500 & 0.019 & -0.001 &-&-&-& -0.00 & 75.7 & 33.7 \\
252.7 & \verb|GT:BBH:621| & 2.3 &-&-&-&-&-&-& 0.00 & 74.9 & 29.0 \\
252.6 & \verb|GT:BBH:609| & 3.0 & -0.335 & -0.317 & -0.192 &-&-&-& -0.14 & 66.9 & 40.6 \\
252.6 & \verb|RIT:BBH:NQ200TH30PH60| & 2 &-&-&-& 0.200 & 0.346 & 0.693 & 0.23 & 80.8 & 32.5 \\
252.5 & \verb|RIT:BBH:NQ200TH30PH150| & 2 &-&-&-& -0.346 & 0.200 & 0.693 & 0.23 & 79.2 & 32.9 \\
252.5 & \verb|RIT:BBH:NQ33TH100PH30| & 3 & 0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 73.5 & 25.7 \\
252.4 & \verb|RIT:BBH:NQ200TH30PH90| & 2 &-&-&-&-& 0.400 & 0.693 & 0.23 & 78.1 & 33.2 \\
252.4 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 76.9 & 29.2 \\
252.4 & \verb|RIT:BBH:A7TH135PH30| & 1.0 & -0.281 & 0.434 & -0.502 & 0.255 & -0.441 & -0.510 & -0.51 & 61.2 & 17.0 \\
252.3 & \verb|RIT:BBH:A7TH60PH30| & 1.0 & -0.376 & 0.493 & 0.376 & 0.339 & -0.532 & 0.356 & 0.37 & 87.7 & 29.8 \\
252.2 & \verb|RIT:BBH:NQ33TH100PH60| & 3 & 0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 73.0 & 27.6 \\
252.0 & \verb|RIT:BBH:NQ200TH30PH120| & 2 &-&-&-& -0.200 & 0.346 & 0.693 & 0.23 & 77.9 & 33.3 \\
252.0 & \verb|RIT:BBH:NQ200TH30PH30| & 2 &-&-&-& 0.346 & 0.200 & 0.693 & 0.23 & 78.0 & 34.1 \\
251.9 & \verb|RIT:BBH:NQ33TH135PH0| & 3 & 0.566 &-& -0.566 &-&-&-& -0.42 & 60.6 & 36.5 \\
251.9 & \verb|RIT:BBH:A7TH135PH90| & 1.0 & -0.510 &-& -0.510 & 0.510 &-& -0.510 & -0.51 & 61.2 & 21.8 \\
251.8 & \verb|RIT:BBH:NQ33TH100PH0| & 3 & 0.788 &-& -0.139 &-&-&-& -0.10 & 76.6 & 23.5 \\
251.8 & \verb|RIT:BBH:NQ200TH30PH0| & 2 &-&-&-& 0.400 &-& 0.693 & 0.23 & 78.5 & 34.4 \\
251.8 & \verb|RIT:BBH:NQ33TH100PH90| & 3 &-& 0.788 & -0.139 &-&-&-& -0.10 & 75.8 & 26.6 \\
251.8 & \verb|RIT:BBH:NTH15PH30| & 1.005 & -0.106 & 0.183 & 0.789 &-& - & - & 0.40 & 88.1 & 32.9 \\
251.5 & \verb|RIT:BBH:A7TH60PH130| & 1.0 & -0.467 & -0.427 & 0.354 & 0.481 & 0.404 & 0.363 & 0.36 & 84.8 & 33.3 \\
251.5 & \verb|RIT:BBH:A7TH135PH130| & 1.0 & -0.390 & -0.328 & -0.510 & 0.390 & 0.328 & -0.510 & -0.51 & 57.9 & 27.5 \\
251.5 & \verb|RIT:BBH:NTH15PH60| & 1.005 & -0.185 & 0.106 & 0.788 &-&-& - & 0.40 & 87.3 & 33.3 \\
251.4 & \verb|GT:BBH:622| & 2.4 &-&-&-&-&-&-& 0.00 & 79.2 & 27.3 \\
251.4 & \verb|RIT:BBH:A7TH60PH110| & 1.0 & -0.587 & -0.241 & 0.351 & 0.590 & 0.215 & 0.363 & 0.36 & 87.4 & 32.5 \\
251.3 & \verb|RIT:BBH:NTH15PH0| & 1.005 & -0.005 & 0.215 & 0.788 &-& - & - & 0.39 & 85.8 & 33.7 \\
251.2 & \verb|RIT:BBH:NQ33TH135PH120| & 3 & -0.283 & 0.490 & -0.566 &-&-&-& -0.42 & 58.8 & 38.1 \\
251.2 & \verb|RIT:BBH:A7TH60PH210| & 1.0 & 0.361 & -0.514 & 0.362 & -0.314 & 0.544 & 0.362 & 0.36 & 87.5 & 30.0 \\
251.0 & \verb|D12.00_q0.50_a0.50_0.10_n100|(*) & 2.0 &-&-& 0.100 &-&-& 0.500 & 0.23 & 81.4 & 18.0 \\
251.0 & \verb|RIT:BBH:NQ33TH100PH120| & 3 & -0.394 & 0.682 & -0.139 &-&-&-& -0.10 & 71.9 & 28.3 \\
251.0 & \verb|RIT:BBH:NTH15PH90| & 1.005 & -0.223 & -0.003 & 0.785 &-&-&-& 0.39 & 87.9 & 33.4 \\
250.9 & \verb|SXS:BBH:0052| & 3.0 & 0.494 & 0.073 & 0.001 & 0.001 & 0.008 & -0.499 & -0.12 & 76.3 & 15.0 \\
250.9 & \verb|DU_D10.90_q2.00_a-0.8_rl10_opt1_n100| & 2.0 &-&-& -0.801 & - & -0.004 & 0.801 & -0.27 & 67.0 & 26.5 \\
250.8 & \verb|RIT:BBH:LPH90| & 1.0 & -0.819 & -0.038 & -0.009 & 0.016 &-& 0.820 & 0.41 & 86.5 & 29.3 \\
250.8 & \verb|GT:BBH:724| & 3.0 & -0.464 & 0.182 & 0.046 &-&-&-& 0.03 & 77.1 & 33.2 \\
250.8 & \verb|GT:BBH:743| & 3.0 & 0.267 & -0.412 & -0.094 &-&-&-& -0.07 & 63.9 & 42.1 \\
250.7 & \verb|RIT:BBH:LPH30| & 1.0 & -0.476 & 0.668 & 0.011 & 0.011 & 0.004 & 0.820 & 0.42 & 86.7 & 29.8 \\
250.7 & \verb|GT:BBH:878| & 2.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.16 & 84.0 & 23.5 \\
250.7 & \verb|RIT:BBH:NQ50TH60PH90| & 2.0 &-& 0.693 & 0.400 &-&-&-& 0.27 & 88.9 & 27.8 \\
250.4 & \verb|GT:BBH:605| & 3.0 & 0.464 & -0.182 & 0.046 &-&-&-& 0.03 & 77.7 & 31.2 \\
250.4 & \verb|RIT:BBH:NTH15PH120| & 1.005 & -0.183 & -0.106 & 0.789 & - & - & - & 0.40 & 84.4 & 34.8 \\
250.3 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 78.3 & 28.5 \\
250.3 & \verb|GT:BBH:651| & 2.6 &-&-&-&-&-&-& 0.00 & 76.9 & 28.0 \\
250.3 & \verb|SXS:BBH:0151| & 1.0 &-& - & -0.600 & - &-& -0.600 & -0.60 & 56.6 & 17.9 \\
250.1 & \verb|RIT:BBH:NQ50TH60PH120| & 2.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 88.9 & 27.9 \\
249.9 & \verb|SXS:BBH:0143| & 1.92 & -0.094 & -0.062 & 0.436 & -0.019 & -0.434 & -0.085 & 0.26 & 86.2 & 11.1 \\
249.9 & \verb|D11_q1.00_a-0.8_-0.8_n100|(*) & 1.0 &-&-& -0.801 &-&-& -0.801 & -0.80 & 50.0 & 38.0 \\
249.8 & \verb|SXS:BBH:0044| & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.00 & 80.3 & 17.6 \\
249.8 & \verb|RIT:BBH:NQ25TH135PH150| & 4.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 58.0 & 41.2 \\
249.8 & \verb|RIT:BBH:NQ50TH60PH30| & 2.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 86.7 & 28.5 \\
249.8 & \verb|RIT:BBH:NQ50TH60PH60| & 2.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.27 & 85.7 & 28.7 \\
249.8 & \verb|GT:BBH:881| & 2.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.18 & 87.3 & 23.3 \\
249.8 & \verb|SXS:BBH:0035| & 3.001 & 0.499 & 0.029 & - &-& - &-& -0.00 & 77.9 & 11.6 \\
249.7 & \verb|D11_q0.75_a-0.5_-0.5_n100|(*) & 1.333 &-&-& -0.500 &-&-& -0.500 & -0.50 & 57.9 & 30.6 \\
249.5 & \verb|RIT:BBH:LPH0| & 1.0 & -0.064 & 0.817 & 0.013 & - & -0.010 & 0.820 & 0.42 & 81.9 & 32.0 \\
249.5 & \verb|D11_q1.00_a-0.5_-0.5_n100|(*) & 1.0 &-&-& -0.500 &-&-& -0.500 & -0.50 & 57.9 & 30.6 \\
249.5 & \verb|GT:BBH:657| & 3.0 & -0.201 & 0.405 & 0.213 &-&-&-& 0.16 & 79.0 & 34.1 \\
249.4 & \verb|RIT:BBH:NQ50TH60PH0| & 2.0 & 0.693 &-& 0.400 &-&-&-& 0.27 & 88.2 & 28.7 \\
249.3 & \verb|GT:BBH:680| & 3.0 & 0.500 & -0.019 & -0.001 &-&-&-& -0.00 & 78.9 & 32.1 \\
249.3 & \verb|SXS:BBH:0042| & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.32 & 66.8 & 21.5 \\
249.2 & \verb|RIT:BBH:LPH60| & 1.0 & -0.746 & 0.341 & -0.002 & 0.016 & -0.002 & 0.820 & 0.41 & 86.0 & 29.6 \\
249.1 & \verb|RIT:BBH:NTH15PH150| & 1.005 & -0.106 & -0.183 & 0.789 & - &-& - & 0.40 & 85.7 & 34.3 \\
249.0 & \verb|RIT:BBH:A7TH60PH90| & 1.0 & -0.632 & -0.052 & 0.351 & 0.628 &-& 0.363 & 0.36 & 85.7 & 31.6 \\
248.8 & \verb|GT:BBH:746| & 3.0 & -0.267 & 0.412 & -0.094 &-&-&-& -0.07 & 64.7 & 42.6 \\
248.8 & \verb|SXS:BBH:0020| & 1.5 &-& - & 0.500 & 0.494 & 0.071 & - & 0.30 & 88.1 & 11.0 \\
248.7 & \verb|D13_q1.00_a-0.80_-0.40_n100|(*) & 1.0 &-&-& -0.400 &-&-& -0.801 & -0.60 & 56.1 & 25.8 \\
248.6 & \verb|D11.25_q0.3333_a0.0_0.0_n100|(*) & 3.0 &-&-&-&-&-& - & 0.00 & 77.4 & 20.1 \\
248.5 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 77.2 & 27.7 \\
248.2 & \verb|SXS:BBH:0311|(*) & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.40 & 87.5 & 13.0 \\
248.2 & \verb|EMu0_D8.80_q1.00_a0.8_n100| & 1.0 &-&-& 0.801 &-&-& - & 0.40 & 91.2 & 25.7 \\
248.1 & \verb|Del0_D10.97_q1.3333_a-0.6_-0.8_n100| & 1.334 &-&-& -0.600 &-&-& -0.801 & -0.69 & 56.1 & 33.1 \\
248.1 & \verb|GT:BBH:635| & 3.0 & 0.201 & -0.405 & 0.213 &-&-&-& 0.16 & 78.2 & 33.5 \\
247.9 & \verb|GT:BBH:857| & 3.0 & 0.047 &-& 0.047 & -0.424 &-& -0.424 & -0.07 & 74.6 & 28.7 \\
247.9 & \verb|SXS:BBH:0037| & 3.001 & 0.498 & 0.038 &-&-& - &-& 0.00 & 80.3 & 12.0 \\
247.8 & \verb|SXS:BBH:0030| & 3.0 &-&-&-& - &-&-& 0.00 & 79.3 & 14.5 \\
247.6 & \verb|GT:BBH:406| & 1.25 &-&-& 0.400 &-&-& 0.400 & 0.40 & 89.7 & 20.8 \\
247.5 & \verb|RIT:BBH:NQ25TH135PH60| & 4.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 62.6 & 38.4 \\
247.5 & \verb|SXS:BBH:0032| & 3.001 & 0.248 & 0.037 & -0.432 &-& - &-& -0.32 & 64.3 & 17.8 \\
247.3 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 77.3 & 28.6 \\
247.2 & \verb|GT:BBH:650| & 2.7 &-&-&-&-&-&-& 0.00 & 77.9 & 28.5 \\
247.2 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 78.1 & 28.1 \\
247.2 & \verb|GT:BBH:747| & 3.0 & 0.335 & 0.317 & -0.192 &-&-&-& -0.14 & 65.0 & 40.9 \\
247.2 & \verb|RIT:BBH:NQ25TH135PH0| & 4.0 & 0.566 &-& -0.566 &-&-&-& -0.45 & 63.6 & 35.8 \\
247.1 & \verb|GT:BBH:422| & 1.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 90.1 & 17.6 \\
247.0 & \verb|SXS:BBH:0026| & 1.5 & - &-& 0.500 & -0.494 & -0.071 & - & 0.30 & 87.6 & 11.2 \\
247.0 & \verb|GT:BBH:554| & 1.0 &-&-& 0.200 &-&-& 0.600 & 0.40 & 90.0 & 17.7 \\
246.9 & \verb|D10_q0.33_a-0.8_xi0_n100|(*) & 2.999 & 0.757 & 0.030 & 0.259 &-&-& -0.800 & -0.01 & 83.3 & 22.7 \\
246.4 & \verb|GT:BBH:453| & 3.0 &-&-&-&-&-&-& 0.00 & 79.7 & 20.2 \\
246.3 & \verb|SXS:BBH:0053| & 3.0 & 0.494 & 0.075 & 0.001 & -0.464 & -0.184 & -0.003 & 0.00 & 77.6 & 14.9 \\
246.3 & \verb|SXS:BBH:0105| & 3.001 &-& - & -0.500 & - & - &-& -0.37 & 63.6 & 11.9 \\
246.2 & \verb|GT:BBH:726| & 3.0 & -0.197 & 0.385 & -0.251 &-&-&-& -0.19 & 61.8 & 45.5 \\
246.1 & \verb|GT:BBH:654| & 2.9 &-&-&-&-&-&-& 0.00 & 77.9 & 27.4 \\
246.1 & \verb|D11_q0.75_a0.0_-0.8_n100|(*) & 1.333 &-&-& -0.801 &-&-& - & -0.46 & 62.0 & 28.5 \\
246.0 & \verb|GT:BBH:653| & 2.8 &-&-&-&-&-&-& 0.00 & 80.6 & 26.5 \\
245.9 & \verb|GT:BBH:551| & 1.0 &-&-&-&-&-& 0.800 & 0.40 & 88.9 & 18.0 \\
245.9 & \verb|RIT:BBH:NQ25TH135PH90| & 4.0 &-& 0.566 & -0.566 &-&-&-& -0.45 & 61.3 & 36.9 \\
245.7 & \verb|RIT:BBH:NQ33TH100PH150| & 3 & -0.682 & 0.394 & -0.139 &-&-&-& -0.10 & 77.3 & 26.2 \\
245.7 & \verb|RIT:BBH:NQ33TH75PH30| & 3 & 0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 85.6 & 23.0 \\
245.6 & \verb|SXS:BBH:0034| & 3.001 & 0.497 & 0.047 & 0.001 &-& - &-& 0.00 & 80.3 & 14.2 \\
245.5 & \verb|RIT:BBH:NQ33TH75PH90| & 3 &-& 0.773 & 0.207 &-&-&-& 0.16 & 85.3 & 25.6 \\
245.4 & \verb|D13.00_q0.50_a0.00_-0.80_n100|(*) & 1.999 &-&-& -0.801 &-&-& - & -0.53 & 57.6 & 23.2 \\
245.4 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 79.2 & 27.5 \\
245.4 & \verb|D13.00_q0.50_a-0.50_-0.60_n100|(*) & 2.0 &-&-& -0.600 &-&-& -0.500 & -0.57 & 57.6 & 22.9 \\
245.3 & \verb|UD_D8.76_q2.00_a0.8_rl10_opt1_n100| & 2.0 &-&-& 0.801 &-&-& -0.801 & 0.27 & 92.0 & 26.1 \\
245.3 & \verb|RIT:BBH:NQ25TH135PH30| & 4.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.45 & 64.4 & 35.6 \\
244.9 & \verb|RIT:BBH:NQ33TH75PH60| & 3 & 0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 83.1 & 25.0 \\
244.9 & \verb|D10_q0.33_a0.8_xi0_n120|(*) & 2.999 & 0.754 & 0.031 & -0.268 &-&-& 0.800 & -0.00 & 78.9 & 24.0 \\
244.8 & \verb|SXS:BBH:0200| & 3.272 & - &-& - &-&-& - & -0.00 & 77.5 & 14.3 \\
244.6 & \verb|SXS:BBH:0050| & 3.0 & 0.494 & 0.072 & 0.002 & 0.467 & 0.176 & 0.005 & 0.00 & 81.9 & 13.7 \\
244.6 & \verb|SXS:BBH:0046| & 3.0 &-&-& -0.500 & - &-& -0.499 & -0.50 & 63.1 & 18.2 \\
244.4 & \verb|RIT:BBH:NQ33TH75PH0| & 3 & 0.773 &-& 0.207 &-&-&-& 0.16 & 83.9 & 23.6 \\
244.1 & \verb|RIT:BBH:NQ50TH60PH150| & 2.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.27 & 90.3 & 28.3 \\
244.1 & \verb|GT:BBH:882| & 2.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.20 & 85.2 & 24.2 \\
243.8 & \verb|GT:BBH:861| & 1.0 & -0.159 & -0.414 & -0.404 & 0.297 & 0.521 & -0.020 & -0.21 & 65.8 & 48.6 \\
243.7 & \verb|RIT:BBH:NQ25TH135PH120| & 4.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.45 & 57.8 & 40.2 \\
243.5 & \verb|(0.4,1.5,'M100')| & 1.5 &-&-& 0.400 &-&-& 0.400 & 0.40 & 91.7 & 20.0 \\
243.3 & \verb|U0_D9.4_q2.00_a0.5_n100_am| & 2.0 &-&-& 0.500 &-&-& - & 0.33 & 90.8 & 21.8 \\
242.9 & \verb|GT:BBH:735| & 3.0 & -0.155 & -0.394 & -0.265 &-&-&-& -0.20 & 62.3 & 45.1 \\
242.6 & \verb|RIT:BBH:A7TH45PH130| & 1.0 & -0.378 & -0.354 & 0.508 & 0.393 & 0.330 & 0.513 & 0.51 & 95.2 & 30.2 \\
242.5 & \verb|GT:BBH:863| & 1.0 & -0.512 & 0.270 & -0.157 & -0.506 & -0.175 & -0.270 & -0.21 & 69.4 & 49.1 \\
242.3 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 79.0 & 26.7 \\
242.2 & \verb|RIT:BBH:NQ33TH75PH120| & 3 & -0.386 & 0.669 & 0.207 &-&-&-& 0.16 & 87.2 & 26.0 \\
242.2 & \verb|GT:BBH:758| & 3.1 &-&-&-&-&-&-& 0.00 & 81.0 & 26.2 \\
242.1 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 80.4 & 26.9 \\
242.1 & \verb|GT:BBH:684| & 3.0 & 0.289 & -0.281 & -0.296 &-&-&-& -0.22 & 66.7 & 42.0 \\
242.1 & \verb|GT:BBH:760| & 3.3 &-&-&-&-&-&-& 0.00 & 80.2 & 26.7 \\
241.7 & \verb|SXS:BBH:0049| & 3.0 & 0.494 & 0.073 & 0.001 & - & -0.008 & 0.499 & 0.13 & 85.0 & 13.3 \\
241.6 & \verb|GT:BBH:759| & 3.2 &-&-&-&-&-&-& 0.00 & 77.7 & 27.3 \\
241.3 & \verb|RIT:BBH:A7TH45PH315| & 1.0 & 0.344 & 0.384 & 0.510 & -0.363 & -0.363 & 0.513 & 0.51 & 95.1 & 28.8 \\
241.3 & \verb|GT:BBH:739| & 3.0 & -0.162 & -0.326 & 0.343 &-&-&-& 0.26 & 84.5 & 25.3 \\
241.1 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 80.5 & 26.3 \\
240.8 & \verb|GT:BBH:606| & 3.0 & -0.411 & 0.149 & 0.242 &-&-&-& 0.18 & 84.5 & 25.1 \\
240.4 & \verb|RIT:BBH:NQ33TH75PH150| & 3 & -0.669 & 0.386 & 0.207 &-&-&-& 0.16 & 87.7 & 26.6 \\
239.8 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 78.9 & 26.8 \\
239.7 & \verb|RIT:BBH:A7TH45PH0| & 1.0 & -0.028 & 0.507 & 0.517 & 0.028 & -0.507 & 0.518 & 0.52 & 95.8 & 28.2 \\
239.7 & \verb|RIT:BBH:NQ25TH90PH120| & 4.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 81.3 & 19.8 \\
239.5 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 80.9 & 25.9 \\
239.4 & \verb|RIT:BBH:A7TH45PH210| & 1.0 & 0.299 & -0.412 & 0.516 & -0.256 & 0.444 & 0.513 & 0.51 & 94.4 & 29.1 \\
239.1 & \verb|GT:BBH:414| & 1.75 &-&-& 0.400 &-&-& 0.400 & 0.40 & 91.4 & 20.7 \\
239.0 & \verb|GT:BBH:761| & 3.4 &-&-&-&-&-&-& 0.00 & 81.8 & 25.6 \\
238.9 & \verb|EMuu_D8.82_q1.00_a0.2_n100| & 1.0 &-&-& 0.801 &-&-& 0.200 & 0.50 & 94.5 & 24.4 \\
238.9 & \verb|SXS:BBH:0167| & 4.0 & - & - &-&-&-&-& 0.00 & 79.5 & 16.7 \\
238.7 & \verb|RIT:BBH:NQ16TH150PH0| & 6.0 & 0.400 &-& -0.693 &-&-&-& -0.59 & 56.1 & 40.9 \\
238.7 & \verb|RIT:BBH:A7TH45PH90| & 1.0 & -0.518 & -0.054 & 0.505 & 0.513 &-& 0.513 & 0.51 & 95.0 & 29.2 \\
238.3 & \verb|GT:BBH:744| & 3.0 & 0.411 & -0.149 & 0.242 &-&-&-& 0.18 & 87.4 & 23.7 \\
238.3 & \verb|DU_D10.60_q3.00_a-0.8_rl11_n120| & 2.999 &-&-& -0.801 &-&-& 0.800 & -0.40 & 60.1 & 32.1 \\
238.2 & \verb|RIT:BBH:NQ25TH90PH0| & 4.0 & 0.800 &-&-&-&-&-& 0.00 & 83.6 & 22.0 \\
238.2 & \verb|GT:BBH:652| & 3.5 &-&-&-&-&-&-& 0.00 & 82.1 & 25.6 \\
238.2 & \verb|GT:BBH:874| & 3.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.21 & 90.4 & 23.4 \\
238.2 & \verb|d0_D10.52_q3.00_a-0.66667_n100| & 2.999 &-&-& -0.667 &-&-& - & -0.50 & 59.4 & 33.2 \\
238.1 & \verb|D11_q0.75_a0.0_0.8_n100|(*) & 1.333 &-&-& 0.801 &-&-& - & 0.46 & 92.8 & 17.3 \\
237.9 & \verb|D11_q1.00_a0.5_0.5_n100|(*) & 1.0 &-&-& 0.500 &-&-& 0.500 & 0.50 & 95.5 & 16.5 \\
237.8 & \verb|RIT:BBH:A7TH45PH30| & 1.0 & -0.299 & 0.411 & 0.518 & 0.256 & -0.444 & 0.513 & 0.52 & 96.5 & 27.8 \\
237.7 & \verb|RIT:BBH:NQ16TH150PH30| & 6.0 & 0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 56.1 & 39.3 \\
237.7 & \verb|RIT:BBH:NQ16TH135PH150| & 6.0 & -0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 64.2 & 33.7 \\
237.4 & \verb|RIT:BBH:NQ25TH90PH90| & 4.0 &-& 0.800 &-&-&-&-& 0.00 & 83.9 & 18.7 \\
237.3 & \verb|RIT:BBH:NQ16TH135PH120| & 6.0 & -0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 64.2 & 35.8 \\
237.3 & \verb|GT:BBH:626| & 3.0 & 0.179 & 0.254 & 0.392 &-&-&-& 0.29 & 91.7 & 22.2 \\
237.3 & \verb|(0.4,2.0,'M100')| & 2.0 &-&-& 0.400 &-&-& 0.400 & 0.40 & 94.2 & 20.5 \\
237.2 & \verb|RIT:BBH:NQ25TH90PH30| & 4.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 83.9 & 20.3 \\
237.0 & \verb|D11.00_q0.2500_a0.0_0.0_n100|(*) & 4.0 &-&-&-&-&-& - & 0.00 & 79.8 & 20.3 \\
237.0 & \verb|RIT:BBH:NQ16TH135PH60| & 6.0 & 0.283 & 0.490 & -0.566 &-&-&-& -0.48 & 58.9 & 36.6 \\
236.7 & \verb|GT:BBH:780| & 3.8 &-&-&-&-&-&-& 0.00 & 82.0 & 25.2 \\
236.7 & \verb|RIT:BBH:NQ16TH150PH150| & 6.0 & -0.346 & 0.200 & -0.693 &-&-&-& -0.59 & 59.6 & 38.0 \\
236.6 & \verb|RIT:BBH:NQ16TH150PH60| & 6.0 & 0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 56.1 & 38.8 \\
236.6 & \verb|RIT:BBH:NQ16TH135PH30| & 6.0 & 0.490 & 0.283 & -0.566 &-&-&-& -0.48 & 58.9 & 38.3 \\
236.2 & \verb|GT:BBH:748| & 3.6 &-&-&-&-&-&-& 0.00 & 79.5 & 26.3 \\
236.1 & \verb|GT:BBH:778| & 3.7 &-&-&-&-&-&-& 0.00 & 79.8 & 26.1 \\
236.0 & \verb|D11_q0.75_a0.5_0.5_n100|(*) & 1.333 &-&-& 0.500 &-&-& 0.500 & 0.50 & 97.1 & 16.5 \\
235.9 & \verb|GT:BBH:613| & 3.0 & 0.176 & -0.221 & 0.413 &-&-&-& 0.31 & 90.2 & 23.8 \\
235.7 & \verb|GT:BBH:741| & 3.0 & 0.162 & 0.326 & 0.343 &-&-&-& 0.26 & 91.2 & 24.3 \\
235.5 & \verb|SXS:BBH:0165| & 6.001 & 0.704 & 0.313 & -0.484 & -0.170 & -0.072 & -0.236 & -0.45 & 65.2 & 29.2 \\
235.2 & \verb|SXS:BBH:0057| & 5.002 & 0.402 & -0.177 & -0.201 & - &-&-& -0.17 & 74.9 & 27.6 \\
235.2 & \verb|RIT:BBH:NQ25TH90PH150| & 4.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 82.5 & 22.8 \\
235.2 & \verb|RIT:BBH:NQ16TH150PH120| & 6.0 & -0.200 & 0.346 & -0.693 &-&-&-& -0.59 & 59.6 & 36.6 \\
235.1 & \verb|GT:BBH:879| & 3.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.24 & 93.1 & 22.5 \\
235.0 & \verb|SXS:BBH:0162| & 2.0 &-& - & 0.600 &-&-&-& 0.40 & 93.4 & 12.3 \\
234.4 & \verb|SXS:BBH:0043| & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.32 & 95.6 & 14.9 \\
234.4 & \verb|GT:BBH:555| & 1.0 &-&-& 0.200 &-&-& 0.800 & 0.50 & 98.1 & 16.3 \\
234.3 & \verb|GT:BBH:797| & 4.1 &-&-&-&-&-&-& 0.00 & 80.4 & 25.4 \\
234.1 & \verb|(0,4,'MXX','D11')| & 4 &-&-&-&-&-&-& 0.00 & 79.0 & 20.6 \\
233.7 & \verb|RIT:BBH:NQ16TH135PH0| & 6.0 & 0.566 &-& -0.566 &-&-&-& -0.48 & 59.4 & 38.2 \\
233.7 & \verb|RIT:BBH:NQ16TH150PH90| & 6.0 &-& 0.400 & -0.693 &-&-&-& -0.59 & 56.8 & 37.1 \\
233.4 & \verb|SXS:BBH:0062| & 5.003 & 0.384 & -0.236 & -0.218 &-& - &-& -0.18 & 75.0 & 0.0 \\
233.4 & \verb|GT:BBH:798| & 4.2 &-&-&-&-&-&-& 0.00 & 80.3 & 25.3 \\
233.3 & \verb|GT:BBH:777| & 3.9 &-&-&-&-&-&-& 0.00 & 82.9 & 24.9 \\
233.3 & \verb|GT:BBH:791| & 4.3 &-&-&-&-&-&-& 0.00 & 81.7 & 24.8 \\
232.6 & \verb|RIT:BBH:NQ25TH90PH60| & 4.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 81.0 & 19.4 \\
232.6 & \verb|RIT:BBH:NQ50TH30PH150| & 2.0 & -0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 98.2 & 26.1 \\
232.5 & \verb|RIT:BBH:NQ16TH115PH150| & 6.0 & -0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 69.0 & 31.8 \\
232.4 & \verb|RIT:BBH:NQ16TH135PH90| & 6.0 &-& 0.566 & -0.566 &-&-&-& -0.48 & 62.1 & 39.1 \\
232.4 & \verb|GT:BBH:607| & 3.0 & -0.276 & 0.148 & 0.390 &-&-&-& 0.29 & 95.9 & 21.4 \\
232.3 & \verb|GT:BBH:795| & 4.4 &-&-&-&-&-&-& 0.00 & 81.0 & 24.9 \\
231.6 & \verb|SXS:BBH:0033| & 3.001 & 0.248 & 0.030 & 0.432 & - & - &-& 0.32 & 98.0 & 11.7 \\
231.3 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 80.8 & 24.9 \\
231.3 & \verb|RIT:BBH:NQ50TH30PH120| & 2.0 & -0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 97.2 & 25.7 \\
230.9 & \verb|GT:BBH:884| & 3.75 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 94.2 & 21.8 \\
230.8 & \verb|RIT:BBH:NQ16TH115PH0| & 6.0 & 0.725 &-& -0.338 &-&-&-& -0.29 & 75.5 & 28.3 \\
230.7 & \verb|GT:BBH:862| & 1.0 & 0.542 & -0.255 & -0.034 & 0.053 & 0.188 & -0.567 & -0.30 & 67.6 & 50.7 \\
230.3 & \verb|RIT:BBH:NQ16TH115PH30| & 6.0 & 0.628 & 0.363 & -0.338 &-&-&-& -0.29 & 75.8 & 27.7 \\
229.7 & \verb|GT:BBH:883| & 3.25 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.22 & 93.6 & 21.5 \\
229.4 & \verb|SXS:BBH:0159| & 1.0 &-&-& -0.900 & - & - & -0.900 & -0.90 & 52.8 & 19.3 \\
229.3 & \verb|GT:BBH:656| & 4.5 &-&-&-&-&-&-& 0.00 & 84.1 & 24.5 \\
228.9 & \verb|RIT:BBH:NQ50TH30PH90| & 2.0 &-& 0.400 & 0.693 &-&-&-& 0.46 & 92.5 & 26.7 \\
228.7 & \verb|SXS:BBH:0190| & 4.499 & - &-& - &-&-&-& -0.00 & 83.1 & 14.5 \\
228.7 & \verb|d0_D11.03_q4.00_a-0.75_v2_n100| & 3.998 &-&-& -0.751 & - &-& - & -0.60 & 57.9 & 31.3 \\
228.2 & \verb|GT:BBH:603| & 3.0 &-&-& 0.500 &-&-&-& 0.38 & 97.3 & 21.1 \\
228.0 & \verb|RIT:BBH:NQ16TH115PH120| & 6.0 & -0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 75.5 & 29.4 \\
227.4 & \verb|SXS:BBH:0107| & 5.0 &-&-&-& - & - &-& 0.00 & 82.2 & 12.1 \\
227.4 & \verb|SXS:BBH:0051| & 3.0 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.37 & 99.0 & 11.5 \\
227.3 & \verb|RIT:BBH:NQ16TH115PH90| & 6.0 &-& 0.725 & -0.338 &-&-&-& -0.29 & 70.5 & 32.5 \\
227.1 & \verb|RIT:BBH:NQ16TH115PH60| & 6.0 & 0.363 & 0.628 & -0.338 &-&-&-& -0.29 & 71.1 & 31.1 \\
226.9 & \verb|SXS:BBH:0174| & 3.001 &-& - & 0.500 & - &-&-& 0.37 & 97.5 & 8.4 \\
226.9 & \verb|RIT:BBH:NQ50TH30PH30| & 2.0 & 0.346 & 0.200 & 0.693 &-&-&-& 0.46 & 101.0 & 25.3 \\
226.8 & \verb|Del0_D8.87_q2.00_a0.4_0.8_n100| & 2.001 &-&-& 0.400 & 0.015 & -0.007 & 0.800 & 0.53 & 97.5 & 23.0 \\
226.6 & \verb|RIT:BBH:NQ50TH30PH0| & 2.0 & 0.400 &-& 0.693 &-&-&-& 0.46 & 101.9 & 25.6 \\
226.4 & \verb|DU_D10.61_q4.00_a-0.8_rl11_n100| & 3.999 &-&-& -0.801 &-&-& 0.800 & -0.48 & 58.4 & 33.5 \\
226.3 & \verb|RIT:BBH:NQ50TH30PH60| & 2.0 & 0.200 & 0.346 & 0.693 &-&-&-& 0.46 & 102.2 & 24.4 \\
226.3 & \verb|SXS:BBH:0048| & 3.0 & - & -0.001 & 0.500 & 0.471 & 0.165 & 0.001 & 0.37 & 99.7 & 11.3 \\
226.2 & \verb|SXS:BBH:0156| & 1.0 &-&-& -0.949 &-&-& -0.949 & -0.95 & 49.5 & 18.0 \\
225.6 & \verb|SXS:BBH:0059| & 5.0 & 0.265 & -0.096 & -0.157 &-& - &-& -0.13 & 80.9 & 24.9 \\
225.4 & \verb|RIT:BBH:NQ25TH60PH90| & 4.0 &-& 0.693 & 0.400 &-&-&-& 0.32 & 101.0 & 21.9 \\
225.2 & \verb|RIT:BBH:NQ25TH60PH60| & 4.0 & 0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 103.7 & 20.0 \\
225.2 & \verb|EMuu_D8.78_q1.00_a0.4_n100| & 1.0 &-&-& 0.801 &-&-& 0.400 & 0.60 & 100.8 & 22.8 \\
224.9 & \verb|SXS:BBH:0187| & 5.039 &-& - &-& - & - & - & 0.00 & 84.5 & 15.0 \\
224.9 & \verb|GT:BBH:875| & 4.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.25 & 100.3 & 21.5 \\
224.3 & \verb|SXS:BBH:0152| & 1.0 &-& - & 0.600 & - &-& 0.600 & 0.60 & 101.2 & 10.0 \\
224.3 & \verb|RIT:BBH:NQ25TH60PH30| & 4.0 & 0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 101.2 & 22.1 \\
224.2 & \verb|RIT:BBH:NQ33TH45PH30| & 3 & 0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 100.4 & 22.0 \\
224.1 & \verb|RIT:BBH:NQ33TH45PH90| & 3 &-& 0.566 & 0.566 &-&-&-& 0.42 & 104.0 & 20.7 \\
224.1 & \verb|RIT:BBH:NQ33TH45PH0| & 3 & 0.566 &-& 0.566 &-&-&-& 0.42 & 100.3 & 22.4 \\
224.1 & \verb|RIT:BBH:NQ25TH60PH0| & 4.0 & 0.693 &-& 0.400 &-&-&-& 0.32 & 104.3 & 21.8 \\
223.8 & \verb|RIT:BBH:NQ33TH45PH60| & 3 & 0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 100.6 & 21.3 \\
223.3 & \verb|GT:BBH:745| & 6.0 & -0.046 & 0.539 & 0.259 &-&-&-& 0.22 & 88.8 & 23.1 \\
223.2 & \verb|SXS:BBH:0058| & 5.002 & 0.498 & 0.027 &-&-& - &-& 0.00 & 82.0 & 11.8 \\
223.0 & \verb|(0.6,1.0,'M200','D11')| & 1.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 100.2 & 15.6 \\
222.6 & \verb|GT:BBH:407| & 1.25 &-&-& 0.600 &-&-& 0.600 & 0.60 & 100.4 & 18.1 \\
222.6 & \verb|RIT:BBH:NQ16TH90PH120| & 6.0 & -0.400 & 0.693 &-&-&-&-& 0.00 & 93.4 & 23.8 \\
221.2 & \verb|RIT:BBH:NQ16TH90PH60| & 6.0 & 0.400 & 0.693 &-&-&-&-& 0.00 & 78.7 & 27.9 \\
221.1 & \verb|RIT:BBH:NQ16TH90PH30| & 6.0 & 0.693 & 0.400 &-&-&-&-& 0.00 & 94.5 & 21.0 \\
221.1 & \verb|SXS:BBH:0108| & 5.002 & - & - & -0.500 &-&-&-& -0.42 & 66.8 & 17.4 \\
221.1 & \verb|RIT:BBH:NQ16TH90PH0| & 6.0 & 0.800 &-&-&-&-&-& 0.00 & 96.9 & 20.9 \\
220.9 & \verb|RIT:BBH:A7TH22.5PH130| & 1.0 & -0.213 & -0.178 & 0.670 & 0.213 & 0.178 & 0.670 & 0.67 & 103.7 & 27.7 \\
220.9 & \verb|GT:BBH:880| & 4.5 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.27 & 100.4 & 20.4 \\
220.8 & \verb|SXS:BBH:0197| & 5.522 & - &-& - &-&-& - & -0.00 & 82.2 & 15.4 \\
220.7 & \verb|RIT:BBH:NQ33TH45PH120| & 3 & -0.283 & 0.490 & 0.566 &-&-&-& 0.42 & 105.8 & 21.4 \\
220.4 & \verb|GT:BBH:411| & 1.5 &-&-& 0.600 &-&-& 0.600 & 0.60 & 102.7 & 17.8 \\
220.3 & \verb|RIT:BBH:NQ25TH60PH120| & 4.0 & -0.346 & 0.600 & 0.400 &-&-&-& 0.32 & 104.2 & 19.9 \\
220.3 & \verb|RIT:BBH:NQ33TH45PH150| & 3 & -0.490 & 0.283 & 0.566 &-&-&-& 0.42 & 106.2 & 22.0 \\
220.2 & \verb|RIT:BBH:A7TH22.5PH90| & 1.0 & -0.288 & -0.026 & 0.665 & 0.278 &-& 0.670 & 0.67 & 103.6 & 27.4 \\
220.1 & \verb|D11.50_q0.50_a0.50_0.60_n100|(*) & 2.0 &-&-& 0.600 &-&-& 0.500 & 0.57 & 104.6 & 14.4 \\
220.1 & \verb|RIT:BBH:A7TH22.5PH315| & 1.0 & 0.196 & 0.196 & 0.670 & -0.196 & -0.196 & 0.670 & 0.67 & 105.3 & 26.6 \\
219.0 & \verb|RIT:BBH:NQ25TH60PH165| & 4.0 & -0.669 & 0.179 & 0.400 &-&-&-& 0.32 & 104.3 & 22.6 \\
218.8 & \verb|RIT:BBH:NQ16TH90PH90| & 6.0 &-& 0.800 &-&-&-&-& 0.00 & 79.3 & 27.0 \\
218.7 & \verb|SXS:BBH:0166| & 6.0 & - & - &-&-&-&-& 0.00 & 85.2 & 14.6 \\
218.3 & \verb|RIT:BBH:A7TH22.5PH0| & 1.0 &-& 0.278 & 0.670 &-& -0.278 & 0.670 & 0.67 & 104.3 & 26.7 \\
218.3 & \verb|RIT:BBH:NQ25TH60PH135| & 4.0 & -0.490 & 0.490 & 0.400 &-&-&-& 0.32 & 103.0 & 21.2 \\
218.2 & \verb|GT:BBH:415| & 1.75 &-&-& 0.600 &-&-& 0.600 & 0.60 & 105.0 & 17.9 \\
218.0 & \verb|RIT:BBH:NQ25TH60PH150| & 4.0 & -0.600 & 0.346 & 0.400 &-&-&-& 0.32 & 103.5 & 22.0 \\
217.7 & \verb|d0_D11.35_q5.00_a-0.8_opt1_n100| & 4.997 &-&-& -0.801 &-&-& - & -0.67 & 60.3 & 28.6 \\
217.6 & \verb|D10.50_q0.1667_a0.0_0.0_n100|(*) & 6.0 &-&-&-&-&-& - & 0.00 & 83.2 & 19.6 \\
217.4 & \verb|SXS:BBH:0047| & 3.0 &-&-& 0.500 & - & - & 0.499 & 0.50 & 102.5 & 11.1 \\
217.3 & \verb|RIT:BBH:A7TH22.5PH30| & 1.0 & -0.160 & 0.221 & 0.672 & 0.139 & -0.240 & 0.670 & 0.67 & 106.9 & 26.1 \\
216.3 & \verb|D11_q0.50_a0.00_0.80_n100|(*) & 1.999 &-&-& 0.801 &-&-& - & 0.53 & 108.9 & 14.6 \\
216.3 & \verb|RIT:BBH:NQ16TH90PH150| & 6.0 & -0.693 & 0.400 &-&-&-&-& 0.00 & 81.8 & 28.6 \\
215.8 & \verb|RIT:BBH:A7TH22.5PH210| & 1.0 & 0.139 & -0.240 & 0.670 & -0.139 & 0.240 & 0.670 & 0.67 & 100.4 & 28.1 \\
215.0 & \verb|(0.6,2.0,'M100')| & 2.0 &-&-& 0.600 &-&-& 0.600 & 0.60 & 109.0 & 17.7 \\
214.9 & \verb|GT:BBH:887| & 5.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.28 & 103.6 & 18.8 \\
214.7 & \verb|GT:BBH:889| & 6.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.30 & 112.6 & 17.1 \\
214.0 & \verb|UD_D8.40_q3.00_a0.8_rl11_n120| & 2.999 &-&-& 0.801 &-&-& -0.800 & 0.40 & 106.6 & 23.0 \\
213.2 & \verb|Del0_D8.83_q1.3333_a0.6_0.8_n100| & 1.334 &-&-& 0.600 &-&-& 0.801 & 0.69 & 105.8 & 21.4 \\
212.9 & \verb|GT:BBH:742| & 7.0 & -0.028 & 0.599 & -0.008 &-&-&-& -0.01 & 87.4 & 22.8 \\
212.8 & \verb|SXS:BBH:0192| & 6.58 & - &-&-& - & - & - & 0.00 & 84.4 & 15.5 \\
211.8 & \verb|U0_D9.07_q3.00_a0.66667_n100| & 2.999 &-&-& 0.667 &-&-& - & 0.50 & 108.7 & 19.3 \\
211.7 & \verb|SXS:BBH:0179| & 1.5 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.65 & 109.7 & 9.6 \\
211.2 & \verb|SXS:BBH:0188| & 7.187 &-& - &-& - &-& - & -0.00 & 87.8 & 14.9 \\
210.8 & \verb|SXS:BBH:0061| & 5.002 &-& - & 0.500 & - &-&-& 0.42 & 113.8 & 9.0 \\
210.6 & \verb|D10_q7.00_a0.0_m320| & 7.0 &-&-&-&-&-&-& 0.00 & 86.5 & 0.0 \\
210.6 & \verb|RIT:BBH:A9TH30PH90| & 1.0 & -0.462 & -0.003 & 0.800 & 0.462 & 0.003 & 0.800 & 0.80 & 112.5 & 24.0 \\
209.2 & \verb|GT:BBH:888| & 7.0 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.32 & 116.8 & 15.8 \\
207.9 & \verb|RIT:BBH:A9TH30PH210| & 1.0 & 0.231 & -0.400 & 0.800 & -0.231 & 0.400 & 0.800 & 0.80 & 111.2 & 23.2 \\
207.8 & \verb|RIT:BBH:A9TH30PH130| & 1.0 & -0.354 & -0.297 & 0.800 & 0.354 & 0.297 & 0.800 & 0.80 & 116.0 & 23.2 \\
206.2 & \verb|RIT:BBH:A9TH30PH315| & 1.0 & 0.327 & 0.327 & 0.800 & -0.327 & -0.327 & 0.800 & 0.80 & 116.0 & 21.8 \\
206.1 & \verb|RIT:BBH:A9TH30PH0| & 1.0 & -0.027 & 0.445 & 0.809 & -0.004 & -0.462 & 0.800 & 0.80 & 113.1 & 22.6 \\
205.4 & \verb|RIT:BBH:A9TH30PH30| & 1.0 & -0.262 & 0.381 & 0.799 & 0.231 & -0.400 & 0.800 & 0.80 & 111.5 & 23.3 \\
205.2 & \verb|SXS:BBH:0195| & 7.761 & - & - &-& - &-& - & 0.00 & 88.1 & 15.3 \\
205.2 & \verb|RIT:BBH:NQ16TH45PH30| & 6.0 & 0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 124.8 & 18.7 \\
205.1 & \verb|RIT:BBH:NQ16TH45PH0| & 6.0 & 0.566 &-& 0.566 &-&-&-& 0.48 & 125.6 & 18.7 \\
203.8 & \verb|RIT:BBH:NQ16TH45PH90| & 6.0 &-& 0.566 & 0.566 &-&-&-& 0.48 & 128.3 & 17.9 \\
203.5 & \verb|RIT:BBH:NQ16TH45PH150| & 6.0 & -0.490 & 0.283 & 0.566 &-&-&-& 0.48 & 127.2 & 19.0 \\
203.1 & \verb|RIT:BBH:NQ16TH45PH60| & 6.0 & 0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 126.2 & 17.3 \\
201.5 & \verb|U0_D8.8_q4.00_a0.75_n100_am| & 3.999 &-&-& 0.751 &-&-& - & 0.60 & 134.2 & 16.1 \\
200.4 & \verb|SXS:BBH:0175| & 1.0 &-& - & 0.750 & - &-& 0.750 & 0.75 & 107.9 & 0.0 \\
199.8 & \verb|RIT:BBH:NQ16TH45PH120| & 6.0 & -0.283 & 0.490 & 0.566 &-&-&-& 0.48 & 130.4 & 18.0 \\
196.5 & \verb|SXS:BBH:0155| & 1.0 & - & - & 0.800 &-&-& 0.800 & 0.80 & 116.0 & 8.3 \\
192.0 & \verb|RIT:BBH:A9TH15PH210| & 1.0 & 0.120 & -0.207 & 0.892 & -0.120 & 0.207 & 0.893 & 0.89 & 118.2 & 22.6 \\
191.9 & \verb|GT:BBH:424| & 1.0 &-&-& 0.800 &-&-& 0.800 & 0.80 & 111.8 & 14.6 \\
191.8 & \verb|D10_q1.00_a0.8_0.8_n100|(*) & 1.0 &-&-& 0.801 &-&-& 0.801 & 0.80 & 110.0 & 16.4 \\
191.6 & \verb|RIT:BBH:A9TH15PH0| & 1.0 &-& 0.239 & 0.893 &-& -0.239 & 0.893 & 0.89 & 120.0 & 22.2 \\
190.2 & \verb|RIT:BBH:A9TH15PH30| & 1.0 & -0.120 & 0.207 & 0.892 & 0.120 & -0.207 & 0.893 & 0.89 & 120.0 & 22.3 \\
190.0 & \verb|RIT:BBH:A9TH15PH90| & 1.0 & -0.258 & 0.005 & 0.887 & 0.258 & -0.005 & 0.888 & 0.89 & 117.5 & 23.0 \\
189.3 & \verb|UU_D8.56_q2.00_a0.8_m100| & 2.0 &-&-& 0.801 & 0.016 & -0.004 & 0.800 & 0.80 & 118.0 & 19.7 \\
189.0 & \verb|RIT:BBH:A9TH15PH315| & 1.0 & 0.169 & 0.169 & 0.893 & -0.169 & -0.169 & 0.893 & 0.89 & 120.0 & 22.1 \\
187.3 & \verb|RIT:BBH:A9TH15PH130| & 1.0 & -0.183 & -0.154 & 0.893 & 0.183 & 0.154 & 0.893 & 0.89 & 120.0 & 22.6 \\
184.5 & \verb|SXS:BBH:0153| & 1.0 & - & - & 0.850 &-&-& 0.850 & 0.85 & 114.4 & 8.9 \\
181.9 & \verb|U0_D8.65_q5.00_a0.8_n100| & 4.997 &-&-& 0.801 &-&-&-& 0.67 & 142.3 & 15.3 \\
178.6 & \verb|SXS:BBH:0160| & 1.0 &-& - & 0.900 &-&-& 0.900 & 0.90 & 119.2 & 8.1 \\
166.0 & \verb|SXS:BBH:0157| & 1.0 & - &-& 0.950 &-& - & 0.950 & 0.95 & 119.2 & 8.3 \\
163.0 & \verb|SXS:BBH:0176| & 1.0 &-& - & 0.960 & - &-& 0.960 & 0.96 & 119.2 & 8.2 \\
160.6 & \verb|U0_D8.51_q6.00_a0.83333_n100_am| & 5.996 & 0.003 & -0.023 & 0.834 & - & - & - & 0.71 & 161.4 & 13.6 \\
153.5 & \verb|SXS:BBH:0177| & 1.0 &-&-& 0.989 & - & - & 0.989 & 0.99 & 119.2 & 8.2 \\
152.7 & \verb|SXS:BBH:0158| & 1.0 &-& - & 0.970 & - &-& 0.970 & 0.97 & 116.0 & 8.6 \\
150.2 & \verb|SXS:BBH:0178| & 1.0 &-&-& 0.994 & - & - & 0.994 & 0.99 & 117.6 & 8.4 \\
149.7 & \verb|SXS:BBH:0172| & 1.0 &-& - & 0.979 & - &-& 0.979 & 0.98 & 116.0 & 8.8 \\
129.8 & \verb|d0_D10.53_q6.00_a-0.83333_n100| & 5.996 &-&-& -0.835 &-&-& - & -0.72 & 121.9 & 16.7 \\
\end{longtable}


==> simulation-table.tex <==
\begin{longtable}{ll|lllllll|ll|clll}
\caption{\label{tab:SimulationList}\textbf{List of simulations}: Table of simulations used in this work. Columns indicate the group; an (internal) shorthand for the simulation; the mass ratio; and the components of the dimensionless spins $\mathbf{\chi}_1 = \mathbf{S}_i/m_i^2$; the effective aligned spin $\xi$; the estimated initial starting orbital frequency $M\omega_0$; and (where available) the final black mass and spin.  [We indicate where the black hole mass and spin was unavailable by using X for the corresponding entry.]  } \\ \hline

\hline Name & Key & $q$ & $\chi_{1,x}$ & $\chi_{1,y}$ & $\chi_{1,z}$ & $\chi_{2,x}$ & $\chi_{2,y}$ & $\chi_{2,z}$ &  $\chi_{\rm eff}$ & $M\omega_0$ & $M_{f}/M$ & $a_{f}$ \\ \hline \endfirsthead \multicolumn{4}{r}{Continued on next page}\\ \endfoot \\ \endlastfoot
{\small RIT-Generic} & {\tiny \verb|D10.50_q0.1667_a0.0_0.0_n100|}(*) & 6.000 &-&-&-&-&-& - &-& 0.025 & 0.986 & 0.372 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.33_a-0.8_xi0_n100|}(*) & 2.999 & 0.757 & 0.030 & 0.259 &-&-& -0.800 & -0.006 & 0.029 & 0.965 & 0.756 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.33_a0.8_xi0_n120|}(*) & 2.999 & 0.754 & 0.031 & -0.268 &-&-& 0.800 & -0.001 & 0.029 & 0.970 & 0.607 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.50_a-0.50_0.50_n100|}(*) & 2.000 &-&-& 0.500 &-&-& -0.500 & 0.167 & 0.028 & 0.953 & 0.751 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.50_a-0.8_xi0_n100|}(*) & 2.000 & 0.696 & 0.059 & 0.392 &-& -0.006 & -0.801 & -0.005 & 0.030 & 0.956 & 0.768 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.50_a0.8_xi0_n100|}(*) & 2.000 & 0.689 & 0.062 & -0.403 & 0.012 & 0.006 & 0.800 & -0.002 & 0.030 & 0.960 & 0.609 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a-0.25_0.25_n100|}(*) & 1.333 &-&-& 0.250 &-&-& -0.250 & 0.036 & 0.029 & 0.952 & 0.702 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a-0.5_0.25_n100|}(*) & 1.333 &-&-& 0.250 &-&-& -0.500 & -0.071 & 0.030 & 0.954 & 0.675 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a-0.8_0.8_n100|}(*) & 1.333 &-&-& 0.801 &-&-& -0.801 & 0.114 & 0.031 & 0.946 & 0.758 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a-0.8_xi0_n100|}(*) & 1.333 & 0.538 & 0.056 & 0.590 &-&-& -0.801 & -0.006 & 0.031 & 0.948 & 0.731 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a0.0_0.25_n100|}(*) & 1.333 &-&-& 0.250 &-&-& - & 0.143 & 0.028 & 0.949 & 0.728 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a0.25_-0.25_n100|}(*) & 1.333 &-&-& -0.250 &-&-& 0.250 & -0.036 & 0.029 & 0.955 & 0.648 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a0.5_-0.25_n100|}(*) & 1.333 &-&-& -0.250 &-&-& 0.500 & 0.071 & 0.029 & 0.953 & 0.674 \\
{\small RIT-Generic} & {\tiny \verb|D10_q0.75_a0.8_xi0_n100|}(*) & 1.333 & 0.528 & 0.062 & -0.598 &-&-& 0.801 & 0.001 & 0.031 & 0.953 & 0.643 \\
{\small RIT-Generic} & {\tiny \verb|D10_q1.00_a0.8_0.8_n100|}(*) & 1.000 &-&-& 0.801 &-&-& 0.801 & 0.801 & 0.028 & 0.911 & 0.908 \\
{\small RIT-Generic} & {\tiny \verb|D11.00_q0.2500_a0.0_0.0_n100|}(*) & 4.000 &-&-&-&-&-& - &-& 0.025 & 0.978 & 0.472 \\
{\small RIT-Generic} & {\tiny \verb|D11.25_q0.3333_a0.0_0.0_n100|}(*) & 3.000 &-&-&-&-&-& - &-& 0.024 & 0.971 & 0.541 \\
{\small RIT-Generic} & {\tiny \verb|D11.25_q0.3333_a0.0_0.0_n110|} & 3.000 &-&-&-&-&-& - &-& 0.024 & 0.971 & 0.541 \\
{\small RIT-Generic} & {\tiny \verb|D11.25_q0.3333_a0.0_0.0_n120|} & 3.000 &-&-&-&-&-& - &-& 0.024 & 0.971 & 0.541 \\
{\small RIT-Generic} & {\tiny \verb|D11.25_q0.3333_a0.0_0.0_n130|} & 3.000 &-&-&-&-&-& - &-& 0.024 & 0.971 & 0.541 \\
{\small RIT-Generic} & {\tiny \verb|D11.25_q0.3333_a0.0_0.0_opt_n140|} & 3.000 &-&-&-&-&-& - & - & 0.024 & 0.971 & 0.541 \\
{\small RIT-Generic} & {\tiny \verb|D11.50_q0.4557_a-0.53_0.35_opt_n100|} & 2.194 & - & - & 0.351 & - &-& -0.534 & 0.074 & 0.023 & 0.959 & 0.699 \\
{\small RIT-Generic} & {\tiny \verb|D11.50_q0.50_a0.50_0.60_n100|}(*) & 2.000 &-&-& 0.600 &-&-& 0.500 & 0.567 & 0.023 & 0.941 & 0.834 \\
{\small RIT-Generic} & {\tiny \verb|D11.50_q0.60_a0.0_0.0_n100|}(*) & 1.667 &-&-& - &-&-& - & - & 0.024 & 0.957 & 0.651 \\
{\small RIT-Generic} & {\tiny \verb|D11.75_q0.6667_a0.0_0.0_n100|} & 1.500 &-&-& - &-&-& - & - & 0.022 & 0.955 & 0.664 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.50_a0.00_0.80_n100|}(*) & 1.999 &-&-& 0.801 &-&-& - & 0.534 & 0.025 & 0.937 & 0.866 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.50_a0.0_0.0_n100|}(*) & 2.000 &-&-& - &-&-& - & - & 0.025 & 0.961 & 0.623 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.50_a0.50_-0.50_n100|}(*) & 2.000 &-&-& -0.500 &-&-& 0.500 & -0.167 & 0.027 & 0.966 & 0.491 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.5_-0.5_n100|}(*) & 1.333 &-&-& -0.500 &-&-& -0.500 & -0.500 & 0.027 & 0.964 & 0.509 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.5_0.0_n100|}(*) & 1.333 &-&-& - &-&-& -0.500 & -0.214 & 0.026 & 0.958 & 0.621 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.5_0.5_n100|}(*) & 1.333 &-&-& 0.500 &-&-& -0.500 & 0.071 & 0.026 & 0.950 & 0.728 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.5_0.8_n100|}(*) & 1.333 &-&-& 0.801 &-&-& -0.500 & 0.243 & 0.025 & 0.942 & 0.788 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.8500_0.6375_n100|} & 1.334 &-&-& 0.638 & 0.001 & 0.003 & -0.851 & - & 0.026 & 0.950 & 0.719 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a-0.8_0.0_n100|}(*) & 1.334 &-&-&-&-&-& -0.801 & -0.343 & 0.027 & 0.960 & 0.588 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.0_-0.5_n100|}(*) & 1.333 &-&-& -0.500 &-&-& - & -0.286 & 0.026 & 0.960 & 0.566 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.0_-0.8_n100|}(*) & 1.333 &-&-& -0.801 &-&-& - & -0.458 & 0.027 & 0.963 & 0.498 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.0_0.0_n100|}(*) & 1.333 &-&-& - &-&-& - & - & 0.026 & 0.954 & 0.675 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.0_0.5_n100|}(*) & 1.333 &-&-& 0.500 &-&-& - & 0.286 & 0.025 & 0.851 & 0.779 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.0_0.8_n100|}(*) & 1.333 &-&-& 0.801 &-&-& - & 0.457 & 0.025 & 0.934 & 0.837 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.4_0.8_PNr500_th1d_n100|}(*) & 1.333 & -0.597 & -0.231 & 0.481 & -0.346 & 0.200 & 0.003 & 0.276 & 0.025 & 0.941 & 0.815 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.5_-0.5_n100|}(*) & 1.333 &-&-& -0.500 &-&-& 0.500 & -0.071 & 0.026 & 0.956 & 0.620 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.5_0.0_n100|}(*) & 1.333 &-&-& - &-&-& 0.500 & 0.214 & 0.025 & 0.948 & 0.726 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.5_0.5_n100|}(*) & 1.333 &-&-& 0.500 &-&-& 0.500 & 0.500 & 0.025 & 0.935 & 0.827 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.6_0.6_PNr500_th1d_n100|}(*) & 1.333 & 0.460 & 0.351 & 0.161 & 0.526 & 0.288 & -0.023 & 0.082 & 0.025 & 0.948 & 0.757 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.8500_-0.6375_n100|}(*) & 1.334 &-&-& -0.638 & -0.001 & 0.003 & 0.851 &-& 0.026 & 0.955 & 0.627 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.8_0.0_n100|}(*) & 1.334 &-&-& - &-&-& 0.801 & 0.343 & 0.025 & 0.944 & 0.756 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.8_0.4_PNr500_th1d_n100|}(*) & 1.334 & 0.074 & -0.374 & 0.123 & -0.420 & -0.531 & -0.427 & -0.113 & 0.026 & 0.953 & 0.687 \\
{\small RIT-Generic} & {\tiny \verb|D11_q0.75_a0.8_0.8_PNr500_th1d_n100|}(*) & 1.333 & -0.308 & 0.640 & 0.369 & -0.006 & 0.763 & -0.243 & 0.107 & 0.026 & 0.947 & 0.807 \\
{\small RIT-Generic} & {\tiny \verb|D11_q1.00_a-0.5_-0.5_n100|}(*) & 1.000 &-&-& -0.500 &-&-& -0.500 & -0.500 & 0.027 & 0.962 & 0.528 \\
{\small RIT-Generic} & {\tiny \verb|D11_q1.00_a-0.8_-0.8_n100|}(*) & 1.000 &-&-& -0.801 &-&-& -0.801 & -0.801 & 0.029 & 0.966 & 0.426 \\
{\small RIT-Generic} & {\tiny \verb|D11_q1.00_a0.0_-0.5_n100|}(*) & 1.000 &-&-& -0.500 &-&-& - & -0.250 & 0.026 & 0.957 & 0.609 \\
{\small RIT-Generic} & {\tiny \verb|D11_q1.00_a0.0_-0.8_n100|}(*) & 1.000 &-&-& -0.801 &-&-& - & -0.400 & 0.027 & 0.960 & 0.559 \\
{\small RIT-Generic} & {\tiny \verb|D11_q1.00_a0.5_0.5_n100|}(*) & 1.000 &-&-& 0.500 &-&-& 0.500 & 0.500 & 0.024 & 0.933 & 0.831 \\
{\small RIT-Generic} & {\tiny \verb|D12.00_q0.50_a0.50_0.10_n100|}(*) & 2.000 &-&-& 0.100 &-&-& 0.500 & 0.233 & 0.023 & 0.956 & 0.684 \\
{\small RIT-Generic} & {\tiny \verb|D12.00_q0.85_a0.0_0.0_n100|}(*) & 1.176 &-&-& - &-&-& - & - & 0.023 & 0.952 & 0.683 \\
{\small RIT-Generic} & {\tiny \verb|D12.25_q0.82_a-0.44_0.33_n100|}(*+) & 1.220 &-&-& 0.330 &-&-& -0.440 & -0.017 & 0.023 & 0.952 & 0.692 \\
{\small RIT-Generic} & {\tiny \verb|D12.25_q0.82_a-0.44_0.33_n110|}(*) & 1.220 &-&-& 0.330 &-&-& -0.440 & -0.017 & 0.023 & 0.952 & 0.692 \\
{\small RIT-Generic} & {\tiny \verb|D12.25_q0.82_a-0.44_0.33_n120|}(*) & 1.220 &-&-& 0.330 &-&-& -0.440 & -0.017 & 0.023 & 0.952 & 0.692 \\
{\small RIT-Generic} & {\tiny \verb|D12.25_q0.82_a-0.44_0.33_n132|} & 1.220 &-&-& 0.330 &-&-& -0.440 & -0.017 & 0.023 & 0.952 & 0.692 \\
{\small RIT-Generic} & {\tiny \verb|D12.50_q0.50_a-0.50_-0.10_n100|}(*) & 2.000 &-&-& -0.100 &-&-& -0.500 & -0.233 & 0.022 & 0.965 & 0.561 \\
{\small RIT-Generic} & {\tiny \verb|D12_q1.00_a-0.25_-0.25_n100|}(*) & 1.000 &-&-& -0.250 &-&-& -0.250 & -0.250 & 0.024 & 0.958 & 0.608 \\
{\small RIT-Generic} & {\tiny \verb|D12_q1.00_a-0.25_0.00_n100|}(*) & 1.000 &-&-& - &-&-& -0.250 & -0.125 & 0.023 & 0.955 & 0.648 \\
{\small RIT-Generic} & {\tiny \verb|D12_q1.00_a-0.25_0.25_n100|}(*) & 1.000 &-&-& 0.250 &-&-& -0.250 & - & 0.023 & 0.952 & 0.686 \\
{\small RIT-Generic} & {\tiny \verb|D12_q1.00_a0.25_0.25_n100|}(*) & 1.000 &-&-& 0.250 &-&-& 0.250 & 0.250 & 0.023 & 0.944 & 0.761 \\
{\small RIT-Generic} & {\tiny \verb|D13.00_q0.50_a-0.50_-0.60_n100|}(*) & 2.000 &-&-& -0.600 &-&-& -0.500 & -0.567 & 0.020 & 0.971 & 0.394 \\
{\small RIT-Generic} & {\tiny \verb|D13.00_q0.50_a0.00_-0.80_n100|}(*) & 1.999 &-&-& -0.801 &-&-& - & -0.534 & 0.021 & 0.971 & 0.359 \\
{\small RIT-Generic} & {\tiny \verb|D13_q1.00_a-0.80_-0.40_n100|}(*) & 1.000 &-&-& -0.400 &-&-& -0.801 & -0.600 & 0.022 & 0.963 & 0.494 \\
{\small RIT-Generic} & {\tiny \verb|D15.00_q0.4557_a0.35_-0.53_n100|} & 2.194 &-&-& -0.530 &-&-& 0.350 & -0.255 & 0.015 & 0.970 & 0.438 \\
{\small RIT-Generic} & {\tiny \verb|D15.00_q0.50_a0.00_0.60_th0_45_n100|} & 2.000 & 0.424 &-& 0.424 & - & - & - & 0.283 & 0.016 & 0.951 & 0.776 \\
{\small RIT-Generic} & {\tiny \verb|D15.00_q0.50_a0.00_0.60_th0_45_n118|} & 2.000 & 0.424 &-& 0.424 & - & - & - & 0.283 & 0.016 & 0.951 & 0.776 \\
{\small RIT-Generic} & {\tiny \verb|D21.5_q1_a0.2_0.8_th104.4775_n100|} & 1.001 &-&-& 0.200 & 0.775 &-& -0.200 & - & 0.011 & 0.949 & 0.704 \\
{\small RIT-Generic} & {\tiny \verb|DD_D10.99_q2.00_a-0.8_n100|} & 2.000 &-&-& -0.801 &-&-& -0.801 & -0.801 & 0.029 & 0.973 & 0.305 \\
{\small RIT-Generic} & {\tiny \verb|DU_D10.60_q3.00_a-0.8_rl11_n120|} & 2.999 &-&-& -0.801 &-&-& 0.800 & -0.400 & 0.030 & 0.978 & 0.206 \\
{\small RIT-Generic} & {\tiny \verb|DU_D10.61_q4.00_a-0.8_rl11_n100|} & 3.999 &-&-& -0.801 &-&-& 0.800 & -0.481 & 0.030 & 0.983 & 0.058 \\
{\small RIT-Generic} & {\tiny \verb|DU_D10.86_q1.3333_a-0.8_opt1_n100|} & 1.333 &-&-& -0.801 &-&-& 0.801 & -0.114 & 0.027 & 0.957 & 0.586 \\
{\small RIT-Generic} & {\tiny \verb|DU_D10.90_q2.00_a-0.8_rl10_opt1_n100|} & 2.000 &-&-& -0.801 & - & -0.004 & 0.801 & -0.267 & 0.027 & 0.968 & 0.410 \\
{\small RIT-Generic} & {\tiny \verb|Del0_D10.01_q2.00_a-0.4_-0.8_n100|} & 2.001 &-&-& -0.400 & -0.011 & 0.003 & -0.800 & -0.533 & 0.033 & 0.970 & 0.442 \\
{\small RIT-Generic} & {\tiny \verb|Del0_D10.97_q1.3333_a-0.6_-0.8_n100|} & 1.334 &-&-& -0.600 &-&-& -0.801 & -0.686 & 0.029 & 0.966 & 0.451 \\
{\small RIT-Generic} & {\tiny \verb|Del0_D8.83_q1.3333_a0.6_0.8_n100|} & 1.334 &-&-& 0.600 &-&-& 0.801 & 0.686 & 0.035 & 0.924 & 0.872 \\
{\small RIT-Generic} & {\tiny \verb|Del0_D8.87_q2.00_a0.4_0.8_n100|} & 2.001 &-&-& 0.400 & 0.015 & -0.007 & 0.800 & 0.533 & 0.035 & 0.945 & 0.790 \\
{\small RIT-Generic} & {\tiny \verb|EMu0_D8.80_q1.00_a0.8_n100|} & 1.000 &-&-& 0.801 &-&-& - & 0.400 & 0.036 & 0.937 & 0.803 \\
{\small RIT-Generic} & {\tiny \verb|EMu0_D8.98_q1.00_a0.6_n100|} & 1.000 &-&-& 0.600 &-&-& - & 0.300 & 0.035 & 0.942 & 0.775 \\
{\small RIT-Generic} & {\tiny \verb|EMu0_D9.16_q1.00_a0.4_n100|} & 1.000 &-&-& 0.400 &-&-& - & 0.200 & 0.034 & 0.945 & 0.746 \\
{\small RIT-Generic} & {\tiny \verb|EMuu_D8.78_q1.00_a0.4_n100|} & 1.000 &-&-& 0.801 &-&-& 0.400 & 0.600 & 0.036 & 0.926 & 0.857 \\
{\small RIT-Generic} & {\tiny \verb|EMuu_D8.82_q1.00_a0.2_n100|} & 1.000 &-&-& 0.801 &-&-& 0.200 & 0.500 & 0.036 & 0.932 & 0.831 \\
{\small RIT-Generic} & {\tiny \verb|Rflop_r500_d11_q0.7_a0.8_m088|}(*) & 1.428 & 0.603 & 0.445 & 0.283 & 0.747 & 0.278 & -0.079 & 0.134 & 0.026 & 0.945 & 0.807 \\
{\small RIT-Generic} & {\tiny \verb|S0_D10.04_q1.3333_a0.45_-0.80_n100|} & 1.334 &-&-& 0.450 &-&-& -0.801 & -0.086 & 0.031 & 0.953 & 0.685 \\
{\small RIT-Generic} & {\tiny \verb|S0_D9.75_q2.00_a-0.20_0.80_n100|} & 2.001 &-&-& -0.200 & 0.015 & -0.006 & 0.800 & 0.133 & 0.031 & 0.960 & 0.606 \\
{\small RIT-Generic} & {\tiny \verb|S0_D9.87_q2.00_a0.20_-0.80_n100|} & 2.001 &-&-& 0.200 & -0.015 & -0.007 & -0.800 & -0.133 & 0.032 & 0.962 & 0.639 \\
{\small RIT-Generic} & {\tiny \verb|S0_D9.96_q1.3333_a-0.45_0.80_n100|} & 1.334 &-&-& -0.450 &-&-& 0.801 & 0.086 & 0.031 & 0.953 & 0.662 \\
{\small RIT-Generic} & {\tiny \verb|U0_D8.51_q6.00_a0.83333_n100_am|} & 5.996 & 0.003 & -0.023 & 0.834 & - & - & - & 0.715 & 0.034 & 0.967 & 0.888 \\
{\small RIT-Generic} & {\tiny \verb|U0_D8.65_q5.00_a0.8_n100|} & 4.997 &-&-& 0.801 &-&-&-& 0.667 & 0.034 & 0.963 & 0.872 \\
{\small RIT-Generic} & {\tiny \verb|U0_D8.8_q4.00_a0.75_n100_am|} & 3.999 &-&-& 0.751 &-&-& - & 0.600 & 0.034 & 0.959 & 0.852 \\
{\small RIT-Generic} & {\tiny \verb|U0_D9.07_q3.00_a0.66667_n100|} & 2.999 &-&-& 0.667 &-&-& - & 0.500 & 0.032 & 0.954 & 0.823 \\
{\small RIT-Generic} & {\tiny \verb|U0_D9.4_q2.00_a0.5_n100_am|} & 2.000 &-&-& 0.500 &-&-& - & 0.333 & 0.031 & 0.949 & 0.779 \\
{\small RIT-Generic} & {\tiny \verb|U0_D9.53_q1.00_a0.0_n100|} & 1.000 &-&-& - &-&-& - & - & 0.033 & 0.952 & 0.686 \\
{\small RIT-Generic} & {\tiny \verb|UD_D10.01_q1.00_a0.4_n100|} & 1.000 &-&-& 0.400 &-&-& -0.400 & - & 0.030 & 0.952 & 0.686 \\
{\small RIT-Generic} & {\tiny \verb|UD_D8.40_q3.00_a0.8_rl11_n120|} & 2.999 &-&-& 0.801 &-&-& -0.800 & 0.400 & 0.038 & 0.952 & 0.856 \\
{\small RIT-Generic} & {\tiny \verb|UD_D8.76_q2.00_a0.8_rl10_opt1_n100|} & 2.000 &-&-& 0.801 &-&-& -0.801 & 0.267 & 0.037 & 0.946 & 0.824 \\
{\small RIT-Generic} & {\tiny \verb|UD_D9.51_q1.00_a0.8_rl10_opt1_n100|} & 1.000 &-&-& 0.801 &-&-& -0.801 & - & 0.034 & 0.951 & 0.684 \\
{\small RIT-Generic} & {\tiny \verb|UD_D9.52_q1.00_a0.6_rl10_opt3_n100|} & 1.000 &-&-& 0.600 &-&-& -0.600 & - & 0.034 & 0.951 & 0.685 \\
{\small RIT-Generic} & {\tiny \verb|UU_D8.56_q2.00_a0.8_m100|} & 2.000 &-&-& 0.801 & 0.016 & -0.004 & 0.800 & 0.801 & 0.036 & 0.924 & 0.903 \\
{\small RIT-Generic} & {\tiny \verb|d0_D10.50_q2.00_a-0.5_n100|} & 2.000 &-&-& -0.500 &-&-& - & -0.333 & 0.029 & 0.968 & 0.460 \\
{\small RIT-Generic} & {\tiny \verb|d0_D10.52_q1.3333_a-0.25_n100|} & 1.333 &-&-& -0.250 &-&-& - & -0.143 & 0.028 & 0.957 & 0.621 \\
{\small RIT-Generic} & {\tiny \verb|d0_D10.52_q3.00_a-0.66667_n100|} & 2.999 &-&-& -0.667 &-&-& - & -0.500 & 0.031 & 0.978 & 0.240 \\
{\small RIT-Generic} & {\tiny \verb|d0_D10.53_q6.00_a-0.83333_n100|} & 5.996 &-&-& -0.835 &-&-& - & -0.715 & 0.031 & 0.990 & 0.172 \\
{\small RIT-Generic} & {\tiny \verb|d0_D11.03_q4.00_a-0.75_v2_n100|} & 3.998 &-&-& -0.751 & - &-& - & -0.600 & 0.028 & 0.983 & 0.067 \\
{\small RIT-Generic} & {\tiny \verb|d0_D11.35_q5.00_a-0.8_opt1_n100|} & 4.997 &-&-& -0.801 &-&-& - & -0.667 & 0.027 & 0.987 & 0.067 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0001|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0010|} & 1.501 & 0.248 & 0.028 & -0.433 & - &-&-& -0.260 & 0.014 & 0.962 & 0.563 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0100|} & 1.500 & - & - &-&-& - &-&-& 0.012 & 0.955 & 0.664 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0101|} & 1.501 &-& - & -0.500 & - & - &-& -0.300 & 0.018 & 0.963 & 0.540 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0102|} & 1.500 & 0.496 & 0.051 & -0.001 & 0.494 & 0.071 & -0.001 & -0.001 & 0.015 & 0.954 & 0.695 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0103|} & 1.501 & 0.496 & 0.058 &-&-&-&-&-& 0.012 & 0.954 & 0.683 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0104|} & 3.000 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.375 & 0.018 & 0.961 & 0.755 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0105|} & 3.001 &-& - & -0.500 & - & - &-& -0.375 & 0.012 & 0.978 & 0.316 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0106|} & 5.000 &-&-&-&-&-&-&-& 0.020 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0107|} & 5.000 &-&-&-& - & - &-&-& 0.015 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0108|} & 5.002 & - & - & -0.500 &-&-&-& -0.416 & 0.018 & 0.987 & 0.117 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0109|} & 5.002 &-& - & -0.500 & - & - &-& -0.416 & 0.020 & 0.987 & 0.117 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0011|} & 1.501 & 0.248 & 0.026 & 0.433 &-&-&-& 0.260 & 0.015 & 0.946 & 0.770 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0110|} & 5.002 &-& - & 0.500 & - & - &-& 0.416 & 0.019 & 0.975 & 0.707 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0111|} & 5.002 &-& - & -0.500 & - & - &-& -0.416 & 0.020 & 0.987 & 0.117 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0112|} & 5.000 &-& - &-&-&-&-&-& 0.018 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0113|} & 5.000 &-&-&-& - &-&-&-& 0.018 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0114|} & 8.003 &-& - & -0.500 &-& - &-& -0.444 & 0.020 & 0.992 & 0.053 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0115|} & 1.070 & 0.019 & 0.013 & -0.204 & 0.243 & -0.067 & 0.291 & 0.035 & 0.017 & 0.951 & 0.695 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0116|} & 1.080 & -0.078 & 0.065 & 0.033 & 0.185 & 0.007 & 0.103 & 0.067 & 0.016 & 0.950 & 0.706 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0117|} & 1.080 & 0.118 & -0.069 & 0.070 & -0.302 & -0.298 & -0.200 & -0.060 & 0.017 & 0.953 & 0.674 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0118|} & 1.120 & -0.010 & 0.030 & 0.343 & -0.190 & -0.146 & 0.258 & 0.303 & 0.016 & 0.942 & 0.777 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0119|} & 1.120 & -0.012 & 0.068 & 0.260 & 0.078 & -0.003 & 0.006 & 0.140 & 0.016 & 0.948 & 0.731 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0012|} & 1.501 &-& - & -0.500 & - & - &-& -0.300 & 0.014 & 0.963 & 0.540 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0120|} & 1.120 & 0.138 & -0.200 & -0.008 & -0.065 & -0.241 & -0.099 & -0.051 & 0.016 & 0.953 & 0.677 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0121|} & 1.120 & -0.061 & -0.109 & 0.356 & -0.323 & -0.127 & -0.297 & 0.048 & 0.017 & 0.950 & 0.714 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0122|} & 1.170 & -0.019 & 0.061 & -0.477 & 0.041 & 0.050 & -0.364 & -0.425 & 0.017 & 0.962 & 0.546 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0123|} & 1.100 & 0.267 & 0.020 & -0.415 & 0.038 & -0.054 & 0.126 & -0.157 & 0.017 & 0.956 & 0.634 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0124|} & 1.260 & 0.250 & -0.058 & 0.071 & 0.075 & -0.095 & 0.286 & 0.166 & 0.016 & 0.948 & 0.730 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0125|} & 1.270 & 0.012 & 0.045 & -0.058 & 0.389 & 0.241 & 0.070 & -0.002 & 0.015 & 0.953 & 0.680 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0126|} & 1.290 & -0.250 & -0.237 & 0.091 & -0.358 & 0.172 & 0.215 & 0.145 & 0.017 & 0.949 & 0.730 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0127|} & 1.340 & 0.010 & -0.077 & -0.017 & -0.061 & -0.065 & -0.179 & -0.086 & 0.016 & 0.955 & 0.653 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0128|} & 1.350 & 0.041 & 0.005 & 0.134 & -0.048 & 0.103 & 0.397 & 0.246 & 0.016 & 0.947 & 0.743 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0129|} & 1.360 & -0.001 & - & 0.088 & 0.193 & -0.289 & -0.075 & 0.019 & 0.016 & 0.953 & 0.687 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0013|} & 1.501 & - & - & 0.500 &-& - &-& 0.300 & 0.014 & 0.945 & 0.781 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0130|} & 1.380 & 0.164 & 0.037 & -0.014 & 0.293 & 0.060 & 0.343 & 0.136 & 0.015 & 0.951 & 0.707 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0131|} & 1.550 & 0.042 & -0.014 & -0.070 & 0.105 & 0.017 & -0.175 & -0.111 & 0.016 & 0.958 & 0.628 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0132|} & 1.630 & -0.005 & -0.114 & -0.007 & 0.041 & -0.087 & 0.310 & 0.114 & 0.015 & 0.954 & 0.678 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0133|} & 1.630 & 0.098 & 0.042 & -0.134 & -0.107 & -0.110 & -0.021 & -0.091 & 0.016 & 0.959 & 0.618 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0134|} & 1.630 & -0.230 & 0.184 & -0.012 & -0.001 & 0.032 & 0.176 & 0.060 & 0.016 & 0.955 & 0.672 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0135|} & 1.640 & -0.110 & 0.027 & 0.024 & 0.211 & -0.144 & -0.229 & -0.072 & 0.016 & 0.958 & 0.643 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0136|} & 1.680 & 0.118 & -0.114 & 0.326 & -0.145 & -0.071 & 0.145 & 0.258 & 0.015 & 0.949 & 0.750 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0137|} & 1.760 & -0.248 & -0.319 & -0.034 & -0.071 & 0.151 & -0.190 & -0.090 & 0.017 & 0.959 & 0.636 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0138|} & 1.700 & -0.044 & 0.425 & 0.042 & -0.012 & -0.008 & -0.111 & -0.015 & 0.016 & 0.957 & 0.671 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0139|} & 1.820 & 0.032 & -0.342 & 0.210 & -0.132 & -0.047 & -0.042 & 0.121 & 0.016 & 0.954 & 0.708 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0014|} & 1.501 &-& - & -0.500 &-&-&-& -0.300 & 0.014 & 0.963 & 0.540 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0140|} & 1.820 & 0.115 & -0.367 & -0.209 & -0.066 & 0.062 & 0.087 & -0.104 & 0.016 & 0.961 & 0.598 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0141|} & 1.840 & -0.182 & 0.052 & 0.086 & -0.093 & 0.124 & 0.040 & 0.070 & 0.016 & 0.957 & 0.670 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0142|} & 1.910 & -0.291 & -0.230 & -0.052 & 0.004 & 0.001 & 0.110 & 0.004 & 0.016 & 0.960 & 0.639 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0143|} & 1.920 & -0.094 & -0.062 & 0.436 & -0.019 & -0.434 & -0.085 & 0.257 & 0.015 & 0.951 & 0.760 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0144|} & 1.940 & 0.061 & 0.104 & -0.288 & -0.050 & -0.022 & 0.215 & -0.117 & 0.015 & 0.964 & 0.554 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0145|} & 1.960 & 0.017 & 0.029 & -0.049 & 0.091 & -0.002 & 0.027 & -0.023 & 0.016 & 0.961 & 0.614 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0146|} & 1.970 & -0.156 & -0.102 & -0.037 & -0.098 & 0.027 & -0.357 & -0.145 & 0.016 & 0.963 & 0.598 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0147|} & 1.000 & 0.404 & 0.294 & -0.001 & -0.404 & -0.294 & -0.001 & -0.001 & 0.027 & 0.951 & 0.681 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0148|} & 1.000 &-&-& -0.438 & - & - & -0.438 & -0.438 & 0.016 & 0.961 & 0.548 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0149|} & 1.000 &-& - & -0.200 & - &-& -0.200 & -0.200 & 0.016 & 0.956 & 0.624 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0015|} & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.001 & 0.012 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0150|} & 1.000 &-& - & 0.200 & - &-& 0.200 & 0.200 & 0.015 & 0.945 & 0.746 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0151|} & 1.000 &-& - & -0.600 & - &-& -0.600 & -0.600 & 0.016 & 0.964 & 0.494 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0152|} & 1.000 &-& - & 0.600 & - &-& 0.600 & 0.600 & 0.016 & 0.927 & 0.858 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0153|} & 1.000 & - & - & 0.850 &-&-& 0.850 & 0.850 & 0.016 & 0.906 & 0.919 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0154|} & 1.000 & - & - & -0.800 &-& - & -0.800 & -0.800 & 0.016 & 0.967 & 0.427 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0155|} & 1.000 & - & - & 0.800 &-&-& 0.800 & 0.800 & 0.015 & 0.911 & 0.908 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0156|} & 1.000 &-&-& -0.949 &-&-& -0.949 & -0.949 & 0.014 & 0.968 & 0.376 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0157|} & 1.000 & - &-& 0.950 &-& - & 0.950 & 0.950 & 0.015 & 0.894 & 0.941 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0158|} & 1.000 &-& - & 0.970 & - &-& 0.970 & 0.970 & 0.015 & 0.891 & 0.945 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0159|} & 1.000 &-&-& -0.900 & - & - & -0.900 & -0.900 & 0.016 & 0.968 & 0.393 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0016|} & 1.501 &-& - & -0.500 & - & - &-& -0.300 & 0.011 & 0.963 & 0.540 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0160|} & 1.000 &-& - & 0.900 &-&-& 0.900 & 0.900 & 0.015 & 0.900 & 0.930 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0161|} & 1.000 & 0.446 & 0.281 & -0.287 & 0.446 & 0.281 & -0.287 & -0.287 & 0.015 & 0.956 & 0.636 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0162|} & 2.000 &-& - & 0.600 &-&-&-& 0.400 & 0.018 & 0.946 & 0.808 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0163|} & 1.000 & 0.441 & 0.290 & -0.284 & 0.424 & 0.266 & 0.331 & 0.023 & 0.015 & 0.950 & 0.728 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0164|} & 1.000 & 0.425 & 0.266 & 0.330 & 0.425 & 0.266 & 0.330 & 0.330 & 0.016 & 0.937 & 0.804 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0165|} & 6.001 & 0.704 & 0.313 & -0.484 & -0.170 & -0.072 & -0.236 & -0.448 & 0.029 & 0.988 & 0.562 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0166|} & 6.000 & - & - &-&-&-&-&-& 0.019 & 0.985 & 0.372 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0167|} & 4.000 & - & - &-&-&-&-&-& 0.021 & 0.978 & 0.472 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0168|} & 3.000 & - & - &-&-&-&-&-& 0.019 & 0.971 & 0.541 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0169|} & 2.000 & - & - &-&-&-&-&-& 0.018 & 0.961 & 0.623 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0017|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0170|} & 1.000 & -0.001 & -0.001 & 0.437 & 0.001 & 0.001 & 0.437 & 0.437 &-& X & X \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0171|} & 1.000 & -0.001 & -0.001 & -0.438 & 0.001 & 0.001 & -0.438 & -0.438 &-& X & X \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0172|} & 1.000 &-& - & 0.979 & - &-& 0.979 & 0.979 & 0.016 & 0.889 & 0.947 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0173|} & 1.500 & 0.235 & 0.146 & -0.161 & 0.091 & 0.065 & -0.101 & -0.137 & 0.015 & 0.958 & 0.624 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0174|} & 3.001 &-& - & 0.500 & - &-&-& 0.375 & 0.013 & 0.961 & 0.756 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0175|} & 1.000 &-& - & 0.750 & - &-& 0.750 & 0.750 &-& 0.916 & 0.896 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0176|} & 1.000 &-& - & 0.960 & - &-& 0.960 & 0.960 & 0.015 & 0.892 & 0.943 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0177|} & 1.000 &-&-& 0.989 & - & - & 0.989 & 0.989 & 0.015 & 0.888 & 0.949 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0178|} & 1.000 &-&-& 0.994 & - & - & 0.994 & 0.994 & 0.015 & 0.887 & 0.950 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0179|} & 1.500 & -0.001 & -0.001 & 0.991 & 0.128 & 0.051 & 0.145 & 0.652 & 0.016 & 0.922 & 0.897 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0018|} & 1.501 & 0.487 & 0.110 & 0.001 &-&-&-& 0.001 & 0.012 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0180|} & 1.000 & - &-& - &-& - & - & - & 0.012 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0181|} & 6.000 &-&-& - & - & - & - & - & 0.018 & 0.985 & 0.372 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0182|} & 4.000 &-& - &-&-&-& - &-& 0.021 & 0.978 & 0.472 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0183|} & 3.000 &-&-&-& - & - & - &-& 0.019 & 0.971 & 0.541 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0184|} & 2.000 & - &-&-&-&-& - & - & 0.018 & 0.961 & 0.623 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0185|} & 9.990 & - &-&-& - & - & - &-& 0.021 & 0.992 & 0.261 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0186|} & 8.267 &-&-&-&-&-& - &-&-& 0.990 & 0.300 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0187|} & 5.039 &-& - &-& - & - & - &-& 0.020 & 0.982 & 0.415 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0188|} & 7.187 &-& - &-& - &-& - & - & 0.020 & 0.988 & 0.331 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0189|} & 9.167 & - &-&-&-&-& - &-& 0.021 & 0.991 & 0.278 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0019|} & 1.500 & - & - & -0.500 & - & - & 0.499 & -0.100 & 0.014 & 0.960 & 0.587 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0190|} & 4.499 & - &-& - &-&-&-& - & 0.019 & 0.980 & 0.443 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0191|} & 2.507 & - &-& - &-&-&-& - & 0.015 & 0.967 & 0.580 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0192|} & 6.580 & - &-&-& - & - & - &-& 0.020 & 0.987 & 0.351 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0193|} & 3.498 & - &-& - &-&-& - & - & 0.018 & 0.975 & 0.504 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0194|} & 1.518 &-& - &-& - &-& - & - & 0.016 & 0.955 & 0.663 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0195|} & 7.761 & - & - &-& - &-& - &-& 0.021 & 0.989 & 0.313 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0196|} & 9.663 & - &-&-&-&-& - & - & 0.022 & 0.991 & 0.267 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0197|} & 5.522 & - &-& - &-&-& - & - & 0.020 & 0.984 & 0.392 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0198|} & 1.202 & - & - & - & - & - &-&-& 0.015 & 0.952 & 0.682 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0199|} & 8.729 &-&-& - &-&-& - & - & 0.021 & 0.990 & 0.288 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0002|} & 1.000 &-& - &-&-&-&-&-& 0.011 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0020|} & 1.500 &-& - & 0.500 & 0.494 & 0.071 & - & 0.300 & 0.015 & 0.945 & 0.789 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0200|} & 3.272 & - &-& - &-&-& - & - & 0.017 & 0.973 & 0.520 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0021|} & 1.500 & 0.496 & 0.053 & - & - & 0.001 & -0.499 & -0.200 & 0.014 & 0.958 & 0.642 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0022|} & 1.500 & 0.497 & 0.049 & - & 0.001 & -0.001 & 0.499 & 0.200 & 0.015 & 0.950 & 0.723 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0023|} & 1.501 & 0.497 & 0.051 & 0.001 & 0.077 & -0.489 &-& 0.001 & 0.015 & 0.954 & 0.684 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0024|} & 1.501 & 0.496 & 0.051 & -0.001 & -0.077 & 0.489 & 0.002 &-& 0.014 & 0.955 & 0.688 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0025|} & 1.500 & - & - & 0.500 & - & - & -0.499 & 0.100 & 0.013 & 0.950 & 0.738 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0026|} & 1.500 & - &-& 0.500 & -0.494 & -0.071 & - & 0.300 & 0.015 & 0.945 & 0.789 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0027|} & 1.500 & 0.497 & 0.051 & - & -0.494 & -0.071 &-&-& 0.016 & 0.954 & 0.675 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0028|} & 1.501 & -0.001 & 0.001 & 0.500 & 0.078 & -0.489 & 0.001 & 0.300 & 0.015 & 0.944 & 0.786 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0029|} & 1.500 & 0.496 & 0.051 & -0.001 & 0.494 & 0.070 & -0.001 & -0.001 & 0.015 & 0.954 & 0.694 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0003|} & 1.000 & 0.497 & 0.053 & - &-&-&-& - & 0.013 & 0.951 & 0.695 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0030|} & 3.000 &-&-&-& - &-&-&-& 0.018 & 0.971 & 0.541 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0031|} & 3.001 &-&-& 0.500 & - &-&-& 0.375 & 0.018 & 0.961 & 0.755 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0032|} & 3.001 & 0.248 & 0.037 & -0.432 &-& - &-& -0.324 & 0.018 & 0.977 & 0.373 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0033|} & 3.001 & 0.248 & 0.030 & 0.432 & - & - &-& 0.324 & 0.018 & 0.962 & 0.739 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0034|} & 3.001 & 0.497 & 0.047 & 0.001 &-& - &-&-& 0.018 & 0.970 & 0.604 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0035|} & 3.001 & 0.499 & 0.029 & - &-& - &-& - & 0.014 & 0.970 & 0.605 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0036|} & 3.001 & - & - & -0.500 &-&-&-& -0.375 & 0.010 & 0.978 & 0.316 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0037|} & 3.001 & 0.498 & 0.038 &-&-& - &-&-& 0.015 & 0.971 & 0.606 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0038|} & 3.001 &-&-& -0.500 &-& - &-& -0.375 & 0.018 & 0.978 & 0.316 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0039|} & 3.001 &-& - & -0.500 &-& - &-& -0.375 & 0.013 & 0.978 & 0.316 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0004|} & 1.000 & - & - & -0.500 & - & - &-& -0.250 & 0.012 & 0.958 & 0.608 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0040|} & 3.001 &-& - & -0.500 &-& - &-& -0.375 & 0.023 & 0.978 & 0.316 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0041|} & 3.001 & - &-& 0.500 &-& - &-& 0.375 & 0.022 & 0.961 & 0.755 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0042|} & 3.001 & 0.249 & 0.040 & -0.431 &-& - &-& -0.324 & 0.022 & 0.977 & 0.373 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0043|} & 3.001 & 0.247 & 0.037 & 0.432 & - & - &-& 0.324 & 0.022 & 0.962 & 0.739 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0044|} & 3.001 & 0.494 & 0.072 & 0.002 & - & - &-& 0.001 & 0.022 & 0.970 & 0.606 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0045|} & 3.000 &-& - & 0.500 & - & - & -0.499 & 0.250 &-& 0.963 & 0.741 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0046|} & 3.000 &-&-& -0.500 & - &-& -0.499 & -0.499 & 0.018 & 0.978 & 0.299 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0047|} & 3.000 &-&-& 0.500 & - & - & 0.499 & 0.500 & 0.018 & 0.959 & 0.769 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0048|} & 3.000 & - & -0.001 & 0.500 & 0.471 & 0.165 & 0.001 & 0.375 & 0.017 & 0.961 & 0.755 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0049|} & 3.000 & 0.494 & 0.073 & 0.001 & - & -0.008 & 0.499 & 0.126 & 0.018 & 0.969 & 0.618 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0005|} & 1.000 &-&-& 0.499 & - & - &-& 0.250 & 0.013 & 0.943 & 0.761 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0050|} & 3.000 & 0.494 & 0.072 & 0.002 & 0.467 & 0.176 & 0.005 & 0.002 & 0.017 & 0.970 & 0.611 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0051|} & 3.000 &-& 0.001 & 0.500 & -0.474 & -0.157 & 0.001 & 0.375 & 0.018 & 0.961 & 0.755 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0052|} & 3.000 & 0.494 & 0.073 & 0.001 & 0.001 & 0.008 & -0.499 & -0.124 & 0.018 & 0.972 & 0.591 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0053|} & 3.000 & 0.494 & 0.075 & 0.001 & -0.464 & -0.184 & -0.003 &-& 0.018 & 0.971 & 0.597 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0054|} & 5.000 &-& - &-& - &-&-&-& 0.022 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0055|} & 5.000 &-& - &-&-&-&-&-& 0.017 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0056|} & 5.000 &-&-&-& - & - &-&-& 0.015 & 0.982 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0057|} & 5.002 & 0.402 & -0.177 & -0.201 & - &-&-& -0.167 & 0.032 & 0.984 & 0.418 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0058|} & 5.002 & 0.498 & 0.027 &-&-& - &-&-& 0.015 & 0.982 & 0.538 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0059|} & 5.000 & 0.265 & -0.096 & -0.157 &-& - &-& -0.131 & 0.031 & 0.984 & 0.376 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0006|} & 1.345 & 0.234 & 0.148 & -0.161 & 0.091 & 0.064 & -0.101 & -0.135 & 0.015 & 0.957 & 0.636 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0060|} & 5.002 & - &-& -0.500 & - & - &-& -0.416 & 0.016 & 0.987 & 0.117 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0061|} & 5.002 &-& - & 0.500 & - &-&-& 0.416 & 0.016 & 0.975 & 0.707 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0062|} & 5.003 & 0.384 & -0.236 & -0.218 &-& - &-& -0.182 &-& 0.984 & 0.421 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0063|} & 8.000 &-& - &-& - &-&-&-& 0.019 & 0.989 & 0.307 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0064|} & 8.003 &-& - & -0.500 & - & - &-& -0.444 & 0.020 & 0.992 & 0.053 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0065|} & 8.003 & - & - & 0.500 &-&-&-& 0.444 & 0.019 & 0.985 & 0.657 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0066|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0067|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0068|} & 1.000 &-& - &-&-&-&-&-& 0.012 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0069|} & 1.000 &-& - &-&-&-&-&-& 0.011 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0007|} & 1.500 & - & - &-&-& - &-&-& 0.013 & 0.955 & 0.664 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0070|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0071|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0072|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0073|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0074|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.687 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0075|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0076|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0077|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.954 & 0.682 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0078|} & 1.501 & 0.497 & 0.049 & - &-&-&-& - & 0.013 & 0.954 & 0.682 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0079|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0008|} & 1.500 & - & - &-& - & - &-&-& 0.015 & 0.955 & 0.664 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0080|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0081|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.684 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0082|} & 1.501 & 0.496 & 0.053 & - &-&-&-& - & 0.016 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0083|} & 1.000 & - &-& 0.500 & - & - &-& 0.250 & 0.011 & 0.944 & 0.761 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0084|} & 1.000 & - &-& 0.500 & - & - &-& 0.250 & 0.013 & 0.944 & 0.761 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0085|} & 1.000 & - &-& 0.500 & - & - &-& 0.250 & 0.013 & 0.944 & 0.760 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0086|} & 1.000 &-& - &-&-&-&-&-& 0.013 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0087|} & 1.000 &-& - &-&-&-&-&-& 0.012 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0088|} & 1.000 & 0.495 & 0.067 &-&-&-&-&-& 0.013 & 0.951 & 0.695 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0089|} & 1.000 &-& - & -0.500 & - &-&-& -0.250 & 0.013 & 0.958 & 0.608 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0009|} & 1.501 & - &-& 0.500 & - & - &-& 0.300 & 0.018 & 0.945 & 0.782 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0090|} & 1.000 &-& - &-&-&-&-&-& 0.011 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0091|} & 1.000 &-& - &-&-&-&-&-& 0.011 & 0.952 & 0.687 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0092|} & 1.501 & 0.248 & 0.029 & -0.433 & - &-&-& -0.260 & 0.014 & 0.962 & 0.563 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0093|} & 1.500 & - & - &-& - &-&-&-& 0.013 & 0.955 & 0.664 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0094|} & 1.501 & 0.496 & 0.059 &-&-&-&-&-& 0.014 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0095|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0096|} & 1.501 & 0.497 & 0.051 & - &-&-&-& - & 0.015 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0097|} & 1.501 & 0.495 & 0.065 & 0.001 &-&-&-&-& 0.017 & 0.955 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0098|} & 1.501 & 0.486 & 0.114 & 0.002 &-&-&-& 0.001 & 0.013 & 0.955 & 0.684 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0099|} & 1.501 & 0.496 & 0.058 &-&-&-&-&-& 0.012 & 0.954 & 0.682 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0303|} & 10.000 &-&-&-& - & - &-&-& 0.024 & 0.992 & 0.261 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0302|} & 9.500 & - & - &-&-& - &-&-& 0.024 & 0.991 & 0.271 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0301|} & 9.000 & - & - &-& - & - &-&-& 0.023 & 0.991 & 0.282 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0300|} & 8.500 &-&-&-& - & - &-&-& 0.023 & 0.990 & 0.294 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0299|} & 7.500 & - &-&-&-&-&-&-& 0.021 & 0.989 & 0.321 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0298|} & 7.000 & - &-&-& - & - &-&-& 0.021 & 0.988 & 0.337 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0297|} & 6.500 &-&-&-& - & - &-&-& 0.021 & 0.987 & 0.354 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0286|} & 3.000 & - &-& 0.500 &-&-& 0.499 & 0.500 & 0.017 & 0.959 & 0.769 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0296|} & 5.500 & - &-&-& - & - &-&-& 0.017 & 0.984 & 0.393 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0283|} & 3.000 &-& - & 0.300 &-&-& 0.300 & 0.300 & 0.017 & 0.965 & 0.680 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0282|} & 3.000 &-&-& 0.300 & - & - &-& 0.225 & 0.017 & 0.966 & 0.671 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0281|} & 3.000 &-& - & 0.300 & - & - & -0.300 & 0.150 & 0.016 & 0.967 & 0.662 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0295|} & 4.500 & - &-&-&-& - &-&-& 0.016 & 0.980 & 0.443 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0276|} & 3.000 & - & - &-& - & - & -0.300 & -0.075 & 0.015 & 0.972 & 0.531 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0251|} & 2.000 & - & - & 0.300 & - & - & 0.300 & 0.300 & 0.015 & 0.953 & 0.734 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0272|} & 3.000 & - & - & -0.300 &-&-& 0.300 & -0.150 & 0.015 & 0.975 & 0.417 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0250|} & 2.000 &-& - & 0.300 &-&-&-& 0.200 & 0.015 & 0.955 & 0.718 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0271|} & 3.000 &-&-& -0.300 & - & - &-& -0.225 & 0.015 & 0.975 & 0.407 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0249|} & 2.000 & - & - & 0.300 & - & - & -0.300 & 0.100 & 0.015 & 0.957 & 0.701 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0246|} & 2.000 &-&-&-&-& - & 0.300 & 0.100 & 0.015 & 0.959 & 0.641 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0270|} & 3.000 &-& - & -0.300 & - & - & -0.300 & -0.300 & 0.014 & 0.976 & 0.397 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0294|} & 3.500 &-& - &-&-& - &-&-& 0.015 & 0.974 & 0.505 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0277|} & 3.000 & - & - &-& - &-& 0.300 & 0.075 & 0.016 & 0.971 & 0.550 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0245|} & 2.000 & - & - &-&-& - & -0.300 & -0.100 & 0.014 & 0.963 & 0.605 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0242|} & 2.000 & - & - & -0.300 &-&-& 0.300 & -0.100 & 0.014 & 0.965 & 0.545 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0223|} & 1.000 &-&-& 0.300 & - &-&-& 0.150 & 0.014 & 0.947 & 0.732 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0253|} & 2.000 & - & - & 0.500 & - &-& 0.499 & 0.500 & 0.014 & 0.945 & 0.805 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0267|} & 3.000 &-&-& -0.500 & - & - & -0.499 & -0.500 & 0.014 & 0.978 & 0.299 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0241|} & 2.000 &-&-& -0.300 &-&-&-& -0.200 & 0.014 & 0.966 & 0.526 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0240|} & 2.000 & - & - & -0.300 &-&-& -0.300 & -0.300 & 0.013 & 0.967 & 0.508 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0259|} & 2.500 &-& - &-& - &-&-&-& 0.013 & 0.967 & 0.581 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0222|} & 1.000 &-&-& -0.300 &-&-&-& -0.150 & 0.013 & 0.955 & 0.640 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0218|} & 1.000 &-& - & -0.500 & - & - & 0.500 &-& 0.012 & 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0304|} & 1.000 &-& - & -0.500 & - & - & 0.500 &-&-& 0.952 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0238|} & 2.000 &-&-& -0.500 &-&-& -0.499 & -0.500 & 0.012 & 0.970 & 0.428 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0306|}(*) & 1.310 & - &-& 0.961 & - & - & -0.899 & 0.156 & 0.020 & 0.944 & 0.775 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0293|} & 2.999 &-& - & 0.850 & - &-& 0.849 & 0.850 & 0.018 & 0.936 & 0.914 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0290|} & 3.000 &-& - & 0.600 & - &-& 0.400 & 0.550 & 0.017 & 0.955 & 0.807 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0291|} & 3.000 & - & - & 0.600 &-&-& 0.600 & 0.600 & 0.017 & 0.954 & 0.812 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0312|}(*) & 1.203 &-& - & 0.390 &-&-& -0.480 & -0.005 & 0.017 & 0.951 & 0.697 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0305|}(*+) & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.017 & 0.018 & 0.952 & 0.692 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0309|} & 1.221 & - &-& 0.330 & - & - & -0.440 & -0.016 & 0.017 & 0.952 & 0.692 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0313|}(*) & 1.217 &-& - & 0.380 &-&-& -0.520 & -0.026 & 0.017 & 0.952 & 0.692 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0310|}(*) & 1.221 & - &-&-& - & - &-&-& 0.017 & 0.953 & 0.681 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0314|} & 1.228 & - & - & 0.310 & - & - & -0.460 & -0.036 & 0.018 & 0.953 & 0.686 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0315|} & 1.272 & - &-& 0.320 & - & - & -0.560 & -0.067 & 0.018 & 0.953 & 0.680 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0289|} & 3.000 &-&-& 0.600 &-&-& - & 0.450 & 0.017 & 0.957 & 0.796 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0292|} & 2.999 &-& - & 0.731 &-& - & -0.849 & 0.336 & 0.017 & 0.956 & 0.827 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0311|}(*) & 1.186 &-&-& 0.420 &-& - & 0.380 & 0.402 & 0.018 & 0.938 & 0.803 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0285|} & 3.000 & - & - & 0.400 &-&-& 0.600 & 0.450 & 0.017 & 0.961 & 0.730 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0288|} & 3.000 & - &-& 0.600 & - &-& -0.400 & 0.350 & 0.017 & 0.959 & 0.785 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0316|}(*) & 1.186 & 0.241 & 0.170 & 0.299 & -0.203 & -0.172 & -0.271 & 0.038 & 0.017 & 0.950 & 0.705 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0280|} & 2.999 & - & - & 0.269 &-& - & 0.850 & 0.414 & 0.017 & 0.963 & 0.682 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0287|} & 3.000 & - & - & 0.600 &-&-& -0.600 & 0.300 & 0.017 & 0.960 & 0.780 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0257|} & 2.000 &-& - & 0.850 & - & - & 0.850 & 0.850 & 0.016 & 0.920 & 0.918 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0284|} & 3.000 &-& - & 0.400 &-&-& -0.600 & 0.150 & 0.016 & 0.965 & 0.696 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0278|} & 3.000 &-&-&-& - &-& 0.600 & 0.150 & 0.016 & 0.970 & 0.559 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0274|} & 2.999 & - &-& -0.231 & - & - & 0.850 & 0.039 & 0.016 & 0.973 & 0.465 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0279|} & 2.999 & - &-& 0.231 & - & - & -0.849 & -0.039 & 0.016 & 0.970 & 0.615 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0255|} & 2.000 &-& - & 0.600 &-& - & - & 0.400 & 0.016 & 0.946 & 0.808 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0258|} & 2.000 & - &-& 0.871 & - & - & -0.849 & 0.298 & 0.015 & 0.944 & 0.842 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0230|} & 1.000 &-& - & 0.800 & - &-& 0.800 & 0.800 & 0.015 & 0.911 & 0.908 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0248|} & 2.000 &-& - & 0.129 &-& - & 0.850 & 0.369 & 0.016 & 0.953 & 0.712 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0275|} & 3.000 & - &-& - &-&-& -0.600 & -0.150 & 0.015 & 0.973 & 0.521 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0232|} & 1.000 &-& - & 0.900 &-& - & 0.500 & 0.700 & 0.015 & 0.920 & 0.883 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0254|} & 2.000 &-& - & 0.600 &-&-& -0.600 & 0.200 & 0.015 & 0.951 & 0.776 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0269|} & 3.000 &-& - & -0.400 & - &-& 0.600 & -0.150 & 0.015 & 0.975 & 0.382 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0225|} & 1.000 &-& - & 0.400 & - &-& 0.800 & 0.600 & 0.015 & 0.927 & 0.857 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0228|} & 1.000 &-& - & 0.600 & - &-& 0.600 & 0.600 & 0.015 & 0.927 & 0.858 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0247|} & 2.000 &-& - & - &-& - & 0.600 & 0.200 & 0.015 & 0.958 & 0.658 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0229|} & 1.000 &-& - & 0.650 & - &-& 0.250 & 0.450 & 0.015 & 0.935 & 0.817 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0231|} & 1.000 &-& - & 0.900 & - &-&-& 0.450 & 0.015 & 0.935 & 0.816 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0263|} & 3.000 & - &-& -0.600 & - &-& 0.600 & -0.300 & 0.015 & 0.977 & 0.291 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0261|} & 2.999 &-&-& -0.731 &-& - & 0.850 & -0.336 & 0.015 & 0.978 & 0.240 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0239|} & 1.999 &-& - & -0.371 & - & - & 0.850 & 0.036 & 0.015 & 0.963 & 0.554 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0252|} & 1.999 &-& - & 0.371 &-& - & -0.849 & -0.036 & 0.015 & 0.959 & 0.691 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0266|} & 3.000 &-&-& -0.600 &-&-& 0.400 & -0.350 & 0.015 & 0.977 & 0.284 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0256|} & 2.000 & - &-& 0.600 & - &-& 0.600 & 0.600 & 0.016 & 0.940 & 0.839 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0219|} & 1.000 & - &-& -0.500 &-&-& 0.900 & 0.200 & 0.014 & 0.945 & 0.744 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0227|} & 1.000 &-& - & 0.600 &-& - &-& 0.300 & 0.014 & 0.942 & 0.775 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0273|} & 2.999 &-&-& -0.269 & - & - & -0.849 & -0.414 & 0.015 & 0.976 & 0.392 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0221|} & 1.000 &-&-& -0.400 & - &-& 0.800 & 0.200 & 0.015 & 0.945 & 0.745 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0268|} & 3.000 & - &-& -0.400 & - & - & -0.600 & -0.450 & 0.014 & 0.977 & 0.341 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0262|} & 3.000 &-&-& -0.600 &-&-& - & -0.450 & 0.014 & 0.978 & 0.271 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0213|} & 1.000 &-& - & -0.800 & - &-& 0.800 &-& 0.014 & 0.951 & 0.684 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0211|} & 1.000 &-&-& -0.900 &-&-& 0.900 &-& 0.014 & 0.951 & 0.684 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0237|} & 2.000 & - &-& -0.600 & - &-& 0.600 & -0.200 & 0.014 & 0.967 & 0.465 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0244|} & 2.000 &-& - & - &-&-& -0.600 & -0.200 & 0.014 & 0.964 & 0.587 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0217|} & 1.000 &-& - & -0.600 & - &-& 0.600 &-& 0.014 & 0.951 & 0.685 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0233|} & 2.000 &-&-& -0.871 &-& - & 0.850 & -0.298 & 0.014 & 0.969 & 0.390 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0265|} & 3.000 &-&-& -0.600 &-&-& -0.400 & -0.550 & 0.014 & 0.979 & 0.257 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0264|} & 3.000 & - & - & -0.600 & - &-& -0.600 & -0.600 & 0.014 & 0.979 & 0.250 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0243|} & 2.000 & - &-& -0.129 &-&-& -0.850 & -0.369 & 0.014 & 0.967 & 0.529 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0224|} & 1.000 & - &-& 0.400 & - & - & -0.800 & -0.200 & 0.014 & 0.956 & 0.623 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0226|} & 1.000 &-&-& 0.500 & - &-& -0.900 & -0.200 & 0.013 & 0.956 & 0.623 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0236|} & 2.000 & - & - & -0.600 & - &-& - & -0.400 & 0.013 & 0.969 & 0.427 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0216|} & 1.000 &-& - & -0.600 & - & - &-& -0.300 & 0.013 & 0.959 & 0.592 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0260|} & 2.999 & - & - & -0.850 & - & - & -0.849 & -0.850 & 0.013 & 0.981 & 0.124 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0235|} & 2.000 & - & - & -0.600 & - & - & -0.600 & -0.600 & 0.012 & 0.971 & 0.388 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0220|} & 1.000 &-& - & -0.400 & - &-& -0.800 & -0.600 & 0.012 & 0.964 & 0.494 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0215|} & 1.000 & - &-& -0.600 &-& - & -0.600 & -0.600 & 0.012 & 0.964 & 0.494 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0214|} & 1.000 &-&-& -0.625 & - & - & -0.250 & -0.437 & 0.012 & 0.961 & 0.548 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0210|} & 1.000 &-& - & -0.900 &-& - & - & -0.450 & 0.012 & 0.961 & 0.543 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0234|} & 2.000 &-& - & -0.850 &-&-& -0.850 & -0.850 & 0.011 & 0.974 & 0.285 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0209|} & 1.000 & - & - & -0.900 & - & - & -0.500 & -0.700 & 0.011 & 0.965 & 0.461 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0212|} & 1.000 & - &-& -0.800 &-& - & -0.800 & -0.800 & 0.012 & 0.967 & 0.427 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0307|}(*) & 1.228 & - & - & 0.320 &-& - & -0.580 & -0.084 & 0.019 & 0.954 & 0.674 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0308[Lev3]|}(*) & 1.228 & 0.072 & 0.072 & 0.325 & 0.201 & 0.285 & -0.571 & -0.077 & 0.019 & 0.953 & 0.680 \\
{\small SXS-All} & {\tiny \verb|SXS:BBH:0308|} & 1.228 & 0.094 & 0.056 & 0.322 & 0.266 & 0.213 & -0.576 & -0.081 & 0.019 & 0.953 & 0.680 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH0|} & 6.000 & 0.725 &-& -0.338 &-&-&-& -0.290 & 0.033 & 0.991 & 0.554 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH120|} & 6.000 & -0.363 & 0.628 & -0.338 &-&-&-& -0.290 & 0.034 & 0.991 & 0.552 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH150|} & 6.000 & -0.628 & 0.363 & -0.338 &-&-&-& -0.290 & 0.034 & 0.991 & 0.556 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH30|} & 6.000 & 0.628 & 0.363 & -0.338 &-&-&-& -0.290 & 0.032 & 0.991 & 0.553 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH60|} & 6.000 & 0.363 & 0.628 & -0.338 &-&-&-& -0.290 & 0.034 & 0.991 & 0.556 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH115PH90|} & 6.000 &-& 0.725 & -0.338 &-&-&-& -0.290 & 0.035 & 0.991 & 0.555 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH0|} & 6.000 & 0.566 &-& -0.566 &-&-&-& -0.485 & 0.035 & 0.993 & 0.419 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH120|} & 6.000 & -0.283 & 0.490 & -0.566 &-&-&-& -0.485 & 0.036 & 0.993 & 0.419 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH150|} & 6.000 & -0.490 & 0.283 & -0.566 &-&-&-& -0.485 & 0.033 & 0.993 & 0.416 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH30|} & 6.000 & 0.490 & 0.283 & -0.566 &-&-&-& -0.485 & 0.035 & 0.993 & 0.417 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH60|} & 6.000 & 0.283 & 0.490 & -0.566 &-&-&-& -0.485 & 0.033 & 0.993 & 0.418 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH135PH90|} & 6.000 &-& 0.566 & -0.566 &-&-&-& -0.485 & 0.038 & 0.993 & 0.417 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH0|} & 6.000 & 0.400 &-& -0.693 &-&-&-& -0.594 & 0.035 & 0.994 & 0.305 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH120|} & 6.000 & -0.200 & 0.346 & -0.693 &-&-&-& -0.594 & 0.034 & 0.994 & 0.305 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH150|} & 6.000 & -0.346 & 0.200 & -0.693 &-&-&-& -0.594 & 0.035 & 0.994 & 0.304 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH30|} & 6.000 & 0.346 & 0.200 & -0.693 &-&-&-& -0.594 & 0.034 & 0.994 & 0.305 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH60|} & 6.000 & 0.200 & 0.346 & -0.693 &-&-&-& -0.594 & 0.034 & 0.994 & 0.306 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH150PH90|} & 6.000 &-& 0.400 & -0.693 &-&-&-& -0.594 & 0.033 & 0.994 & 0.306 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH0|} & 6.000 & 0.566 &-& 0.566 &-&-&-& 0.485 & 0.036 & 0.979 & 0.828 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH120|} & 6.000 & -0.283 & 0.490 & 0.566 &-&-&-& 0.485 & 0.036 & 0.980 & 0.829 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH150|} & 6.000 & -0.490 & 0.283 & 0.566 &-&-&-& 0.485 & 0.037 & 0.981 & 0.835 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH30|} & 6.000 & 0.490 & 0.283 & 0.566 &-&-&-& 0.485 & 0.036 & 0.980 & 0.829 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH60|} & 6.000 & 0.283 & 0.490 & 0.566 &-&-&-& 0.485 & 0.034 & 0.979 & 0.828 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH45PH90|} & 6.000 &-& 0.566 & 0.566 &-&-&-& 0.485 & 0.036 & 0.979 & 0.829 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH0|} & 6.000 & 0.800 &-&-&-&-&-&-& 0.031 & 0.989 & 0.695 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH120|} & 6.000 & -0.400 & 0.693 &-&-&-&-&-& 0.034 & 0.989 & 0.694 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH150|} & 6.000 & -0.693 & 0.400 &-&-&-&-&-& 0.036 & 0.988 & 0.692 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH30|} & 6.000 & 0.693 & 0.400 &-&-&-&-&-& 0.031 & 0.989 & 0.695 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH60|} & 6.000 & 0.400 & 0.693 &-&-&-&-&-& 0.034 & 0.988 & 0.692 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ16TH90PH90|} & 6.000 &-& 0.800 &-&-&-&-&-& 0.033 & 0.988 & 0.691 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH0|} & 2.000 &-&-&-& 0.566 &-& -0.566 & -0.189 & 0.021 & 0.972 & 0.585 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH120|} & 2.000 &-&-&-& -0.283 & 0.490 & -0.566 & -0.189 & 0.023 & 0.972 & 0.585 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH150|} & 2.000 &-&-&-& -0.490 & 0.283 & -0.566 & -0.189 & 0.023 & 0.971 & 0.591 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH30|} & 2.000 &-&-&-& 0.490 & 0.283 & -0.566 & -0.189 & 0.020 & 0.972 & 0.585 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH60|} & 2.000 &-&-&-& 0.283 & 0.490 & -0.566 & -0.189 & 0.021 & 0.972 & 0.587 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH135PH90|} & 2.000 &-&-&-&-& 0.566 & -0.566 & -0.189 & 0.023 & 0.972 & 0.592 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH0|} & 2.000 &-&-&-& 0.400 &-& 0.693 & 0.231 & 0.042 & 0.967 & 0.665 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH120|} & 2.000 &-&-&-& -0.200 & 0.346 & 0.693 & 0.231 & 0.040 & 0.967 & 0.665 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH150|} & 2.000 &-&-&-& -0.346 & 0.200 & 0.693 & 0.231 & 0.040 & 0.967 & 0.665 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH30|} & 2.000 &-&-&-& 0.346 & 0.200 & 0.693 & 0.231 & 0.041 & 0.968 & 0.663 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH60|} & 2.000 &-&-&-& 0.200 & 0.346 & 0.693 & 0.231 & 0.041 & 0.967 & 0.665 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH30PH90|} & 2.000 &-&-&-&-& 0.400 & 0.693 & 0.231 & 0.040 & 0.967 & 0.665 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH0|} & 2.000 &-&-&-& 0.693 &-& 0.400 & 0.133 & 0.042 & 0.969 & 0.651 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH120|} & 2.000 &-&-&-& -0.346 & 0.600 & 0.400 & 0.133 & 0.040 & 0.968 & 0.649 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH150|} & 2.000 &-&-&-& -0.600 & 0.346 & 0.400 & 0.133 & 0.041 & 0.969 & 0.650 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH30|} & 2.000 &-&-&-& 0.600 & 0.346 & 0.400 & 0.133 & 0.041 & 0.969 & 0.651 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH60|} & 2.000 &-&-&-& 0.346 & 0.600 & 0.400 & 0.133 & 0.040 & 0.969 & 0.650 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH60PH90|} & 2.000 &-&-&-&-& 0.693 & 0.400 & 0.133 & 0.040 & 0.969 & 0.650 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH0|} & 2.000 &-&-&-& 0.800 &-&-&-& 0.024 & 0.969 & 0.628 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH120|} & 2.000 &-&-&-& -0.400 & 0.693 &-&-& 0.024 & 0.969 & 0.628 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH150|} & 2.000 &-&-&-& -0.693 & 0.400 &-&-& 0.022 & 0.969 & 0.627 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH30|} & 2.000 &-&-&-& 0.693 & 0.400 &-&-& 0.025 & 0.970 & 0.624 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH60|} & 2.000 &-&-&-& 0.400 & 0.693 &-&-& 0.026 & 0.969 & 0.629 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ200TH90PH90|} & 2.000 &-&-&-&-& 0.800 &-&-& 0.025 & 0.970 & 0.623 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH0|} & 4.000 & 0.566 &-& -0.566 &-&-&-& -0.453 & 0.035 & 0.988 & 0.397 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH120|} & 4.000 & -0.283 & 0.490 & -0.566 &-&-&-& -0.453 & 0.036 & 0.988 & 0.398 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH150|} & 4.000 & -0.490 & 0.283 & -0.566 &-&-&-& -0.453 & 0.037 & 0.989 & 0.399 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH30|} & 4.000 & 0.490 & 0.283 & -0.566 &-&-&-& -0.453 & 0.036 & 0.988 & 0.396 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH60|} & 4.000 & 0.283 & 0.490 & -0.566 &-&-&-& -0.453 & 0.037 & 0.988 & 0.395 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH135PH90|} & 4.000 &-& 0.566 & -0.566 &-&-&-& -0.453 & 0.035 & 0.988 & 0.395 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH0|} & 4.000 & 0.400 &-& -0.693 &-&-&-& -0.554 & 0.018 & 0.989 & 0.272 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH120|} & 4.000 & -0.200 & 0.346 & -0.693 &-&-&-& -0.554 & 0.026 & 0.989 & 0.273 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH150|} & 4.000 & -0.346 & 0.200 & -0.693 &-&-&-& -0.554 & 0.029 & 0.989 & 0.273 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH30|} & 4.000 & 0.346 & 0.200 & -0.693 &-&-&-& -0.554 & 0.018 & 0.989 & 0.271 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH60|} & 4.000 & 0.200 & 0.346 & -0.693 &-&-&-& -0.554 & 0.022 & 0.989 & 0.271 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH150PH90|} & 4.000 &-& 0.400 & -0.693 &-&-&-& -0.554 & 0.024 & 0.989 & 0.272 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH0|} & 4.000 & 0.400 &-& 0.693 &-&-&-& 0.554 & 0.036 & 0.969 & 0.863 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH120|} & 4.000 & -0.200 & 0.346 & 0.693 &-&-&-& 0.554 & 0.034 & 0.969 & 0.860 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH150|} & 4.000 & -0.346 & 0.200 & 0.693 &-&-&-& 0.554 & 0.036 & 0.969 & 0.854 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH30|} & 4.000 & 0.346 & 0.200 & 0.693 &-&-&-& 0.554 & 0.036 & 0.969 & 0.855 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH60|} & 4.000 & 0.200 & 0.346 & 0.693 &-&-&-& 0.554 & 0.036 & 0.969 & 0.854 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH30PH90|} & 4.000 &-& 0.400 & 0.693 &-&-&-& 0.554 & 0.036 & 0.967 & 0.857 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH0|} & 4.000 & 0.693 &-& 0.400 &-&-&-& 0.320 & 0.035 & 0.974 & 0.803 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH120|} & 4.000 & -0.346 & 0.600 & 0.400 &-&-&-& 0.320 & 0.032 & 0.976 & 0.803 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH135|} & 4.000 & -0.490 & 0.490 & 0.400 &-&-&-& 0.320 & 0.034 & 0.973 & 0.799 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH150|} & 4.000 & -0.600 & 0.346 & 0.400 &-&-&-& 0.320 & 0.035 & 0.973 & 0.799 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH165|} & 4.000 & -0.669 & 0.179 & 0.400 &-&-&-& 0.320 & 0.037 & 0.973 & 0.801 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH30|} & 4.000 & 0.600 & 0.346 & 0.400 &-&-&-& 0.320 & 0.035 & 0.974 & 0.804 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH60|} & 4.000 & 0.346 & 0.600 & 0.400 &-&-&-& 0.320 & 0.032 & 0.974 & 0.803 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH60PH90|} & 4.000 &-& 0.693 & 0.400 &-&-&-& 0.320 & 0.034 & 0.976 & 0.805 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH0|} & 4.000 & 0.800 &-&-&-&-&-&-& 0.028 & 0.981 & 0.689 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH120|} & 4.000 & -0.400 & 0.693 &-&-&-&-&-& 0.025 & 0.981 & 0.688 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH150|} & 4.000 & -0.693 & 0.400 &-&-&-&-&-& 0.029 & 0.980 & 0.683 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH30|} & 4.000 & 0.693 & 0.400 &-&-&-&-&-& 0.026 & 0.981 & 0.689 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH60|} & 4.000 & 0.400 & 0.693 &-&-&-&-&-& 0.024 & 0.980 & 0.685 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ25TH90PH90|} & 4.000 &-& 0.800 &-&-&-&-&-& 0.024 & 0.981 & 0.685 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH0|} & 3.000 & 0.788 &-& -0.139 &-&-&-& -0.104 & 0.028 & 0.977 & 0.642 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH120|} & 3.000 & -0.394 & 0.682 & -0.139 &-&-&-& -0.104 & 0.031 & 0.977 & 0.642 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH150|} & 3.000 & -0.682 & 0.394 & -0.139 &-&-&-& -0.104 & 0.031 & 0.978 & 0.646 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH30|} & 3.000 & 0.682 & 0.394 & -0.139 &-&-&-& -0.104 & 0.029 & 0.977 & 0.640 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH60|} & 3.000 & 0.394 & 0.682 & -0.139 &-&-&-& -0.104 & 0.031 & 0.977 & 0.640 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH100PH90|} & 3.000 &-& 0.788 & -0.139 &-&-&-& -0.104 & 0.031 & 0.977 & 0.639 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH0|} & 3.000 & 0.566 &-& -0.566 &-&-&-& -0.424 & 0.034 & 0.984 & 0.425 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH120|} & 3.000 & -0.283 & 0.490 & -0.566 &-&-&-& -0.424 & 0.035 & 0.984 & 0.423 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH150|} & 3.000 & -0.490 & 0.283 & -0.566 &-&-&-& -0.424 & 0.035 & 0.984 & 0.426 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH30|} & 3.000 & 0.490 & 0.283 & -0.566 &-&-&-& -0.424 & 0.034 & 0.984 & 0.423 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH60|} & 3.000 & 0.283 & 0.490 & -0.566 &-&-&-& -0.424 & 0.036 & 0.984 & 0.422 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH135PH90|} & 3.000 &-& 0.566 & -0.566 &-&-&-& -0.424 & 0.034 & 0.984 & 0.421 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH0|} & 3.000 & 0.566 &-& 0.566 &-&-&-& 0.424 & 0.035 & 0.961 & 0.835 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH120|} & 3.000 & -0.283 & 0.490 & 0.566 &-&-&-& 0.424 & 0.035 & 0.963 & 0.838 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH150|} & 3.000 & -0.490 & 0.283 & 0.566 &-&-&-& 0.424 & 0.036 & 0.962 & 0.836 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH30|} & 3.000 & 0.490 & 0.283 & 0.566 &-&-&-& 0.424 & 0.034 & 0.962 & 0.835 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH60|} & 3.000 & 0.283 & 0.490 & 0.566 &-&-&-& 0.424 & 0.033 & 0.962 & 0.836 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH45PH90|} & 3.000 &-& 0.566 & 0.566 &-&-&-& 0.424 & 0.033 & 0.963 & 0.837 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH0|} & 3.000 & 0.773 &-& 0.207 &-&-&-& 0.155 & 0.031 & 0.971 & 0.758 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH120|} & 3.000 & -0.386 & 0.669 & 0.207 &-&-&-& 0.155 & 0.035 & 0.971 & 0.754 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH150|} & 3.000 & -0.669 & 0.386 & 0.207 &-&-&-& 0.155 & 0.036 & 0.970 & 0.752 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH30|} & 3.000 & 0.669 & 0.386 & 0.207 &-&-&-& 0.155 & 0.031 & 0.972 & 0.758 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH60|} & 3.000 & 0.386 & 0.669 & 0.207 &-&-&-& 0.155 & 0.032 & 0.972 & 0.757 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ33TH75PH90|} & 3.000 &-& 0.773 & 0.207 &-&-&-& 0.155 & 0.034 & 0.972 & 0.757 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH0|} & 2.000 & 0.566 &-& -0.566 &-&-&-& -0.377 & 0.023 & 0.976 & 0.500 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH120|} & 2.000 & -0.283 & 0.490 & -0.566 &-&-&-& -0.377 & 0.019 & 0.975 & 0.497 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH150|} & 2.000 & -0.490 & 0.283 & -0.566 &-&-&-& -0.377 & 0.020 & 0.976 & 0.500 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH30|} & 2.000 & 0.490 & 0.283 & -0.566 &-&-&-& -0.377 & 0.027 & 0.976 & 0.499 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH60|} & 2.000 & 0.283 & 0.490 & -0.566 &-&-&-& -0.377 & 0.027 & 0.976 & 0.497 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH135PH90|} & 2.000 &-& 0.566 & -0.566 &-&-&-& -0.377 & 0.022 & 0.975 & 0.496 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH0|} & 2.000 & 0.400 &-& 0.693 &-&-&-& 0.462 & 0.040 & 0.950 & 0.849 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH120|} & 2.000 & -0.200 & 0.346 & 0.693 &-&-&-& 0.462 & 0.039 & 0.951 & 0.850 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH150|} & 2.000 & -0.346 & 0.200 & 0.693 &-&-&-& 0.462 & 0.040 & 0.950 & 0.849 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH30|} & 2.000 & 0.346 & 0.200 & 0.693 &-&-&-& 0.462 & 0.040 & 0.950 & 0.849 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH60|} & 2.000 & 0.200 & 0.346 & 0.693 &-&-&-& 0.462 & 0.039 & 0.951 & 0.850 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH30PH90|} & 2.000 &-& 0.400 & 0.693 &-&-&-& 0.462 & 0.038 & 0.951 & 0.851 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH0|} & 2.000 & 0.693 &-& 0.400 &-&-&-& 0.267 & 0.039 & 0.957 & 0.797 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH120|} & 2.000 & -0.346 & 0.600 & 0.400 &-&-&-& 0.267 & 0.038 & 0.959 & 0.801 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH150|} & 2.000 & -0.600 & 0.346 & 0.400 &-&-&-& 0.267 & 0.039 & 0.957 & 0.797 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH30|} & 2.000 & 0.600 & 0.346 & 0.400 &-&-&-& 0.267 & 0.038 & 0.958 & 0.799 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH60|} & 2.000 & 0.346 & 0.600 & 0.400 &-&-&-& 0.267 & 0.038 & 0.958 & 0.800 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH60PH90|} & 2.000 &-& 0.693 & 0.400 &-&-&-& 0.267 & 0.038 & 0.959 & 0.801 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH0|} & 2.000 & 0.800 &-&-&-&-&-&-& 0.018 & 0.966 & 0.705 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH120|} & 2.000 & -0.400 & 0.693 &-&-&-&-&-& 0.020 & 0.967 & 0.707 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH150|} & 2.000 & -0.693 & 0.400 &-&-&-&-&-& 0.021 & 0.967 & 0.709 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH30|} & 2.000 & 0.693 & 0.400 &-&-&-&-&-& 0.018 & 0.965 & 0.703 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH60|} & 2.000 & 0.400 & 0.693 &-&-&-&-&-& 0.018 & 0.965 & 0.702 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ50TH90PH90|} & 2.000 &-& 0.800 &-&-&-&-&-& 0.019 & 0.965 & 0.702 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH0|} & 1.500 & 0.693 &-& 0.400 &-&-&-& 0.240 & 0.040 & 0.953 & 0.788 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH120|} & 1.500 & -0.346 & 0.600 & 0.400 &-&-&-& 0.240 & 0.039 & 0.956 & 0.793 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH150|} & 1.500 & -0.600 & 0.346 & 0.400 &-&-&-& 0.240 & 0.040 & 0.955 & 0.790 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH30|} & 1.500 & 0.600 & 0.346 & 0.400 &-&-&-& 0.240 & 0.040 & 0.953 & 0.788 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH60|} & 1.500 & 0.346 & 0.600 & 0.400 &-&-&-& 0.240 & 0.039 & 0.954 & 0.789 \\
{\small RIT-Kicks} & {\tiny \verb|RIT:BBH:NQ66TH60PH90|} & 1.500 &-& 0.693 & 0.400 &-&-&-& 0.240 & 0.038 & 0.955 & 0.791 \\
{\small RIT-Kicks} & {\tiny \verb|q_1_a1_0_a2_0_d_20|} & 1.000 &-&-&-&-&-&-&-&-& X & X \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH0|} & 1.000 & -0.026 & 0.304 & 0.760 & -0.008 & 0.310 & -0.759 & 0.001 & 0.042 & 0.960 & 0.695 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH120|} & 1.000 & -0.272 & -0.157 & 0.757 & -0.272 & -0.157 & -0.757 & - & 0.043 & 0.961 & 0.698 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH150|} & 1.000 & -0.157 & -0.272 & 0.757 & -0.157 & -0.272 & -0.757 & - & 0.043 & 0.961 & 0.697 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH30|} & 1.000 & -0.185 & 0.257 & 0.756 & -0.157 & 0.272 & -0.757 & -0.001 & 0.042 & 0.960 & 0.695 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH60|} & 1.000 & -0.297 & 0.138 & 0.751 & -0.272 & 0.157 & -0.757 & -0.003 & 0.042 & 0.960 & 0.695 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH22.5PH90|} & 1.000 & -0.331 & -0.026 & 0.749 & -0.314 & -0.007 & -0.757 & -0.004 & 0.042 & 0.960 & 0.696 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH0|} & 1.000 & -0.037 & 0.570 & 0.587 & -0.021 & 0.578 & -0.580 & 0.004 & 0.041 & 0.959 & 0.733 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH105|} & 1.000 & -0.567 & -0.177 & 0.564 & -0.560 & -0.150 & -0.579 & -0.008 & 0.040 & 0.958 & 0.726 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH120|} & 1.000 & -0.502 & -0.290 & 0.579 & -0.502 & -0.290 & -0.579 & - & 0.041 & 0.957 & 0.725 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH135|} & 1.000 & -0.410 & -0.410 & 0.579 & -0.410 & -0.410 & -0.579 & - & 0.042 & 0.957 & 0.726 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH150|} & 1.000 & -0.290 & -0.502 & 0.579 & -0.290 & -0.502 & -0.579 & - & 0.042 & 0.958 & 0.729 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH165|} & 1.000 & -0.119 & -0.558 & 0.588 & -0.150 & -0.560 & -0.579 & 0.004 & 0.042 & 0.959 & 0.732 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH30|} & 1.000 & -0.355 & 0.443 & 0.590 & -0.290 & 0.502 & -0.579 & 0.005 & 0.041 & 0.959 & 0.731 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH60|} & 1.000 & -0.549 & 0.217 & 0.568 & -0.502 & 0.290 & -0.579 & -0.006 & 0.040 & 0.959 & 0.729 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:KTH45PH90|} & 1.000 & -0.595 & -0.035 & 0.562 & -0.591 & - & -0.568 & -0.003 & 0.040 & 0.958 & 0.727 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH0|} & 1.000 & -0.064 & 0.817 & 0.013 & - & -0.010 & 0.820 & 0.417 & 0.041 & 0.944 & 0.816 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH120|} & 1.000 & -0.703 & -0.422 & -0.009 & 0.016 & 0.006 & 0.820 & 0.405 & 0.039 & 0.945 & 0.819 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH150|} & 1.000 & -0.385 & -0.724 & 0.002 & 0.012 & 0.003 & 0.820 & 0.411 & 0.040 & 0.945 & 0.818 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH30|} & 1.000 & -0.476 & 0.668 & 0.011 & 0.011 & 0.004 & 0.820 & 0.416 & 0.040 & 0.943 & 0.815 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH60|} & 1.000 & -0.746 & 0.341 & -0.002 & 0.016 & -0.002 & 0.820 & 0.409 & 0.039 & 0.943 & 0.814 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:LPH90|} & 1.000 & -0.819 & -0.038 & -0.009 & 0.016 &-& 0.820 & 0.405 & 0.039 & 0.944 & 0.816 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH0|} & 1.000 & -0.034 & 0.569 & 0.589 & 0.002 & -0.591 & -0.568 & 0.010 & 0.042 & 0.960 & 0.681 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH120|} & 1.000 & -0.498 & -0.319 & 0.567 & 0.502 & 0.290 & -0.579 & -0.006 & 0.041 & 0.960 & 0.679 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH150|} & 1.000 & -0.290 & -0.502 & 0.579 & 0.290 & 0.502 & -0.579 & - & 0.041 & 0.960 & 0.679 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH30|} & 1.000 & -0.337 & 0.463 & 0.585 & 0.290 & -0.502 & -0.579 & 0.003 & 0.041 & 0.961 & 0.684 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH60|} & 1.000 & -0.537 & 0.242 & 0.570 & 0.502 & -0.290 & -0.579 & -0.005 & 0.040 & 0.961 & 0.683 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:STH45PH90|} & 1.000 & -0.591 & -0.053 & 0.565 & 0.568 & -0.003 & -0.591 & -0.013 & 0.040 & 0.961 & 0.681 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH0|} & 1.005 & -0.062 & 0.702 & -0.407 &-&-&-& -0.204 & 0.039 & 0.966 & 0.644 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH120|} & 1.005 & -0.611 & -0.353 & -0.407 &-&-& - & -0.204 & 0.036 & 0.965 & 0.640 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH150|} & 1.005 & -0.322 & -0.617 & -0.422 & - & - &-& -0.212 & 0.037 & 0.965 & 0.642 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH30|} & 1.005 & -0.408 & 0.580 & -0.399 & - &-& - & -0.200 & 0.038 & 0.966 & 0.645 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH60|} & 1.005 & -0.643 & 0.299 & -0.399 &-& - & - & -0.200 & 0.037 & 0.966 & 0.643 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH120PH90|} & 1.005 & -0.706 & -0.033 & -0.403 & - &-& - & -0.202 & 0.037 & 0.966 & 0.642 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH0|} & 1.005 & -0.034 & 0.576 & -0.574 &-&-&-& -0.288 & 0.039 & 0.968 & 0.611 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH120|} & 1.005 & -0.498 & -0.288 & -0.576 & - & - & - & -0.289 & 0.037 & 0.968 & 0.612 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH150|} & 1.005 & -0.259 & -0.498 & -0.590 & - & - &-& -0.296 & 0.038 & 0.968 & 0.612 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH30|} & 1.005 & -0.343 & 0.468 & -0.571 & - & - & - & -0.286 & 0.038 & 0.967 & 0.610 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH60|} & 1.005 & -0.520 & 0.265 & -0.568 &-& - &-& -0.285 & 0.037 & 0.967 & 0.610 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH135PH90|} & 1.005 & -0.579 & -0.025 & -0.572 & - &-& - & -0.287 & 0.037 & 0.967 & 0.610 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH0|} & 1.005 & -0.005 & 0.215 & 0.788 &-& - & - & 0.395 & 0.045 & 0.949 & 0.800 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH120|} & 1.005 & -0.183 & -0.106 & 0.789 & - & - & - & 0.395 & 0.045 & 0.949 & 0.800 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH150|} & 1.005 & -0.106 & -0.183 & 0.789 & - &-& - & 0.395 & 0.045 & 0.949 & 0.800 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH30|} & 1.005 & -0.106 & 0.183 & 0.789 &-& - & - & 0.395 & 0.045 & 0.949 & 0.801 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH60|} & 1.005 & -0.185 & 0.106 & 0.788 &-&-& - & 0.395 & 0.045 & 0.949 & 0.801 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH15PH90|} & 1.005 & -0.223 & -0.003 & 0.785 &-&-&-& 0.394 & 0.045 & 0.949 & 0.801 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH0|} & 1.005 & -0.009 & 0.195 & -0.790 & - & - & - & -0.396 & 0.037 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH120|} & 1.005 & -0.187 & -0.098 & -0.786 & - &-& - & -0.394 & 0.036 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH150|} & 1.005 & -0.105 & -0.182 & -0.786 & - & - & - & -0.394 & 0.037 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH30|} & 1.005 & -0.103 & 0.188 & -0.785 & - &-& - & -0.393 & 0.037 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH60|} & 1.005 & -0.182 & 0.105 & -0.786 &-& - &-& -0.394 & 0.037 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH165PH90|} & 1.005 & -0.211 &-& -0.786 & - &-& - & -0.394 & 0.036 & 0.970 & 0.566 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH0|} & 1.005 & -0.033 & 0.386 & 0.718 &-& - & - & 0.360 & 0.044 & 0.950 & 0.793 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH120|} & 1.005 & -0.353 & -0.204 & 0.707 & - &-& - & 0.354 & 0.045 & 0.950 & 0.792 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH150|} & 1.005 & -0.204 & -0.353 & 0.707 & - &-& - & 0.354 & 0.046 & 0.950 & 0.792 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH30|} & 1.005 & -0.232 & 0.338 & 0.706 &-& - & - & 0.354 & 0.044 & 0.951 & 0.794 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH60|} & 1.005 & -0.378 & 0.185 & 0.700 & - &-& - & 0.351 & 0.044 & 0.951 & 0.793 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH30PH90|} & 1.005 & -0.423 & -0.024 & 0.698 &-&-& - & 0.350 & 0.045 & 0.950 & 0.793 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH0|} & 1.005 & -0.034 & 0.568 & 0.584 &-& - & - & 0.293 & 0.044 & 0.953 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH10|} & 1.005 & -0.153 & 0.539 & 0.593 &-& - & - & 0.297 & 0.044 & 0.953 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH1125|} & 1.005 & -0.531 & -0.251 & 0.566 &-&-& - & 0.284 & 0.045 & 0.952 & 0.778 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH120|} & 1.005 & -0.500 & -0.289 & 0.577 &-& - & - & 0.289 & 0.045 & 0.952 & 0.778 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH1275|} & 1.005 & -0.458 & -0.351 & 0.577 & - & - &-& 0.289 & 0.046 & 0.952 & 0.779 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH150|} & 1.005 & -0.289 & -0.500 & 0.577 &-&-&-& 0.289 & 0.045 & 0.952 & 0.780 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH20|} & 1.005 & -0.251 & 0.511 & 0.584 &-& - & - & 0.293 & 0.044 & 0.953 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH30|} & 1.005 & -0.341 & 0.464 & 0.578 &-& - & - & 0.290 & 0.044 & 0.953 & 0.780 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH40|} & 1.005 & -0.417 & 0.401 & 0.575 &-& - & - & 0.288 & 0.044 & 0.953 & 0.780 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH45|} & 1.005 & -0.453 & 0.365 & 0.572 &-& - & - & 0.287 & 0.044 & 0.953 & 0.780 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH50|} & 1.005 & -0.485 & 0.328 & 0.568 & - &-&-& 0.285 & 0.044 & 0.953 & 0.779 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH60|} & 1.005 & -0.536 & 0.241 & 0.566 & - &-&-& 0.284 & 0.044 & 0.952 & 0.779 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH75|} & 1.005 & -0.582 & 0.097 & 0.564 &-& - & - & 0.283 & 0.044 & 0.952 & 0.778 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH90|} & 1.005 & -0.590 & -0.050 & 0.562 &-& - & - & 0.282 & 0.045 & 0.952 & 0.778 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH45PH975|} & 1.005 & -0.580 & -0.104 & 0.565 & - & - &-& 0.283 & 0.045 & 0.952 & 0.778 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH0|} & 1.005 & -0.058 & 0.692 & 0.429 &-& - & - & 0.215 & 0.045 & 0.955 & 0.760 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH120|} & 1.005 & -0.612 & -0.353 & 0.408 &-&-& - & 0.205 & 0.045 & 0.956 & 0.763 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH150|} & 1.005 & -0.353 & -0.612 & 0.408 & - &-& - & 0.204 & 0.045 & 0.956 & 0.763 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH30|} & 1.005 & -0.426 & 0.555 & 0.420 & - &-& - & 0.210 & 0.044 & 0.954 & 0.759 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH60|} & 1.005 & -0.656 & 0.274 & 0.401 &-& - & - & 0.201 & 0.044 & 0.954 & 0.759 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:NTH60PH90|} & 1.005 & -0.716 & -0.035 & 0.389 & - & - &-& 0.195 & 0.044 & 0.955 & 0.760 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH0|} & 1.012 & -0.062 & 0.725 & 0.549 & - &-& - & 0.276 & 0.040 & 0.953 & 0.782 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH120|} & 1.012 & -0.373 & -0.647 & 0.523 &-&-& - & 0.263 & 0.041 & 0.953 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH150|} & 1.012 & -0.373 & -0.646 & 0.523 &-&-& - & 0.263 & 0.041 & 0.953 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH30|} & 1.012 & -0.432 & 0.609 & 0.522 & - &-& - & 0.263 & 0.041 & 0.953 & 0.780 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH60|} & 1.012 & -0.686 & 0.321 & 0.507 & - &-& - & 0.255 & 0.041 & 0.952 & 0.777 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:N9TH55PH90|} & 1.012 & -0.759 & -0.029 & 0.505 &-& - & - & 0.254 & 0.041 & 0.951 & 0.776 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH0|} & 1.000 & -0.055 & 0.621 & -0.362 &-& -0.625 & -0.361 & -0.361 & 0.020 & 0.967 & 0.568 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH130|} & 1.000 & -0.478 & -0.401 & -0.361 & 0.478 & 0.401 & -0.361 & -0.361 & 0.023 & 0.968 & 0.572 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH210|} & 1.000 & 0.361 & -0.512 & -0.358 & -0.312 & 0.541 & -0.361 & -0.359 & 0.027 & 0.967 & 0.569 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH30|} & 1.000 & -0.361 & 0.515 & -0.352 & 0.312 & -0.541 & -0.361 & -0.356 & 0.021 & 0.967 & 0.569 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH315|} & 1.000 & 0.442 & 0.442 & -0.361 & -0.442 & -0.442 & -0.361 & -0.361 & 0.022 & 0.968 & 0.572 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH120PH90|} & 1.000 & -0.629 & -0.027 & -0.353 & 0.625 &-& -0.361 & -0.357 & 0.023 & 0.968 & 0.574 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH0|} & 1.000 & -0.028 & 0.512 & -0.506 &-& -0.510 & -0.510 & -0.508 & 0.016 & 0.970 & 0.525 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH130|} & 1.000 & -0.390 & -0.328 & -0.510 & 0.390 & 0.328 & -0.510 & -0.510 & 0.025 & 0.971 & 0.526 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH210|} & 1.000 & 0.281 & -0.431 & -0.505 & -0.255 & 0.441 & -0.510 & -0.507 & 0.024 & 0.970 & 0.523 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH30|} & 1.000 & -0.281 & 0.434 & -0.502 & 0.255 & -0.441 & -0.510 & -0.506 & 0.016 & 0.970 & 0.523 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH315|} & 1.000 & 0.360 & 0.360 & -0.510 & -0.360 & -0.360 & -0.510 & -0.510 & 0.018 & 0.971 & 0.527 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH135PH90|} & 1.000 & -0.510 &-& -0.510 & 0.510 &-& -0.510 & -0.510 & 0.021 & 0.970 & 0.524 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH0|} & 1.000 &-& 0.278 & 0.670 &-& -0.278 & 0.670 & 0.670 & 0.043 & 0.934 & 0.870 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH130|} & 1.000 & -0.213 & -0.178 & 0.670 & 0.213 & 0.178 & 0.670 & 0.670 & 0.044 & 0.934 & 0.869 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH210|} & 1.000 & 0.139 & -0.240 & 0.670 & -0.139 & 0.240 & 0.670 & 0.670 & 0.044 & 0.934 & 0.871 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH30|} & 1.000 & -0.160 & 0.221 & 0.672 & 0.139 & -0.240 & 0.670 & 0.671 & 0.043 & 0.934 & 0.871 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH315|} & 1.000 & 0.196 & 0.196 & 0.670 & -0.196 & -0.196 & 0.670 & 0.670 & 0.043 & 0.934 & 0.869 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH22.5PH90|} & 1.000 & -0.288 & -0.026 & 0.665 & 0.278 &-& 0.670 & 0.668 & 0.044 & 0.935 & 0.870 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH0|} & 1.000 & -0.028 & 0.507 & 0.517 & 0.028 & -0.507 & 0.518 & 0.518 & 0.042 & 0.941 & 0.824 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH130|} & 1.000 & -0.378 & -0.354 & 0.508 & 0.393 & 0.330 & 0.513 & 0.510 & 0.044 & 0.943 & 0.827 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH210|} & 1.000 & 0.299 & -0.412 & 0.516 & -0.256 & 0.444 & 0.513 & 0.515 & 0.042 & 0.941 & 0.825 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH30|} & 1.000 & -0.299 & 0.411 & 0.518 & 0.256 & -0.444 & 0.513 & 0.515 & 0.042 & 0.941 & 0.825 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH315|} & 1.000 & 0.344 & 0.384 & 0.510 & -0.363 & -0.363 & 0.513 & 0.511 & 0.042 & 0.943 & 0.827 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH45PH90|} & 1.000 & -0.518 & -0.054 & 0.505 & 0.513 &-& 0.513 & 0.509 & 0.043 & 0.944 & 0.830 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH0|} & 1.000 & -0.053 & 0.616 & 0.379 & 0.028 & -0.624 & 0.368 & 0.373 & 0.041 & 0.949 & 0.784 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH10|} & 1.000 & -0.161 & 0.600 & 0.373 & 0.137 & -0.612 & 0.364 & 0.369 & 0.042 & 0.949 & 0.783 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH110|} & 1.000 & -0.587 & -0.241 & 0.351 & 0.590 & 0.215 & 0.363 & 0.357 & 0.044 & 0.950 & 0.788 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH130|} & 1.000 & -0.467 & -0.427 & 0.354 & 0.481 & 0.404 & 0.363 & 0.358 & 0.044 & 0.950 & 0.789 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH210|} & 1.000 & 0.361 & -0.514 & 0.362 & -0.314 & 0.544 & 0.362 & 0.362 & 0.041 & 0.948 & 0.782 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH30|} & 1.000 & -0.376 & 0.493 & 0.376 & 0.339 & -0.532 & 0.356 & 0.366 & 0.040 & 0.948 & 0.782 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH315|} & 1.000 & 0.424 & 0.464 & 0.361 & -0.444 & -0.444 & 0.363 & 0.362 & 0.041 & 0.951 & 0.789 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH40|} & 1.000 & -0.445 & 0.444 & 0.362 & 0.404 & -0.481 & 0.362 & 0.362 & 0.042 & 0.948 & 0.781 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH80|} & 1.000 & -0.632 & 0.058 & 0.351 & 0.618 & -0.109 & 0.363 & 0.357 & 0.043 & 0.948 & 0.784 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A7TH60PH90|} & 1.000 & -0.632 & -0.052 & 0.351 & 0.628 &-& 0.363 & 0.357 & 0.042 & 0.949 & 0.785 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH0|} & 1.000 &-& 0.239 & 0.893 &-& -0.239 & 0.893 & 0.893 & 0.041 & 0.913 & 0.921 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH130|} & 1.000 & -0.183 & -0.154 & 0.893 & 0.183 & 0.154 & 0.893 & 0.893 & 0.042 & 0.914 & 0.922 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH210|} & 1.000 & 0.120 & -0.207 & 0.892 & -0.120 & 0.207 & 0.893 & 0.893 & 0.041 & 0.913 & 0.921 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH30|} & 1.000 & -0.120 & 0.207 & 0.892 & 0.120 & -0.207 & 0.893 & 0.893 & 0.041 & 0.913 & 0.921 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH315|} & 1.000 & 0.169 & 0.169 & 0.893 & -0.169 & -0.169 & 0.893 & 0.893 & 0.041 & 0.914 & 0.922 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH15PH90|} & 1.000 & -0.258 & 0.005 & 0.887 & 0.258 & -0.005 & 0.888 & 0.887 & 0.042 & 0.914 & 0.922 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH0|} & 1.000 & -0.027 & 0.445 & 0.809 & -0.004 & -0.462 & 0.800 & 0.805 & 0.039 & 0.923 & 0.898 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH130|} & 1.000 & -0.354 & -0.297 & 0.800 & 0.354 & 0.297 & 0.800 & 0.800 & 0.042 & 0.920 & 0.895 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH210|} & 1.000 & 0.231 & -0.400 & 0.800 & -0.231 & 0.400 & 0.800 & 0.800 & 0.040 & 0.923 & 0.898 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH30|} & 1.000 & -0.262 & 0.381 & 0.799 & 0.231 & -0.400 & 0.800 & 0.800 & 0.040 & 0.923 & 0.898 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH315|} & 1.000 & 0.327 & 0.327 & 0.800 & -0.327 & -0.327 & 0.800 & 0.800 & 0.039 & 0.920 & 0.895 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH30PH90|} & 1.000 & -0.462 & -0.003 & 0.800 & 0.462 & 0.003 & 0.800 & 0.800 & 0.042 & 0.921 & 0.896 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH0|} & 1.000 & -0.043 & 0.791 & 0.474 & 0.023 & -0.797 & 0.465 & 0.470 & 0.038 & 0.944 & 0.822 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH130|} & 1.000 & -0.613 & -0.514 & 0.462 & 0.612 & 0.514 & 0.462 & 0.462 & 0.043 & 0.945 & 0.819 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH210|} & 1.000 & 0.458 & -0.653 & 0.465 & -0.400 & 0.692 & 0.462 & 0.463 & 0.037 & 0.941 & 0.813 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH30|} & 1.000 & -0.455 & 0.653 & 0.468 & 0.400 & -0.692 & 0.462 & 0.465 & 0.037 & 0.941 & 0.813 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH315|} & 1.000 & 0.565 & 0.565 & 0.462 & -0.565 & -0.565 & 0.462 & 0.462 & 0.039 & 0.945 & 0.822 \\
{\small RIT-OlderWork} & {\tiny \verb|RIT:BBH:A9TH60PH90|} & 1.000 & -0.809 & -0.030 & 0.443 & 0.808 & -0.006 & 0.446 & 0.444 & 0.039 & 0.945 & 0.818 \\
{\small RIT-OlderWork} & {\tiny \verb|q150_a8_a0_th_60_ph_0|} & 1.492 & - &-& - & -0.087 & 0.682 & 0.435 & 0.174 & 0.042 & 0.962 & 0.706 \\
{\small RIT-OlderWork} & {\tiny \verb|q150_a8_a0_th_60_ph_120|} & 1.492 & - & - &-& -0.595 & -0.380 & 0.405 & 0.162 & 0.041 & 0.961 & 0.704 \\
{\small RIT-OlderWork} & {\tiny \verb|q150_a8_a0_th_60_ph_30|} & 1.492 &-& - & - & -0.430 & 0.556 & 0.410 & 0.164 & 0.043 & 0.962 & 0.707 \\
{\small RIT-OlderWork} & {\tiny \verb|th_0_alt|} & 1.000 & -0.043 & 0.791 & 0.474 & 0.023 & -0.797 & 0.465 & 0.470 & 0.038 & 0.944 & 0.822 \\
{\small RIT-OlderWork} & {\tiny \verb|th_130_alt|} & 1.000 & -0.613 & -0.514 & 0.462 & 0.612 & 0.514 & 0.462 & 0.462 & 0.043 & 0.945 & 0.819 \\
{\small RIT-OlderWork} & {\tiny \verb|th_210_alt|} & 1.000 & 0.458 & -0.653 & 0.465 & -0.400 & 0.692 & 0.462 & 0.463 & 0.037 & 0.941 & 0.813 \\
{\small RIT-OlderWork} & {\tiny \verb|th_30_alt|} & 1.000 & -0.455 & 0.653 & 0.468 & 0.400 & -0.692 & 0.462 & 0.465 & 0.037 & 0.941 & 0.813 \\
{\small RIT-OlderWork} & {\tiny \verb|th_315_alt|} & 1.000 & 0.565 & 0.565 & 0.462 & -0.565 & -0.565 & 0.462 & 0.462 & 0.039 & 0.945 & 0.822 \\
{\small RIT-OlderWork} & {\tiny \verb|th_90_alt|} & 1.000 & -0.809 & -0.030 & 0.443 & 0.808 & -0.006 & 0.446 & 0.444 & 0.039 & 0.945 & 0.818 \\
{\small GT} & {\tiny \verb|GT:BBH:564|} & 1.000 &-&-& -0.400 &-&-& -0.400 & -0.400 & 0.026 & 0.961 & 0.560 \\
{\small GT} & {\tiny \verb|GT:BBH:476|} & 1.000 &-&-& -0.200 &-&-& -0.200 & -0.200 & 0.025 & 0.956 & 0.624 \\
{\small GT} & {\tiny \verb|(0.0,1.0)|} & 1.000 &-&-&-&-&-&-&-& 0.030 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|(0,1.0,'M100')|} & 1.000 &-&-&-&-&-&-&-& 0.029 & 0.951 & 0.687 \\
{\small GT} & {\tiny \verb|(0.0,1.0,'M120','D11')|} & 1.000 &-&-&-&-&-&-&-& 0.029 & 0.951 & 0.686 \\
{\small GT} & {\tiny \verb|(0.0,1.0,'M160','D11')|} & 1.000 &-&-&-&-&-&-&-& 0.025 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|(0.0,1.0,'M160','D9')|} & 1.000 &-&-&-&-&-&-&-& 0.035 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|(0.0,1.0,'M200','D11')|} & 1.000 &-&-&-&-&-&-&-& 0.025 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|GT:BBH:448|} & 1.000 &-&-&-&-&-&-&-& 0.025 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|GT:BBH:717|} & 1.100 &-&-&-&-&-&-&-& 0.035 & 0.952 & 0.685 \\
{\small GT} & {\tiny \verb|GT:BBH:370|} & 1.150 &-&-&-&-&-&-&-& 0.030 & 0.952 & 0.684 \\
{\small GT} & {\tiny \verb|(0.0,1.2,'M160','D9')|} & 1.200 &-&-&-&-&-&-&-& 0.035 & 0.952 & 0.682 \\
{\small GT} & {\tiny \verb|(0,1.25,'M100')|} & 1.250 &-&-&-&-&-&-&-& 0.029 & 0.952 & 0.680 \\
{\small GT} & {\tiny \verb|GT:BBH:371|} & 1.300 &-&-&-&-&-&-&-& 0.030 & 0.953 & 0.677 \\
{\small GT} & {\tiny \verb|(0.0,1.3,'M160','D9')|} & 1.300 &-&-&-&-&-&-&-& 0.035 & 0.953 & 0.677 \\
{\small GT} & {\tiny \verb|GT:BBH:730|} & 1.400 &-&-&-&-&-&-&-& 0.035 & 0.954 & 0.671 \\
{\small GT} & {\tiny \verb|GT:BBH:372|} & 1.450 &-&-&-&-&-&-&-& 0.030 & 0.955 & 0.667 \\
{\small GT} & {\tiny \verb|(0.0,1.5)|} & 1.500 &-&-&-&-&-&-&-& 0.030 & 0.955 & 0.664 \\
{\small GT} & {\tiny \verb|(0,1.5,'M100')|} & 1.500 &-&-&-&-&-&-&-& 0.029 & 0.955 & 0.664 \\
{\small GT} & {\tiny \verb|(0.0,1.5,'M160','D9')|} & 1.500 &-&-&-&-&-&-&-& 0.034 & 0.955 & 0.664 \\
{\small GT} & {\tiny \verb|GT:BBH:477|} & 1.500 &-&-&-&-&-&-&-& 0.025 & 0.955 & 0.664 \\
{\small GT} & {\tiny \verb|GT:BBH:374|} & 1.600 &-&-&-&-&-&-&-& 0.030 & 0.956 & 0.656 \\
{\small GT} & {\tiny \verb|(0.0,1.6,'M160','D9')|} & 1.600 &-&-&-&-&-&-&-& 0.034 & 0.956 & 0.656 \\
{\small GT} & {\tiny \verb|GT:BBH:615|} & 1.700 &-&-&-&-&-&-&-& 0.034 & 0.958 & 0.649 \\
{\small GT} & {\tiny \verb|(0.0,1.75)|} & 1.750 &-&-&-&-&-&-&-& 0.030 & 0.958 & 0.644 \\
{\small GT} & {\tiny \verb|(0.0,1.75,'M100')|} & 1.750 &-&-&-&-&-&-&-& 0.030 & 0.958 & 0.645 \\
{\small GT} & {\tiny \verb|GT:BBH:618|} & 1.800 &-&-&-&-&-&-&-& 0.034 & 0.959 & 0.640 \\
{\small GT} & {\tiny \verb|GT:BBH:376|} & 1.900 &-&-&-&-&-&-&-& 0.029 & 0.960 & 0.632 \\
{\small GT} & {\tiny \verb|(0.0,1.9,'M160','D9')|} & 1.900 &-&-&-&-&-&-&-& 0.034 & 0.960 & 0.632 \\
{\small GT} & {\tiny \verb|(0.0,2.0)|} & 2.000 &-&-&-&-&-&-&-& 0.030 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|(0,2.0,'M100')|} & 2.000 &-&-&-&-&-&-&-& 0.030 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|(0.0,2.0,'M160','D9')|} & 2.000 &-&-&-&-&-&-&-& 0.034 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|(0.0,2.0,'M180','D11')|} & 2.000 &-&-&-&-&-&-&-& 0.026 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|GT:BBH:446|} & 2.000 &-&-&-&-&-&-&-& 0.025 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|GT:BBH:378|} & 2.050 &-&-&-&-&-&-&-& 0.029 & 0.962 & 0.619 \\
{\small GT} & {\tiny \verb|GT:BBH:617|} & 2.100 &-&-&-&-&-&-&-& 0.034 & 0.962 & 0.615 \\
{\small GT} & {\tiny \verb|GT:BBH:379|} & 2.200 &-&-&-&-&-&-&-& 0.030 & 0.964 & 0.606 \\
{\small GT} & {\tiny \verb|(0.0,2.2,'M160','D9')|} & 2.200 &-&-&-&-&-&-&-& 0.034 & 0.963 & 0.606 \\
{\small GT} & {\tiny \verb|GT:BBH:621|} & 2.300 &-&-&-&-&-&-&-& 0.034 & 0.965 & 0.597 \\
{\small GT} & {\tiny \verb|GT:BBH:380|} & 2.350 &-&-&-&-&-&-&-& 0.030 & 0.965 & 0.593 \\
{\small GT} & {\tiny \verb|GT:BBH:622|} & 2.400 &-&-&-&-&-&-&-& 0.034 & 0.966 & 0.589 \\
{\small GT} & {\tiny \verb|(0.0,2.5)|} & 2.500 &-&-&-&-&-&-&-& 0.030 & 0.967 & 0.581 \\
{\small GT} & {\tiny \verb|(0.0,2.5,'M160','D9')|} & 2.500 &-&-&-&-&-&-&-& 0.033 & 0.967 & 0.581 \\
{\small GT} & {\tiny \verb|GT:BBH:565|} & 2.500 &-&-&-&-&-&-&-& 0.025 & 0.967 & 0.581 \\
{\small GT} & {\tiny \verb|GT:BBH:651|} & 2.600 &-&-&-&-&-&-&-& 0.033 & 0.968 & 0.572 \\
{\small GT} & {\tiny \verb|GT:BBH:650|} & 2.700 &-&-&-&-&-&-&-& 0.033 & 0.969 & 0.564 \\
{\small GT} & {\tiny \verb|GT:BBH:653|} & 2.800 &-&-&-&-&-&-&-& 0.033 & 0.970 & 0.556 \\
{\small GT} & {\tiny \verb|GT:BBH:654|} & 2.900 &-&-&-&-&-&-&-& 0.033 & 0.970 & 0.548 \\
{\small GT} & {\tiny \verb|(0.0,3.0,'M160','D9')|} & 3.000 &-&-&-&-&-&-&-& 0.033 & 0.971 & 0.540 \\
{\small GT} & {\tiny \verb|GT:BBH:453|} & 3.000 &-&-&-&-&-&-&-& 0.025 & 0.971 & 0.540 \\
{\small GT} & {\tiny \verb|GT:BBH:758|} & 3.100 &-&-&-&-&-&-&-& 0.033 & 0.972 & 0.533 \\
{\small GT} & {\tiny \verb|GT:BBH:759|} & 3.200 &-&-&-&-&-&-&-& 0.033 & 0.973 & 0.525 \\
{\small GT} & {\tiny \verb|GT:BBH:760|} & 3.300 &-&-&-&-&-&-&-& 0.033 & 0.974 & 0.518 \\
{\small GT} & {\tiny \verb|GT:BBH:761|} & 3.400 &-&-&-&-&-&-&-& 0.032 & 0.974 & 0.511 \\
{\small GT} & {\tiny \verb|GT:BBH:652|} & 3.500 &-&-&-&-&-&-&-& 0.032 & 0.975 & 0.504 \\
{\small GT} & {\tiny \verb|GT:BBH:748|} & 3.600 &-&-&-&-&-&-&-& 0.032 & 0.976 & 0.497 \\
{\small GT} & {\tiny \verb|GT:BBH:454|} & 4.000 &-&-&-&-&-&-&-& 0.025 & 0.978 & 0.472 \\
{\small GT} & {\tiny \verb|(0,4,'MXX','D11')|} & 4.000 &-&-&-&-&-&-&-& 0.025 & 0.978 & 0.472 \\
{\small GT} & {\tiny \verb|GT:BBH:656|} & 4.500 &-&-&-&-&-&-&-& 0.032 & 0.980 & 0.443 \\
{\small GT} & {\tiny \verb|GT:BBH:568|} & 9.996 &-&-&-&-&-&-&-& 0.041 & 0.992 & 0.261 \\
{\small GT} & {\tiny \verb|(0.2,1,'M100')|} & 1.000 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.028 & 0.945 & 0.746 \\
{\small GT} & {\tiny \verb|GT:BBH:420|} & 1.000 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.025 & 0.946 & 0.746 \\
{\small GT} & {\tiny \verb|GT:BBH:405|} & 1.250 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.029 & 0.946 & 0.740 \\
{\small GT} & {\tiny \verb|(0.2,1.5,'M100')|} & 1.500 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.029 & 0.949 & 0.729 \\
{\small GT} & {\tiny \verb|GT:BBH:479|} & 1.500 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.025 & 0.949 & 0.729 \\
{\small GT} & {\tiny \verb|GT:BBH:413|} & 1.750 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.029 & 0.952 & 0.714 \\
{\small GT} & {\tiny \verb|(0.2,2.0,'M100')|} & 2.000 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.030 & 0.956 & 0.698 \\
{\small GT} & {\tiny \verb|GT:BBH:471|} & 2.000 &-&-& 0.200 &-&-& 0.200 & 0.200 & 0.026 & 0.956 & 0.698 \\
{\small GT} & {\tiny \verb|GT:BBH:422|} & 1.000 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.025 & 0.938 & 0.804 \\
{\small GT} & {\tiny \verb|GT:BBH:406|} & 1.250 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.029 & 0.939 & 0.800 \\
{\small GT} & {\tiny \verb|(0.4,1.5,'M100')|} & 1.500 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.028 & 0.941 & 0.792 \\
{\small GT} & {\tiny \verb|GT:BBH:558|} & 1.500 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.025 & 0.942 & 0.792 \\
{\small GT} & {\tiny \verb|GT:BBH:414|} & 1.750 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.029 & 0.945 & 0.781 \\
{\small GT} & {\tiny \verb|(0.4,2.0,'M100')|} & 2.000 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.030 & 0.949 & 0.768 \\
{\small GT} & {\tiny \verb|GT:BBH:472|} & 2.000 &-&-& 0.400 &-&-& 0.400 & 0.400 & 0.025 & 0.949 & 0.770 \\
{\small GT} & {\tiny \verb|(0.6,1,'M100')|} & 1.000 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.028 & 0.926 & 0.858 \\
{\small GT} & {\tiny \verb|(0.6,1.0,'M200','D11')|} & 1.000 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.024 & 0.927 & 0.858 \\
{\small GT} & {\tiny \verb|GT:BBH:407|} & 1.250 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.028 & 0.928 & 0.855 \\
{\small GT} & {\tiny \verb|GT:BBH:411|} & 1.500 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.028 & 0.931 & 0.851 \\
{\small GT} & {\tiny \verb|GT:BBH:415|} & 1.750 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.029 & 0.935 & 0.845 \\
{\small GT} & {\tiny \verb|(0.6,2.0,'M100')|} & 2.000 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.030 & 0.939 & 0.839 \\
{\small GT} & {\tiny \verb|(0.6,2.0,'M160','D11')|} & 2.000 &-&-& 0.600 &-&-& 0.600 & 0.600 & 0.025 & 0.940 & 0.839 \\
{\small GT} & {\tiny \verb|(0.8,1,'M100')|} & 1.000 &-&-& 0.800 &-&-& 0.800 & 0.800 & 0.029 & 0.912 & 0.908 \\
{\small GT} & {\tiny \verb|GT:BBH:424|} & 1.000 &-&-& 0.800 &-&-& 0.800 & 0.800 & 0.025 & 0.912 & 0.909 \\
{\small GT} & {\tiny \verb|GT:BBH:546|} & 1.000 &-&-&-&-&-& 0.200 & 0.100 & 0.025 & 0.949 & 0.716 \\
{\small GT} & {\tiny \verb|GT:BBH:547|} & 1.000 &-&-&-&-&-& 0.400 & 0.200 & 0.025 & 0.945 & 0.746 \\
{\small GT} & {\tiny \verb|GT:BBH:548|} & 1.000 &-&-&-&-&-& 0.600 & 0.300 & 0.025 & 0.942 & 0.775 \\
{\small GT} & {\tiny \verb|GT:BBH:551|} & 1.000 &-&-&-&-&-& 0.800 & 0.400 & 0.025 & 0.937 & 0.802 \\
{\small GT} & {\tiny \verb|GT:BBH:549|} & 1.000 &-&-& 0.200 &-&-& 0.400 & 0.300 & 0.025 & 0.942 & 0.775 \\
{\small GT} & {\tiny \verb|GT:BBH:554|} & 1.000 &-&-& 0.200 &-&-& 0.600 & 0.400 & 0.025 & 0.937 & 0.803 \\
{\small GT} & {\tiny \verb|GT:BBH:555|} & 1.000 &-&-& 0.200 &-&-& 0.800 & 0.500 & 0.025 & 0.932 & 0.830 \\
{\small GT} & {\tiny \verb|('Unbalanced',3.0,0.0,0.0,'M240','D10')|} & 3.000 &-&-&-&-&-&-&-&-& 0.971 & 0.541 \\
{\small GT} & {\tiny \verb|('Unbalanced',3.0,0.2,0.0,'M240','D10')|} & 3.000 &-&-& 0.200 &-&-&-& 0.150 &-& 0.968 & 0.627 \\
{\small GT} & {\tiny \verb|GT:BBH:596|} & 3.000 &-&-& 0.400 &-&-&-& 0.300 &-& 0.963 & 0.713 \\
{\small GT} & {\tiny \verb|GT:BBH:600|} & 3.000 &-&-& 0.600 &-&-&-& 0.450 &-& 0.957 & 0.796 \\
{\small GT} & {\tiny \verb|('Unbalanced',4.0,0.0,0.0,'M240','D10')|} & 4.000 &-&-&-&-&-&-&-&-& 0.978 & 0.472 \\
{\small GT} & {\tiny \verb|GT:BBH:570|} & 4.000 &-&-& 0.200 &-&-&-& 0.160 &-& 0.975 & 0.577 \\
{\small GT} & {\tiny \verb|GT:BBH:573|} & 4.000 &-&-& 0.400 &-&-&-& 0.320 &-& 0.971 & 0.678 \\
{\small GT} & {\tiny \verb|GT:BBH:578|} & 4.000 &-&-& 0.600 &-&-&-& 0.480 &-& 0.965 & 0.778 \\
{\small GT} & {\tiny \verb|GT:BBH:765|} & 5.000 &-&-& -0.730 &-&-&-& -0.608 &-& 0.987 & -0.022 \\
{\small GT} & {\tiny \verb|GT:BBH:769|} & 5.000 &-&-& -0.720 &-&-&-& -0.600 &-& 0.987 & -0.016 \\
{\small GT} & {\tiny \verb|GT:BBH:768|} & 5.000 &-&-& -0.710 &-&-&-& -0.592 &-& 0.987 & -0.010 \\
{\small GT} & {\tiny \verb|GT:BBH:577|} & 5.000 &-&-&-&-&-&-&-&-& 0.982 & 0.417 \\
{\small GT} & {\tiny \verb|GT:BBH:599|} & 5.000 &-&-& 0.200 &-&-&-& 0.167 &-& 0.980 & 0.535 \\
{\small GT} & {\tiny \verb|GT:BBH:602|} & 5.000 &-&-& 0.400 &-&-&-& 0.333 &-& 0.977 & 0.650 \\
{\small GT} & {\tiny \verb|GT:BBH:611|} & 5.000 &-&-& 0.600 &-&-&-& 0.500 &-& 0.972 & 0.762 \\
{\small GT} & {\tiny \verb|GT:BBH:604|} & 6.000 &-&-&-&-&-&-&-&-& 0.986 & 0.373 \\
{\small GT} & {\tiny \verb|GT:BBH:608|} & 6.000 &-&-& 0.200 &-&-&-& 0.171 &-& 0.983 & 0.501 \\
{\small GT} & {\tiny \verb|GT:BBH:610|} & 6.000 &-&-& 0.400 &-&-&-& 0.343 &-& 0.981 & 0.626 \\
{\small GT} & {\tiny \verb|GT:BBH:612|} & 6.000 &-&-& 0.600 &-&-&-& 0.514 &-& 0.976 & 0.748 \\
{\small GT} & {\tiny \verb|('Unbalanced',7.0,0.0,0.0,'M320','D10')|} & 7.000 &-&-&-&-&-&-&-&-& 0.988 & 0.337 \\
{\small GT} & {\tiny \verb|GT:BBH:688|} & 7.000 &-&-& 0.200 &-&-&-& 0.175 &-& 0.986 & 0.472 \\
{\small GT} & {\tiny \verb|GT:BBH:740|} & 7.000 &-&-& 0.400 &-&-&-& 0.350 &-& 0.983 & 0.606 \\
{\small GT} & {\tiny \verb|GT:BBH:456|} & 1.500 & 0.346 &-& 0.200 &-&-& 0.400 & 0.280 & 0.024 & 0.947 & 0.753 \\
{\small GT} & {\tiny \verb|GT:BBH:455|} & 1.500 & 0.424 &-& 0.424 &-&-& 0.600 & 0.495 & 0.020 & 0.937 & 0.822 \\
{\small GT} & {\tiny \verb|GT:BBH:457|} & 1.500 & 0.520 &-& 0.300 &-&-& 0.600 & 0.420 & 0.021 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:764|} & 1.500 & 0.600 &-&-&-&-& 0.600 & 0.240 & 0.021 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:458|} & 2.000 & 0.346 &-& 0.200 &-&-& 0.400 & 0.267 & 0.023 & 0.954 & 0.722 \\
{\small GT} & {\tiny \verb|GT:BBH:460|} & 2.000 & 0.424 &-& 0.424 &-&-& 0.600 & 0.483 & 0.023 & 0.945 & 0.804 \\
{\small GT} & {\tiny \verb|GT:BBH:461|} & 2.000 & 0.520 &-& 0.300 &-&-& 0.600 & 0.400 & 0.021 & 0.948 & 0.777 \\
{\small GT} & {\tiny \verb|GT:BBH:463|} & 2.000 & 0.600 &-&-&-&-& 0.600 & 0.200 & 0.011 & 0.955 & 0.698 \\
{\small GT} & {\tiny \verb|GT:BBH:459|} & 2.500 & 0.283 &-& 0.283 &-&-& 0.400 & 0.316 & 0.033 & 0.958 & 0.715 \\
{\small GT} & {\tiny \verb|GT:BBH:462|} & 2.500 & 0.346 &-& 0.200 &-&-& 0.400 & 0.257 & 0.032 & 0.960 & 0.693 \\
{\small GT} & {\tiny \verb|GT:BBH:464|} & 2.500 & 0.400 &-&-&-&-& 0.400 & 0.114 & 0.019 & 0.964 & 0.626 \\
{\small GT} & {\tiny \verb|GT:BBH:465|} & 2.500 & 0.424 &-& 0.424 &-&-& 0.600 & 0.475 & 0.062 & 0.952 & 0.787 \\
{\small GT} & {\tiny \verb|GT:BBH:466|} & 2.500 & 0.520 &-& 0.300 &-&-& 0.600 & 0.386 & 0.054 & 0.955 & 0.756 \\
{\small GT} & {\tiny \verb|GT:BBH:467|} & 2.500 & 0.600 &-&-&-&-& 0.600 & 0.171 & 0.033 & 0.962 & 0.671 \\
{\small GT} & {\tiny \verb|GT:BBH:468|} & 4.000 & 0.424 &-& 0.424 &-&-& 0.600 & 0.459 & 0.022 & 0.968 & 0.749 \\
{\small GT} & {\tiny \verb|GT:BBH:469|} & 4.000 & 0.520 &-& 0.300 &-&-& 0.600 & 0.360 & 0.016 & 0.970 & 0.715 \\
{\small GT} & {\tiny \verb|GT:BBH:470|} & 4.000 & 0.600 &-&-&-&-& 0.600 & 0.120 & 0.037 & 0.975 & 0.610 \\
{\small GT} & {\tiny \verb|GT:BBH:428|} & 2.000 &-&-& 0.600 & -0.600 &-&-& 0.400 & 0.053 & 0.946 & 0.809 \\
{\small GT} & {\tiny \verb|GT:BBH:431|} & 2.000 & 0.300 &-& 0.520 & -0.600 &-&-& 0.346 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:434|} & 2.000 & 0.600 &-&-& -0.600 &-&-&-& 0.060 & 0.960 & 0.652 \\
{\small GT} & {\tiny \verb|GT:BBH:437|} & 2.000 & 0.300 &-& -0.520 & -0.600 &-&-& -0.346 & 0.059 & 0.969 & 0.457 \\
{\small GT} & {\tiny \verb|GT:BBH:440|} & 2.000 &-&-& -0.600 & -0.600 &-&-& -0.400 & 0.060 & 0.970 & 0.429 \\
{\small GT} & {\tiny \verb|GT:BBH:443|} & 2.000 & -0.600 &-& - & -0.600 &-&-& - & 0.056 & X & X \\
{\small GT} & {\tiny \verb|Sq4_d6.2_a0.6_oth.000_rr_M140|} & 4.000 &-&-& 0.600 & -0.600 &-&-& 0.480 & 0.048 & 0.966 & 0.781 \\
{\small GT} & {\tiny \verb|GT:BBH:432|} & 4.000 & 0.300 &-& 0.520 & -0.600 &-&-& 0.416 & 0.044 & 0.967 & 0.758 \\
{\small GT} & {\tiny \verb|Sq4_d6.2_a0.6_oth.090_rr_M140|} & 4.000 & 0.600 &-&-& -0.600 &-&-&-& 0.054 & 0.977 & 0.594 \\
{\small GT} & {\tiny \verb|Sq4_d6.2_a0.6_oth.150_rr_M140|} & 4.000 & 0.300 &-& -0.520 & -0.600 &-&-& -0.416 & 0.068 & 0.983 & 0.255 \\
{\small GT} & {\tiny \verb|Sq4_d6.2_a0.6_oth.180_rr_M140|} & 4.000 &-&-& -0.600 & -0.600 &-&-& -0.480 & 0.066 & 0.983 & 0.146 \\
{\small GT} & {\tiny \verb|Sq4_d6.2_a0.6_oth.270_rr_M140|} & 4.000 & -0.600 & - & - & -0.600 &-&-& - & 0.043 & 0.976 & 0.616 \\
{\small GT} & {\tiny \verb|GT:BBH:430|} & 4.000 &-&-& 0.600 & -0.600 &-&-& 0.480 & 0.023 & 0.965 & 0.779 \\
{\small GT} & {\tiny \verb|GT:BBH:433|} & 4.000 & 0.600 &-&-& -0.600 &-&-&-& 0.046 & 0.976 & 0.593 \\
{\small GT} & {\tiny \verb|GT:BBH:435|} & 4.000 & 0.300 &-& -0.520 & -0.600 &-&-& -0.416 & 0.056 & 0.983 & 0.258 \\
{\small GT} & {\tiny \verb|GT:BBH:438|} & 4.000 &-&-& -0.600 & -0.600 &-&-& -0.480 & 0.042 & 0.983 & 0.150 \\
{\small GT} & {\tiny \verb|GT:BBH:441|} & 4.000 & -0.300 &-& -0.520 & -0.600 &-&-& -0.416 & 0.033 & 0.982 & 0.285 \\
{\small GT} & {\tiny \verb|Sq4_d9_a0.6_oth.270_rr_M100|} & 4.000 & -0.601 & - &-& -0.601 & - &-&-& 0.049 & X & X \\
{\small GT} & {\tiny \verb|Sq4_d9_a0.6_oth.270_rr_M120|} & 4.000 & -0.601 & - &-& -0.601 & - &-&-& 0.049 & 0.975 & 0.613 \\
{\small GT} & {\tiny \verb|Sq4_d9_a0.6_oth.270_rr_M140|} & 4.000 & -0.600 &-& - & -0.600 &-&-& - & 0.036 & 0.975 & 0.612 \\
{\small GT} & {\tiny \verb|Sq4_d9_a0.6_oth.270_rr_M160|} & 4.000 & -0.601 & - &-& -0.601 & - &-&-& 0.031 & 0.975 & 0.612 \\
{\small GT} & {\tiny \verb|GT:BBH:560|} & 4.000 & -0.600 &-& - & -0.600 &-&-& - & 0.035 & 0.975 & 0.613 \\
{\small GT} & {\tiny \verb|GT:BBH:647|} & 2.500 &-&-& 0.600 & -0.600 &-&-& 0.429 & 0.057 & 0.952 & 0.805 \\
{\small GT} & {\tiny \verb|GT:BBH:648|} & 2.500 & 0.155 &-& 0.580 & -0.600 &-&-& 0.414 & 0.057 & 0.952 & 0.797 \\
{\small GT} & {\tiny \verb|GT:BBH:649|} & 2.500 & 0.300 &-& 0.520 & -0.600 &-&-& 0.371 & 0.056 & 0.955 & 0.783 \\
{\small GT} & {\tiny \verb|GT:BBH:646|} & 2.500 & 0.424 &-& 0.424 & -0.600 &-&-& 0.303 & 0.053 & 0.957 & 0.758 \\
{\small GT} & {\tiny \verb|GT:BBH:645|} & 2.500 & 0.520 &-& 0.300 & -0.600 &-&-& 0.214 & 0.048 & 0.958 & 0.724 \\
{\small GT} & {\tiny \verb|GT:BBH:644|} & 2.500 & 0.580 &-& 0.155 & -0.600 &-&-& 0.111 & 0.046 & 0.963 & 0.686 \\
{\small GT} & {\tiny \verb|Sq_D6.2_q2.50_a0.6_th090_m140|} & 2.499 & 0.600 & 0.005 & -0.001 & -0.600 & -0.030 & -0.002 & -0.001 & 0.050 & 0.965 & 0.631 \\
{\small GT} & {\tiny \verb|GT:BBH:642|} & 2.500 & 0.520 &-& -0.300 & -0.600 &-&-& -0.214 & 0.055 & 0.970 & 0.510 \\
{\small GT} & {\tiny \verb|GT:BBH:659|} & 2.500 & 0.300 &-& -0.520 & -0.600 &-&-& -0.371 & 0.060 & 0.974 & 0.389 \\
{\small GT} & {\tiny \verb|GT:BBH:660|} & 2.500 &-&-& -0.600 & -0.600 &-&-& -0.429 & 0.064 & 0.975 & 0.344 \\
{\small GT} & {\tiny \verb|GT:BBH:667|} & 2.500 & -0.300 & - & -0.520 & -0.600 &-&-& -0.371 & 0.065 & 0.973 & 0.421 \\
{\small GT} & {\tiny \verb|GT:BBH:663|} & 2.500 & -0.520 & - & -0.300 & -0.600 &-&-& -0.214 & 0.060 & 0.970 & 0.552 \\
{\small GT} & {\tiny \verb|GT:BBH:662|} & 2.500 & -0.600 & - & - & -0.600 &-&-&-& 0.048 & 0.964 & 0.668 \\
{\small GT} & {\tiny \verb|GT:BBH:628|} & 2.500 & -0.520 & - & 0.300 & -0.600 &-&-& 0.214 & 0.055 & 0.958 & 0.750 \\
{\small GT} & {\tiny \verb|GT:BBH:630|} & 2.500 & -0.424 & - & 0.424 & -0.600 &-&-& 0.303 & 0.049 & 0.955 & 0.776 \\
{\small GT} & {\tiny \verb|GT:BBH:666|} & 2.500 & -0.300 & - & 0.520 & -0.600 &-&-& 0.371 & 0.045 & 0.953 & 0.795 \\
{\small GT} & {\tiny \verb|GT:BBH:668|} & 2.500 & -0.155 & - & 0.580 & -0.600 &-&-& 0.414 & 0.052 & 0.952 & 0.804 \\
{\small GT} & {\tiny \verb|GT:BBH:694|} & 3.000 &-&-& 0.600 & -0.600 &-&-& 0.450 & 0.058 & 0.957 & 0.798 \\
{\small GT} & {\tiny \verb|GT:BBH:698|} & 3.000 & 0.155 &-& 0.580 & -0.600 &-&-& 0.435 & 0.056 & 0.958 & 0.791 \\
{\small GT} & {\tiny \verb|GT:BBH:689|} & 3.000 & 0.300 &-& 0.520 & -0.600 &-&-& 0.390 & 0.053 & 0.959 & 0.774 \\
{\small GT} & {\tiny \verb|GT:BBH:690|} & 3.000 & 0.424 &-& 0.424 & -0.600 &-&-& 0.318 & 0.050 & 0.962 & 0.752 \\
{\small GT} & {\tiny \verb|GT:BBH:691|} & 3.000 & 0.520 &-& 0.300 & -0.600 &-&-& 0.225 & 0.047 & 0.964 & 0.715 \\
{\small GT} & {\tiny \verb|GT:BBH:692|} & 3.000 & 0.580 &-& 0.155 & -0.600 &-&-& 0.116 & 0.043 & 0.967 & 0.674 \\
{\small GT} & {\tiny \verb|GT:BBH:693|} & 3.000 & 0.600 &-&-& -0.600 &-&-&-& 0.046 & 0.969 & 0.615 \\
{\small GT} & {\tiny \verb|GT:BBH:685|} & 3.000 & 0.520 &-& -0.300 & -0.600 &-&-& -0.225 & 0.054 & 0.975 & 0.479 \\
{\small GT} & {\tiny \verb|GT:BBH:686|} & 3.000 & 0.300 &-& -0.520 & -0.600 &-&-& -0.390 & 0.065 & 0.978 & 0.333 \\
{\small GT} & {\tiny \verb|GT:BBH:710|} & 3.000 &-&-& -0.600 & -0.600 &-&-& -0.450 & 0.068 & 0.978 & 0.269 \\
{\small GT} & {\tiny \verb|GT:BBH:709|} & 3.000 & -0.300 & - & -0.520 & -0.600 &-&-& -0.390 & 0.064 & 0.977 & 0.364 \\
{\small GT} & {\tiny \verb|GT:BBH:713|} & 3.000 & -0.520 & - & -0.300 & -0.600 &-&-& -0.225 & 0.054 & 0.974 & 0.517 \\
{\small GT} & {\tiny \verb|GT:BBH:714|} & 3.000 & -0.600 & - & - & -0.600 &-&-&-& 0.040 & 0.969 & 0.648 \\
{\small GT} & {\tiny \verb|GT:BBH:723|} & 3.000 & -0.520 & - & 0.300 & -0.600 &-&-& 0.225 & 0.048 & 0.963 & 0.736 \\
{\small GT} & {\tiny \verb|GT:BBH:720|} & 3.000 & -0.424 & - & 0.424 & -0.600 &-&-& 0.318 & 0.040 & 0.960 & 0.765 \\
{\small GT} & {\tiny \verb|GT:BBH:721|} & 3.000 & -0.300 & - & 0.520 & -0.600 &-&-& 0.390 & 0.046 & 0.959 & 0.785 \\
{\small GT} & {\tiny \verb|GT:BBH:722|} & 3.000 & -0.155 & - & 0.580 & -0.600 &-&-& 0.435 & 0.057 & 0.957 & 0.796 \\
{\small GT} & {\tiny \verb|GT:BBH:550|} & 2.000 & 0.424 &-& -0.424 &-&-& 0.600 & -0.083 & 0.032 & 0.964 & 0.549 \\
{\small GT} & {\tiny \verb|GT:BBH:545|} & 2.000 &-&-& -0.600 &-&-& 0.600 & -0.200 & 0.033 & 0.967 & 0.465 \\
{\small GT} & {\tiny \verb|GT:BBH:556|} & 2.000 & -0.600 &-& - &-&-& 0.600 & 0.200 & 0.032 & 0.955 & 0.698 \\
{\small GT} & {\tiny \verb|EK_D6.2_a0.6_th000_M77|} & 1.000 & 0.584 & 0.143 & 0.002 & -0.584 & -0.143 & 0.002 & 0.002 & 0.070 & 0.951 & 0.686 \\
{\small GT} & {\tiny \verb|GT:BBH:482|} & 1.000 & 0.520 & 0.300 &-& -0.520 & -0.300 &-&-& 0.071 & 0.951 & 0.684 \\
{\small GT} & {\tiny \verb|GT:BBH:483|} & 1.000 & 0.424 & 0.424 &-& -0.424 & -0.424 &-&-& 0.071 & 0.950 & 0.683 \\
{\small GT} & {\tiny \verb|GT:BBH:484|} & 1.000 & 0.300 & 0.520 &-& -0.300 & -0.520 &-&-& 0.072 & 0.950 & 0.681 \\
{\small GT} & {\tiny \verb|GT:BBH:485|} & 1.000 &-& 0.600 &-& - & -0.600 &-&-& 0.072 & 0.949 & 0.680 \\
{\small GT} & {\tiny \verb|GT:BBH:486|} & 1.000 & -0.300 & 0.520 &-& 0.300 & -0.520 &-&-& 0.072 & 0.950 & 0.682 \\
{\small GT} & {\tiny \verb|GT:BBH:487|} & 1.000 & -0.520 & 0.300 &-& 0.520 & -0.300 &-&-& 0.071 & 0.951 & 0.685 \\
{\small GT} & {\tiny \verb|EK_D6.2_a0.6_th180_M77|} & 1.000 & -0.584 & -0.143 & 0.002 & 0.584 & 0.143 & 0.002 & 0.002 & 0.071 & 0.951 & 0.686 \\
{\small GT} & {\tiny \verb|GT:BBH:489|} & 1.000 & -0.520 & -0.300 &-& 0.520 & 0.300 &-&-& 0.072 & 0.951 & 0.684 \\
{\small GT} & {\tiny \verb|GT:BBH:490|} & 1.000 & -0.300 & -0.520 &-& 0.300 & 0.520 &-&-& 0.072 & 0.950 & 0.681 \\
{\small GT} & {\tiny \verb|GT:BBH:491|} & 1.000 & - & -0.600 &-&-& 0.600 &-&-& 0.072 & 0.949 & 0.680 \\
{\small GT} & {\tiny \verb|GT:BBH:492|} & 1.000 & 0.300 & -0.520 &-& -0.300 & 0.520 &-&-& 0.072 & 0.950 & 0.682 \\
{\small GT} & {\tiny \verb|GT:BBH:493|} & 1.000 & 0.520 & -0.300 &-& -0.520 & 0.300 &-&-& 0.071 & 0.951 & 0.685 \\
{\small GT} & {\tiny \verb|GT:BBH:500|} & 1.000 & 0.336 &-& 0.497 & -0.336 &-& 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:501|} & 1.000 & 0.291 & 0.168 & 0.497 & -0.291 & -0.168 & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:502|} & 1.000 & 0.237 & 0.237 & 0.497 & -0.237 & -0.237 & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:503|} & 1.000 & 0.168 & 0.291 & 0.497 & -0.168 & -0.291 & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:504|} & 1.000 &-& 0.336 & 0.497 & - & -0.336 & 0.497 & 0.497 & 0.060 & 0.932 & 0.827 \\
{\small GT} & {\tiny \verb|GT:BBH:505|} & 1.000 & -0.168 & 0.291 & 0.497 & 0.168 & -0.291 & 0.497 & 0.497 & 0.060 & 0.933 & 0.828 \\
{\small GT} & {\tiny \verb|GT:BBH:506|} & 1.000 & -0.291 & 0.168 & 0.497 & 0.291 & -0.168 & 0.497 & 0.497 & 0.060 & 0.933 & 0.829 \\
{\small GT} & {\tiny \verb|GT:BBH:507|} & 1.000 & -0.336 &-& 0.497 & 0.336 & - & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:508|} & 1.000 & -0.291 & -0.168 & 0.497 & 0.291 & 0.168 & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:509|} & 1.000 & -0.168 & -0.291 & 0.497 & 0.168 & 0.291 & 0.497 & 0.497 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:510|} & 1.000 & - & -0.336 & 0.497 &-& 0.336 & 0.497 & 0.497 & 0.060 & 0.932 & 0.827 \\
{\small GT} & {\tiny \verb|GT:BBH:511|} & 1.000 & 0.168 & -0.291 & 0.497 & -0.168 & 0.291 & 0.497 & 0.497 & 0.060 & 0.933 & 0.828 \\
{\small GT} & {\tiny \verb|GT:BBH:512|} & 1.000 & 0.291 & -0.168 & 0.497 & -0.291 & 0.168 & 0.497 & 0.497 & 0.060 & 0.933 & 0.829 \\
{\small GT} & {\tiny \verb|GT:BBH:513|} & 1.000 & 0.548 &-& 0.244 & -0.548 &-& 0.244 & 0.244 & 0.063 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:514|} & 1.000 & 0.475 & 0.274 & 0.244 & -0.475 & -0.274 & 0.244 & 0.244 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:515|} & 1.000 & 0.274 & 0.475 & 0.244 & -0.274 & -0.475 & 0.244 & 0.244 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:516|} & 1.000 &-& 0.548 & 0.244 & - & -0.548 & 0.244 & 0.244 & 0.065 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:517|} & 1.000 & -0.274 & 0.475 & 0.244 & 0.274 & -0.475 & 0.244 & 0.244 & 0.065 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:518|} & 1.000 & -0.475 & 0.274 & 0.244 & 0.475 & -0.274 & 0.244 & 0.244 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|aa_b5_a0.2_M77|} & 1.000 &-&-& 0.200 &-&-& -0.200 &-& 0.027 & X & X \\
{\small GT} & {\tiny \verb|aa_b5_a0.4_M77|} & 1.000 &-&-& 0.400 &-&-& -0.400 &-& 0.028 & X & X \\
{\small GT} & {\tiny \verb|aa_b5_a0.6_M77|} & 1.000 &-&-& 0.600 &-&-& -0.600 &-& 0.029 & X & X \\
{\small GT} & {\tiny \verb|aa_b5_a0.8_M77|} & 1.000 &-&-& 0.800 &-&-& -0.800 &-& 0.031 & X & X \\
{\small GT} & {\tiny \verb|fr_b5_a0.6_random2_M77|} & 1.000 &-&-& 0.600 &-&-& -0.600 &-& 0.027 & X & X \\
{\small GT} & {\tiny \verb|fr_b5_a0.6_random_M77|} & 1.000 & -0.212 & -0.367 & 0.424 &-&-& 0.600 & 0.512 & 0.028 & X & X \\
{\small GT} & {\tiny \verb|ro_b5_a0.6_oth.000_M077|} & 1.000 & 0.424 &-& 0.424 &-&-& 0.600 & 0.512 & 0.026 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:803|} & 1.000 & 0.424 &-& 0.424 &-&-& 0.600 & 0.512 & 0.027 & X & X \\
{\small GT} & {\tiny \verb|ro_b5_a0.6_oth.120_M077|} & 1.000 & -0.212 & 0.367 & 0.424 &-&-& 0.600 & 0.512 & 0.027 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:805|} & 1.000 & -0.212 & 0.367 & 0.424 &-&-& 0.600 & 0.512 & 0.028 & X & X \\
{\small GT} & {\tiny \verb|ro_b5_a0.6_oth.240_M077|} & 1.000 & -0.212 & -0.367 & 0.424 &-&-& 0.600 & 0.512 & 0.027 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:807|} & 1.000 & -0.212 & -0.367 & 0.424 &-&-& 0.600 & 0.512 & 0.028 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.000_M77|} & 1.000 &-&-& 0.600 & -0.600 &-&-& 0.300 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.015_M77|} & 1.000 & 0.155 &-& 0.580 & -0.600 &-&-& 0.290 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.030_M77|} & 1.000 & 0.300 &-& 0.520 & -0.600 &-&-& 0.260 & 0.058 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.045_M77|} & 1.000 & 0.424 &-& 0.424 & -0.600 &-&-& 0.212 & 0.058 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.060_M77|} & 1.000 & 0.520 &-& 0.300 & -0.600 &-&-& 0.150 & 0.059 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.075_M77|} & 1.000 & 0.580 &-& 0.155 & -0.600 &-&-& 0.078 & 0.060 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.090_M77|} & 1.000 & 0.600 &-&-& -0.600 &-&-&-& 0.062 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.105_M77|} & 1.000 & 0.580 &-& -0.155 & -0.600 &-&-& -0.078 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.120_M77|} & 1.000 & 0.520 &-& -0.300 & -0.600 &-&-& -0.150 & 0.066 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.135_M77|} & 1.000 & 0.424 &-& -0.424 & -0.600 &-&-& -0.212 & 0.068 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.150_M77|} & 1.000 & 0.300 &-& -0.520 & -0.600 &-&-& -0.260 & 0.070 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.165_M77|} & 1.000 & 0.155 &-& -0.580 & -0.600 &-&-& -0.290 & 0.071 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.180_M77|} & 1.000 &-&-& -0.600 & -0.600 &-&-& -0.300 & 0.071 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.195_M77|} & 1.000 & -0.155 &-& -0.580 & -0.600 &-&-& -0.290 & 0.069 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.210_M77|} & 1.000 & -0.300 &-& -0.520 & -0.600 &-&-& -0.260 & 0.067 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.225_M77|} & 1.000 & -0.424 &-& -0.424 & -0.600 &-&-& -0.212 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.240_M77|} & 1.000 & -0.520 &-& -0.300 & -0.600 &-&-& -0.150 & 0.061 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.255_M77|} & 1.000 & -0.580 &-& -0.155 & -0.600 &-&-& -0.078 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.260_M77|} & 1.000 & -0.591 &-& -0.104 & -0.600 &-&-& -0.052 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.265_M77|} & 1.000 & -0.598 &-& -0.052 & -0.600 &-&-& -0.026 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.270_M77|} & 1.000 & -0.600 &-& - & -0.600 &-&-& - & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.285_M77|} & 1.000 & -0.580 &-& 0.155 & -0.600 &-&-& 0.078 & 0.055 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.300_M77|} & 1.000 & -0.520 &-& 0.300 & -0.600 &-&-& 0.150 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.315_M77|} & 1.000 & -0.424 &-& 0.424 & -0.600 &-&-& 0.212 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.330_M77|} & 1.000 & -0.300 &-& 0.520 & -0.600 &-&-& 0.260 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|fr_b3.1_a0.6_oth.345_M77|} & 1.000 & -0.155 &-& 0.580 & -0.600 &-&-& 0.290 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:382|} & 1.000 &-&-& 0.800 & -0.800 &-&-& 0.400 & 0.057 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:384|} & 1.000 & 0.400 &-& 0.693 & -0.800 &-&-& 0.346 & 0.056 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:385|} & 1.000 & 0.693 &-& 0.400 & -0.800 &-&-& 0.200 & 0.055 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:388|} & 1.000 & 0.800 &-&-& -0.800 &-&-&-& 0.058 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:390|} & 1.000 & 0.693 &-& -0.400 & -0.800 &-&-& -0.200 & 0.065 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:391|} & 1.000 & 0.400 &-& -0.693 & -0.800 &-&-& -0.346 & 0.069 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:393|} & 1.000 &-&-& -0.800 & -0.800 &-&-& -0.400 & 0.071 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:395|} & 1.000 & -0.400 &-& -0.693 & -0.800 &-&-& -0.346 & 0.064 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:396|} & 1.000 & -0.693 &-& -0.400 & -0.800 &-&-& -0.200 & 0.054 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:397|} & 1.000 & -0.773 &-& -0.207 & -0.800 &-&-& -0.104 & 0.051 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:398|} & 1.000 & -0.800 &-& - & -0.800 &-&-& - & 0.051 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:400|} & 1.000 & -0.693 &-& 0.400 & -0.800 &-&-& 0.200 & 0.051 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:401|} & 1.000 & -0.400 &-& 0.693 & -0.800 &-&-& 0.346 & 0.054 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.000_M77|} & 1.000 &-&-& 0.600 & -0.600 & -0.001 &-& 0.300 & 0.038 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.045_M77|} & 1.000 & 0.424 &-& 0.424 & -0.600 & -0.001 &-& 0.212 & 0.034 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.090_M77|} & 1.000 & 0.600 & 0.001 &-& -0.600 & -0.001 &-&-& 0.037 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.135_M77|} & 1.000 & 0.424 & 0.001 & -0.424 & -0.600 & -0.001 & - & -0.212 & 0.039 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.180_M77|} & 1.000 & - & - & -0.600 & -0.600 & -0.001 & - & -0.300 & 0.039 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.225_M77|} & 1.000 & -0.424 & -0.001 & -0.424 & -0.600 & -0.001 & - & -0.212 & 0.038 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.240_M77|} & 1.000 & -0.520 & -0.001 & -0.300 & -0.600 & -0.001 &-& -0.150 & 0.038 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.255_M77|} & 1.000 & -0.580 & -0.001 & -0.155 & -0.600 & -0.001 &-& -0.078 & 0.037 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.270_M77|} & 1.000 & -0.600 & -0.001 &-& -0.600 & -0.001 &-&-& 0.036 & X & X \\
{\small GT} & {\tiny \verb|fr_b4_a0.6_oth.315_M77|} & 1.000 & -0.424 & - & 0.424 & -0.600 & -0.001 &-& 0.212 & 0.039 & X & X \\
{\small GT} & {\tiny \verb|D10_q7.00_a0.0_m320|} & 7.000 &-&-&-&-&-&-&-&-& X & X \\
{\small GT} & {\tiny \verb|GT:BBH:860|} & 1.000 & 0.109 & 0.481 & 0.342 & 0.460 & -0.287 & 0.257 & 0.299 & 0.042 & 0.940 & 0.783 \\
{\small GT} & {\tiny \verb|GT:BBH:861|} & 1.000 & -0.159 & -0.414 & -0.404 & 0.297 & 0.521 & -0.020 & -0.212 & 0.049 & 0.957 & 0.620 \\
{\small GT} & {\tiny \verb|GT:BBH:862|} & 1.000 & 0.542 & -0.255 & -0.034 & 0.053 & 0.188 & -0.567 & -0.301 & 0.053 & 0.958 & 0.607 \\
{\small GT} & {\tiny \verb|GT:BBH:863|} & 1.000 & -0.512 & 0.270 & -0.157 & -0.506 & -0.175 & -0.270 & -0.214 & 0.053 & 0.956 & 0.663 \\
{\small GT} & {\tiny \verb|GT:BBH:864|} & 1.000 & -0.269 & -0.536 & -0.014 & -0.269 & -0.536 & -0.014 & -0.014 & 0.046 & 0.949 & 0.736 \\
{\small GT} & {\tiny \verb|GT:BBH:865|} & 1.000 & -0.096 & 0.467 & 0.364 & 0.208 & 0.562 & 0.033 & 0.199 & 0.043 & 0.943 & 0.782 \\
{\small GT} & {\tiny \verb|GT:BBH:866|} & 1.000 & -0.354 & 0.233 & 0.424 & 0.494 & -0.341 & -0.001 & 0.212 & 0.042 & 0.945 & 0.749 \\
{\small GT} & {\tiny \verb|GT:BBH:867|} & 1.000 & 0.599 & 0.030 & - & -0.599 & -0.030 & - &-& 0.045 & 0.949 & 0.679 \\
{\small GT} & {\tiny \verb|GT:BBH:603|} & 3.000 &-&-& 0.500 &-&-&-& 0.375 & 0.032 & 0.960 & 0.755 \\
{\small GT} & {\tiny \verb|GT:BBH:607|} & 3.000 & -0.276 & 0.148 & 0.390 &-&-&-& 0.292 & 0.032 & 0.963 & 0.718 \\
{\small GT} & {\tiny \verb|GT:BBH:613|} & 3.000 & 0.176 & -0.221 & 0.413 &-&-&-& 0.309 & 0.033 & 0.963 & 0.718 \\
{\small GT} & {\tiny \verb|GT:BBH:626|} & 3.000 & 0.179 & 0.254 & 0.392 &-&-&-& 0.294 & 0.031 & 0.964 & 0.719 \\
{\small GT} & {\tiny \verb|GT:BBH:606|} & 3.000 & -0.411 & 0.149 & 0.242 &-&-&-& 0.182 & 0.033 & 0.965 & 0.689 \\
{\small GT} & {\tiny \verb|GT:BBH:739|} & 3.000 & -0.162 & -0.326 & 0.343 &-&-&-& 0.257 & 0.033 & 0.965 & 0.688 \\
{\small GT} & {\tiny \verb|GT:BBH:744|} & 3.000 & 0.411 & -0.149 & 0.242 &-&-&-& 0.182 & 0.032 & 0.965 & 0.689 \\
{\small GT} & {\tiny \verb|GT:BBH:741|} & 3.000 & 0.162 & 0.326 & 0.343 &-&-&-& 0.257 & 0.034 & 0.965 & 0.689 \\
{\small GT} & {\tiny \verb|GT:BBH:605|} & 3.000 & 0.464 & -0.182 & 0.046 &-&-&-& 0.035 & 0.038 & 0.970 & 0.604 \\
{\small GT} & {\tiny \verb|GT:BBH:657|} & 3.000 & -0.201 & 0.405 & 0.213 &-&-&-& 0.160 & 0.042 & 0.970 & 0.602 \\
{\small GT} & {\tiny \verb|GT:BBH:636|} & 3.000 & -0.500 & 0.019 & -0.001 &-&-&-& -0.001 & 0.039 & 0.970 & 0.605 \\
{\small GT} & {\tiny \verb|GT:BBH:724|} & 3.000 & -0.464 & 0.182 & 0.046 &-&-&-& 0.035 & 0.040 & 0.970 & 0.604 \\
{\small GT} & {\tiny \verb|GT:BBH:635|} & 3.000 & 0.201 & -0.405 & 0.213 &-&-&-& 0.160 & 0.040 & 0.970 & 0.602 \\
{\small GT} & {\tiny \verb|GT:BBH:680|} & 3.000 & 0.500 & -0.019 & -0.001 &-&-&-& -0.001 & 0.039 & 0.970 & 0.605 \\
{\small GT} & {\tiny \verb|GT:BBH:609|} & 3.000 & -0.335 & -0.317 & -0.192 &-&-&-& -0.144 & 0.042 & 0.974 & 0.488 \\
{\small GT} & {\tiny \verb|GT:BBH:743|} & 3.000 & 0.267 & -0.412 & -0.094 &-&-&-& -0.070 & 0.042 & 0.974 & 0.490 \\
{\small GT} & {\tiny \verb|GT:BBH:747|} & 3.000 & 0.335 & 0.317 & -0.192 &-&-&-& -0.144 & 0.041 & 0.974 & 0.488 \\
{\small GT} & {\tiny \verb|GT:BBH:746|} & 3.000 & -0.267 & 0.412 & -0.094 &-&-&-& -0.070 & 0.043 & 0.974 & 0.490 \\
{\small GT} & {\tiny \verb|GT:BBH:684|} & 3.000 & 0.289 & -0.281 & -0.296 &-&-&-& -0.222 & 0.043 & 0.975 & 0.427 \\
{\small GT} & {\tiny \verb|GT:BBH:726|} & 3.000 & -0.197 & 0.385 & -0.251 &-&-&-& -0.188 & 0.044 & 0.975 & 0.427 \\
{\small GT} & {\tiny \verb|GT:BBH:735|} & 3.000 & -0.155 & -0.394 & -0.265 &-&-&-& -0.199 & 0.043 & 0.975 & 0.428 \\
{\small GT} & {\tiny \verb|D9_q1.0_a0.0_m160|} & 1.000 &-&-& - &-&-& - & - & 0.036 & 0.952 & 0.686 \\
{\small GT} & {\tiny \verb|GT:BBH:717|} & 1.100 &-&-&-&-&-&-&-& 0.036 & 0.952 & 0.685 \\
{\small GT} & {\tiny \verb|D9_q1.2_a0.0_m160|} & 1.200 &-&-& - & - & - & - & - & 0.036 & 0.952 & 0.682 \\
{\small GT} & {\tiny \verb|D9_q1.3_a0.0_m160|} & 1.300 &-&-& - & - & - & - & - & 0.036 & 0.953 & 0.677 \\
{\small GT} & {\tiny \verb|GT:BBH:730|} & 1.400 &-&-&-&-&-&-&-& 0.036 & 0.954 & 0.671 \\
{\small GT} & {\tiny \verb|D9_q1.5_a0.0_m160|} & 1.500 &-&-& - & - & - & - & - & 0.036 & 0.955 & 0.664 \\
{\small GT} & {\tiny \verb|D9_q1.6_a0.0_m160|} & 1.600 &-&-& - & - & - & - & - & 0.035 & 0.956 & 0.656 \\
{\small GT} & {\tiny \verb|GT:BBH:615|} & 1.700 &-&-&-&-&-&-&-& 0.035 & 0.958 & 0.649 \\
{\small GT} & {\tiny \verb|GT:BBH:618|} & 1.800 &-&-&-&-&-&-&-& 0.035 & 0.959 & 0.640 \\
{\small GT} & {\tiny \verb|D9_q1.9_a0.0_m160|} & 1.900 &-&-& - &-&-& - & - & 0.035 & 0.960 & 0.632 \\
{\small GT} & {\tiny \verb|D9_q2.0_a0.0_m160|} & 2.000 &-&-& - & - &-& - & - & 0.035 & 0.961 & 0.623 \\
{\small GT} & {\tiny \verb|GT:BBH:890|} & 2.000 &-&-& 0.600 &-&-& -0.600 & 0.200 & 0.032 & 0.951 & 0.775 \\
{\small GT} & {\tiny \verb|GT:BBH:891|} & 2.000 & 0.328 & -0.270 & -0.423 & -0.425 & -0.076 & 0.417 & -0.143 & 0.035 & 0.965 & 0.536 \\
{\small GT} & {\tiny \verb|D9_q2.0_a0.6_0.6_th180_r100_res140_CE|} & 2.000 & - & - & -0.600 & - &-& 0.601 & -0.200 & 0.035 & 0.967 & 0.464 \\
{\small GT} & {\tiny \verb|GT:BBH:893|} & 2.000 & -0.328 & 0.270 & -0.423 & 0.425 & 0.076 & 0.417 & -0.143 & 0.036 & 0.965 & 0.536 \\
{\small GT} & {\tiny \verb|GT:BBH:894|} & 2.000 & -0.500 & 0.324 & -0.070 & 0.188 & 0.556 & 0.122 & -0.006 & 0.035 & 0.959 & 0.666 \\
{\small GT} & {\tiny \verb|GT:BBH:895|} & 2.000 & 0.511 & -0.009 & 0.314 & 0.565 & 0.025 & -0.200 & 0.143 & 0.036 & 0.953 & 0.754 \\
{\small GT} & {\tiny \verb|GT:BBH:896|} & 2.000 & -0.511 & 0.009 & 0.314 & -0.565 & -0.025 & -0.200 & 0.143 & 0.032 & 0.953 & 0.754 \\
{\small GT} & {\tiny \verb|GT:BBH:897|} & 2.000 & 0.500 & -0.324 & -0.070 & -0.188 & -0.556 & 0.122 & -0.006 & 0.033 & 0.959 & 0.666 \\
{\small GT} & {\tiny \verb|GT:BBH:617|} & 2.100 &-&-&-&-&-&-&-& 0.035 & 0.962 & 0.615 \\
{\small GT} & {\tiny \verb|D9_q2.2_a0.0_m160|} & 2.200 &-&-& - &-&-& - & - & 0.035 & 0.964 & 0.606 \\
{\small GT} & {\tiny \verb|GT:BBH:621|} & 2.300 &-&-&-&-&-&-&-& 0.035 & 0.965 & 0.598 \\
{\small GT} & {\tiny \verb|GT:BBH:622|} & 2.400 &-&-&-&-&-&-&-& 0.035 & 0.966 & 0.589 \\
{\small GT} & {\tiny \verb|D9_q2.5_a0.0_m160|} & 2.500 &-&-& - & - & - & - & - & 0.035 & 0.967 & 0.581 \\
{\small GT} & {\tiny \verb|GT:BBH:651|} & 2.600 &-&-&-&-&-&-&-& 0.035 & 0.968 & 0.572 \\
{\small GT} & {\tiny \verb|GT:BBH:650|} & 2.700 &-&-&-&-&-&-&-& 0.034 & 0.969 & 0.564 \\
{\small GT} & {\tiny \verb|GT:BBH:653|} & 2.800 &-&-&-&-&-&-&-& 0.034 & 0.970 & 0.556 \\
{\small GT} & {\tiny \verb|GT:BBH:654|} & 2.900 &-&-&-&-&-&-&-& 0.034 & 0.970 & 0.548 \\
{\small GT} & {\tiny \verb|D9_q3.0_a0.0_m180|} & 3.000 &-&-& - & - & - & - & - & 0.034 & 0.971 & 0.540 \\
{\small GT} & {\tiny \verb|GT:BBH:758|} & 3.100 &-&-&-&-&-&-&-& 0.034 & 0.972 & 0.533 \\
{\small GT} & {\tiny \verb|GT:BBH:759|} & 3.200 &-&-&-&-&-&-&-& 0.033 & 0.973 & 0.525 \\
{\small GT} & {\tiny \verb|GT:BBH:760|} & 3.300 &-&-&-&-&-&-&-& 0.033 & 0.974 & 0.518 \\
{\small GT} & {\tiny \verb|GT:BBH:761|} & 3.400 &-&-&-&-&-&-&-& 0.033 & 0.974 & 0.511 \\
{\small GT} & {\tiny \verb|GT:BBH:652|} & 3.500 &-&-&-&-&-&-&-& 0.033 & 0.975 & 0.504 \\
{\small GT} & {\tiny \verb|GT:BBH:748|} & 3.600 &-&-&-&-&-&-&-& 0.032 & 0.976 & 0.497 \\
{\small GT} & {\tiny \verb|GT:BBH:778|} & 3.700 &-&-&-&-&-&-&-& 0.032 & 0.976 & 0.491 \\
{\small GT} & {\tiny \verb|GT:BBH:780|} & 3.800 &-&-&-&-&-&-&-& 0.032 & 0.977 & 0.484 \\
{\small GT} & {\tiny \verb|GT:BBH:777|} & 3.900 &-&-&-&-&-&-&-& 0.032 & 0.977 & 0.478 \\
{\small GT} & {\tiny \verb|D9_q4.0_a0.0_m160|} & 4.000 &-&-& - & - & - & - & - & 0.032 & 0.978 & 0.472 \\
{\small GT} & {\tiny \verb|GT:BBH:797|} & 4.100 &-&-&-&-&-&-&-& 0.032 & 0.978 & 0.466 \\
{\small GT} & {\tiny \verb|GT:BBH:798|} & 4.200 &-&-&-&-&-&-&-& 0.031 & 0.979 & 0.460 \\
{\small GT} & {\tiny \verb|GT:BBH:791|} & 4.300 &-&-&-&-&-&-&-& 0.031 & 0.979 & 0.454 \\
{\small GT} & {\tiny \verb|GT:BBH:795|} & 4.400 &-&-&-&-&-&-&-& 0.031 & 0.980 & 0.448 \\
{\small GT} & {\tiny \verb|GT:BBH:656|} & 4.500 &-&-&-&-&-&-&-& 0.031 & 0.980 & 0.443 \\
{\small GT} & {\tiny \verb|GW15_D12_q1.19_a0.42_-0.38_m140|}(*) & 1.190 & - &-& 0.420 & - &-& -0.380 & 0.055 & 0.021 & 0.950 & 0.714 \\
{\small GT} & {\tiny \verb|GW15_D12_q1.22_a0.33_-0.44_m140|}(*+) & 1.220 & - &-& 0.330 & - &-& -0.440 & -0.017 & 0.022 & 0.952 & 0.692 \\
{\small GT} & {\tiny \verb|GT:BBH:898|}(*) & 1.200 &-&-&-&-&-&-&-& 0.021 & 0.952 & 0.682 \\
{\small GT} & {\tiny \verb|GT:BBH:745|} & 6.000 & -0.046 & 0.539 & 0.259 &-&-&-& 0.222 & 0.032 & 0.984 & 0.571 \\
{\small GT} & {\tiny \verb|GT:BBH:742|} & 7.000 & -0.028 & 0.599 & -0.008 &-&-&-& -0.007 & 0.031 & 0.987 & 0.566 \\
{\small GT} & {\tiny \verb|GT:BBH:847|} & 1.500 & 0.600 &-&-& -0.424 &-& 0.424 & 0.170 & 0.036 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:858|} & 1.500 & -0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.170 & 0.032 & 0.948 & 0.734 \\
{\small GT} & {\tiny \verb|GT:BBH:871|} & 1.500 & -0.600 &-&-& -0.424 &-& 0.424 & 0.170 & 0.030 & 0.948 & 0.741 \\
{\small GT} & {\tiny \verb|GT:BBH:848|} & 1.500 & 0.424 & 0.424 &-& -0.424 &-& 0.424 & 0.170 & 0.032 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:870|} & 1.500 &-& 0.600 &-& -0.424 &-& 0.424 & 0.170 & 0.032 & 0.949 & 0.724 \\
{\small GT} & {\tiny \verb|GT:BBH:876|} & 1.250 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.047 & 0.035 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:900|}(*) & 1.200 & 0.400 &-&-& 0.400 &-&-&-& 0.025 & 0.951 & 0.703 \\
{\small GT} & {\tiny \verb|GT:BBH:873|} & 1.500 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.085 & 0.033 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:877|} & 1.750 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.116 & 0.032 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:885|} & 1.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 &-& 0.035 & X & X \\
{\small GT} & {\tiny \verb|q1_Seff_D9_a_0.6_-0.6_th1_45_m140|} & 1.000 & 0.425 & 0.003 & 0.424 & -0.424 & -0.004 & -0.425 & - & 0.035 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:878|} & 2.250 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.163 & 0.030 & 0.956 & 0.748 \\
{\small GT} & {\tiny \verb|GT:BBH:881|} & 2.500 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.182 & 0.032 & 0.959 & 0.751 \\
{\small GT} & {\tiny \verb|GT:BBH:882|} & 2.750 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.198 & 0.032 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:872|} & 2.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.141 & 0.031 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:859|} & 2.000 & -0.106 &-& -0.106 & 0.424 &-& 0.424 & 0.071 & 0.033 & 0.961 & 0.615 \\
{\small GT} & {\tiny \verb|GT:BBH:856|} & 2.000 & 0.106 &-& 0.106 & -0.424 &-& -0.424 & -0.071 & 0.032 & 0.962 & 0.632 \\
{\small GT} & {\tiny \verb|GT:BBH:883|} & 3.250 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.225 & 0.031 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:879|} & 3.500 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.236 & 0.032 & 0.967 & 0.737 \\
{\small GT} & {\tiny \verb|GT:BBH:884|} & 3.750 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.246 & 0.032 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:874|} & 3.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.212 & 0.033 & 0.963 & 0.745 \\
{\small GT} & {\tiny \verb|GT:BBH:857|} & 3.000 & 0.047 &-& 0.047 & -0.424 &-& -0.424 & -0.071 & 0.033 & 0.972 & 0.548 \\
{\small GT} & {\tiny \verb|GT:BBH:880|} & 4.500 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.270 & 0.032 & 0.973 & 0.721 \\
{\small GT} & {\tiny \verb|GT:BBH:875|} & 4.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.255 & 0.033 & 0.970 & 0.729 \\
{\small GT} & {\tiny \verb|GT:BBH:887|} & 5.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.283 & 0.030 & X & X \\
{\small GT} & {\tiny \verb|GT:BBH:889|} & 6.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.303 & 0.030 & 0.979 & 0.704 \\
{\small GT} & {\tiny \verb|GT:BBH:888|} & 7.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.318 & 0.029 & 0.983 & 0.695 \\
{\small GT} & {\tiny \verb|GT:BBH:886|} & 8.000 & 0.424 &-& 0.424 & -0.424 &-& -0.424 & 0.330 & 0.033 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:31|}(*) & 1.200 & 0.384 & -0.135 & -0.119 & -0.354 & 0.218 & 0.086 & -0.026 & 0.026 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:1|}(*) & 1.200 & 0.384 & -0.135 & -0.119 & -0.354 & 0.218 & 0.086 & -0.026 & 0.025 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:29|}(*) & 1.200 & 0.123 & 0.366 & -0.175 & 0.136 & -0.460 & 0.469 & 0.118 & 0.027 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:18|}(*) & 1.200 & -0.161 & -0.207 & 0.145 & 0.378 & 0.352 & 0.428 & 0.274 & 0.023 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:26|}(*) & 1.200 & -0.095 & 0.404 & -0.088 & 0.605 & -0.442 & 0.399 & 0.133 & 0.029 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:11|}(*) & 1.200 & -0.463 & -0.481 & 0.069 & 0.217 & 0.608 & 0.181 & 0.120 & 0.030 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:28|}(*) & 1.200 & -0.168 & -0.322 & -0.218 & -0.171 & 0.364 & 0.537 & 0.125 & 0.026 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:2|}(*) & 1.200 & -0.099 & -0.377 & -0.167 & -0.108 & 0.484 & 0.452 & 0.114 & 0.025 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:17|}(*) & 1.200 & -0.297 & 0.031 & 0.028 & -0.176 & -0.184 & 0.340 & 0.170 & 0.021 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:16|}(*) & 1.200 & 0.272 & -0.108 & 0.063 & 0.424 & 0.370 & 0.366 & 0.201 & 0.023 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:10|}(*) & 1.200 & 0.587 & 0.102 & 0.074 & 0.120 & 0.087 & 0.398 & 0.221 & 0.024 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:15|}(*) & 1.200 & 0.276 & -0.106 & 0.052 & 0.144 & 0.268 & 0.295 & 0.163 & 0.022 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:3|}(*) & 1.200 & 0.299 & 0.028 & 0.008 & 0.192 & 0.092 & 0.367 & 0.171 & 0.022 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:25|}(*) & 1.200 & 0.119 & -0.407 & 0.017 & 0.125 & 0.656 & -0.064 & -0.020 & 0.025 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:9|}(*) & 1.200 & 0.554 & -0.314 & 0.212 & 0.008 & 0.643 & -0.191 & 0.028 & 0.031 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:24|}(*) & 1.200 & 0.151 & 0.396 & 0.017 & -0.278 & -0.605 & -0.085 & -0.029 & 0.020 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:4|}(*) & 1.200 & 0.159 & -0.393 & -0.016 & 0.149 & 0.654 & -0.014 & -0.015 & 0.025 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:14|}(*) & 1.200 & 0.662 & -0.015 & 0.106 & -0.384 & 0.113 & -0.141 & -0.006 & 0.026 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:5|}(*) & 1.200 & 0.649 & 0.149 & 0.086 & -0.385 & -0.130 & -0.124 & -0.009 & 0.024 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:6|}(*) & 1.200 & 0.662 & -0.070 & 0.083 & -0.358 & 0.201 & -0.106 & -0.003 & 0.027 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:30|}(*) & 1.200 & 0.391 & 0.100 & -0.131 & -0.392 & -0.130 & 0.097 & -0.028 & 0.021 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:8|}(*) & 1.200 & -0.395 & 0.100 & -0.116 & 0.381 & -0.167 & 0.083 & -0.026 & 0.022 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:13|}(*) & 1.200 & -0.360 & 0.181 & -0.131 & 0.277 & -0.304 & 0.105 & -0.023 & 0.021 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:22|}(*) & 1.500 & -0.337 & 0.011 & -0.258 & -0.093 & -0.207 & 0.632 & 0.098 & 0.026 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:21|}(*) & 1.500 & -0.272 & 0.107 & 0.069 & 0.079 & -0.347 & 0.230 & 0.134 & 0.028 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:20|}(*) & 1.500 & -0.259 & -0.236 & -0.238 & -0.470 & 0.317 & 0.358 &-& 0.028 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:12|}(*) & 1.500 & -0.624 & -0.197 & -0.148 & -0.143 & 0.185 & 0.354 & 0.053 & 0.032 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:19|}(*) & 1.500 & 0.318 & 0.087 & -0.266 & 0.219 & 0.004 & 0.363 & -0.015 & 0.023 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:7|}(*) & 1.500 & 0.293 & 0.173 & -0.253 & 0.178 & -0.218 & 0.317 & -0.025 & 0.022 & X & X \\
{\small BAM-GitAnnex} & {\tiny \verb|BAM150914:23|}(*) & 1.500 & 0.306 & 0.140 & -0.259 & 0.216 & -0.127 & 0.342 & -0.018 & 0.028 & X & X \\
\end{longtable}

